Quantum Geometric Machine Learning

The use of geometric and symmetry techniques in quantum and classical information processing has a long tradition across the physical sciences as a means of theoretical discovery and applied problem solving. In the modern era, the emergent combination of such geometric and symmetry-based methods with quantum machine learning (QML) has provided a rich opportunity to contribute to solving a number of persistent challenges in fields such as QML parametrisation, quantum control, quantum unitary synthesis and quantum proof generation. In this thesis, we combine state-of-the-art machine learning methods with techniques from differential geometry and topology to address these challenges. We present a large-scale simulated dataset of open quantum systems to facilitate the development of quantum machine learning as a field. We demonstrate the use of deep learning greybox machine learning techniques for estimating approximate time-optimal unitary sequences as geodesics on subRiemannian symmetric space manifolds. Finally, we present novel techniques utilising Cartan decompositions and variational methods for analytically solving quantum control problems for certain classes of Riemannian symmetric space. Owing to its multidisciplinary nature, this work contains extensive supplementary background information in the form of Appendices. Each supplementary Appendix is tailored to provide additional background material in a relatively contained way for readers whom may be familiar with some, but not all, of these diverse scientific disciplines. The Appendices reproduce or paraphrase standard results in the literature with source material identified at the beginning of each Appendix. Proofs are omitted for brevity but can be found in the cited sources and other standard texts.

==> ebackupChapter2a.tex <==
% %==========
% %==========
% %===QUANTUM INFORMATION PROCESSING
% \chapter{Background: Quantum Information Processing} \label{chapter:Background: Quantum Information Processing}
% \section{Overview}
% Quantum information processing is characterised by constraints upon how information is represented and processed arising from the foundational postulates of quantum mechanics. While information as the subject of enquiry within physics has a long lineage, it quantum information processing as an emergent and distinct discipline arose largely through the convergence (and often synthesis) of concepts in computational and informational sciences and quantum physics, principally through the vision of quantum computing envisaged by Feynman \cite{feynman_simulating_1982} and others. As we discuss below, the field incorporates concepts from quantum physics, computer science and information and communication theory (pioneered by Shannon and others \cite{shannon_mathematical_1948}).


% Below we provide an overview of key elements of quantum postulates \cite{nielsen_quantum_2010} and quantum information processing for classical machine learning practitioners solving optimisation problems for quantum engineering. In particular, we describe ways in which quantum data are typically represented (such as via tensors), how quantum processes are usually expressed in common programming languages. Quantum information processing draws upon formalism and conceptual framing from a range of disciplines, including analysis, information theory and complexity theory, together with algebra, geometry and other numerous branches of mathematics. All quantum information processing rests, however, upon the mathematical formalism of quantum mechanics itself. The study of such formalism usually begins with the study of quantum axioms or postulates, a set of assumptions about quantum systems and their evolution derived from observation (rather than deduced from assumptions) and from which other results and properties of quantum systems are deduced. There are a variety of ways to express such axioms according to chosen formalism (and indeed debate continues within fields such as quantum foundations, mathematics and philosophy as to the appropriateness of such postulates). 

% In this work, we partly frame postulates information-theoretic fashion concurrently with traditional formulations. The axioms form a structured ordering of this background material, anchoring various definitions, theorems and results relevant to establishing and justifying methods and results in later chapters. Following our exposition, we then proceed to discussing key elements of open quantum systems (relevant to, for example, the simulated quantum machine learning dataset the subject of Chapter \ref{chapter:QDataSet and Quantum Greybox Learning}) together with elements of the theory of quantum control (which we later expand upon in terms of algebraic and geometric formulations). For those familiar with quantum mechanics and quantum information processing, this section can be skipped without loss of benefit. Most of the material below is drawn from standard texts in the literature, including \cite{nielsen_quantum_2010,hall_quantum_2013,watrous_theory_2018}. Proofs are omitted for the most part (being accessible in the foregoing or other textbooks on the topic). We begin with the first axiom of quantum mechanics, that related to quantum states.


% % \subsection{Axioms of quantum mechanics}
 
% % The first axiom concerns representations of quantum systems in terms of states.
% % \begin{axiom}[Quantum states]\label{axiom:quantumstates}
% % The state of a quantum system is represented by a unit vector $\psi$ in an appropriate Hilbert space $\mathcal{H}$. Two unit vectors $\psi_1, \psi_2\in\mathcal{H}$, where $\psi_2 = c\psi_1$ for $c \in \mathbb{C}$, correspond to the same physical state. In density operator formalism, the quantum system is described by the linear operator $\rho \in \mathcal{B}(\Hilb)$ acting on $\Hilb$. For bounded $A \in \mathcal{B}(\Hilb)$, the expectation value of $A$ is $\Tr(\rho A).$ 
% % \end{axiom}
% % We set out background theory and more developed representations of quantum states (such as in terms of operators) in section (\ref{sec:chapter1:quantum:statespace}). 

% % \begin{axiom}[Observable Operators]\label{axiom:observableoperators}
% % For every real-valued function $O$ defined on classical phase space, there exists a self-adjoint (Hermitian) operator $\hat{O}$ defined on $\mathcal{H}$.
% % \end{axiom}

% % \begin{axiom}[Measurement]\label{axiom:probabilitymeasurement}
% % Given $\psi \in \mathcal{H}$, the probability distribution for the measurement of an observable $f$ is such that $E[O^m] = \braket{ \psi, (\hat{O})^m \psi }$. Given an orthonormal basis $\{e_j\}$, we may write $\psi = \sum_j^\infty a_j e_j, a_j \in \C$ with the probability of observing measurement outcome $\lambda_j$ given by $P(O=\lambda_j)=|a|^2$.
% % \end{axiom}

% % \begin{axiom}[Wave Function Collapse]
% % Measurement of observable $O$ with measurement outcome $\lambda \in \mathbb{R}$, causes a quantum system transition to $\psi' \in \Hilb$ such that $\hat{O}\psi' = \lambda\psi'$. 
% % \end{axiom}

% % \begin{axiom}[Evolution]
% % Quantum state evolution is described by the Schr\"{o}dinger equation: $\frac{d\psi}{dt} = H\psi$, where $\hat{H}$ is the Hamiltonian. In density operator 
% % \end{axiom}

% \subsection{State space}\label{sec:chapter1:quantum:statespace}
% The first axiom concerns representations of quantum systems in terms of states.
% \begin{axiom}[Quantum states]\label{axiom:quant:quantumstates}
% The state of a quantum system is represented by a unit vector $\psi$ in an appropriate Hilbert space $\mathcal{H}$. Two unit vectors $\psi_1, \psi_2\in\mathcal{H}$, where $\psi_2 = c\psi_1$ for $c \in \mathbb{C}$, correspond to the same physical state. In density operator formalism, the quantum system is described by the linear operator $\rho \in \mathcal{B}(\Hilb)$ acting on $\Hilb$. For bounded $A \in \mathcal{B}(\Hilb)$, the expectation value of $A$ is $\Tr(\rho A)$. Composite quantum systems are represented by tensor products $\psi \otimes \psi$ (or equivalently in operator formalism, $\rho_k \otimes \rho_j$). 
% \end{axiom}
% We set out background theory and more developed representations of quantum states (such as in terms of operators) in section (\ref{sec:chapter1:quantum:statespace}). 

% Quantum systems are represented by (unit) state vectors within a complex-valued vector (Hilbert) space $\mathcal{H}$ whose dimensionality is determined according to the physics of the problem. There are various formalisms for representing such state vectors. A common form in quantum information processing `bra-ket' notation. In this notation, the state vector is represented as a `ket' $\ketpsi \in \mathcal{H}$. Associated with a ket is a corresponding `bra' notation $\bra{\psi}$ which strictly speaking is a linear (one) form (or function) that acts on $\ketpsi$ such that $\braket{\psi_1|\psi_2} \in \Complex$ for two states $\ket{\psi_1},\ket{\psi_2}$. In this section, we set out a number of standard formulations for conceptualising quantum information and quantum control problems. Advanced readers familiar with quantum formalism can progress to other sections without loss of generality. We begin with vector spaces, introductory measure theory and some results from functional analysis. In later chapters, we will equate typical Hilbert space formalism in terms of geometric and algebraic concepts related to manifolds, fibres and connections. Quantum states are typically defined as elements of a Hilbert space, a vector space over $\C$ equipped with an inner product.

% %=====Defn: Vector Space
% \begin{definition}[State space]\label{defn:quant:State space}
%     A state space $V(\mathbb{K})$ is a vector space over a field $\mathbbm{K}$, typically $\mathbbm{C}$. Elements $\psi \in V$ represent possible states of a quantum system. In particular, for $a_k\in\C$ and $\psi_k \in V$, the state $\psi = \sum_k a_k \psi_k \in V$. 
% \end{definition}
% Evolutions of quantum systems over time are described by mappings within this state space (e.g. linear operators on $V$). The state space of a quantum system is fundamental in the description of quantum states, where the vectors are typically normalized to have a unit norm due to the probabilistic interpretation of quantum mechanics. Later on we refine our working definition of state space in terms of Hilbert spaces, operators and other concepts such as channels. We moreover in later chapters connect quantum state space with concepts from algebra, representation theory, geometry and statistical learning. We set out below a few key concepts relevant to the formalism adopted. A more quantum information-theoretic approach is provided by Watrous \cite{watrous_theory_2018} who defines states in terms of \textit{registers} (alphabets or tuples thereof) as descriptions of quantum states according to an alphabet $\Sigma$. 
% \begin{definition}[Classical registers and states]\label{defn:quant:Classical registers and states}
%     A classical register $X$ is either (a) a simple register, being an alphabet $\Sigma$ (describing a state); or (b) a compound register, being an n-tuple of registers $X=(Y_k)$.\\
%     A classical state set $\Gamma$ of $X$ is then either (i) $\Gamma=\Sigma$ or (ii) in the case of a compound register, the Cartesian product of those state sets $\Sigma = \times_k \Gamma_k$  
% \end{definition}
% The formulation of classical states here maps largely to that found in computer science literature where states are constructed from alphabets etc. For classical states and subregisters determine each other's state. A register has configurations (states) it may adopt (with subregisters determining higher-order registers). Probabilistic states are distributions over classical states the register may assume, denoted $\mathcal{P}(\Sigma)$ with states represented by probability vectors $p(a)\in \mathcal{P}(\Sigma)$. From the classical case, we can then construct the quantum information representation of a quantum register and states which are represented by density operators (defined below).
% \begin{definition}[Quantum registers and states]\label{defn:quant:Quantum registers and states}
%     A quantum state is defined as an element of a complex (Euclidean) space $\C^\Sigma$ for a classical state set $\Sigma$ satisfying specifications imposed by axioms of quantum mechanics (see below) as they apply to states.  
% \end{definition}
% In the terminology of operators (see below) a quantum state is defined as a density operator $\rho \in D(\Hilb)$.
%  We refer in parts to this formulation below and in later chapters.
% %=====Defn: Norm

% \begin{definition}[Norm]\label{defn:Norm}
% Define a norm on a vector space \( V \) over \( \mathbbm{K} = \mathbb{R}\) or \( \mathbb{C} \) as a mapping \( \lVert . \rVert: V \to \mathbb{R} \), \( \psi \mapsto \lVert \psi \rVert \), such that for $\psi,\phi \in V$ and $c \in \mathbbm{K}$:
% \begin{align*}
%     1. & \quad \lVert \psi \rVert \geq 0 \text{ and } \psi = 0 \Longleftrightarrow \lVert \psi \rVert=0 . \\
%     2. & \quad \lVert c\psi \rVert = |c| \lVert \psi \rVert. \\
%     3. & \quad \lVert \phi + \psi \rVert \leq \lVert \phi \rVert + \lVert \psi \rVert.
% \end{align*}
% A norm \( \lVert . \rVert \) on \( V \) defines a distance (metric) function \( d \) on \( V \) as $d(\phi, \psi) = \lVert \psi - \phi \rVert$.
% \end{definition}

% %=====Defn: Banach
% A normed vector space is a Banach space
% if it is complete with respect to the associated distance function (e.g. inner product). Banach spaces are equipped with certain convergence and boundedness properties which enable among other things definitions of bounded linear functionals and dual spaces, both of which are relevant to results in later chapters. Banach spaces allow us to define an \textit{operator norm}.
% %===Operator norm
% \begin{definition}[Operator norm]\label{defn:quant:Operator norm}
% If $V_1(\mathbb{K})$ and $V_2(\mathbb{K})$ are normed spaces, the linear mapping $A \colon V_1(\mathbb{K}) \rightarrow V_2(\mathbb{K})$ is bounded if
% \begin{align*}
% \sup_{\psi \in V_1 \setminus \{0\}} \frac{\|A\psi\|}{\|\psi\|} < \infty.
% \end{align*}
% \end{definition}
% Intuitively this tells us that linear mappings on $V(\mathbb{K})$ remain within the closure of $V(\mathbb{K})$

% The set of such linear forms forms a complementary vector space denoted the dual space.

% %=====Defn: bounded linear functional
% \begin{definition}[Dual space]\label{defn:quant:Dual space}
%     A bounded linear functional on a normed vector space $V(\mathbbm{K})$ is a bounded linear map $\chi: V \to \mathbbm{K}, \psi \mapsto a||\psi||$ for some (scaling) $a \in \mathbbm{K}$. The norm is given via the field norm $||.|| = |.| \in \mathbbm{K}$. The set of all such bounded linear functionals is denoted the dual space $V^*(\mathbb{K})$ to $V(\mathbbm{K})$.\\
%     If $V(\mathbbm{K})$ is normed then $V^*(\mathbb{K})$ is also a Banach space. Moreover, we have that for $\psi \in V$ and $\chi \in V^*$: 
%     \begin{align*}
%         1.&\quad \chi(\psi) \in \mathbb{K}.\\
%         2.&\quad |\chi(\psi)|= ||\chi||||\psi||.\\
%         3.&\quad \forall \chi \in V^*, \chi(\psi) = 0 \Longleftrightarrow \psi = 0.
%     \end{align*}
% \end{definition}
% We discuss dual spaces and functionals in further chapters, particularly in relation to representations of Lie algebras and differential forms. With the concept of a dual space, we can now define a central operation on vector spaces, the inner product.


% %=====Defn: dual space


% %=====Defn: Inner Product
% \begin{definition}[Inner Product]\label{defn:quant:Inner Product}
% An inner product on $V(\mathbbm{K})$ is a mapping from a vector space to a field $\mathbbm{K}$ \( \langle \cdot, \cdot \rangle: V \times V \rightarrow \mathbbm{K}, (\psi,\phi) \mapsto \langle \psi,\phi \rangle \) for $\psi,\phi \in V, c \in \mathbbm{K}$ satisfying:
% \begin{enumerate}[(i)]
%     \item $\braket{\psi | \phi} = \braket{\phi | \psi}$.
%     \item $\braket{\phi | \phi} \in \mathbb{R}^+ \text{ and } \braket{\phi | \phi} = 0 \Longleftrightarrow \phi = 0$.
%     \item $\braket{c\phi | \psi} = c \braket{\phi | \psi} \text{ and } \braket{\phi | c\psi} = c^* \braket{\phi | \psi}$.
%     \item $\braket{\phi + \psi | \chi} = \braket{\phi | \chi} + \braket{\psi | \chi} \text{ and } \braket{\phi | \psi + \chi} = \braket{\phi | \psi} + \braket{\phi | \chi}$.
% \end{enumerate}
% \end{definition}
% Inner products and bilinear forms are crucial components across quantum, algebraic and geometric methods in quantum information processing. In particular, we examine the relationship between differential (\textit{n}-)forms and inner products (see Chapter \ref{chapter:Background: Geometry, Lie Algebras and Representation Theory}) which are relevant to variational results in Chapter \ref{chapter:Time optimal quantum geodesics using Cartan decompositions} [where the inner product is analogous to a bilinear mapping of $V \times V^* \to \mathbb{K}$, implicit in the commonplace `braket' notation of quantum information (where kets $\ketpsi$ and $\bra{\psi}$ are duals to each other and inner products are given by $\braket{\psi|\psi}$)]. Moreover, in later chapters we adopt (and argue for the utility of) a geometric approach where inner products and norms are defined in terms of metric tensors $g$ over manifolds and vector space relationships to fibers. We also note the Plancherel formula which provides that the inner product of two functions equals the inner product of their transforms, such that for unitary transformations. The inner product defined on a vector space $V$ then gives rise to a norm via the Cauchy-Schwartz inequality.








% %=====Defn: Cauchy-Schwarz

% \begin{definition}[Cauchy-Schwarz Inequality]\label{defn:quant:Cauchy-Schwarz Inequality}
% The Cauchy-Schwarz inequality applies to inner product spaces $V(\mathbbm{K})$ such that for \( \phi, \psi \in V \):
% \begin{align*}
% |\langle \phi, \psi \rangle|^2 \leq \langle \phi, \phi \rangle \langle \psi, \psi \rangle.
% \end{align*}
% If \( ||\cdot||: V \rightarrow \mathbb{R} \) where $||\psi|| = \sqrt{\langle \psi, \psi \rangle}$, then the inner product defines a norm on $V$.
% \end{definition}
% As standard we can then define a generalised angle given two vectors \( \phi, \psi \in V \) in an inner product space where the cosine of the angle \( \theta \) between \( \phi \) and \( \psi \) is given by:
% \begin{align}
% \cos(\theta) = \frac{\langle \phi, \psi \rangle}{\| \phi \| \cdot \| \psi \|} \label{eqn:quant:cosinevector}
% \end{align}

% %=====Defn: Hilbert Space
% Equipped with a vector space and inner product, we now come to the definition of a Hilbert space as a Banach space where the norm is defined in terms of the inner product above.
% \begin{definition}[Hilbert Space]\label{defn:quant:Hilbert Space}
% A Hilbert space is a vector space $\mathcal{H}(\mathbbm{K})$ with an inner product \( \langle \cdot, \cdot \rangle \) complete in the norm defined by the inner product $||\psi|| = \sqrt{\langle \psi, \psi \rangle}$.
% \end{definition}
% Often [we are interested in direct sums or direct (tensor) products of Hilbert spaces. For example, tensor product states (crucial to multi-qubit quantum computations) are considered to belong to a tensor product of Hilbert spaces. We discuss these in later chapters. It should be noted that in some cases, mulitipartite Hilbert spaces may be characterised by direct sums rather than direct (tensor) products. This is the case where a Hilbert space is decomposable into disjoint regions such as, in particular, our discussion of Cartan decompositions in later chapters. In such cases, we observe the following.

% %=====Defn: Hilbert space direct sum
% \begin{proposition}[Hilbert Space Direct Sum]\label{prop:quant:Hilbert Space Direct Sum} The direct sum of a sequence \( \Hilb \) of separable Hilbert spaces denoted by
% \begin{align*}
% H := \bigoplus_{j=1}^{\infty} H_j,
% \end{align*}
% has a representation as a space of sequences \( \psi = (\psi_1, \psi_2, \psi_3, \ldots) \) where \( \psi_j \in \Hilb_j \). The norm on $\Hilb$ satisfies:
% \begin{align*}
% ||\psi||^2 := \sum_{j=1}^{\infty} ||\psi_j||^2 < \infty.
% \end{align*}
% \end{proposition}
% A direct sum of each \( H_j \) is the set of \( \psi = (\psi_1, \psi_2, \psi_3, \ldots) \) where \( \psi_j = 0 \) for all but finitely many $\psi_j$. An inner product on the direct sum can be defined via:
% \begin{align*}
% \langle \phi, \psi \rangle = \sum_{j=1}^{\infty} \langle \phi_j, \psi_j \rangle,
% \end{align*}
% for all \( \phi_j, \psi_j \in H_j \) and $\psi,\phi \in \Hilb$. Each subspce inherits the inner product and associated completeness properties of $\Hilb$, confirming each $\Hilb_j$ as a Hilbert space. The partitioning of a Hilbert space via a Cartan decomposition of Lie algebraic generators (which form a Hilbert space as a vector space upon which an inner produt is defined) $\g$ into $\g= \k \oplus \p$ is an example of such a decomposition which preserves the overall structure of the Hilbert space within which quantum information vectors subsist [\textbf{SCHUE}]. Thus the essential properties of quantum state vectors are retained in the case of such decomposition. 
% Hilbert spaces have a number of features of importance to quantum computational contexts. These include certain orthogonality relations which are important to their decomposition in ways that can simplify problems (such as those of unitary synthesis that we examine in later chapters).
% \begin{definition}[Orthogonality and orthonormality]\label{defn:quant:Orthogonality and orthonormality}
%     A Hilbert space $\mathcal{H}$ exhibits the following relations related to orthogonality:
%     \begin{enumerate}
%         \item $\psi,\phi \in \mathcal{H}$ are orthogonal if $\innerproduct{\psi}{\phi}=0$.
%         \item (Orthogonal space) If $\mathcal{H}_i \subset \mathcal{H}$, the orthogonal subspace $\mathcal{H}_i^\perp \subset \mathcal{H}$ of $H_i$ is:
%         \begin{align*}
%     \mathcal{H}_i^\perp &= \{ \phi \in \mathcal{H} | \innerproduct{\psi}{\phi} = 0 \text{ for all } \psi \in H_i \}
%         \end{align*}
%     \end{enumerate}
% \end{definition}
% In many quantum information tasks, we assume that states $\psi \in \mathcal{H}$ can be decomposed into a direct sum $\mathcal{H}_i \oplus \mathcal{H}_i^\perp = \mathcal{H}$ such that $\psi = \psi_i + \psi_i^\perp$. States are then represented in terms of an orthonormal basis for $\mathcal{H}$.
% \begin{definition}[Orthonormal Basis]\label{defn:quant:Orthonormal Basis}
% The set $\{e_j\}, e_j \in \mathcal{H}$, $j=1,...,\dim\mathcal{H}$ is an \textit{orthonormal} basis if $\braket{e_j, e_k}=\delta_{jk}$ (the Kronecker delta)
% and $\mathcal{H}=span\{ae_j | a\in \C\}$. In this case:
% \begin{align}
%     ||\psi||^2&=\sum_j |a_j|^2 \label{defn:2.2.10sumjaj2}
% \end{align}
% \end{definition}
% States are expressible as (convergent) sums $\psi = \sum_j a_j e_j, a_j \in \C$ where $a_j = \braket{e_j, \psi} \in \C$ . 

% \subsubsection{Tensor product states}\label{sec:quant:Tensor product states}
% In many cases of interest, we have disjoint or multi-state (e.g. multi-qubit) quantum systems of interest. This is especially the case with the multi-qubit systems the subject of Chapters \ref{chapter:QDataSet and Quantum Greybox Learning} 
%  and \ref{chapter:Quantum Geometric Machine Learning}. Vector spaces for multi-state systems are represented by tensor products of vector spaces and Hilbert spaces which we define below.

% \begin{definition}[Tensor Product]\label{defn:quant:Tensor Product}
% A tensor product of two vector spaces $V_1(\mathbb{K}), V_2(\mathbb{K})$ is itself a vector space $W(\mathbb{F})$ equipped with a bilinear map $T : V_1(\mathbb{K}) \times V_2(\mathbb{K}) \rightarrow W(\mathbb{K})$.
% \end{definition}
% To allow us to represent a single (equivalent) tensor product between two such vector spaces, we note the following `universal property' \cite{hall_quantum_2013} which allows elements of $W$ to be written as elements $u \otimes v$ where $u \in V_1, v, v \in V_2$. Given another vector space $Z(\mathbb{K})$ along with a bilinear mapping $\Phi : V_1 \times V_2 \rightarrow Z$, it can be shown that there exists a unique linear map $\widetilde{\Phi}: W \rightarrow Z$ such that the diagram below commutes:
% \begin{figure}[h!]
% \centering
% \begin{tikzcd}[row sep=huge, column sep=huge]
% V_1(\mathbb{K})\times V_2(\mathbb{K}) \arrow[rd, "\Phi"'] \arrow[r, "T"] & W(\mathbb{K}) \arrow[d, "\tilde\Phi"] \\
% & U
% \end{tikzcd}
% \caption{Commutative diagram with spaced out arrows.}
% \end{figure}
% It can then be shown that the tensor product of $V_1,V_2$ exists and is unique up to a canonical isomorphism. This allows us to represent the mapping $T$ in terms of the direct product $T:V_1 \times V_2 \to V_1 \otimes V_2, (u,v) \mapsto u\otimes v$. 

% The universal property guarantees that given $\Phi: V_1 \times V_2 \to Z$, there will exist a map $\tilde\Phi: V_1 \otimes V_2 \to Z$ with $\tilde\Phi(u \otimes v = \Phi(u,v)$. Among other things this means that $\dim(V_1 \otimes V_2 = (\dim V_1)(\dim V_2)$. Under such assumptions, arbitrary $\psi \in V_1 \otimes V_2$ can then be decomposed as linear compositions of $u\otimes v$ for a given basis. It also allows the space of operators (linear maps $A_k \in End(V_k)$) to be [constructed] in tensor-product form by guaranteeing the existence of $A_k \otimes A_j: V_k \otimes V_j \to V_k \otimes V_j$ exhibiting (a) homomorphic structure $(A_k \otimes A_j)(u \times v) = (A_ku) \otimes (A_j v)$ and linear compositionality $(A_k \otimes A_j)(A_p \otimes A_q)=(A_kA_p) \otimes (A_jA_r)$. For tensor products of Hilbert spaces, we note that given multiple inner product spaces $V_k$ with inner products $\braket{v_p,v_q}_k$, there exists an inner product on the tensor product space $\otimes_k V_k$ given by:
% \begin{align*}
%     \braket{u_p \otimes v_p, u_q \otimes v_q} = \braket{u_p,u_q}_k \braket{v_p,v_q}_j
% \end{align*}
% where $u_p,u_q \in V_k$ and $v_p,v_q \in V_j$. In this way, a Hilbert tensor product $\otimes_k \Hilb_k$ space is equipped with sufficient structure via the inner product and bounded operators as per above (allowing, among other things, metric calculations relevant to machine learning and variational techniques to be implemented). We note for completeness that orthonormal bases $\{e_j\}_k$ for $\Hilb_k$ form a tensorial orthonormal basis for the Hilbert space $\otimes \Hilb_k$ given by $\{ \times_k e_{j,k}\}$ (tensor product of orthonormal bases). Note also that for $A_k \in \mathcal{B}(\Hilb)_k$, we have $||\otimes_k A_k||= \prod_k ||A_k||$.

% \subsubsection{Quantum State formalism}\label{sec:quant:Quantum State formalism}
% A significant proportion of quantum information research concentrates on single (or multi) qubits (quantum bits), being arbitrary two-level (and their corresponding operator representations below) quantum systems (two-dimensional state spaces) of qubits with arbitrary state vectors with orthonormal bases $\{\kz,\ko\}$. In this formalism:
% \begin{align}
% \ketpsi = a\kz + b\ko
% \label{eqn:qubit}
% \end{align}
% Qubits are normalised such that they are unit vectors $\braket{\psi | \psi} = 1$ (that is $|a|^2 + |b|^2=1)$, where $a,b \in \Complex$ are amplitudes and their squared moduli, the probabilities, for measuring outcomes of 0 or 1 (corresponding to states $\kz,\ko$ respectively). Here $\braket{\psi | \psi'}$ denotes the inner product of quantum states $\ketpsi,\ket{\psi'}$). As can be observed in (\ref{eqn:qubit}), as distinct from a classical (deterministic or stochastic) state, quantum states may subsist ontologically in a superposition of their basis states.

% The stateful characteristic of quantum systems is also manifest in the first postulate of quantum mechanics, which associates Hilbert spaces to enclosed physical systems under the assumption that $\psi \in \mathcal{H}$ provides complete information about the system \cite{nielsen_quantum_2010}. For problems in quantum computing and control, we are interested in how quantum systems evolve, how they are measured and how they may be controlled. To this end, we include below a brief synopsis of operator formalism and evolution of quantum systems. In Chapter \ref{chapter:Background: Geometry, Lie Algebras and Representation Theory}, we characterise these formal features of quantum information processing algebraic and geometric terms.

   
% \subsection{Operators and evolution}\label{sec:quant:Operators and evolution}

% Often it is more convenient to work with (and consider evolutions of) functions and algebras associated with operators on $\Hilb$ rather than $\psi \in \Hilb$ directly. This operator formalism manifests in both recasting state spaces in terms of density operators and considering maps between operators in terms of quantum channels. Such mappings also serve to connect quantum formalism with the types of mappings and formalism common within machine learning and geometry. We now consider formalism associated with the second axiom of quantum mechanics, namely that physical observables correspond to real eigenvalues of (measurement) operators. 
% \begin{axiom}[Observable Operators]\label{axiom:quant:observableoperators}
% For every measureable physical observable quantity is defined by a real-valued function $M$ defined on classical phase space, there exists a self-adjoint (Hermitian) linear measurement operator $M$ acting on $\mathcal{H}$. The results of measurement of the state must be a real-valued eigenvalue of the measurement operator.
% \end{axiom}



% \subsubsection{Operator formalism}\label{sec:quant:Operator formalism}
% In quantum information, operators are thought of as maps between Hilbert spaces. We begin by considering the general class of endomorphisms on $\Hilb$ (and later describe Hilbert-Schmidt space and channels) and define $\mathcal{B}(\mathcal{H})$ as the space of bounded endomorphic linear maps of $\Hilb$:
% \begin{definition}[Bounded linear operators]\label{defn:quant:Bounded linear operators}
%     The space $\mathcal{B}(\mathcal{H})$ of bounded linear operators $T$ is defined by
% \begin{align*}
% \mathcal{B}(\mathcal{H}) = \{ T : \mathcal{H} \rightarrow \mathcal{H} \mid T \text{ is linear and bounded} \},
% \end{align*}
% where $T$ is bounded if there exists a non-negative real number $M$ such that:
% \begin{align*}
% \| T\psi \| &\leq M\|\psi\| \quad \text{for all } \psi \in \mathcal{H}.
% \end{align*}
% The smallest such $M$ is the operator norm of $T$, denoted by $\| T \|$.
% \end{definition}
% We also note Reisz's Theorem that for any bounded linear functional $\xi:\mathcal{H} \to \C$, there exists a dual element $\chi$ such that $\xi(\psi) = \braket{\chi,\psi}$ (i.e. and so an equivalence of norms). Reisz's Theorem guarantees the existence in such cases of an adjoint operator $A^\dagger$ which crucial for Hermitian operators. \hl{check}
% \begin{definition}[Adjoint of an Operator]\label{defn:quant:Adjoint of an Operator}
% For any $A \in \mathcal{B}(\Hilb)$, there exists a unique linear operator $A^\dagger \colon \Hilb \to \Hilb$, called the adjoint of $A$, such that
% \begin{align*}
% \langle \phi, A\psi \rangle = \langle A^\dagger\phi, \psi \rangle
% \end{align*}
% for all $\phi, \psi \in H$.
% \end{definition}
% The adjoint is also known as the Hermitian conjugate. In physics, sometimes the adjoint of such an operator, $A^\dagger$ is denoted $A^*$ (we reserve the $*$ notation for dual spaces). This can occasionally lead to some confusion as sometimes $A^*$ is just considered the complex (entry-wise) conjugate. 
% % [For the avoidance of doubt, in this work $A^*$ represents $\overline{A}^T$] with $\overline{A}$ representing the entry-wise conjugate.
% %=====djoint Operator Properties and Hermitian Operators
% \begin{proposition}[Adjoint Operator Properties and Hermitian Operators]\label{prop:quant:djoint Operator Properties and Hermitian Operators}
% For all $A, B \in \mathcal{B}(H)$ and $\alpha, \beta \in \mathbb{C}$ we have
% \begin{align*}
% (A^\dagger)^\dagger &= A \qquad (AB)^\dagger = B^\dagger A^\dagger, \\
% (\alpha A + \beta B)^\dagger &= \bar{\alpha}A^\dagger + \bar{\beta}B^\dagger \qquad
% I^\dagger = I.
% \end{align*}
% Note too that $\|A^\dagger\| = \|A\| < \infty$. If $A^\dagger = A$, then $A$ is self-adjoint which we denote as Hermitian (or skew-self-adjoint if $A^\dagger = -A$). 
% \end{proposition}
% Matrix representation of Hermitian conjugation is via the (complex)-conjugate transpose $A^\dagger = A^\dagger$. Note also that $\braket{\phi,A(\psi)}=\braket{A^\dagger(\phi),\psi}$. In braket notation we define $\ket{\psi}^\dagger\dot=\bra{\psi}$. The adjoint operator is also important practically as an element used when determining Cartan involutions (and thus Cartan decompositions) with respect to symmetric and anti-symmetric subalgebras of $\g$. We can now introduce unitary operators which are crucial to quantum information processing and our results herein. A few standard important operator classes are set out below.
% \begin{definition}[Positive Semidefinite Operators]\label{defn:Positive Semidefinite Operators}
% An operator $A \in \mathcal{B}(\mathcal{H})$ is positive semidefinite if $A = B^\daggerB$ for some operator $B \in \mathcal{B}(\mathcal{H})$. Denote the set of such operators as:
% \begin{align*}
% \text{Pos}(\mathcal{H}) = \{B^\daggerB : B \in \mathcal{B}(\mathcal{H})\}.
% \end{align*}
% \end{definition}
% Positive semidefinite operators are Hermitian. A \textit{positive definite operator} is a positive-semi definite operator that is also invertible i.e. $A \in Pos(\Hilb)$ such that $\det(A) \neq 0$. Positive semi-definite operators are commonly expressed via constraints on the inner product, namely that $\braket{Av,v} \geq 0$ for $v \in \Hilb$. Using these definitions we can then specify two important classes, projection operators and isometries.

% %=====Defn: projection and isometries
% \begin{definition}[Projection Operators]
% \label{defn:quant:projection_operators}
% An operator $P \in \text{Pos}(\mathcal{H})$ is an (orthogonal) projection operator if $\Pi^2 = \Pi$ and, for some closed $V \in \Hilb$, $P(V)=I$ and $P(V^\perp)=0$.
% \end{definition}
% The set of projection operators is denoted $\text{Proj}(\mathcal{H})$. For each $V$ there exists a $P$ such that the imat of $P$ is $V$.
% %=====Defn: isometries
% \begin{definition}[Isometries]
% \label{defn:isometries} \hl{Update}
% $A \in \mathcal{B}(\mathcal{H}, \mathcal{Y})$ is an \textit{isometry} if $\|Av\| = \|v\|$ for all $v \in \mathcal{H}$. This is equivalent to $A^\daggerA = I_{\mathcal{H}}$. The set of such isometries is denoted:
% \begin{align*}
% U(\mathcal{H}, \mathcal{Y}) = \{A \in \mathcal{B}(\mathcal{H}, \mathcal{Y}) : A^\daggerA = I_{\mathcal{H}}\}
% \end{align*} 
% \end{definition}
% In order for an isometry of the form $A \in U(\mathcal{H}, \mathcal{Y})$ to exist, it must hold that $\text{dim}(\mathcal{Y}) \geq \text{dim}(\mathcal{H})$. Every isometry preserves not only the Euclidean norm, but inner products as well: $\langle Au, Av \rangle = \langle u, v \rangle$ for all $u, v \in \mathcal{H}$. Isometries allow us to then define unitaries operators as the set of isometries $U:(\Hilb,\Hilb) \to \Hilb$ (which map $\Hilb$ to itself).

% %====Defn: unitary operator
% \begin{definition}[Unitary Operator]\label{defn:quant:Unitary Operator}
% An operator $U \in \mathcal{B}(\Hilb)$ is unitary if:
% \begin{align*}
% \langle U\phi, U\psi \rangle = \langle \phi, \psi \rangle
% \end{align*}
% (i.e. is surjective and maintains inner products) for all $\phi, \psi \in \Hilb$. Unitary operators preserve norms $\| U\psi \| = \| \psi \|$. 
% \end{definition}
% From this definition, we deduce that $\|U\| = 1$. $U$ is unitary if and only if $U^\dagger = U^{-1}$ such that $UU^\dagger = U^\daggerU = I$. Hermitian operators, unitary operators and positive semi-definite operators are central to quantum information processing (and the theory of quantum mechanics generally). Importantly, there is a bijection from the space of hermitian operators on the complex space $\Hilb$ to real Euclidean spaces. 
% Unitary operators represent propagators of quantum state vectors $\psi(t) \in \Hilb$ and, moreover, represent solutions to Schr\"{o}dinger's equation (which we discuss in more detail), forming a group. Not all evolution is unitary (e.g. open quantum systems) and measurement itself, however evolution of quantum systems modelled via unitary operators is usually the foundational basis for more complex models.

% From normal operators we obtain the spectral theorem which states that every normal operator $X \in \mathcal{B}(\Hilb)$ can be expressed as a linear combination of projection $\prod_k$ operators onto distinct orthogonal subspaces that allows the decomposition of such normal operator into the sum of (complex) eigenvalues and such projection operators. This fact is expressed via the spectral theorem.

% \begin{theorem}[Spectral Theorem]\label{thm:quant:spectral}
% Given $\Hilb$ with normal operator $X \in\mathcal{B}(\Hilb)$, there exists $\lambda_k \in \C$ ($k = 1,...,\dim\Hilb)$ and projection operators $\sum_k\Pi_k=I$ in $\text{Proj}(\Hilb)$ such that:
% \begin{align*}
% X = \sum_{k=1}^{m} \lambda_k \Pi_k
% \label{eqn:quant:spectral}
% \end{align*}
% \end{theorem}
% This decomposition is unique in the sense that each $\lambda_k$ corresponds to an eigenvalue of $X$, and each $\Pi_k$ projects onto a subspace formed by the eigenvectors associated with $\lambda_k$. Normal operators that may be decomposed in this way have an orthonormal basis, and the same basis may be used for decomposing commuting normal operators. In particular, both Hamiltonians $H$ and measurement operators are Hermitian [with real eigenvalues] such that the eigenvalues in equation (\ref{eqn:quant:spectral}) above are real. Among other things, this allows the Jordan-Hahn decomposition \cite{watrous_quantum_2002} where the spectral decomposition of $H=\sum_k \lambda_k \Pi_k$ is obtained via partitioning into:
% \begin{align}
%     P&=\sum_k\max\{ \lambda_k,0\} \Pi_k \qquad Q = \sum_k \max\{ -\lambda_k,0\} \Pi_k
% \end{align}
% for $P,Q \in Pos(\Hilb), PQ=0$, allowing $H$ to be written as:
% \begin{align}
%     H = P-Q
%     \label{eqn:quant:jordanhahn}
% \end{align}
% The spectral decomposition allows functions $f \in \C^m$ to be written as $f(X) = \sum_k f(\lambda_k) \Pi_k$. The spectral decomposition is also related to more general decompositions, such as singular value decompositions which hold for arbitrary $X \in \mathcal{B}(\Hilb)$, and polar decompositions (see \cite{watrous_theory_2018,hall_quantum_2013}) which are commonly used in machine learning contexts. They are also related to the later focus of this work in terms of generalised decompositions of Lie group manifolds, such as Cartan decompositions. We now define an important operator, the trace.
% \begin{definition}[Trace]\label{defn:quant:Trace}
% Given a non-negative self-adjoint $A \in \mathcal{B}(\Hilb)$ the trace of $A$ is given by:
% \begin{align*}
% \Tr(A)&=\sum_j \langle e_j, Ae_j \rangle,
% \end{align*}
% for an orthonormal basis $\{ e_j \}$ of $\Hilb$ (where $A$ is denoted `trace class' if $\Tr(A)$ is finite).
% \end{definition}
% Note that for any $A \in B(H)$, $A^\dagger$ is self-adjoint and non-negative. As a result, $\sqrt{A^\daggerA}$ is well-defined given that for such self-adjoint operators, for a bounded and measureable functional $f:\sigma(A) \to \C$ we have:
% \begin{align*}
% f(A)&=\int_{\sigma(A)}f(x)d\mu^A(x) \qquad A = \int_{\sigma(A)}x d\mu^A(x)
% \end{align*}
% where $\sigma(A)$ is a Borel $\sigma-$algebra and $\mu^A$ is a projection-valued measure on $\mu^A:\sigma(A) \to \Pi(\Hilb)$ (ee Appendix (\ref{app:Analysis and Measure Theory} for background)). The trace is independent of choice of orthonormal basis with standard properties such as cyclicity $\Tr(AB)=\Tr(BA)$ for $A,B \in \mathcal{B}(\Hilb)$. The trace operation can sometimes usefully be considered as a tensorial contraction of $A=A^i_j$ with $\delta^j_i$ i.e. $Tr(A)=A^i{}_j \delta^j_i$. For self-adjoint operators, the trace has associated eigenvalues $\lambda_j$ such that $\Tr(A)=\sum_j \lambda_j < \infty$. 

% An important operation to note from a measurement and machine learning perspective is the \textit{partial trace} operation below. We can define the partial trace as follows.
% \begin{definition}[Partial trace]\label{defn:quant:partialtrace}
% Given a tensor product of $X_k \in \mathcal{B}(\Hilb)$, the partial trace of $X_k$ with respect to the product state is:
%     \begin{align}
%     (\Tr_k \otimes I)(X_{k-1} \otimes X_k \otimes X_{k+1}) = \Tr(X_k)(X_{k-1} \otimes X_{k+1}) = \Tr_{X_k}(X_{k-1} \otimes X_{k+1})
% \end{align}
% \end{definition}
% Here $\Tr_k \otimes I$ is shorthand for the application of the trace operator to $X_k$. The partial trace has the effect of, in geometric terms (see below) contracting the relevant (tensor) product space (along the dimension associated with $X_k$) and scaling the residual tensor by the value of that trace in $\C$. In density operator formalism, the partial trace gives rise to a \textit{reduced density operator}. For $\rho_T$ representing the tensor product state $\Hilb_A \otimes \Hilb_B$, the partial tracing-out of $\Hilb_B$ in effect contracts the total tensor state up to a scalar $\trace_A$, that is:
% \begin{align}
%     \rho_A = \trace_B \rho_T \label{eqn:quant:reduceddensityoperator}
% \end{align}

% In later sections below, we note the relation of the trace to [differential forms] and quantum measurement. \hl{CHECK THIS IS DONE}



% \subsection{Density operators and multi-state systems}\label{sec:quant:Density operators and multi-state systems}
% Modelling multi-state and multi-qubit systems is an important feature of quantum information systems' research. It is also the primary focus of results in Chapters \ref{chapter:QDataSet and Quantum Greybox Learning} to \ref{chapter:Time optimal quantum geodesics using Cartan decompositions}. In the foregoing, typically a quantum system is described as an element of a Hilbert space $\psi \in \Hilb$ whose evolution is characterised by the operation of linear operators $\ket{\psi(t)}=U(t)\ket{\psi_0}$. However, for multi-state systems, this state formalism becomes convoluted when considering measurement and expectation outcomes of quantum systems. For multi-state systems, instead we introduce [completely positive] self-adjoint operators, denoted \textit{density operators}. Such operators are akin to generalised probability distributions over [expectations of observables]. Thus for a distribution $\phi$ of expectation values of observables of a measurement operator $M$, it can be shown that there exists a density operator $\rho$ where $\phi(M) = \Tr(\rho A)$. For unit vectors in $\Hilb$, this reduces to the projection of $M$ onto $\psi$ with expectation given by $\braket{\psi,M\psi}$. We now define a Hilbert-Schmidt operator in terms of the trace.
% %=====Defn:Hilbert-Schmidt
% \begin{definition}[Hilbert-Schmidt Operator]\label{defn:quant:Hilbert-Schmidt Operator}
% An operator $A \in \mathcal{B}(\mathcal{H})$ is Hilbert-Schmidt if $\text{trace}(A^\dagger A) < \infty$.
% \end{definition}
% All trace-class operators are Hilbert-Schmidt and the trace exhibits the usual cyclic property $\Tr(AB) =\Tr(BA)$. The inner product is given by $\braket{A,B}=\Tr(A^\dagger B)$ with the norm as per above $||A||^2 = \braket{A,A}$. With the concept of the trace we can also note a number of norms (and metrics) used further on, in particular relating to norms (and thus metrics) for comparing quantum states (such as trace-distance related measures) and in Chapter \ref{chapter:Time optimal quantum geodesics using Cartan decompositions} for variational techniques. Schatten p-norms are given by:
% \begin{align*}
%     ||X||_p = \left( \Tr \left((A^\dagger A)^{\frac{1}{2}}  \right)\right)^\frac{1}{p} \label{eqn:quant:Schatten p-norms}
% \end{align*}
% for $X \in \mathcal{B}(\Hilb)$. 
% Schatten norms are important in quantum information processing in that they are preserved under unitary transformations. Schatten 2-norms (where $p=2$) are sometimes denoted the \textit{Frobenius norm} which corresponds to the Euclidean norm of an operator $X$ represented as a vector $M \in M_c(\C)$:
% \begin{align}
%     ||M||_2 =\left( \sum_{j,k}|M(j,k)|^2\right)^{1/2} \label{eqn:quant:Frobenius norm}
% \end{align}
% ranging over indices $j,k$. For trace distance we have as follows.
% \begin{definition}[Trace distance]\label{defn:quant:Trace distance}
%     A Schatten p-norm such that $p=1$ is denoted the trace distance:
%     \begin{align}
%         ||X||_1 = \Tr(\sqrt{X^\daggerX})
%     \end{align}
% \end{definition}
% which also equals the sum of singular values of $X$. The trace distance is commonly used to compare distances of quantum states via their operator representation as density operators (matrices). 


% %====Density matrices
% \begin{definition}[Density operator]\label{defn:quant:Density operator}
% A density operator is an operator $\rho \in \mathcal{B}(\mathcal{H})$ that is self-adjoint and non-negative with $\Tr(\rho)=1$.
% \end{definition}
% Density operators tend to be the more formal representation of quantum states. The set of density operators is denoted $D(\Hilb)$ which can be shown to be a convex set. As Bengtsson et al. note \cite{bengtsson_geometry_2006} (see \S 8.7), this is crucial for the additional structure required for the set of such operators to form an algebra. For a state description given by alphabet $\Gamma$, such that $\rho_a \in D(\Hilb)$ (the density operator for the state described by $a$, which in practice depends upon measurement outcome expectations), it can be shown that:
% \begin{align}
%     \rho = \sum_{a\in\Gamma}p(a) \rho_a
% \label{eqn:quant:rhomixedstate}
% \end{align}
% Here $p$ describes the probability of observing (observations that characterise the system in state) $\rho_a$. Equation (\ref{eqn:quant:rhomixedstate}) describes a \textit{mixed state}. Such a description is of an \textit{ensemble} of quantum states which can be construed as a function $\eta:\Gamma \to Pos(\Hilb)$ such that $\Tr(\sum_{a\in\Gamma}\eta(a))=1$. Here the trace acts as a sort of normalising measure such that $\rho_a = \eta(a)/\Tr(\eta(a))$. Density matrices characterise expectation values of observables as families of expectation values via:
% \begin{align}
%     \Phi_\rho(A) = \Tr(\rho A) = \Tr(A\rho) \label{eqn:quant:measurementdensitymatrixtrace}
% \end{align}
% where $\Phi_\rho$ is a linear functional $\Phi_\rho:\mathcal{B}(\Hilb) \to \C$, associating operators on $\Hilb$ to scalar values in $\C$. The map $\Phi_\rho$ reflects a distribution of measurement outcomes satisfying $\Phi_\rho(I)=1$, $\Phi_\rho(A) \in \R$ for $A$ self-adjoint and non-negative if $A$ is non-negative. We denote $\rho=\ket{\psi}\bra{\psi}$ with $\Tr(\ket{\psi}\bra{\psi} A)=\braket{\psi,A\psi}$. Note also that relative phases $\psi_1 = e^{i\theta}\psi_2$ indicate the same states $\rho_1 = \rho_2$, reflecting the physical equivalence of states that differ only by a global phase. The trace norm above can then be used to calculate \textit{trace distance} as a measure of similarity as the Schatten 1-norm:
% %=====Trace distance
% \begin{definition}[Trace distance]\label{defn:quant:Tracedistance}
% Given two operators $\rho,\sigma \in \mathcal{B}(\Hilb)$ representing quantum systems, the trace distance between such operators is given by:
% \begin{align}
%     d_T(\rho,\sigma) = \frac{1}{2}||\rho - \sigma||_1 
% \end{align}
% \end{definition}
% Trace distance is considere a generalisation (in the quantum setting) of total variation distance between two probability distributions. The metric is a central component of the quantum machine learning objective (loss) functions used in Chapters \ref{chapter:QDataSet and Quantum Greybox Learning} and \ref{chapter:Time optimal quantum geodesics using Cartan decompositions}. Density matrices allow distinction between \textit{pure} states and \textit{mixed} states.

% \begin{definition}[Pure and Mixed States] \label{defn:quant:Pure and Mixed States}
% A density operator $\rho \in \mathcal{B}(\mathcal{H})$ represents a pure state if there exists a unit vector $\psi \in \mathcal{H}$ such that $\rho$ is equal to the orthogonal projection onto $span\{\psi\}$. The density matrix $\rho$ is called a mixed state if no such unit vector $\psi$ exists.
% \end{definition}
% Closed-system pure states remain pure under the action generated by Hamiltonians. For pure states, $\Tr(\rho^2)=1$ while for mixed $\Tr(\rho^2) < 1$. Density matrices form a convex set such that $\lambda \rho_1 + (1-\lambda)\rho2, \lambda \in (0,1)$. Pure states are those that cannot be expressed as $\rho = \lambda \rho_1 + (1-\lambda)\rho_2$ for $\rho_1 \neq \rho_2$. Mixed and pure states can also be conceived of such that if the state of a quantum system is known exactly $\ketpsi$, i.e. where $\psi = \ketpsi\bra{\psi}$ then it is denoted as a \textit{pure state}, while where there is (epistemic) uncertainty about its state, it is a mixed state i.e. $\rho = \sum_i p_i \rho_i$ where $\text{tr}(\rho^2)< 1$ (as all $p_i < 1$). Such properties of pure and mixed states are important tests for the effects of, for example, decoherence arising from various sources of noise (see Chapter \ref{chapter:QDataSet and Quantum Greybox Learning} for more detail).

% In many applications of quantum information processing, we seek a metric to ascertain similarity between quantum states. Density matrices can be used to define a metric such as quantum relative or von Neumann entropy noted in our discussion of metrics (relevant to quantum machine learning below in subsection \ref{sec:quant:quantummetrics}):
% \begin{definition}[Quantum relative (von Neumann) entropy]\label{defn:quant:quantumrelativeentropy}
%     Given a density matrix $\rho \in \mathcal{B}(\Hilb)$ for a quantum state and trace operation, we define the von Neumann entropy or quantum relative entropy as:
%     \begin{align*}
%         S(\rho) = \Tr(-\rho \log \rho)
%     \end{align*}
% \end{definition}
% A state $\rho$ is pure if an only if $S(\rho)=0$ and mixed otherwise. Density matrix formalism can be used to formally understand and express quantum superposition in terms of coherent (quantum) and incoherent superposition.

% \begin{definition}[Coherent Superposition]
% \label{defn:quant:coherent_superposition} For two quantum two states $\psi_1, \psi_2 \in \mathcal{H}$ with amplitudes $c_1, c_2 \in \mathbb{C}$, the state $c_1\psi_1 + c_2\psi_2$ is called \emph{coherent} if it cannot be transformed into another state with different relative phases. That is, such a state is coherent if the only case where:
% \begin{align*}
%     c_1e^{i\theta_1}\psi_1 + c_2e^{i\theta_2}\psi_2 = c_1\psi_1 + c_2\psi_2
% \end{align*}
% are physically the same state when $e^{i\theta_1} = e^{i\theta_2}$ for $\theta_1, \theta_2 \in \mathbb{R}$.
% \end{definition}
% Coherence is characterized by preservation of relative phases. By contrast, an \emph{incoherent superposition} of states $\psi_1, \psi_2 \in \mathcal{H}$ with probabilities $p_1, p_2 \geq 0$ such that $p_1 + p_2 = 1$ is described by the density operator $\rho = p_1 |\psi_1\rangle\langle\psi_1| + p_2 |\psi_2\rangle\langle\psi_2|$. The expectation value of an observable $A$ in this state is given by:
% \begin{align*}
% \Tr(\rho A) = p_1 \langle\psi_1, A\psi_1\rangle + p_2 \langle\psi_2, A\psi_2\rangle \label{eqn:quant:incoherent_superposition}
% \end{align*}
% We now briefly describe quantum channels due to their relevance, in our context, to measurement and system evolution.

% %====Quatum channels

% \subsubsection{Quantum channels}\label{sec:quant:Quantum channels}
% The concept of a \textit{channel} derives from information theory \cite{shannon_mathematical_1948} as a way of abstracting a medium or instrument of information transfer. The concept has since been adapted for application in quantum information theory such that a\textit{ quantum channel} is a linear map from one space of square operators to another, that satisfies the two conditions of (complete) positivity and trace preservation.

% %====(Definition of a quantum channel)
% \begin{definition}[Quantum Channel]\label{defn:quant:Quantum Channel}
% A quantum channel  is a linear map
% \begin{align*}
%     \Phi \colon \mathcal{B}(\mathcal{H}_1) \to \mathcal{B}(\mathcal{H}_2)
% \end{align*}
% such that $\Phi$ is (a) completely positive and (b) trace-preserving. Maps satisfying these two properties are denoted CPTP maps.
% \end{definition}
% The set of such channels is denoted \(C(\mathcal{H}_1, \mathcal{H}_2)\). Denote \(C(\mathcal{H})\) for \(C(\mathcal{H}, \mathcal{H})\). Of particular importance is the concept of \textit{unitary channels}.
% %====(Example of a unitary channel)
% \begin{definition}[Unitary Channel]\label{defn:quant:Unitary Channel}
% Given the unitary operator \(U \in \mathcal{B}(\mathcal{H})\), then the following map is a unitary channel:
% \begin{align*}
%     \Phi(X) = U X U^\dagger
% \end{align*}
% for every \(X \in \mathcal{B}(\mathcal{X})\) (e.g. $X = \rho)$ is an example of a channel, being a completely positive, trace-preserving (CPTP) map. 
% \end{definition}
% Such channels represent an idealised channel or memory operator, as operating on the quantum state causes no change in the state of the register \(\psi\) it acts upon (in this sense representing a fixed point operator with respect to the register state) \cite{watrous_theory_2018}. For multi-state systems, there exist product channels $C(\otimes_k\mathcal{X}_k,\otimes_k\mathcal{Y}_k)$. The trace operator can also be construed as a channel. For problems in quantum control and geometry explored below, we are mainly interested in learning the CPTP map $\Phi:U(0) \to U(T)$ satisfying some optimality condition, such as minimisation of evolution time or energy. Channels play a crucial role across quantum information processing, giving rise to considerations such as optimal representations (distinct from Lie group representations) for such channels. Importantly, the class of channels we seek to learn preserves those essential properties of quantum operators above, such as Hermiticity and trace-preservation (ensuring, for example, we remain within the closure of unitary or special unitary groups when formulating unitary sequences). Other standard results for channels, such as that for $\Hilb_1,\Hilb_2$, the set $C(\Hilb_1,\Hilb_2)$ is compact and convex are important in guaranteeing the controllability and reachability of target unitaries. We direct the reader to \cite{watrous_theory_2018} for more detailed exposition.

% In the formalism of quantum information, we can also cast measurements as channels mapping to classical registers in $\R^n$. For this purpose, we introduce the notion of a quantum-classical channel.
% \begin{definition}[Quantum-classical channel]\label{defn:quant:Quantum-classical channel}
%     A quantum-classical channel is a CPTP map
%     \begin{align*}
%         \Phi \in C(\Hilb_1,\Hilb_2)
%     \end{align*}
%     which transforms a quantum state $\rho_1 \in \mathcal{B}(\Hilb_1)$ into a classical distribution of states represented by a diagonal density matrix $\rho_2 \in \mathcal{B}(\Hilb_2)$. The channel is realised via a measurement comprising a dephasing channel component $\Delta$ that eliminates off-diagonal (coherent) elements i.e. it is a quantum-classical channel if $\Phi=\Delta\Phi$ where $\Delta \in C$ is a dephasing channel which has the effect of transforming off-diagonal entries in $\rho_1 \in \mathcal{B}(\Hilb_1)$ to zero while preserving diagonal entries.
% \end{definition}
% Reiterating our discussion of density operators above, this equivalent to $\Phi:\rho \to \rho'$ where $\rho'$ is a diagonal density operator. As Watrous notes, these quantum-classical channels are those which can be represented as measurements of quantum registers $X$, formally described by $\rho$, with measurement outcomes $m$ stored in a register $Y$ with classical state set $\Sigma$. It can be shown that for every such channel $\phi \in C$, there exists a unique (measurement) $\mu:\Sigma \to Pos(\Hilb)$ such that (connecting standard notation with Watrous's notation):
% \begin{align}
%     \Phi(X) &=\sum_{m\in\Sigma}\braket{\mu(m),X}E_{a,a}\\
%     &=\Phi(\rho) = \sum_{m \in \Sigma} (M_m \rho M_m^\dagger) = \sum_{m \in \Sigma} p_m E_m \label{eqn:quant:measurementaschannel}
% \end{align}
% where $p_m = \mathrm{Tr}(M_m \rho M_m^\dagger)$ is the probability of obtaining outcome $m$, and $E_m$ represents the eigenstates corresponding to outcome $m$ projected onto a diagonal basis (i.e. diagonalised with entries corresponding to measurement outcomes equivalent to $E_{a,a}$ diagonal basis operators) to represent the post-measurement state. Quantum-classical channels are general measurement channels in quantum information. Other features of quantum-classical channels, such as their compactness and convexity over $\Hilb$ and the existence of product measurements (for multi-state systems) are noted in the literature (and ultimately important to both control/ reachability and the learnability (via machine learning algorithms) of such mappings explored in later chapters). We explore their implementation in terms of machine learning techniques in later chapters. Another concept of importance in measurement and quantum machine learning is that of partial measurements, especially the relationship between partial measurements and the partial trace operation.
% \begin{definition}[Partial measurement]\label{defn:quant:Partial measurement}
%     For a compound (quantum) state register $X=(Y_k), k=1,...,n$ a measurement on a single register $\mu:\Sigma \to Pos(Y_k)$ is denoted a partial measurement.
% \end{definition}
% Partial measurements thus related to partial traces and, in geometric contexts (as discussed below), contraction operations over tensor fields (where the trace operation can, under certain geometric conditions relevant to quantum control, be related to tensorial contraction).

% %====Quantum evolution: Hamiltonian formalism
% \subsection{Quantum evolution}\label{sec:quant:Quantum evolution}
% We now consider the evolution of quantum systems, beginning with the evolution axiom (adapted from the literature including \cite{hall_quantum_2013}).

% \begin{axiom}[Evolution]\label{axiom:quant:evolution}
% Quantum state evolution is described by the following first-order differential equation, denoted the Schr\"{o}dinger equation: 
% \begin{align}
%     i\frac{d\psi}{dt} = H\psi \label{eqn:quant:schrodingersequation}
% \end{align}
% where $\psi \in \Hilb$ and  $H\in\mathcal{B}(\Hilb)$ is a fixed Hermitian operator denoted as the Hamiltonian. In the standard way we set $\hbar=1$ for convenience. 
% \end{axiom}
% We examine the formalism and consequences of this axiom below. In later chapters, we connect the evolution of quantum systems to geometric and algebraic formalism (in terms of transformations along Lie group manifolds). Before we do so, we include a short digression on the two perspectives of quantum evolution formalism.
% \subsubsection{Two pictures of quantum evolution}\label{sec:quant:Two pictures of quantum evolution}
% Quantum mechanics is traditionally portrayed as being describable by two somewhat different but mathematically equivalent formulations, the Schr{\"o}dinger picture, focusing on state evolution and the Heisenberg picture, focusing on operator evolution \cite{sakurai_modern_1995}.  In the Schr{\"o}dinger picture, the quantum system is represented by a wavefunction $\ket{\psi(t)}$ parametrised by time $t$ and which evolves according to equation (\ref{eqn:quant:schrodingersequation}). In this picture, the operators, representing observable, that act on $\ket{\psi(t)}$ are time-independent. Measurement probabilities of an observable (see below) are given by the inner product of $\ket{\psi(t)}$ with the observable eigenvector. By contrast, in the Heisenberg picture quantum state vectors are time-independent $\ketpsi$ and it is the operators $\hat{O}(t)$, corresponding to measureable observables, which evolve in time as:
% \begin{align*}
%     \hat{O}(t) = e^{iHt}\hat{O}(0)e^{-iHt}
% \end{align*}
% % Quantum computing formalism often adopts a more Heisenberg-style picture, particularly because of the requirements of unitarity (where $\hat{O}(t) \dot = U(t)$).
% We also mention these well-known formalisms as we can connect both with a more geometric formalism for expressing quantum evolution in Chapters \ref{chapter:Quantum Geometric Machine Learning} and \ref{chapter:Time optimal quantum geodesics using Cartan decompositions}, such as the Maurer-Cartan forms and the adjoint action of Lie groups. It is also worth mentioning the hybrid \textit{interaction} (or von Neumann) picture in which both states and operators evolve, expressed (as we discuss further on) in terms of the Liouville von Neumann equation (for closed quantum systems) and  equation (for open quantum systems \cite{wiseman_quantum_2010}):
% \begin{align}
% \dot{\rho} & = -i[H, \rho] + \kappa \mathcal{D}[\hat{O}]\rho \qquad \mathcal{D}[\hat{O}]\rho = \hat{O}\rho\hat{O}^\dagger  - \frac{1}{2}(\hat{O}^\dagger \hat{O}\rho + \rho \hat{O}^\dagger \hat{O}) \label{eqn:quant:masterequation}
% \end{align}
% where each term is parametrised by $t$ (omitted for brevity). Here $\hat{O}$ is an arbitrary operator, $\mathcal{D}$ is a superoperator term acting to transition quantum (density) operators (in this case, density operators) $\rho$ and $\kappa$ the decoherence rate.
% The interaction picture is specifically relevant to our greybox open quantum systems' simulations for machine learning that is the subject of Chapter \ref{chapter:QDataSet and Quantum Greybox Learning}. We include below a number of standard definitions and results relevant to understanding the operator formalism used throughout this work. Later we connect such formalism to geometric and algebraic methods, along with formalism in quantum machine learning. [We also briefly mention the role of time $t$ in Chapter \ref{chapter:Background: Geometry, Lie Algebras and Representation Theory}] in terms of the matrix exponential $e^{tX}$ which, for Lie algebra generators $X \in \g$ (and corresponding group $G$), is expressed as the unique one-parameter (i.e. a parameter denoted as time) subgroup of $G$ whose tangent vector $d/dt$ at the identity is $X$ (i.e. $d(e^{tX})/dt \big|_{t=0} \to X(e^{tX})$ .

% %=====Hamiltonian formalism

% \subsection{Hamiltonian formalism}\label{sec:chapter1:evolution:Hamiltonian formalism}
% In density operator formalism, state evolution in Axiom (\ref{axiom:quant:evolution}) is described via:
% \begin{align}
%     \frac{d\rho}{dt} = -i[H,\rho] \qquad \rho(t) = e^{-iHt}\rho_0e^{iHt}
% \end{align}
% for $\rho_0=\rho(t=0)$. In unitary operator formalism, the above can be written:
% \begin{align}
%     dU U^\inv = -iHdt \label{eqn:quant:schrodingerdUUinv}
% \end{align}
% where $\psi(t) = U(t)\psi_0$. It is useful to unpack this formalism. First, we define the Hamiltonian. In later chapters, we connect the Hamiltonian to geometric, algebraic and variational principles (such as the framing of equation (\ref{eqn:quant:schrodingerdUUinv}) in terms of the Maurer-Cartan form).
% \begin{definition}[Hamiltonian operator]\label{defn:quant:Hamiltonian}
%     The operator $H \in \mathcal{B}(\Hilb)$ described in equation (\ref{eqn:quant:schrodingerdUUinv}) is a self-adjoint (Hermitian) denoted the Hamiltonian. The Hamiltonian operator is described as the generator of quantum evolutions. 
% \end{definition}
% The Hamiltonian $H(t) \in \mathcal{B}(\Hilb)$ of a system is the primary means of mathematically characterising the dynamics of quantum systems. Hamiltonians specify the data-encoding process by which information is encoded into quantum states along with how the system evolves and how the quantum computation may be controlled.  Solutions to equation (\ref{eqn:quant:schrodingerdUUinv}) are of the form:
% \begin{align}
%     U = \mathcal{T}_+\exp\left(-i\int_0^{\Delta t} H(t) dt\right) \label{eqn:quant:unitarysolutiontimedependentschrod}
% \end{align}
% where $\mathcal{T}_+$ is the time-ordering operator (described below). As can be seen, $U$ is unitary as $UU^\dagger = I$ (the adjoint action has no effect on $\mathcal{T}_+$). Being unitary, these solutions at once can be represented as linear operators on $\Hilb$ that preserve inner products (see definition \ref{defn:alg:Unitary matrix and unitary group}) and Haar measure (see definition \ref{defn:app:Haarmeasure} in the Appendix). As per definition (\ref{defn:quant:Unitary Channel}), these solutions can be represented as unitary channels acting on density operators via $\Phi(\rho) = U\rho U^\dagger$. Unitary evolution itself is required to preserve quantum coherence and probability measures of systems (which give rise to the enhanced computational power of quantum systems). Moreover, as we discuss in Chapter \ref{chapter:Background: Geometry, Lie Algebras and Representation Theory}, the set of unitaries forms a Lie group (see definition \ref{defn:alg:Unitary matrix and unitary group}) and so has a natural geometric interpretation in terms of a Lie group manifold $G$ whose evolution is described by a Hamiltonian composed of generators of the corresponding Lie algebra $\g$. 


% \subsubsection{Time-independent approximations}\label{sec:quant:Time-independent approximations}
% Solving the time dependent Schr\"odinger equation given in definition \ref{eqn:quant:schrodingersequation} is often challenging or unfeasible, requiring perturbation methods or other techniques. A common approximation used in quantum information processing and quantum control is the \textit{time-independent} approximation to the Schr\"odinger equation. Recall from equation (\ref{eqn:quant:unitarysolutiontimedependentschrod}) the time-dependent solution to the close-system Schr\"odinger equation is given by:
% \begin{align}
%         U(T) &= \mathcal{T}_{+} e^{-i\int_0^T H(t) dt}
%     \end{align}
% The time-ordering reflects the fact that the generators within the time-dependent Hamiltonian do not, in general, commute at different time instants (i.e. $[H(t_i), H(t_j)]\neq 0$). In certain cases, a time-independent approximation to equation (\ref{eqn:quant:unitarysolutiontimedependentschrod}) may be adopted:
% \begin{align}
%     U(t) &= \mathcal{T}_{+} e^{-i\int_0^T H(t) dt}\\
%     &\simeq \lim_{N\to \infty} e^{-i H(t_N) \Delta T} e^{-i H(t_{N-1}) \Delta T} \cdots  e^{-i H(\Delta t_0) \Delta T} \label{eqn:quant:timeindependentschrodunitary}
% \end{align}
% where $\Delta T = T/N$ and $t_j = j \Delta T$. 
% Note also the Suzuki-Trotter decomposition \cite{childs_theory_2021,suzuki_generalized_1976} and Lie-Trotter formulation:
%     \begin{align}
%         e^{-i(H_1+H_2)}= \lim_{n\to \infty}\left( e^{-i(H_1/n)}e^{-i(H_2/n)}\right)^n \label{eqn:quant:suzukitrotter}
%     \end{align}
%     which under certain conditions allows the time-varying Hamiltonian to be approximated by a piece-wise constant Hamiltonian. Equation (\ref{eqn:quant:suzukitrotter}) can be seen via:
%     \begin{align*}
%     e^{-i(H_1+H_2)t} &= \lim_{n\to\infty} \left(1 + \frac{-i(H_1 + H_2)t}{n}\right)^n \\
%     &= \lim_{n\to\infty} \left(1 + \frac{-iH_1t}{n}\right)^n\left(1 + \frac{-iH_2t}{n}\right)^n \\
%     &= \lim_{n\to\infty} \left(e^{-iH_1t/n} e^{-iH_2t/n}\right)^n
% \end{align*}
% where we have applied equation (\ref{eqn:alg:exponentiallimit}).  Here the time interval $[0,T]$ is divided into equal segments of length $\Delta t$ while the Hamiltonian is considered constant over that interval. Moreover, even when only a subset of the Lie algebra $\g$ is available, we may be able to achieve universal control (that is, the ability to synthesise all generators, by repeated application of the control Hamiltonian) via commutator terms that in turn allow us to generate the full generators of the corresponding Lie algebra. This is discuss in later chapter in terms of the distribution $\Delta$ (a geometric framing of our set of generators) being `bracket-generating'. This can be shown via the approximation:
%     \begin{align}
%         e^{-i[H1,H2]}= \lim_{n\to \infty}\left( e^{-iH_1/n}e^{-iH_2/n}e^{iH_1/n}e^{iH_2/n}\right)^n
%     \end{align}
%     The approximation is generally available under the assumption that the Hamiltonian over increments $\Delta t$. Of central importance to time-independent approximations it the \textit{Baker Campbell Hausdorff} formula (definition \ref{defn:alg:Baker-Campbell-Hausdorff}). For universal control in quantum systems, repeated application of the control Hamiltonian allows us to synthesize all generators of the Lie algebra corresponding to the system's dynamics. This is where the BCH formula becomes crucial, as it allows for the generation of effective Hamiltonians that include commutator terms, thus expanding the set of reachable operations. For example, the BCH formula shows us that by carefully sequencing the application of $H_1$ and $H_2$, we can effectively implement the commutator $[H_1, H_2]$ as part of the evolution:
% \begin{align}
%     e^{-i[H_1,H_2]\Delta t} \approx \left( e^{-iH_1\Delta t/n}e^{-iH_2\Delta t/n}e^{iH_1\Delta t/n}e^{iH_2\Delta t/n}\right)^n
% \end{align}
% for sufficiently large $n$ and small $\Delta t$. This approximation is powerful for designing control sequences in quantum systems with non-commuting dynamics.
    

    

% \subsubsection*{Expectation evolution}\label{sec:quant:Expectation evolution}
% The evolution of quantum states can also be characterised in terms of changes in measurement statistics over time. That is, equation \ref{eqn:quant:schrodingerdUUinv} can also be used to model the evolution of the measurement statistics \cite{hall_quantum_2013}. Recall that if $A \in \mathcal{B}(\Hilb)$ is Hermitian then the expectation value of $A$ for state $\psi \in \Hilb$ is:
% \begin{align}
%     \braket{A}_\psi = \braket{\psi,A\psi} = \trace(\rho A)\label{eqn:quant:averagevalue}
% \end{align}
% Equation (\ref{eqn:quant:averagevalue}) above expresses the same principle of equation (\ref{defn:app:Expectation}) in operator formalism with the inner product. The uncertainty (variance) in measurements of $A$ is given by:
% \begin{align}
%     (\Delta A)^2 = \braket{A^2}_\psi - (\braket{A}_\psi)^2
% \end{align}
% The expectation value together with the uncertainty of measurements of $A$ are important measurement statistics of $A$ with respect to state $\psi$. We are also often interested in how measurement statistics evolve over time which can be modelled as:
% \begin{align}
%     \frac{d}{dt}\braket{A}_\psi = \braket{-i[A,H]}
% \end{align}
% where $[\cdot,\cdot]$ denotes the commutator $[A,B]=AB-BA$. The commutator (in the form of the Lie derivative) is more fully described in Chapter \ref{chapter:Background: Geometry, Lie Algebras and Representation Theory} and proposition (\ref{prop:alg:Lie derivative properties}).






     


% \subsection{Measurement}\label{sec:quant:Measurement}
% Measurement is at the centre of quantum mechanics and quantum information processing. In the section below, we set out two further axioms relating to measurement, adapted from the literature (see \cite{hall_quantum_2013,nielsen_quantum_2011}). The first concerns measurement and operators. The second concerns the characterisation of post-measurement states. Measurement formalism varies to some degree depending on how information-theoretic an approach adopted is. We incorporate elements of both the traditional and information-based formalism. We have aimed to present a useful coverage of measurement formalism specifically tailored to later chapters, where measurement plays a critical role, for example, in both simulated quantum systems (for use in state description and other tasks) and machine learning. The first axiom defines measurement. We split this into two in terms of (a) measurement probabilities (e.g. the Born rule) and (b) the effect of measurement (wave collapse). Note here we adopt an operator formalism where measurement is represented by a set of operators $\{M \}$ the outcomes of which are measurements $m \in \Sigma$ (i.e. mapping to our register configurations). Connecting to above, we can write $\{M_m | m \in \Sigma \} \subset Pos(\Hilb)$.

% \begin{axiom}[Measurement]\label{axiom:quant:probabilitymeasurement}
% Given $\psi \in \mathcal{H}$, the probability distribution for the measurement of an observable $m$ is such that $E[M^k] = \braket{ \psi, M^k \psi }$. Given an orthonormal basis $\{e_j\}$, we may write $\psi = \sum_j^\infty a_j e_j, a_j \in \C$ with measurement probability of observing $m_j$ given by $P(M=m_j)=|a_j|^2$ (the Born rule).
% \end{axiom}
% The reference to $M^k$ (following Hall) is to the fact that the $k$-th power of the measurement operator $M$ corresponds to the $k$-th moment of the probability distribution for measurement outcomes associated with $M$ (i.e. expectation, variance and so on). 
% The second measurement axiom (which can be viewed as an extension of the first) describes the effect of measurement on quantum states, namely the collapse of the wave function into eigenstates of the measurement operator. 
% \begin{axiom}[Effect of Measurement]\label{axiom:quant:effectofmeasurement}
% Measurement via measurement operator $M$ with measurement outcome $m \in \mathbb{R}$, causes a quantum system transition to $\psi' \in \Hilb$ such that $M\psi' = m\psi'$ where \( m \) is the eigenvalue of \( M_m \) corresponding to the observed outcome, and \( \psi' \) is the corresponding eigenstate of \( M_m \). 
% \end{axiom}
% These postulates can be expanded to encompass multiple possible measurement outcomes whereby quantum measurements are framed as sets of measurement operators $\{ M_m\}$, where $m$ indexes the outcome of a measurement (e.g. an energy level or state indicator), i.e. an observable. The probability $p(m)$ of observable $m$ upon measuring $\ketpsi$ is represented by such operators acting on the state such that measurement probability is given by:
% \begin{align}
%     p(m) = \braket{\psi | M_m^\dagger M_m |\psi}  = \text{tr}(M_m^\dagger M_m \rho)
% \label{eqn:quant:measurementprobinnerproduct}
% \end{align}
% with the post-measurement state $\ket{\psi'}$ given by: 
%     \begin{align}
%         \ket{\psi'} &= \frac{M_m \ketpsi}{\sqrt{\braket{\psi | M_m^\dagger M_m | \psi}}}
%         \label{eqn:quant:postmeasurementstate}\\
% \rho'&=\frac{M_m\rhoM_m^\dagger}{\braket{M_m^\dagger M_m,\rho}} \label{eqn:quant:postmeasurementstatedensity}
%     \end{align}
%     The set of measurement operators $\sum_m M_m^\dagger M_m = I$ reflects the probabilistic nature of measurement outcomes. Importantly, measurement is modelled as a random variable in $\Sigma$, described by the probability distribution $p \in \mathcal{P}(\Sigma)$.
%     % calculated via the inner product $p(m) = \braket{\mu(m),\rho}$. 
%     The act of measurement transitions $M:\rho \to \rho'$ described by equation (\ref{eqn:quant:postmeasurementstate}). 
    
%     In quantum information theory, we further refine the concept of measurement as per below.
% \begin{definition}[Measurement]\label{defn:quant:Measurementchannel}
%     A measurement is defined in terms of a probability measure from the set of measurement outcomes to the set $Pos(\Hilb)$:
%     \begin{align}
%         \mu: \Sigma \to Pos(\Hilb) \qquad m \mapsto \mu(m) := M_m \qquad \sum_{m\in\Sigma} \mu(m)= I
%     \end{align}
% \end{definition}
% \hl{Check $\mu(m)$ def here and channel below; also make clear for each operator $M$ have $m_j$ different outcomes and may have a number of operators $M$ (not entirely clear here)}
% Here $\Sigma$ is the set of measurement outcomes $m$ (which describe our quantum state $\rho$) following application of $M_m$ (note we include $\mu(m) := M_m$ as a bridge between the commonplace formalism of Nielsen et al. \cite{nielsen_quantum_2011} and the slightly more information theoretic form in Watrous \cite{watrous_theory_2018}. In this notation (from \cite{watrous_theory_2018}), $p(m) = \braket{\mu(m),\rho}$.
% When a measurement is performed on a system described by the density operator $\rho$, the probability of obtaining outcome $m$ is given by 
% \begin{align}
% p(m) = \text{Tr}(M_m \rho M_m^\dagger),
% \end{align}
% and the state of the system after the measurement (post-measurement state) is 
% \begin{align}
% \rho_m = \frac{M_m \rho M_m^\dagger}{p(m)}.
% \end{align}
% Recall the expectation 
% This measurement process can be described by a quantum channel $\mathcal{E}$ that maps the initial density operator $\rho$ to a final density operator $\rho'$ that is a mixture of the post-measurement states, weighted by their respective probabilities:
% \begin{align}
% \rho' = \mathcal{E}(\rho) = \sum_m p(m) \rho_m = \sum_m M_m \rho M_m^\dagger \label{eqn:quant:measurementsuperoperatordensity}
% \end{align}
%     Connecting the standard terminology with the more information terminology for measurement, we note that $\{M_m | m \in \Sigma \} \subset \mathcal{B}(\Hilb)$ such that $\sum_{m}M^\dagger_m M_m = I$. Measurement then corresponds $m \in \Sigma$ being selected at random (i.e. modelled as a random variable) with probability given by equation (\ref{eqn:quant:measurementprobinnerproduct}) and post-measurement state given by equation (\ref{eqn:quant:postmeasurementstatedensity}). Such measurements are described as \textit{non-destructive measurements}. 

%     \subsubsection{POVMs and Kraus Operators} \label{sec:quant:POVMs and Kraus Operators}
%     In more advanced treatments, positive-operator valued measure (POVM) formalism more fully describes the measurement statistics and post-measurement state of the system. For a POVM, we define a set of positive operators $\{  E_m \}=\{M^\dagger_m M_m\}$ satisfying $\sum_m E_m=\mathbb{I}$ in a way that gives us a complete set of positive operators (such formalism being more general than simply relying on projection operators). In this way the measurement operators $M$ can be regarded as \textit{Kraus operators} satisfying the requisite completeness relation [\textbf{KRAUS STATES},\textbf{HELLWIG KRAUS}]. 
%     As we are interested in probability distributions rather than individual probabilities from a single measurement, we calculate the probability distribution over outcomes via Born rule using the trace:
%     \begin{align}
%         p(E_i) = \Tr(\rho E_i)  \qquad \braket{A} = \trace(\rho A) \label{eqn:quant:measurementtracePOVM}
%     \end{align} noting the expectation as per equation (\ref{eqn:quant:measurementdensitymatrixtrace}).
%     Measurement thus has a representation as a quantum to classical channel $\Phi_M \in C(\X,\Y)$ (see definition (\ref{defn:quant:Quantum-classical channel})) under the condition that it is completely dephasing with $\Phi_M(\rho)$ is diagonal for all $\rho \in D(\X)$. Such quantum-to-classical channels are those that can be realised as a measurement of a register $X$. As Watrous ($\S$2.3) notes, there is a correspondence between the mapping of measurement outcomes $m$ to operators $M \in \Pos(\X)$. Combining Watrous and Nielsen et al.'s formalism, $\Phi(X)$ describes a classical description (distribution) of the outcome probabilities when a quantum state $\rho$ is measured:
% \begin{align*}
%     \Phi_M(\rho) = \sum_{m \in \Sigma} \trace(M_m \rho M_m^\dagger)\ketbra{m}{m} = \sum_{m \in \Sigma} \braket{\mu(m),\rho}E_m \label{eqn:quant:measurementchannel1}
% \end{align*}
%     \\
%     \\
%     Further discussion of measurement procedures is set out below (such as in Chapter \ref{chapter:QDataSet and Quantum Greybox Learning}). Note that measurements described in the section give rise to a set of measurement statistics and that these are used, e.g. via process or state tomography, to reconstruct or infer the state $\ket{\psi}$ or channel $U$. Note that the outcome of meausrements is a set of measurements $\{ m_j \}$ from which measurement statistics are calculated. Such statistics are then used to infer or reconstruct data describing quantum states (or in operator formalism the channels or operators $U(t)$ themselves. In practice, for sequences of unitaries $(U_n(t))$ or quantum states $\ket{\psi}$, because of state collapse (\ref{axiom:quant:effectofmeasurement}), we assume that we cannot measure each unitary at each time point $t$ (albeit see discussion on post-selection measurement based quantum computing).

% \subsubsection*{Composite system measurement}\label{sec:quant:Composite system measurement}
%     For composite systems, a measurement of the $k$-th state $\rho_k$ (or $X_k$ depending on formalism) will result in a post-measurement state conditional upon that measurement. The state $\rho_k$ will `collapse' onto one of the eigenvectors of the measurement operator $M_m$ corresponding to the observable $m$ obtained. In composite systems, because of the distributivity of scalar multiplication, the post-measurement state is then a tensor product of the original states with that eigenvector state scaled by the measurement outcome (then renormalised). This can be expressed as:
% \begin{align}
%     \eta&:\Sigma \to Pos(\otimes_k X_k)\\
%     \eta(m)&=\Tr_{X_k}(I_{k-1} \otimes \mu(m) \otimes I_{k+1})(\rho)
% \end{align}
% where $X_k \in \Hilb_k$ (note sometimes the trace above is denoted $\trace_{\Hilb_k}$ to indicate tracing out of the $k$-th subsystem). The measurement $\mu(m)$ essentially maps $X_k$ (which, recall, could be a superposition state) to a classical state scaled by $m$ (and in this sense we can think of measurement as a tensorial contraction as discussed in later chapters). In this formalism, the post-measurement state in equation (\ref{eqn:quant:postmeasurementstate}) becomes where the denominator is the normalisation scalar:
% \begin{align}
%     \rho'&=\frac{\eta(m)}{\Tr(\eta(m)} = \frac{\Tr_{X_k}(I_{k-1} \otimes \mu_k(m) \otimes I_{k+1})(\rho)}{\braket{\mu(m),\rho_k}}
% \end{align}
% We are also concerned in particular with projective measurements where each measurement is a projection operator i.e. $\mu(m) \in Proj(\Hilb)$. Each projective measurement projects the state $\rho$ into an eigenstate of the respective projection operator. The set of such operators $\{ \mu(m) | m \in \Sigma \}$ is an orthogonal set, which means there are at most $\dim \Hilb$ distinct observables $m$. It can be shown that any measurement can be framed as a projective measurement.

% %=====POVM
% \subsubsection{Informational completeness and POVMs}\label{sec:quant:Informational completeness and POVMs}
% In more advanced treatments, positive-operator valued measure (POVM) formalism more fully describes the measurement statistics and post-measurement state of the system. For a POVM, we define a set of positive semi-definite operators $\{  E_m \}=\{M^\dagger_m M_m\}$ satisfying $\sum_m E_m=\mathbb{I}$ in a way that gives us a complete set of positive operators (such formalism being more general than simply relying on projection operators). 
% %====(Definition of Positive Operator-Valued Measures (POVMs))
% \begin{definition}[POVM]\label{defn:quant:POVM}
% A \textit{Positive Operator-Valued Measure (POVM)} on a Hilbert space $\mathcal{H}$ is a set $\{E_m\}$ of operators that satisfies the following conditions:
% \begin{align}
%     &E_m \geq 0 \quad \forall m \qquad \sum_m E_m = I_{\mathcal{H}}.
% \end{align}
% \end{definition}
% Here, $E_m$ represents the effect corresponding to the measurement outcome $m$, and $I_{\mathcal{H}}$ is the identity operator on $\mathcal{H}$. The operators $E_m$ are positive semi-definite and the set $\{E_m\}$ is complete in the sense that it sums to the identity, ensuring that probabilities over all outcomes sum to one.

%     To estimate probability distributions, we calculate the probability distribution over outcomes via Born rule using the trace $p(E_i) = \Tr(\rho E_i)$. Further discussion of measurement procedures is set out below (such as in Chapter \ref{chapter:QDataSet and Quantum Greybox Learning}). 

% We are also interested, in a quantum machine learning context, to utilise informationally-complete measurements, where the set of measurements span the entire space $\mathcal{B}(\Hilb)$. This is because quantum states are uniquely determined by their measurement statistics. For problems such as state identification (tomography) and other typical tasks, understanding the underlying probability distribution for each measurement outcome enables a complete description of that state (or in Watrous's terminology, a full description of the register). 
% \begin{definition}[Informationally-complete measurements]\label{defn:quant:Informationally-complete measurements}
%     A measure $\mu:\Sigma \to Pos(\Hilb)$, is informationally complete if $\spn \{ \mu(m) | m \in \Sigma \} = \mathcal{B}(\Hilb)$.
% \end{definition}
% For diagonal states $\rho \in D(\Hilb)$, the probability vector $p \in \mathcal{P}(\Sigma)$ completely specifies $p$, which intuitively shows how density operators can be thought of as operator-analogues of probability distributions over classical states (registers). See \cite{watrous_theory_2018} for more generalised descriptions in terms of instruments. An example of a choice of informationally complete 

% Finally we briefly note extremal measurements, which is a quantum-classical channel corresponding to an extreme point of all quantum-classical channels $C(\Hilb)$. A measurement $\mu$ is extremal if for all measurement choices $\mu_j,\mu_k$ with $\mu = \lambda \mu_j + (1-\lambda)\mu_k$ for $\lambda \in (0,1)$ we have $\mu_j = \mu_k$, Extremal measurements are those that cannot be expressed as non-trivial convex combinations of other POVM elements. We don't expand upon these types of measurements but note that extremal POVMs are often associated with obtaining maximum information about a quantum system. They are optimal in the sense that no other measurement can provide strictly more information about the quantum state with the fewest measurement outcomes (hence potentially providing better training data sets from a statistical learning perspective for tasks such as state discrimination). Extremal measurements are relevant to optimal design of experiments in order to assist statistical learning processes by offering data that captures the most distinct features of the quantum state's behavior.



% % \subsection{Functional analysis and measure theory}
% % We briefly note a few key elements of functional analysis and measure theory, in particular the role and relevance of the Haar measure. In quantum information processing, we are usually interested in unitarily invariant measures, being Borel measures (for quantum states or operators) invariant under hte action of unitary groups. Apart from their general application in quantum information processing theory, such considerations are important to sampling strategies when training machine learning models.
% % \hl{NB: move up to earlier stage, paraphrase key results in Watrous 1.2, 2.3 etc. Consider discussion maybe re Watrous register and states (may be too convoluted); also Watrous Channel section - paragraphse; for Fidelity, see Watrous 3.2}


% \subsection{Quantum entanglement}\label{sec:quant:Quantum entanglement}
% A fundamental (or in Schr\"odinger's estimatin, \textit{the} fundamental) distinguishing property of quantum mechanics from its classical counterpart is the phenomenon of entanglement. Entanglement has a few different but equivalent defintiions, such as being a state $\rho$ which cannot be represented as a tensor product state (definition \ref{defn:quant:Tensor Product}). More formally, entanglement can be defined as per below.
% \begin{definition}[Entanglement]
% Given Hilbert spaces $\mathcal{H}_A$ and $\mathcal{H}_B$ and composite system $\mathcal{H} = \mathcal{H}_A \otimes \mathcal{H}_B$. A pure state $\ket{\psi} \in \mathcal{H}$ is \textit{entangled} if it cannot be written as a product of states from each subsystem, i.e., there do not exist $\ket{\phi_A} \in \mathcal{H}_A$ and $\ket{\phi_B} \in \mathcal{H}_B$ such that:
% \begin{align}
% \ket{\psi} = \ket{\phi_A} \otimes \ket{\phi_B}.
% \end{align}
% A mixed state $\rho \in \mathcal{B}(\mathcal{H})$ is \textit{entangled} if it cannot be expressed as a convex combination of product states:
% \begin{align}
% \rho \neq \sum_i p_i \rho_i^A \otimes \rho_i^B,
% \end{align}
% where $\{p_i\}$ are probabilities, $\rho_i^A \in \mathcal{B}(\mathcal{H}_A)$, and $\rho_i^B \in \mathcal{B}(\mathcal{H}_B)$ are density matrices for the subsystems $A$ and $B$, respectively.
% \end{definition}
% In particular, for EPR pairs (Bell states) this means that certain states such as:
% \begin{align}
%     \ket{\psi} = \frac{1}{\sqrt{2}}(\ket{00} + \ket{11})
% \end{align}
% cannot be represented as a tensor product state. We mention entanglement only tangentially in this work but it is of course of central importance across quantum information processing.

% \subsection{Quantum metrics} \label{sec:quant:quantummetrics}
% Metrics play a central technical role in classical machine learning, fundamentally being the basis upon which machine learning algorithms update, via techniques such as backpropagation. Indeed metrics at their heart concern the ability to quantifiably distinguish objects in some way and to this extent have been integral to the very concept of \textit{information} as portended by Hartley in which information refers to quantifiable ability of a receiver to distinguish symbolic sequences \textbf{HARTLEY}. Hartley's original measure of information prefigured advanced approaches to quantifying and describing information, such as Kolmogorov and others [\textbf{COVER Kolmogorov}]. 

% Metrics for quantum information processing are related but distinct from their classical counterparts and understanding these differences is important for researchers applying classical machine learning algorithms to solve problems involving quantum data. As is commonplace within machine learning, chosen metrics will differ depending on the objectives, optimisation strategies and datasets. For a classical bit string, there are a variety of classical information distance metrics used in general \cite{nielsen_quantum_2010}. In more theoretical and advanced treatments, available metrics will depend upon the underlying structure of the problem (e.g. topology) (see \cite{watrous_theory_2018} for a comprehensive discussion). Metrics used will depend also upon whether quantum states or operators are used as the comparators, though one can relatively easily translate between operator and state metrics. We outline a number of commonly used quantum metrics below and discuss their implementation in classical contexts, such as in loss functions. Note below we take license with the term metric as certain measures below, such as quantum relative entropy, do not (as with their classical counterparts) strictly constitute metrics as such.

% Being able to quantify the difference or similarity of quantum sates is fundamental to the application of any machine learning protocols in quantum information processing. This problem of state discrimination, of how accurately states can be distinguished using measurement, is examined briefly below. In particular, we focus on the key metric in later chapters of \textit{fidelity} among target unitary operators and those generated via our algorithmic methods. We summarise briefly a few key results in the area, including the Holevo-Helstrom theorem (for providing a weighted difference between states). In machine learning, state discrimination is also central to classification methods. Indeed difference measures and metrics are central to underlying objective (loss) functions underpinning the learnability of classical and quantum machine learning algorithms. 

%  \subsubsection{State discrimination}\label{sec:quant:State discrimination}
%  State discrimination for both quantum and probabilistic classical states requires incorporation of stochasticity (the probabilities) together with a similarity measure. The Holevo-Helstrom theorem quantifies the probability of distinguishing between two quantum states given a single measurement $\mu$. State discrimination here is a binary classification problem. 
%  \begin{definition}[Holevo-Helstrom theorem]\label{defn:quant:Holevo-Helstrom theorem}
%      Given diagonal $\rho_k \in D(\Hilb)$ with $\lambda\in[0,1]$, for each choice of measurement $\mu:\{0,1 \}\to Pos(\Hilb)$, the probability of correctly ($\lambda$) or incorrectly $(1-\lambda)$ distinguishing a state is given by:
%      \begin{align}
%          \lambda \braket{\mu(0),\rho_0} + (1-\lambda)\braket{\mu(1),\rho_1} \leq \frac{1}{2} + \frac{1}{2}||\lambda \rho_0 + (1-\lambda)\rho_1||_1
%      \end{align}
%  \end{definition}
%  Where, for a suitably chosen projective measurement $\mu$, the relation is one of equality. State discrimination is central to results in this work, especially in Chapters 5 and 6 where discriminating states (measuring their similarity) is the key to training quantum machine learning models. A detailed exposition of state discrimination from an information theoretic perspective can be found \cite{watrous_theory_2018}. For our primary results relating to state (and by extension operator) discrimination in later chapters, we focus on the fidelity metric as the basis for distinguishing quantum states and operators (central to, for example, our objective functions in machine learning applications we use). We focus on fidelity below. Briefly we also mention an important feature of quantum information (especially as its relates to machine learning applications) in the form of the \textit{no cloning theorem} which provides that quantum information cannot be identically copied. That is, no procedure exists for identically replicating any arbitrary quantum state $\ket{\psi}$ on a Hilbert space $\mathcal{H}$.

%  \begin{definition}[No-Cloning Theorem]\label{defn:quant:No-Cloning Theorem}
%  The no cloning theorem provides that here does not exist a completely positive, trace-preserving (CPTP) map $\Phi: \mathcal{B}(\mathcal{H}) \to \mathcal{B}(\mathcal{H} \otimes \mathcal{H})$ such that for any pure state $\ket{\psi} \in \mathcal{H}$,
% \begin{align}
% \Phi(\ket{\psi}\bra{\psi}) = \ket{\psi}\bra{\psi} \otimes \ket{\psi}\bra{\psi}.
% \end{align}

% \end{definition}
% The no cloning theorem illustrates the fundamentally non-classical nature of quantum information. Note, however, that it does not prevent the preparation of identical quantum states (essential to machine learning protocols including those explored in Chapter \ref{chapter:Background: Classical, Quantum and Geometric Machine Learning}) i.e. identical `copies' of quantum states $\rho$ can be produced via identical preparation procedures.

% \subsubsection*{Fidelity function}\label{sec:quant:Fidelity function}
%  Of central importance to later results in Chapters \ref{chapter:QDataSet and Quantum Greybox Learning} and \ref{chapter:Quantum Geometric Machine Learning} is the fidelity function which quantifies the degree of similarity or overlap between two quantum states (or their operator representations in $Pos(\Hilb)$). Fidelity is a key metric in quantum information processing, especially in quantum control and quantum unitary synthesis problems. It is central to the quantum machine learning loss function architecture adopted in this work. As such, we provide a more in-depth assessment of the metric with regard to quantum state comparison.
% \begin{definition}[Fidelity]\label{defn:quant:Fidelity}
%     The fidelity between two operators $\rho,\sigma \in Pos(\Hilb)$ is given by:
%     \begin{align}
%         F(\rho,\sigma) = \big|\big|\sqrt{\rho}\sqrt{\sigma}  \big|\big|_1 =  \Tr\left(\sqrt{\sqrt{\sigma}\rho\sqrt{\sigma}}\right) \label{eqn:quant:fidelityfunction}
%     \end{align}
% \end{definition}
% The fidelity function exhibits a number of properties including: (a) continuity - it is continuous at $(\rho,\sigma)$ (important for statistical learning performance); (b) symmetric $F(\rho,\sigma) = F(\sigma,\rho)$; (c) positive semi-definiteness $F(\rho,\sigma) \geq 0$ else $\rho \sigma=0$; (d) $F(\rho,\sigma) \leq \Tr(\rho)\Tr(\sigma)$ (equality if not independent); (e) preservation under conjugation by isometries (unitary channels) $V\in U(\Hilb,\Hilb)$ such that $F(\rho,\sigma)=F(V \rho V^*,V \sigma V^*)$; (f) $F(\lambda \rho,\sigma)=\sqrt{\lambda}F(\rho,\sigma)=F(\rho,\lambda \sigma)$. In terms of density operators $\rho,\sigma \in Pos(\Hilb)$, we have that  $F(\rho,\sigma) \in [0,1]$ with $F=0$ if and only if $\rho \perp \sigma$ and $F=1$ if and only if $\rho = \sigma$. The fidelity function can be shown to be jointly concave in its arguments and monotonic under the action of channels. The latter of these properties provides that for $\Phi \in C(\Hilb)$ with $\rho,\sigma \in Pos(\Hilb)$:
% \begin{align}
%     F(\rho,\sigma) \leq F(\Phi(\rho),\Phi(\sigma))
% \label{eqn:chapter1:fidelitymonotonicity}
% \end{align}
% Finally, the relationship of fidelity $F$ and trace function $||\cdot ||_1$ for state $\rho,\sigma \in D(\Hilb)$ is given by Fuchs-van de Graaf inequalities, which can be expressed as:
% \begin{align}
%     2-2F(\rho,\sigma) \leq ||\rho - \sigma||_1 \leq 2\sqrt{1-F(\rho,\sigma)^2} \label{eqn:quant:fidelityfuchs}
% \end{align}
% Note in some texts that equation (\ref{eqn:quant:fidelityfunction}) is sometimes denoted \textit{root fidelity} while fidelity is its square (see \cite{bengtsson_geometry_2006}) and that fidelity can be related to transition probability between mixed states [\textbf{UHLMANN}].  

% Other metrics common in quantum machine learning literature include:
% \begin{enumerate}
%     \item \textit{Hamming distance}, the number of places at which two bit strings are unequal. Hamming distance is important in error-correcting contexts and quantum communication \cite{doriguello_quantum_2019}.
%     \item \textit{Trace distance} or $L1$-\textit{Kolmogorov distance} described in definition (\ref{defn:quant:Tracedistance}). Trace distance is a metric preserved under unitary transformations. It is therefore a widely used similarity metric in quantum information.
% %     For two probability distributions $\{p_x \},\{q_x \}$ we can construct the metric $D(p_x,q_x)=\frac{1}{2}\sum_x|p_x - q_x|$ . In the quantum setting, for states represented by density matrices $\rho,\sigma$ \cite{nielsen_quantum_2010}, their trace distance can be calculated as:
% % \begin{align}
% %     D(\rho,\sigma) = \frac{1}{2} \text{tr}|\rho - \sigma|
% % \end{align}
% % where $|\rho| = \sqrt{\rho^\dagger \rho}$ is taken as the positive square root. 
%        \item \textit{Fidelity} described above in definition \ref{defn:quant:Fidelity} is another  common metric by which to assess state or operator similarity. Note in density matrix terms that $F(\rho,\sigma) = \trace\sqrt{\rho^{1/2}\sigma \rho^{1/2}}$. Specifically, fidelity can be interpreted as a metric by calculating the angle $\zeta=\arccos F(\rho,\sigma)$. Fidelity and trace distance are related via $D(\rho,\sigma) = \sqrt{1 - F(\rho,\sigma)^2}$.
%     \item \textit{Quantum relative entropy} (see definition \ref{defn:quant:quantumrelativeentropy}) is the quantum analogue of Shannon entropy \cite{bengtsson_geometry_2006}. It is found given by $S(\rho) = -\trace(\rho \log \rho)$ The quantum analogue of (binary) cross-entropy is in turn given by:
%     \begin{align}
%         S(\rho||\sigma) = \trace(\rho \log \rho) - \trace(\rho \log \sigma)
%     \end{align} These measures provide a further basis for comparing for the output of algorithms to labelled data during training. 
% \end{enumerate}
% We discuss the use and relationship of such metrics to quantum machine learning algorithms deployed in further chapters in more detail in Chapter \ref{chapter:Background: Classical, Quantum and Geometric Machine Learning}.


% %======QUANTUM CONTROL
% \section{Quantum Control}\label{sec:quant:Quantum Control}
% \subsection{Overview}
% Quantum information tasks can be modelled in terms of a two-step experiment (a) a quantum state and measurement instrument preparation procedure (isolating the quantum system in a particular state); (ii) a measurement step where the instrument interacts with the quantum system to yield measurement statistics. Obtaining such statistics (by which the state preparation can potentially be confirmed) occurs via multiple repetitions of such experiments. While quantum systems are represented distinctly from classical systems, their state preparation, control and measurement is classically parametrised (e.g. by parameters in $\R$ or $\C$). Information can be distinguished between classically described and evolving (classical information) as distinct from being described and evolving according to quantum formalism (quantum information) In certain cases, such as with certain classes of quantum machine learning or variational algorithms \cite{verdon_quantum_2019,verdon_quantum_2019-3,verdon_quantum_2019-1,schuld_introduction_2015}, parameter registers may themselves be represented (or stored within) quantum registers. However, as noted above, quantum registers themselves concern [distributions and evolution] over classical registers (albeit with certain non-classical features). Thus ultimately quantum information processing, and tasks involving quantum systems, involve constructions using classical information. 

% As Wiseman et al. note \cite{wiseman_quantum_2010} the preparation-evolve-measure procedure of quantum parameter estimation can be framed as one where a quantum system mediates (and transforms) the classical parameters of a state preparation procedure to the classical measurement statistics. Construed as a transformation mediating the transition from classical (input) to classical (measurement/output) information, quantum systems can be seen as establishing constraints upon the accuracy of the estimation of such parameters (albeit ontological limits given the fundamental grounding of physics in quantum mechanics). For example, modelling the synthesis of a particular computation or state can be modelled as the task of quantum parameter estimation where parameters $\theta \in \C$ (such as control pulses, see below) are estimated from measurement outcomes of a state whose evolution is modelled as:
% \begin{align}
%     \rho_0 \to \rho_T = e^{-i Ht}\rho_0e^{i Ht} = U\rho_0 U^\dagger
% \end{align}
% Here the Hamiltonian is parameterised by $\theta$ as $H = \sum_\k \theta_k G_k$ where $G_k$ are generators (see below). Assuming $\rho_0$ is (sufficiently) known along with $G_k$, then ascertaining the set of controls $\theta_k$ to (optimally - say minimising time or energy) synthesise $\rho_T$ is contingent on estimates $\hat\theta$ via minimising a cost function $|\theta_k - \hat\theta_k|$. The estimates $\hat\theta$ are themselves usually constructed via comparing the measurement statistics of the estimate $\hat\rho_T$ against $\rho_T$. This is also the case when seeking to estimate, for example, state preparation parameters from measurement statistics. Thus constraints upon measurement statistics, such as as the Helstrom-Holevo bound (see definition (\ref{defn:quant:Holevo-Helstrom theorem})) act as constraints or bounds upon how accurately quantum parameter estimation (and tasks dependent on it, such as unitary synthesis) may be performed. In this work, we primarily base our optimisations (in later chapters) upon the fidelity measure (discussed below), assuming the existence of an (optimal) measurement protocol by which to construct our estimates of, for example, target unitaries $\hat U_T$. Below we set out a few of the key assumptions and features of quantum control formalism used in later chapters. We revisit this formalism in the next chapter in terms of Lie theoretic and differential geometric models of quantum control.

% \subsection{Evolution, Hamiltonians and control}\label{sec:quant:Evolution, Hamiltonians and control}
% Our work and results in later chapters are focused upon typical quantum control problems \cite{sachkov_control_2009, dalessandro_introduction_2007,wiseman_quantum_2010}, where it is assumed there exist a set of controls (such as pulses or voltages) with which the quantum system may be controlled or steered towards a target state (or unitary). Recall that in density matrix formalism, the Schr{\"o}dinger equation is:
%     %
%     \begin{align}
%         i \frac{d \rho}{dt} = [H(t), \rho(t)] \label{eqn:quant:schroddensitycontrol1}
%     \end{align}
%     %
%     where the commutator $[A,B] = AB-BA$ and $H(t)$ is a Hermitian operator called the Hamiltonian. In physical systems, it corresponds to the total energy (sum of kinetic and potential energies) of the system under consideration.
%     In control theory, we can separate out the Hamiltonian in equation (\ref{eqn:quant:schroddensitycontrol1}) into drift and control forms.
%     For a closed system (i.e. a noiseless isolated system with no interaction with the surrounding environment), it can be expressed in the general form:
%     %
%     \begin{align}
%         H(t) = H_0(t) \doteq H_d(t) + H_{\text{ctrl}}(t).
%     \end{align}
%     %
%     $H_d(t)$ is called the drift Hamiltonian and corresponds to the natural evolution of the system in the absence of any control. The second term $H_{\text{ctrl}}(t)$ is called the control Hamiltonian and corresponds to the controlled external forces we apply to the system (such as electromagnetic pulses applied to an atom, or a magnetic field applied to an electron). This is also sometimes described as an interaction Hamiltonian (representing how the system interacts with classical controls e.g. pulses or other signals). This allows us to define a control-theoretic form of the Schr\"odinger equation.
% \begin{definition}[Control (Schr\"odinger) equation]\label{defn:quant:controlequation}
%     Given quantum state $\rho \in \mathcal{B}(\Hilb)$ with Hamiltonian given by $H_0(t) =  H_d(t) + H_{\text{ctrl}}(t)$ define the control form of equation (\ref{eqn:quant:schroddensitycontrol1}) as:
%     \begin{align}
%         i \frac{d \rho}{dt} = [ H_d(t) + H_{\text{ctrl}}(t), \rho(t)] \label{eqn:quant:schroddensitycontrol2}
%     \end{align}
%     The solution of the evolution equation at time $t=T$ is given by:
%     \begin{align}
%         \rho(T) = U(T) \rho(0) U^{\dagger}(T),
%     \end{align}
%     where $\rho(0)$ is the initial state of the system, the unitary evolution matrix $U(t)$ is given by equation (\ref{eqn:quant:schrodingersequation}). 
% \end{definition}
% We discuss control and its application in some detail in later chapters, specifically relating to geometric quantum control as expressed by formal (Pontryagin) control theory where targets are unitaries $U_T \in G$ for unitary groups $G$. As D'Alessandro \cite{dalessandro_introduction_2007} notes, the typical quantum control methodology covers: (a) obtaining the Hamiltonian of the system in an appropriate form, (b) identifying the internal and interaction components of the Hamiltonian (and often calculating the energy eigenstates for a time-independent approximation) and (c) specifying a finite dimensional and bounded control system for control coefficients. \\
% \\
% \subsection{Control systems and strategies}\label{sec:quant:controlsystem}
% We sketch some of the discussion of control theory in later chapters here. D'Alessandro \cite{dalessandro_introduction_2007} notes that a general control system has the following form (which as we discuss is due to Pontryagin):
% \begin{align}
%     \dot x = f(t,x,u)    \label{eqn:quant:controlsystem1}
% \end{align}
% where $x$ represents the system state, $f$ is a fector field while $u=u(t)$ are real-valued time varying (or constant over small $\Delta t$ interval) control functions. The state is inaccessible in general, only via some other function or channel e.g. $g(x)$, say a measurement operation. In quantum settings, equation (\ref{eqn:quant:controlsystem1}) is described by the Schr\"odinger equation. In unitary form this is equivalent to:
% \begin{align}
%     \dot x \sim  \dot U \qquad f(x,t,u) \sim -iH(u(t)) U \label{eqn:quant:control-state-eqn}
% \end{align}
% where $H(u(t))$ is a Hamiltonian comprising controls and generators (for us, drawn from a Lie algebra $\g$). We leave detailed exposition of classical and quantum control (particularly based upon so-called dynamical Lie algebras) for Chapter [3/4] (see section (\ref{sec:geo:variationalgeometrictechniques})). The drift Hamiltonian $H_d$ and control Hamiltonian $H_c$ combine as:
% \begin{align}
%     H(u) = H_d + \sum_k H_k u_k
% \end{align}
% where $f$ in equation (\ref{eqn:quant:control-state-eqn}) is thought of as a linear function of $x$ and an affine function of the controls $u$. For ensembles, the evolution can be described via control Hamiltonians acting upon the set of denisty matrices as well. Overall the generic control solution is then:
% \begin{align}
%     \rho(t) = U(t) \rho(0) U^\dagger(t) \qquad \dot U = -iH(u) U \qquad U(0) = \mathbb{I} \label{eqn:quant:control-math-form}
% \end{align}
% Such solutions are drawn from Jurdjevic \cite{jurdjevic_geometric_1997} from geometric control theory literature. These are a major focus of our final chapter, where we show equivalent results can be obtained for certan symmetric space quantum control problems by using a global Cartan decomposition together with certain variational techniques. The form of equation (\ref{eqn:quant:control-math-form}) can be easily construed in an information-theoretic fashion, such as when logic gates (e.g. upon qubits) are sought to be engineered. 

% As noted in \cite{dalessandro_introduction_2007}, an important distinction between classical and quantum control is the unavailability of classical feedback control in the quantum case as a result of the measurement axiom \ref{axiom:quant:effectofmeasurement}, namely the collapse of $\rho \to \rho'$: the modification of the state $\rho$ by measurement means that evolution must be considered as starting from a different initial condition $\rho(0)'$. Instead, \textit{open loop control schemes} which rely upon an \textit{a priori} control system. In this case, control inputs are applied without observing the current state $\rho(t)$ i.e. meaning no adjustment during the control strategy (the sequence of controls and their characteristics), such as to the sequence or amplitude of control pulses. This is distinct from \textit{feedback control} where the control strategy is dynamically adaptable based on the state (e.g. as say in reinforcement learning). 

% We also note other conditions regarding reachability of targets $U_T \in G$. In particular, we [rely] upon the \textit{quantum recurrence theorem} \textbf{ Bocchieri, liu}\hl{EDIT}
% \begin{definition}[Quantum Recurrence Theorem]
% For any $U \in G$ where $G$ represents a unitary Lie group acting on $\Hilb$ represented by $U(0)$, there exist a $\epsilon,T > 0$ such that:
% \begin{align*}
% \left| U(0) - U(T)U(0)(T)^\dagger \right| < \epsilon,
% \end{align*}
% where $|\cdot|$ denotes the operator norm. This theorem is denoted the quantum recurrence theorem.
% \end{definition}
% The action of the group element $U \in G$ on $\Hilb$ is the quantum analog of the classical flow in dynamical systems. The quantum recurrence theorem guarantees that quantum evolution on the action of $G$ (via conjugation) will evolve the quantum state $U$ arbitrarily close to $U_0$ after some finite time $T$, reflecting the the quasi-periodic nature of the evolution in a finite-dimensional Hilbert space and follows from the spectral properties of the unitary group on such a space.



% Before moving to our next chapter on Lie groups and associated algebraic concepts, we mention a few concepts from open quantum systems relevant to later chapters.

% \section{Open quantum systems}\label{sec:quant:Open quantum systems}
% \subsection{Overview}
% We conclude this background chapter with a brief synopsis of open quantum systems and quantum control. This is of particular relevance to Chapter 5 where our QDataSet models the influence of noise upon one- and two-qubit systems. Moreover, it is of seminal importance in any quantum information processing task. As Wiseman and Howard note, projective measurements (see above) are inadequate for describing real measurements because, among other reasons, such measurement never measure directly the system of interest in a closed state \cite{wiseman_quantum_2010}. Rather, the system always interacts with an environment. Even if this logic is extended back to the interaction of the observer themselves, some truncation of the phenomena into system (measured via applying the measurement postulates above for projective measurement) and environment must be made (so-called Heisenberg cuts). While the focus of this work is on geometric and machine learning techniques, we briefly summarise a few relevant and key aspects of open quantum systems modelling. This is of particular relevance to Chapter 5 where our quantum simulations explicitly factor in a variety of noise sources. Most of our results in Chapters 6 and 7 assume a simplified control problem, one of a closed quantum system, while Chapter 5 demonstrates (through the $V_O$ operator) how machine learning can be used to learn those features of an open or noisy system in a way that can allow for mitigation or noise cancellation to a degree.  
    
% Open quantum systems construct an overall quantum system comprising the \textit{system} (or closed quantum evolution) and the \textit{environment} (i.e. interactions with the environment). A simple Hamiltonian model for such open systems:
%     \begin{align}
%         H(t) = H_0(t) + H_1(t) \doteq \underbrace{H_d(t) + H_{\text{ctrl}}(t)}_{H_0(t)} + \underbrace{H_{SE}(t) + H_E(t)}_{H_1(t)} \label{eqn:quant:openquantHamiltonianSE}
%     \end{align}
%     %
%     $H_0(t)$ is defined as before to encompass the drift and control parts of the Hamiltonian. The new term $H_1(t)$ now consists of two terms: $H_{SE}(t)$ represents an interaction term with the environment, while $H_E(t)$ represents the free evolution of the environment in the absence of the system. In this case, the  Hamiltonian controls the dynamics of both the system and environment combined in a highly non-trivial way. In other words, the state becomes the joint state between the system and environment. The combined system and environment then become closed. Modelling such open quantum systems is complex and challenging and is typically undertaken using a variety of stochastic master equations \cite{wiseman_quantum_2010} or sophisticated noise spectroscopy. As detailed below, the QDataSet contains a variety of noise realisations for one and two qubit systems together with details of a recent novel operator \cite{youssry_characterization_2020} for characterising noise in quantum systems. As such we briefly summarise a few key concepts relating to open quantum systems. Detail can be found in Wiseman and Milburn \cite{wiseman_quantum_2010} and other standard texts.

% \subsection{Noise and quantum evolution}\label{sec:quant:Noise and quantum evolution}
% Of importance to practical development and applications of quantum computing, especially the control of quantum systems, is understanding the role of noise and other environmental interactions. Of central importance to the modelling of environmental and noise-like interactions in quantum information theory are superoperators, defined as follows.
% \begin{definition}[Superoperators]\label{eqn:quant:superoperators}
%     A superoperator $\mathcal{S}$ is a linear map on the space of bounded linear operators on a Hilbert space $\mathcal{H}$ given as $\mathcal{S}: \mathcal{B}(\mathcal{H}) \rightarrow \mathcal{B}(\mathcal{H})$, $\hat A \mapsto \mathcal{S} \hat A$. 
% \end{definition}
% For a superoperator $\mathcal{S}$ to correspond to a physical process, such as a quantum channel, it must satisfy the following conditions: \hl{fix}
% \begin{enumerate}
%     \item \textit{Trace-Preserving or Decreasing:} For any state $\rho$ we have that $0 \leq \text{Tr}[\mathcal{S}\rho] \leq 1$.
%     \item \textit{Convex Linearity:} for probabilities $\{p_j\}$,
%     \begin{align}
%         \mathcal{S} \left( \sum_j p_j \rho_j \right) = \sum_j p_j \mathcal{S}\rho_j.
%     \end{align}
%     \item \textit{Complete Positivity:} $\mathcal{S}$ must not only map positive operators to positive operators for the system but also when tensored with the identity operator on any auxiliary system $\mathcal{R}$,
%     \begin{align}
%         (\mathbb{I}_{\mathcal{R}} \otimes \mathcal{S}) (\rho_{\mathcal{R} \mathcal{S}}) \geq 0.
%     \end{align}
%     i.e. the identity superoperator $\mathcal{I}_\mathcal{R}$ acts as the identity map on the auxiliary system.
% \end{enumerate}
% A superoperator $\mathcal{S}$ that satisfies these properties is a CPTP map and therefore a quantum channel (by definition \ref{defn:quant:Quantum Channel}, often represented by the Kraus operators $\{E_k\}$ in the form:
% \begin{align}
%     \mathcal{S}(\rho) = \sum_k E_k \rho E_k^\dagger \qquad \sum_k E_k^\dagger E_k = \mathbb{I}_{\mathcal{H}}
% \end{align}


% \subsection{Noise and decoherence}\label{sec:quant:Noise and decoherence}
% Noise effects are of fundamental importance to simulating quantum systems (the subject of Chapter 5) but also the ability of machine learning algorithms to learn patterns in data. 
% As shown above, open quantum systems are described by the evolution of their density operators. The formal and most common method of representing such open-state evolution is via the \textit{Lindblad master equation} which formalises non-unitary evolution arising as a result of interaction with noise sources, such as baths. The most general form of the master equation for the density operator $\rho$ of an open quantum system, preserving complete positivity and the trace of $\rho$, is given by the Lindblad equation:
% \begin{definition}[Lindblad Master Equation]\label{defn:quant:lindbladmasterequation}
% The mixed unitary and non-unitary time-evolution of a quantum system represented by $\rho$ interacting with its environment is given by the Lindblad master equation:
%  \begin{align}
%      \frac{d\rho}{dt} = -i[H, \rho] + \sum_{k} \gamma_k\left( L_k \rho L_k^\dagger - \frac{1}{2} \left\{ L_k^\dagger L_k, \rho \right\} \right) \label{eqn:quant:lindbladmasterequation}
%  \end{align}   
%  \end{definition}
% Here $\rho$ is the density matrix of the quantum system, $H$ is the Hamiltonian of the system, dictating the unitary evolution due to the system's internal dynamics, $\sum_{k}$ indicates a sum over all possible noise channels $k$ affecting the system and $\gamma_k$ are the rates at which the system interacts with the environment through the $k^{th}$ channel, quantifying the strength of the non-unitary processes. Of importance are $L_k$, the Lindblad operators associated with each noise channel, describing how the system interacts with its environment and, in particular, how the environment transforms $\rho$ in a way that affects properties of interest, such as its coherence. 


% Lindblad operators $L_k$ are not superoperators themselves, but they are integral components in the definition of the \textit{Lindblad superoperator}, which describes specific physical processes (e.g., photon emission, absorption, or scattering). In contrast, the superoperator $\mathcal{L}$, represents the entire evolution of the quantum system including the dissipative dynamics. To understand this within the context of quantum trajectories, where the evolution of a system is modeled under continuous measurement, the stochastic master equation can be written as:
% \begin{align}
%     \frac{d\rho}{dt} = -i[H, \rho] dt + \sum_{k} \mathcal{L}[L_k]\rho dt + \sqrt{\eta}\mathcal{H}[L]\rho dW_t
% \end{align} In the equations above, $L$ represents the Lindblad operator, $\rho$ is the density matrix of the system, $\eta$ is the efficiency of the measurement, and $dW_t$ is the Wiener increment representing the stochastic process of the measurement that models the infinitesimal evolution of processes that have continuous paths. The equation comprises:
% \begin{enumerate}[(i)]
%     \item a Hamiltonian term $-i[H, \rho]$, describing the unitary evolution of a closed system;
%     \item a \textit{Lindbladian (superoperator)} term $\mathcal{L}[L]\rho$, which describes the average effects of system-environment interactions and is given by:
%     \begin{align}
%         % \mathcal{L}[L]\rho = L\rho L^\dagger - \frac{1}{2}\left(L^\dagger L\rho + \rho L^\dagger L\right),
%         \mathcal{L}[L_k]\rho = \gamma_k\left( L_k \rho L_k^\dagger - \frac{1}{2} \left\{ L_k^\dagger L_k, \rho \right\} \right)
%     \end{align}
%     \item a \textit{backaction (superoperator)} term $\mathcal{H}[L]\rho$, which accounts for the changes in the system due to measurement and is given by:
% %     \begin{align}
% % \mathcal{H}_k[\rho] = \sqrt{\eta_k}\left(L_k\rho + \rho L_k^\dagger - \mathrm{Tr}[L_k\rho + \rho L_k^\dagger]\rho\right).
% % \end{align}
%     \begin{align}
%        \sqrt{\eta}\mathcal{H}[L]\rho = \sqrt{\eta}(L\rho + \rho L^\dagger - \rho \, \text{tr}(L\rho + \rho L^\dagger)).
%     \end{align}
%     where $\eta$ denotes the influence of the backaction term.  As Wiseman and Milburn note, in the Heisenberg picture the backaction is manifest in the system operators rather than state. 
% \end{enumerate}
% Note for completeness that the $L_k$ terms represent the channels through which the quantum system interacts with its environment i.e. the quantum trajetories. By contrast, the backaction term seeks to model the effect of the (usually single) measurement channel (which is why we do not sum over $k$). 

% \subsection{Noise and spectral density}\label{sec:quant:Noise and spectral density}
% We conclude with a few remarks relevant in particular to discussions of noise spectral density in Chapter \ref{chapter:QDataSet and Quantum Greybox Learning} (section \ref{sec:qdata:Noise profile details}). In quantum control, complete knowledge of environmental noise is usually (if not always) impossible to obtain. However, in certain cases, even partial knowledge of open system dynamics can assist in achieving gate fidelities. One such example is where the control pulse is band-limited. To understand this, consider the frequency domain representation of a control pulse $u(t)$:
% \begin{align}
%    F(\omega) = \int^\infty_{-\infty} u(t)\exp(-i\omega t) dt
% \end{align}
% with frequency $\omega$ of the pulse (e.g. some signal) and $F(\omega)$ represents the amplitude of the control pulse. If $F(\omega)$ is confined within a specific frequency band, $|\omega| \leq \Omega_0$, then the quantum system's response to environmental noise can be represented by the convolution:
% \begin{align}
%     I(\omega) = \int_{-\infty}^\infty d\omega F(\omega) S(\omega),
% \end{align}
% where $S(\omega)$ is the noise power spectral density (PSD), a measure of noise intensity. In such cases, only noise components within the control's effective bandwidth, $|\omega| \leq \Omega_0$, are relevant to solving the quantum control problem. Connecting with the Lindblad master equation \ref{eqn:quant:lindbladmasterequation}, each Lindblad operator $L_k$ corresponds to a type of noise interaction between the quantum system and the environment. The decoherence rates $\gamma_k$ can be derived from correlation functions of noise operators coupling to the system as represented via the $L_k$ operators. Correlation functions capture temporal correlations of the noise operators $B$ on the system. The (two-time or interval) correlation function $G(t)$ is defined as:
% \begin{align}
%     G(t) = \langle B(t) B(0)^\dagger \rangle,
% \end{align}
% where $\langle \cdot \rangle$ denotes the expectation with respect to the environmental state, and $B(t) = e^{iH_{\text{env}}t} B e^{-iH_{\text{env}}t}$ in the Heisenberg picture with $H_{\text{env}}$ being the Hamiltonian of the environment. The PSD $S(\omega)$ is then obtained from the Fourier transform of $G(t)$:
% \begin{align}
%     S(\omega) = \int_{-\infty}^{\infty} G(t) e^{-i\omega t} \, dt.
% \end{align}
% This quantity characterizes the strength of noise or fluctuations in the environment at frequency $\omega$. As [\textbf{CLERK}] notes, classical PSD indicates the magnitude of noise at a particular frequency $\omega$, while quantum noise PSD indicates the magnitude of Golden rule transition rates for emission or absorption events. Dephasing rates $\gamma_k$ can thus be shown to be related to (proportional to) $S(\omega)$ (see \textbf{[CLERK]}).





==> ebackupChapter3a.tex <==
% %========DIFFERENTIAL GEOMETRY
% \chapter{Background: Differential Geometry}\label{chapter:background:Differential Geometry}
% The study of geometric methods usually begins with the definition and study of the properties of differentiable manifolds. One begins with the simplest concept of a set of elements, characterised only by their distinctiveness (non-identity), akin to pure spacetime points $\M$. The question becomes how to impose structure upon $\M$ in a useful or illuminating manner for explaining or modelling phenomena. To do so, in practice one assumes that $\M$ is a topological space, following which additional structural complexity, necessary for certain operations, such as analytical (differentiation etc) or measures (for integration), is added. The material on differential geometry in this chapter is drawn from standard texts in the field \cite{isham_modern_1999,frankel_geometry_2011,montgomery_tour_2002,do_carmo_differential_2016,knapp_lie_1996,helgason_differential_1979,goldstein_classical_2002,kobayashi_foundations_1963}. Most results are presented without proofs which can be found in the collection of resources noted above. The chapter begins with an outline of basic conceptualisation of manifolds, tangent planes, pushforwards and bundles. It them moves onto vector (and tensor) fields, $n$-forms, connections, parallel transport and [cohomology]. The second section of this chapter concentrates on geometric control theory, drawn primarily from the work of Jurdjevic \cite{jurdjevic_geometric_1997,jurdjevic_non-euclidean_1995,jurdjevic_control_1981,jurdjevic_optimal_1999,jurdjevic_hamiltonian_2001}, Boscain \cite{boscain_introduction_2021,boscain_invariant_2008}, D'Alessandro \cite{dalessandro_introduction_2007} and others. It focuses primarily on classical geometric control theory, but the results, especially where controls are constructed from semi-simple Lie groups and algebras carry over to the quantum realm.

% \section{Differential geometry}
% \subsection{Manifolds and charts}\label{sec:geo:Manifolds and charts}

% % \begin{definition}
% % This is a definition.
% % \end{definition}

% % \begin{theorem}
% % This is a theorem.
% % \end{theorem}

% % \begin{lemma}
% % This is a lemma.
% % \end{lemma}

% We begin with the concept of a \textit{topological manifold} $\M$, being a connected Hausdorff ($T_2$) space (a topological space such that for any two distinct points there exist disjoint neighbourhoods). From this point, we defined coordinate charts and atlases as follows.
% \begin{definition}[Coordinate charts and atlases]\label{defn:geo:Coordinate charts and atlases}
%     \normalfont A \textit{coordinate chart} is a pair $(U,\phi)$ on $\M$ where $U \subset \M$ (an open subset) and $\phi:U \to \Km^m$ with $p \mapsto \phi(p)$ (usually taking $\Km = \R $ or $\C$) is a homeomorphism. The charts $\phi,\phi^\inv$ together form a family denoted as an \textit{atlas}.
% \end{definition}
% An atlas constitutes the assignment of a collection of open charts to the underlying manifold, which in turn allows the imposition of differential structure on the manifold. 

% \begin{definition}[Differentiable manifold]\label{defn:geo:Differentiable manifold}
%     A differentiable manifold is a Hausdorff topological space $\M$ together with a global differentiable structure.
% \end{definition}
% The coordinates of a point $p$ are maps from $p\in U \subset  \mathcal{M}$ to the Euclidean space $\K^m$ i.e. $(\phi^1(p),...,\phi^m(p))$. The \textit{coordinate functions} are each of these individual functions $\phi^\mu: U \to \K$. We have $m$ of them so that's how we get the map from $U$ to $\K^m$. These functions are defined in terms of a chain, or rather, composition that takes information from $p$, to $\K^m$ to $\K$. An example is Euclidean space $\Real^m$ which can be equipped with a differential structure via imposing a globally-defined coordinate chart, where the coordinates of vectors $v \in \Real^m$ are the components $(x^1,...,x^m)$. Any finite dimensional vector space $V$ can be regarded as a differentiable manifold by choosing a basis set of vectors and using this to map $V$ isomorphically to $\R^m$ e.g. if $\{e_1,...,e_m \}$ is a basis of $V$, then the vector $v = \sum_i^m v^i e_i$ which becomes mapped to the $n$-tuple $(v^1,...,v^m)\in \R^m$. Again, the key point is that $\{e_i\}$ is the basis of $V$, whereas the coordinate functions (or set thereof) are the elements parametrised by $\R^m$. For certain manifolds, such as the sphere $S^1$ or the torus, there is no way of parametrising the space with a single coordinate function, hence we may require an atlas with different coordinate functions. In this case a mapping between coordinate functions that preserves smoothness is required. Of crucial importance for our analysis, a Lie group $G$ (see definition \ref{defn:alg:liegroups}) is a group that is also a smooth manifold via the smoothness of group operations.
% \begin{proposition}[Lie Group (Manifold)]\label{prop:geo:Lie Group (Manifold)} A Lie group $G$ equipped with a differentiable structure is a smooth differentiable manifold via the smoothness of group operations (arising from the continuity properties of $G$ i.e. being a topological group) given by multiplication $m: G \times G \to G$, defined by $m(g, h) = gh$, and inversion $i: G \to G$, defined by $i(g) = g^{-1}$.
% \end{proposition}
% Functions defined on $p \in \M$ that overlap multiple charts are required to be differentiable. Functions that preserve such structure are played by the role of $C^r$ functions, those which are differentiable up to order $r$. In particular we are interested in local representatives, being functions between manifolds $f: \M \to \N$ which have a representation (in a geometric sense) as a function between the coordinate charts $(U,\phi)_{\mathcal{M}} \to (V,\psi)_\mathcal{N}$. The idea is that we can say the function $f$ between manifolds is a $C^r$ function \textit{if all local representatives between the two coverings are themselves} $C^r$ functions i.e. we can designate $f$ as a $C^r$ function if for all coverings (basically atlases) of $\mathcal{M},\mathcal{N}$ by charts (or rather coordinate neighbourhoods), the local representative functions are $C^r$. Functions that are differentiable require $r \geq 1$, while smooth functions require $C^\infty$.
% \\
% \\
% Usually we are working with $(C^\infty)$ spaces. The complete atlas (a $C^\infty$ atlas) provides the differential structure required for differential calculus and analytic approximations on the manifold. A differentiable structure is imposed on $\M$ (where $\Km = \C$ one also imposes holomorphic constraints upon functions defined on $\M$). For brevity, we denote a manifold as differentiable whether complex or real. In differential geometry, the structure (topology) preserving map is fulfilled by a $C^\infty$ (or technically $C^r$ where $r$ may or may not be finite) function such that the function $f:\M \to \N$ is a $C^\infty$ diffeomorphism assuming $f$ is a bijection and $f,f^\inv$ are both $C^\infty$. Two diffeomorphic manifolds can be regarded as `equivalent' or `copies' of a single abstract manifold. 
% \\
% \\
% We denote $F$ as the set of smooth differentiable functions $C^\infty(\M)$ (with which we shall mainly be concerned with). Such functions compose differentiably and remain homoemorphic. The set of such functions $C^\infty$ forms an algebraic derivation (see below). It can be shown under typical criteria for $A \in V_{open} \in M$, there exists a $\varphi \in C^m$ such that $\varphi(C)=1,\varphi(\Bar{V})=0$ (something of relevance to statistical learning of, for example, classifiers). Of relevance to product spaces in quantum information, product spaces of two manifolds $M \times N$ are represented by products in the vector space representation (see paper), so that the product is itself a manifold (topologically). We also assume under typical criteria the existence of an indicator function $\varphi$ on $\M$. We leave as understood usual features such as definitions of covering, paracompactness and normality of $\M$. With these concepts, we now move onto basic concepts of curves and tangent spaces. 

% \subsubsection{Tangent spaces}\label{sec:geo:Tangent spaces}
% Tangent spaces are particularly important in algebraic geometry, geometric control and geometric approaches to machine learning. The most basic example of a tangent space for a point in some vector space $x \in S^n$ with the tangent space typically denoted as $T\M$, representing the tangent space to the manifold $\M$. It is often illustrated by reference to the real vector algebra as:
% \begin{align}
%         T_x S^n:= \{ v \in \R^{n+1} | x \cdot v = 0 \}\label{eqn:geo:tangentspaceTxSn}
%     \end{align}
% To indicate the changed dimensionality (intuitively being constructed from derivatives at $p \in \M$) hence being orthogonal. More constructively for our purposes, tangent spaces can be thought of in a more algebraic way connected with the local differentiable properties of functions on the manifold. A key issue is that tangent spaces, like differentiable manifolds, make no reference to \textit{ambient spaces} in their defintion e.g. higher-dimensional vector spaces. As Isham notes ``[t]he crucial question, therefore, is to understand what should replace the intuitive idea of a tangent vector as something that is tangent to a surface in the usual sense and which, in particular, `sticks out' into the containing space'' (p.72). To answer to this question is to construe the tangent as a property of curves in the manifold. We define a tangent vector in terms of properties of curves $\gamma \in \M$ which are in turn usually parametrised in a particular way (using affine parameters or arc length). Moreover, because there are many curves that are tangent to a curve, the concept of a tangent vector as an equivalence class of curves is used. 

% \begin{definition}[Curves on manifold]\label{defn:geo:Curves on manifold}
%     A curve $\gamma$ on a manifold $\M$ is a smooth (i.e. $C^\infty$) map:
%     \begin{align*}
%         \gamma: &\R \supset (-\epsilon,\epsilon) \to \mathcal{M} \qquad t \mapsto \gamma(t)
%     \end{align*}
%      (i.e. from an interval in $\R$ crossing 0 into $\mathcal{M}$), such that, $\gamma(0)=p$.
% \end{definition}

% \begin{figure}
%     \centering
%     \begin{tikzpicture}[>=Stealth]
%   % Real line with epsilon markings
%   \draw[->] (0,-1) -- (0,1) node[above] {0};
%   \draw[-] (-0.1,-0.5) -- (0.1,-0.5) node[right] {$-\varepsilon$};
%   \draw[-] (-0.1,0.5) -- (0.1,0.5) node[right] {$\varepsilon$};

%   % Curved arrow to manifold
%   \draw[->, very thick] (0.3,0.0) to [bend left=45] (3,0.0);

%   % Contorted trapezoid
%   \begin{scope}[shift={(3.5,0)}, rotate=0, scale=0.8]
%     \draw (0,0.5) -- (0.5,1) -- (1,0.5) -- (0.5,0) -- cycle;
    
%     % Label the trapezoid M
%     \node at (1.5,0.5) {$\mathcal{M}$};
%   \end{scope}
% \end{tikzpicture}
%     \caption{Caption}
%     \label{fig:geo:timetocurve}
% \end{figure}
% As $t$ varies `infinitesimally' within $\epsint$, the curve moves infinitesimally away from $p \in \M$ but that it stays within the neighbourhood $U_p$. We have the definition then of a tangent as a property of curves.
% \begin{definition}[Tangent]\label{defn:geo:Tangent}
%     Curves are tangent if the image of two curves (i.e. two maps) at $t=0, t\in (-\epsilon,\epsilon)$ and their derivatives are identical. Formally, two curves $\gamma_1, \gamma_2$ are \textit{tangent} at a point $p \in \mathcal{M}$ if:
%     \begin{enumerate}[(i)]
%         \item $\gamma_1(0) = \gamma_2(0) = p$; and
%         \item The derivatives of two curves in a local coordinate system are the same i.e. in some local coordinate system $(x^1,...,x^m)$ around the point $p$, the two curves are `tangent' in the usual sense as curves in $\R^m$ i.e:
%         \begin{align*}
%             \left.\frac{dx^i}{dt}(\gamma_1(t))\right|_0 = \left.\frac{dx^i}{dt}(\gamma_2(t))\right|_0 \qquad i=1,...,m
%         \end{align*}
%     \end{enumerate}
% \end{definition}
% If $\gamma_1,\gamma_2$ are tangent in one coordinate system, then they are tangent in any other coordinate system that covers $p \in \mathcal{M}$. Hence the definition of tangent is independent of the coordinate system chosen. The equivalence class of curves satisfying this condition at $p \in \M$ is sometimes denoted $[\gamma]$ which can be shown to form a vector space, hence we can reasonably denote tangents at $p$ as vectors. Note that curves may not be tangent at another point $q \in \M$, hence tangent vectors are thought of as local (around $p$) equivalence relations, hence the importance of connections (see below) that, intuitively speaking, tell us how to map between tangent spaces across a manifold. The idea here is that the equivalence relation among curves arises from the tangent relation (curves are equivalent where at $p$ (for $t=0$) their differentials with respect to coordinate functions are identical. From this construction of the tangent we obtain a number of important definitions:
% \begin{enumerate}[(i)]
%     \item \textit{Tangent space}: the tangent space $T_p\mathcal{M}$ to $\mathcal{M}$ at $p \in \mathcal{M}$ is the set of all tangent vectors at $p$.
%     \item \textit{Tangent bundle}: is defined as the union of tangent spaces i.e. $T\mathcal{M}:= \bigcup_{p \in \mathcal{M}} T_p \mathcal{M}$.
%     \item \textit{Projection map}: a map $\pi: T \mathcal{M} \to \mathcal{M}$ from the tangent bundle to $\mathcal{M}$ associated with each point $p \in \mathcal{M}$. This map is `natural' in the sense that it associates each tangent plant (set of tangent vectors) with the point $p\in\mathcal{M}$.
% \end{enumerate}
% The tangent vector $v \in T_p\mathcal{M}$ can be also be construed as a \textit{directional derivative} on functions that are defined on the manifold, $f$ on $\mathcal{M}$ by defining their `action' on the function $f$ (which we denote $v(f)$ in terms of a differential operator on $f$ evaluated at the identity of the parametrisation of the curve itself (i.e. 0 point of interval)):
%     \begin{align*}
%         v(f) = \frac{df(\gamma(t))}{dt}\bigg|_0
% \label{eqn:geo:directionalderivative}
%     \end{align*}
% The directional derivative points in the direction of steepest ascent. From this, we can define the \textit{gradient} as follows.
% \begin{definition}[Gradient]\label{defn:geo:gradient}
%      Given a smooth function $f: \mathcal{M} \rightarrow \mathbb{R}$ on a differentiable manifold $\mathcal{M}$, the gradient of $f$ at a point $p \in \mathcal{M}$, denoted $\nabla f(p)$, is the unique vector in the tangent space $T_p\mathcal{M}$ that satisfies:
%     \begin{align*}
%         v(f) = \langle \nabla f(p), v \rangle 
%     \end{align*}
%     for all $v \in T_p\mathcal{M}$ where $v(f)$ denotes the directional derivative of $f$ in the direction of $v$ (as above), and $\langle \cdot , \cdot \rangle$ denotes the applicable metric (see below) on $\mathcal{M}$.  
% \end{definition}
% In a coordinate frame $(U, \phi)$ around $p$, with $\phi = (x^1, \dots, x^n)$, the gradient of $f$ can be expressed as:
%     \begin{align*}
%         \nabla f(p) = \sum_{j=1}^{n} \left( \frac{\partial f}{\partial x^j} \circ \phi^{-1} \right)(\phi(p)) \frac{\partial}{\partial x^j}\bigg|_{\phi(p)}
%     \end{align*}
%     where $\frac{\partial}{\partial x^j}\big|_{\phi(p)}$ are the basis vectors of the tangent space $T_p\mathcal{M}$ in the coordinate chart, and $\frac{\partial f}{\partial x^j}$ are the partial derivatives of $f$ with respect to the coordinates $x^j$. The inverse $\phi^{-1}$ reverses this mapping, translating coordinates in $\mathbb{R}^n$ (or $\mathbb{C}^n$) back to points on the manifold $\mathcal{M}$. We can understand how the $\nabla$ `points' in the direction of steepest ascen by noting that that:
%     \begin{align}
%         \nabla(f(p)) \cdot v = |\nabla(f(p))||v|\cos\theta
%     \end{align}
%     where $\cos\theta$ is given by equation (\ref{eqn:quant:cosinevector}). Then $|\nabla(f(p))|$ is maximal for $\cos(\theta)=1$ which occurs when $v$ and $\nabla(f(p))$ are parallel. Hence $\nabla(f(p))$ as a vector points in the direction of maximal increase i.e. steepest ascent. To obtain the steepest gradient descent, we utilise $-\nabla$.
%     %
%     %
% Although in this work we only touch upon the geometric machine learning, this type of framing of tangents is important for geometric framing of statistical learning methods, such as gradient descent (see section \ref{sec:ml:Optimisation and Gradient Descent}), specifically in relation to stochastic gradient descent optimisation (definition \ref{defn:ml:Gradien descent optimisation}).

% As is shown in the literature, tangent spaces $T_p\M$ at $p$ can be considered as real vector spaces. The intuition for this is that two curves $\gamma_i,\gamma_j$ cannot be added directly because $\M$ lacks the structure to do so. However, the coordinate space to which we have a mapping $\Real^m$ is a vector space, thus one considered how each curve $\gamma_i,\gamma_j$ is represented in $\Real^m$ such that $t \mapsto \phi \circ \sigma_1(t) +  \phi \circ \sigma_2(t)$ which we can think of as mapping from $\R$ into $\mathcal{M}$ then into $\R^m$. The object $\phi \circ \sigma_1(t) +  \phi \circ \sigma_2(t)$ is considered a curve in $\R^m$ which itself passes through the origin $\R^m$ when $t=0$. This additive object is then considered a curve in $\mathcal{M}$ that passes through $p$ when $t=0$. We then define vector addition and scalar multiplication.  From this we can show that $T_p \mathcal{M}$ is a real vector space and that the definitions above that allow assertion of the existence of a vector space of tangent vectors independent of the choice of chart and distinct from curves $\gamma_i$. Because of this vector structure, the tangent bundle is a \textit{vector bundle}.



% \subsubsection{Push-forwards}
% An important map to mention in geometry is that of a \textit{push-forward}. Recall that tangent spaces are akin to a local linearisation of the manifold. That is, a map $h: \M \to \N$ can be linearised via the architecture of tangent spaces and their vector space structure. Given this map between manifolds $\M,\N$, we are interested in maps between their corresponding tangent spaces $T\M,T\N$. This map is denoted the push-forward $h_*$ and is defined as follows.
% %Definition:pushforwards
% \begin{definition}[Push-forward]\label{defn:geo:Push-forward}
% Given the mapping $h: \mathcal{M} \to \mathcal{N}$ and $v \in T_p \mathcal{M}$, then a \textit{push-forward} is a function taking a vector in the tangent space associated with $p \in \mathcal{M}$, namely $v \in T_p \mathcal{M}$ and represented as $h_*(v)$ to the tangent space associated with the element of $\mathcal{N}$ we denote via the map $h(p) \in \mathcal{N}$:
%      \begin{align}
%          h_*:& T\M \to T\N\\
%          v &\mapsto h_*(v)\\
%          h_*(v)&:=h \circ v \label{eqn:geo:pushforward}
%      \end{align}
%      where $v = [\gamma]$.
% \end{definition}
% Pushfowards are \textit{compositions} and they are important because they are mappings between tangent spaces. Pushfowards compose linearly and it can be shown that certain commutativity diagrams hold with respect to pushforwards such that, as maps between tangent spaces, they are independent of intermediate tangent spaces/manifolds through which they transition.

% %Tensor fields and tangent spaces
% \subsection{Tensor fields and tangent spaces}\label{sec:geo:Tensor fields and tangent spaces}
% To understand the connection between geometry and Lie algebras, and ultimately symmetry groups relevant to quantum machine learning, we focus on tensor fields. Recall that a derivation is a function on an algebra which generalizes certain features of the derivative operator. For an algebra $A$ over a field $K$ (also a ring), a \textit{derivation} of $A$ is a map $D: A \to A$ such that:
%     \begin{align}
%         D(\alpha f + \beta g) &= \alpha Df + \beta Dg \qquad \text{(scalar distributivity)}\\
%         D(fg) &= f D(g) + gD(f) \qquad \text{(product rule aka Liebniz's law)}
%     \end{align}
%     where $\alpha,\beta \in \Km; f,g \in A$. Intuitively, we can think of derivations as typical linear operators that allow differentiation along a direction. $C^m$ forms an algebra such that (this also relates to the condition of being a \textit{derivation}):
%     \begin{align}
%         (\lambda f)(p) &= \lambda f(p) \qquad \text{(Scalar multiplicative distributivity)}\\
%         (f + g) (p) &= f(p) + g(p) \qquad \text{(Additive distributivity)}\\
%         (fg) (p) &= f(p) g(p) \qquad \text{(Multiplicative distributivity)}
%     \end{align}
%     for $\lambda \in \mathbb{F}$ (the field), $p \in M$ and $f,g \in C^\infty$. Importantly, tangents vectors can be construed as operators or linear maps acting on functions $f \in \cinfm \to \M$ by noting they satisfy the requirements of a derivation. This is a useful way to build intuition around tangent vectors as differential operators upon a space and can be seen via the definition of tangent vectors themselves i.e:
%      \begin{align*}
%         v(f) = \frac{df(\gamma(t))}{dt}|_0
%     \end{align*}
%     where $v=[\gamma]$, the equivalence class of curves tangent at $p \in \mathcal{M}$ (sometimes tangent vectors are described as a derivation map from such a ring of functions on $\cinfm$ into $\Real$). The space of derivations $D_p\M$ (i.e. $D$ at $p \in \M$) satisfies the requirements of being a real vector space if we define:
%     \begin{align*}
%         (v_1 + v_2)f = v_1(f) + v_2(f), (rv)f = rv(f)\qquad v_1,v_2,v\in D_p(\M), r \in \R, f \in C^\infty(\M)
%     \end{align*}
%     As shown in the literature, it can be shown that the vectors in such a space of derivations have a representation as vectors in the space constituted by partial derivatives as vectors, allowing the equating of derivations at $p$ with the tangent space at $p$. In this representation, the partial derivatives represent the basis vectors of the vector space with coefficients (component or coordinate functions) as:
%     \begin{align*}
%       v \in D_p(\M) \implies v = \sum_{\mu = 1}^m v(x^\mu)\pardiv = \sum_{\mu = 1}^m v\mu\pardiv
%     \end{align*}
%     where the set of real numbers $\{ v^1,...,v^m \}$ or $\{ v^\mu \}$ are the components of the vector in the `direction' of $partial_{x^\mu}$. That is, it can then be shown that there exists an isomorphism between $T_p\M$ and $D_p\M$ allowing, in particular expression of important terms such as the Jacobian in terms of local representatives of push-forward maps between tangent planes.

%     %Vector fields and n-forms
%     \subsubsection{Vector fields and $n$-forms}\label{sec:geo:Vector fields and n-forms}
%     Of particular importance to quantum information and algebraic transformations in this work is the concept of a \textit{vector field} as an assignment of vectors in tangent planes to each point in $\M$.

% \begin{definition}[Vector field]\label{defn:geo:vectorfield}
% A vector field $X$ on a $C^\infty$ manifold $\M$ is a \textit{derivation} of the algebra $C^\infty(M)$ by way of an assignment of $X_p \in T_p\M, \forall p \in \M$. Given $f \in C^\infty(\M)$ and vector fields $X,Y \in D(\M)$, then $Xf$ and $X + Y$ are also vector fields as follows:
%     \begin{align}
%         X_p f: \M \to \Real & \qquad p \mapsto (Xf)(p) \\         X + Y&: p \to Xp + Yp
%     \end{align}
%     for $p \in \M$.
% \end{definition}
% To each $p \in \M$ is associated a vector field. We think of vector fields as operators on functions $f$ which are themselves defined on $\M$. Note in the set of vector fields,  Helgason \cite{helgason_differential_1979} denotes $X,Y \in D(M)$ as $\mathcal{D}^1(\M)$. If the above conditions are met, then $D(\M)$ is a module over the ring of functions $F$ on $C^\infty(M)$. If both vector fields are in this module, i.e. if $X,Y \in D(\M)$, then we have that $XY-YX$ is also a derivation of $C^\infty(M)$ and is itself a vector field. This vector field (again, a mapping of the algebra over the field, in this case over $C^\infty(M)=A$ in the above definition of derivation) is denoted:
%     \begin{align}
%         [X,Y] = XY-YX
%     \end{align}
% and aligns as the Lie derivative (commutator) (see definition (\ref{defn:alg:Lie algebraliederivative})). That is, for the map $X:C^\infty(\M) \to C^\infty(\M)$, the map above from $\M \to \R$ defined by $(Xf)(p) = X_p F$ defines a geometric characterisation of the Lie derivative of the function $f$ along the vector field (assignment of tangent vectors which are operators) $X$. The set of all vector fields $X$ on $\M$ is sometimes denoted $VFld(\M)$ \cite{isham_modern_1999} or $\mathfrak{X}(\mathcal{M})$ (or $\Gamma(\M)$) and carries the structure of a real vector space.
% \\
% \\
% Note that a vector field can be regarded as a first-order differential operator. Recall the tangent vector $X_p \in T_p\M$ is differential operator $C^\infty$ functions defined on $\M$. A vector field, as an assignment of such tangent vectors, can be considered first-order differential operator on $\M$. Thus for a neighbourhood around $p$ given by $U\in\M$, the vector field related to $X$ can be defined as:
%     \begin{align*}
%         X = \sum_{\mu =1}^m (Xx^\mu)\frac{\partial}{\partial x^\mu}
%     \end{align*}
%     where $Xx^\mu$ are the coefficient functions and the partial derivatives the basis. The functions $Xx^\mu$ are the \textit{components} of the vector field $X$ with respect to the coordinate system associated with the chart $(U,\phi)$. The components are sometimes denoted $X^\mu$ (though notation may vary) i.e. they are the coordinate functions that tell us the components of the vector at some point $p\in\M$ given a coordinate system. The form of the components depends upon the coordinate chart in use. Given two coordinate charges $(U,\phi),(U',\phi')$ with $U \bigcup U' \neq \emptyset$, the tangent vector should be defined in a way that it is equivalent across two coordinate systems, that is:
%     \begin{align*}
%         X = \sum_\mu Xx^\mu \partial_{x^\mu} = \sum_\nu Xx'^\nu \partial_{x'^\nu}
%     \end{align*}
% \hl{fix} Defining $Xx^\mu=X^\mu,Xx^\nu=X^{\nu'}$ and removing the summation over $\nu$ allows us to then express the coefficient functions in one coordinate chart (or frame) in terms of another:
%     \begin{align*}
%         X^{\nu'} = \sum_\mu X^\mu \frac{\partial x'^\nu}{\partial x^\mu}
%     \end{align*}
% \subsubsection{Vector fields and commutators}
% We explicate a number of relevant features of vector fields and commutators, given their importance in both quantum and geometric methods adopted in later chapters. Commutators arise in this context by considering composition of vector fields: naively multiplying two vector fields does not obtain a third. $X,Y$ can be viewed as linear maps from $C^\infty(\M) \to \cinfm$. So we can define the composition $X \circ Y: \cinfm \to \cinfm$ as $X \circ Y(f) = X(Y(f))$ however this is not a vector field because the Leibnizian derivation property (`product rule') isn't satisfied. Instead, it can be shown that $X \circ Y - Y \circ X$ satisfies the derivation criteria (see text) and so is a vector field:
%     \begin{align*}
%         (X \circ Y - Y \circ X)(fg) = g(X \circ Y - Y \circ X)f + f(X \circ Y - Y \circ X)g
%     \end{align*}
%     This composed vector field is the \textit{commutator} of vector fields $X,Y$ and is denoted $[X,Y]$. In component form the commutator is represented as:
%      \begin{align}
%         [X,Y]^\mu = \sum_\nu (X^\nu Y^\mu_{\nu} - Y^\nu X^\mu_{\nu}) \label{eqn:geo:commutatorcomponentform}
%     \end{align}
% As discussed above, the commutator is both antisymmetric $[X,Y]=-[Y,X]$ and importantly satisfies the Jacobi identity. The relation to Lie algebras is apparent. In general a Lie algebra defined as a real vector space $\mathcal{L}$ together with a bilinear map $\mathcal{L} \times \mathcal{L} \to \mathcal{L},(A,B) \mapsto [A,B]$ satisfies (a) antisymmetry and (b) the Jacobi identity for elements $A,B \in \mathcal{L}$. This bilinear mapping is not associative (ordering matters), forming a non-associative algebra. Note that the Lie algebra `bracket' is defined as compositions which satisfy antisymmetry and Jacobi, rather than directly as the commutator. It turns out that for certain vector spaces (those with which we are concerned in this work), the commutator will satisfy the requirements for being a Lie algebra. One such example is the set of $M(n,\C)$ where the Lie bracket is defined to be the commutator $[AB]:=AB-BA$ as discussed above. For our purposes, the results relating to vector antisymmetry and satisfaction of the Jacobi equation imply that the set of vector fields $X$ on $\M$ (using the same notation for a set as an individual field) have the structure of a real Lie algebra. Note also that, if $h: \M \to \N$ and the associated pushforward satisfies $h_*:T_p\M \to T_{h(p)}\N$ then each manifold is considered $h$-related.

% \subsubsection{Integral curves and Hamiltonian flow} \label{sec:geo:Integral curves and Hamiltonian flow}
% We now connect the theory of vector fields with integral curves and [Hamiltonian] flow, on our way towards understanding the theory of Riemannian and sub-Riemannian geodesic curves. Vector fields can be regarded as generators of an `infinitesimal' diffeomorphism of a manifold e.g. in the form $\delta(x^\mu) = \epsilon X^\mu(x)$. Recall that tangent vectors can be regarded as (a) equivalence classes of curves or (b) derivations defined at a point in the manifold. The question is: given a vector field $X$ on $\M$, is it possible to `fill' $\M$ with a family of curves in such a way that the tangent vector to the curve that passes through any particular point $p \in \M$ is just the vector field $X$ evaluated at that point, i.e. the derivation $X_p$? This idea is important in general canonical theory of classical mechanics, where the state space of a system is represented by a certain (even-dimensional e.g. symplectic phase-space) manifold $\mathcal{M}$ and physical quantities are represented by real-valued differentiable functions on $\mathcal{M}$. The manifold $\mathcal{M}$ is equipped with a structure that associates to each such function (representing physical quantities) $f:\mathcal{M} \to \R$ a vector field $X_f$ on $\mathcal{M}$. The family of curves that `fit' $X_f$ play an important role in the theory. In particular for quantum systems, curves associated with the vector field $X_H$ where $H: \mathcal{M} \to \R$ is the \textit{energy function}, are dynamical trajectories of the system i.e. [the Hamiltonian flow]. \hl{Query whether to discuss Hamiltonian flow a bit more}
% \\
% \\
% Of particular importance to our search for time-optimal curves (geodesics) in later chapters are integral curves. We want to find a single curve that (i) passes through $p\in\M$ and (ii) is such that the tangent vector at each point along the curve agrees with the vector field at that point. For this we use the definition of an \textit{integral curve}.
% %
% %definition integral curves
% \begin{definition}[Integral curves]\label{defn:geo:Integral curves}
% Given vector field $X$ on $\M$, the integral curve of $X$ passing through $p \in \M$ is a curve $\gamma: (-\epsilon,\epsilon) \to \M, t \mapsto \gamma(t) $ such that (at the identity in $\R$) we have $\gamma(0) = p$ and the push-forward satisfies:
%     \begin{align*}
%         \gamma_*\left( \frac{d}{dt} \right)_t = X_{\gamma(t)} \qquad \forall t \in (-\epsilon,\epsilon) \subset \R
%     \end{align*}
% \end{definition}
% The components of $X^\mu$ of the vector field $X$ determine the form taken by the integral curve $t \mapsto \gamma(t)$. Remember, the vector field (and tangent vectors) should be thought of as differential operators, so we have:
%     \begin{align*}
%         X^\mu(\gamma(t)) = \frac{d}{dt}x^\mu (\gamma(t))
%     \end{align*}
%     with the boundary condition that $x^\mu(\gamma(0)) = x^\mu (p)$. Certain other properties are also sought on integral curves, such as completeness properties such that the curves are defined for all $t$ (associated with assumptions regarding the compactness of the manifold).  
% \\
% \\
% We are also interested in the extent to which a vector field can be regarded as the generator of infinitesimal translations on the manifold $\M$. To this end we define a one-parameter group of local diffeomorphisms (see definition \ref{defn:alg:one_parameter_subgroup}) at a point $p \in \M$ consists of the following (a triple with certain properties): (i) an open neighbourhood $U(p)$, (ii) a real constant $\epsilon > 0$ and (iii) a family of diffeomorphisms of $U$, given by $\{ \phi_t | |t|>\epsilon\}$ onto the open set $\phi_t(U) \subset \M$, i.e. $\phi_t: \epsint \times U \to \M$ and $(t,q) \mapsto \phi_t(q)$. The group has the following properties: (a) maps from the parameter and neighbourhood to $\M$ are smooth, i.e. $\epsint \times U \to \M, (t,q) \mapsto \phi_t(q)$ is smooth on both domains; (b) compositions follow $\phi_s(\phi_t(q)) = \phi_{s + t}(q)$ and $\M$, i.e. $\phi_0 (q) = q$. The set of local diffeomorphisms is denoted Diff($\M$). The term \textit{one-parameter subgroup} refers to the composition property (b) above and that the map $t \to \phi_t$ can be thought of as a representation (vector space with map) of part of the additive group of the real line. Families of local diffeomorphisms can be thought of as \textit{inducing} vector fields. Through each point $q\in\M$, there passes a local curve $t \mapsto \phi_t(q)$. Because of the existence of this curve, we can construct a vector field on $U$ by taking tangents to this family of curves at $q$. This vector field is denoted $X^\phi$, the vector field induced by the diffeomorophism $\phi$, more formally:
%         \begin{align*}
%             X_q^\phi (f):=\frac{d}{dt}f(\phi_t(q))|_0 \qquad \forall q \in U \subset \M
%         \end{align*}
%  There is then a theorem that: $\forall q \in U$ the curve $t \mapsto \phi_t(q)$ is an integral curve of $X^\phi$ for $|t|<\epsilon$.

%  \subsubsection{Local flows}\label{sec:geo:Local flows}
%  We now briefly mention local flows and its connection with Diff$(\M)$. A \textit{local flow} of a vector field is a one-parameter local diffeomorphic group such that the vector fields induced by the group are the vector field itself. More formally, for a vector field $X$ defined on an open subset $U \subset \M$, the local flow of $X$ at $p$ is a one-parameter group of local diffeomorphisms defined on some open subset $V \subset U$ such that $p \in V \subset U$ and such that the vector field induced by this family equals $X$. In a local coordinate system, local flow - the  family of diffeomorphisms $\phi_t^X$ - is expressed in the following way:
%     \begin{align*}
%         X^\mu(\phi_t^X(q)) = \frac{d}{dt}x^\mu (\phi_t^X(q))
%     \end{align*}
%     around $q \in U \subset \M$. We then Taylor expand the coordinates (which are in a vector space) $x^\mu(\phi_t^X(q))$ of the transformed point $\phi_t^X(q)$ near $t=0$, resulting in:
%     \begin{align*}
%         x^\mu(\phi_t^X(q)) = x^\mu(q) + tX^\mu (q) + O(t^2)
%     \end{align*}
%   Recalling that $x^\mu(\phi_t^X(q)) \in \Real^m$, the expansion shows that the coordinates $x^\mu$ of the transformed of $q \to \phi_t^X(q)$ are approximated by the original coordinates $x^\mu(q)$ translated to first order by $tX^\mu(q)$. As $X^\mu$ belongs to the vector field, this is what allows us to say that the vector field generates `infinitesimal' transformations on the manifold because it is responsible (up to approximation) for `shifting' from $q$ to $\phi_t^X(q)$ in terms of a local coordinate system on the manifold. We discuss the relationship of integral curves and local flows to time-optimal geodesics in the context of geometric control theory further on in section \ref{sec:geo:Symplectic manifolds and Hamiltonian flow} on Hamiltonian flow, providing a connection between geometric formalism and quantum information processing.

% %======SECTION: Cotangent vectors and dual spaces
% \subsection{Cotangent vectors and dual spaces}
% In this section, we discuss important concepts of one-forms, cotangent vectors, leading to discussion of pullbacks, tensors and $n$-forms along with corresponding definitions of covariance and contravariance. 

% \subsubsection{Dual spaces and one forms}\label{sec:geo:Dual spaces and one forms}
% Recall from above the definition (\ref{defn:quant:Dual space}) that for any vector space $V = V(\mathbb{K})$ we define the associated dual space $V^*$ as the space of all bounded linear maps $L:V \to \mathbb{K}$ (see definition \ref{defn:quant:Bounded linear operators}). Here we focus on $\mathbb{K}=\R$ for exposition. In this mapping formulation, the \textit{dual} of a real vector space $V$ is the collection $V^*$ of all linear maps $L:V \to \R$. The action of $L \in V^*$ on $v \in V$ is usually denoted $\braket{L,v}$ or sometimes with the subscript $V$ as well. Note that here $\braket{\cdot,\cdot}$ represents the evaluation of the functional at a vector in the sense of assigning a scalar to each vector $v \in V$. Note that by the Riesz representation theorem (for finite dimensional $V$), the isomorphism between $V$ and $V^*$ means that we can associate to each vector $v$ a unique such functional $L_v$, thus allowing us to view the evaluation of functionals in this way as a generalisation of the inner product (hence the notational similarity). The dual itself can be given the structure of a real vector space by leveraging the vector-space properties of $\R$ into which $L$ maps i.e.:
%     \begin{enumerate}[(i)]
%         \item $\braket{L_1 + L_2,v} := \braket{L_1,v} + \braket{L_2,v}$ i.e. we in some sense induce addition in $V^*$ by reference to the two images;
%         \item $\braket{rL,v}:= r\braket{L,v}, r \in \Real$.
%     \end{enumerate}
% If $V$ with $\dim V < \infty$ has a basis $\{e_1,...,e_n\}$, then the \textit{dual basis} for $V^*$ is a collection of vectors $\{f^1,...,f^n \}$ (they are vectors because they are just linear maps $L \in V^*$ which is a vector space). This set $\{f^i \}$ is uniquely specified by the criterion that:
%     \begin{align}
%         \braket{f^i, e_j} = \delta^i_j         \label{eqn:geo:dualdelta}
%         \end{align}
% Note equation (\ref{eqn:geo:dualdelta}) may also be written as $f^i(e_j) = \delta^i_j$ where duals take (or act upon) vectors as their arguments, which is in essence an application of the Riesz representation theorem. Because of the isomorphism between a vector and its dual, one can `invert' dual and vector spaces, so the dual is the argument of a vector map to a scalar, but for clarity one usually maintains the formalism above. For maps between different vector spaces $L: V \to W$, then $L$ induces a dual mapping $L^*: W^* \to V^*$ on $k \in W^*$ by:
%     \begin{align*}
%         \braket{L^*k,v}_V:=\braket{k,Lv}_W
%     \end{align*}
%     which says that the dual-map $L^*$ acting on $k$ in $W^*$ (itself a dual space) generates a map $L^*k$ which lives in $V^*$. This map then acts on $v \in V$ (taking it to $\R$), acting as a pullback (discussed below): $L^*$ is pulling back the linear functional $k$ from $W^*$ to a linear functional in $V^*$. To explicate the relationship between $V$ and $V^*$, it can be shown that there exists a canonical map $\chi:V \to (V^*)^*$ where $\braket{\chi(V),\ell}_{V^*} = \braket{\ell,v}_V$ where $V \in V, \ell \in V^*$ which is an isomorphism if $\dim V < \infty$. This concept captures the spirit of what is sometimes described as $V$ being equivalent to the `dual of its dual'. With these concepts to hand, we can now define cotangent structures.

%     \begin{definition}[Cotangent vectors]\label{defn:geo:Cotangent vectors}
%         A cotangent vector is a map from tangent space to $\R$. At a point $p\in\M$, it is defined as a \textit{real linear map}: 
%     \begin{align*}
%         k:T_p\M \to \R
%     \end{align*}
%     The value (which is in $\R$) of $k$ when acting on $v\in \tpn$ is denoted $\braket{k,v}$ or $\braket{k,v}_p$ (analogous to using inner-product symbolism for mapping to scalar or contraction).
%     \end{definition}
% The \textit{cotangent space} is the space of all cotangent vectors i.e. at $p \in \M$ it is the set $T^*_p\M$ of all such linear maps constituting cotangent vectors. It is a vector space and is the dual of the vector space $\tpn$. Similarly, the \textit{cotangent bundle} $T^*\M$ is the collection (a vector bundle) of all such cotangent for all $p \in \M$ i.e. $T^*\M = \bigcup_{p\in\M} T^*_p\M$. 


% We now come to the important definition of a one-form. In the field of geometric optimal control, one-forms are essential for formulating and solving control problems. One-forms can represent constraints and objectives in control problems, particularly in the context of Hamiltonian systems, where the dynamics can be expressed in terms of symplectic geometry (which we discuss in section \ref{sec:geo:Symplectic manifolds and Hamiltonian flow}).
% %one-form definition
% \begin{definition}[One-form]\label{defn:geo:One-form}
% A one form $\omega$ defined on $\M$ is an assignment of a cotangent vector (being a smooth linear map) $\omega_p$ to every point $p \in \M$. We can consider a one-form as a map from a vector field (as a vector space) to $\R$ i.e. $\omega: X \to \R$ for $X \in \mathfrak{X}(\M)$ i.e. a one-form is a field of cotangent vectors, meaning it assigns a cotangent vector to each point in a smoothly varying manner.
% \end{definition}
% One-forms are useful and important for understanding tensorial contractions and, under certain conditions, relate to inner products. Noting that $\braket{\omega,X}(p):=\braket{\omega_p,X_p}_p$, we observe that the one-form as an assignment of a cotangent vector to each point $p \in \M$, in turn induces a map from the tangent plane at $p$ to $\R$. In this sense the representation $\braket{\omega_p,X_p}_p$ specifies a map $\omega$ from the vector field at $p$ to $\R$ and that this mapping is smooth i.e. infinitely-differentiable. Connecting with the definition of the inner product (equation (\ref{defn:quant:Inner Product})) above, we can consider an inner product in terms of tangent spaces:
% \begin{align}
%     \braket{\cdot,\cdot}: T_p\M \times T_p\M \to \R \label{eqn:geo:oneforminner product}
%     \end{align}
% and one forms. Consider a metric tensor $g$ which is a type $(0,2)$-tensor meaning it takes two vectors as an argument and returns a scalar. Choosing an inner product $\braket{\cdot,\cdot}$ on a vector (tangent) space $T_p\M$ gives rise to an isomorphism:
%     \begin{align*}
%         \varphi:& T_p\M \to T^*_p\M \qquad
%         v \mapsto \braket{v,\cdot}
%     \end{align*}
% The function $\varphi(u)$ takes $u \in \tpn$ and returns its dual such that that $\varphi(u)(v) = \braket{u,v}$ i.e we have a function taking a vector, obtaining its dual then taking the inner product with $v$ and returning a real number. In this sense, we can identify the inner product as the action of a covector on a vector i.e:
%     \begin{align*}
%         \braket{u,v} = \varphi(u) v
%     \end{align*}
%    In terms of components of the metric tensor, this is equivalent to:
%     \begin{align*}
%         \braket{u,v} = g_{ij}u^i v^j = u_jv^j
%         \label{eqn:tensordualinnerproductmetric}
%     \end{align*}
%     but noting that there is no canonical identification of $V$ with $V^*$. Such concepts are important in quantum and geometric methods, especially Hamiltonian dynamics where, if a system has a configuration space $Q$ then the space of classical states is defined to be the cotangent bundle i.e. set of all linear maps from the tangent plane into $\R$ (see \cite{isham_modern_1999}). We briefly note the expression of dual vectors in terms of components and basis elements.\\
%     \\
% As discussed above, selecting a local coordinate system around $p \in \M$ (i.e. a mapping from $p$ to $R^m$ gives rise to a basis set associated with $p \in \M$:
%         \begin{align*}
%             \bigg\{ \pardivx \bigg\}
%         \end{align*}
%         This is a basis for the set of derivations and thus of the tangent space at $p$ by the isomorphism above. There is also an associated basis about $p$ for the corresponding dual $\tpndual$. It is denoted by what via differential operators:
%         \begin{align*}
%             (dx^1)_p,...,(dx^m)_p
%         \end{align*}
%         As with the basis of the dual space above, the basis for the dual space $\tpndual$ is given via a set of linear operators in the dual space which when composed with the basis vectors of $\tpn$ (i.e. the $\pardivx$ operators), leads to deltas. That is:
%         \begin{align}
%             \bigg\langle{(dx^\mu)_p,\left( \frac{\partial}{\partial x^\nu} \right)\bigg\rangle}_p := \delta^\mu_\nu 
%             % \label{eqn:geo:innerproductvectordualdelta}
%         \end{align}
%         In this way, we can expand dual vectors $k \in \tpndual$ in terms of component functions and this basis:
%         \begin{align*}
%             k = \sum_\mu^m k_\mu (dx^\mu)_p
%         \end{align*}
%         where the components $k_\mu \in \R$ of the vector for the coordinate system and thus the basis vectors $\pardivxdual$ are given via the bilinear map (e.g. inner product in certain contexts) of the dual vector $k$ with the basis element of the tangent vector:
%         \begin{align*}
%             k_\mu = \bigg\langle{k,\left( \pardivx \right)_p\bigg\rangle}_p
%         \end{align*}
%         Remembering that $k$ is a map acting on $v \in \tpn$, then we can write the bilinear map pairing $\braket{k,v}$ similarly as:
%         \begin{align*}
%             \braket{k,v} = \sum_\mu^m k_\mu v^\mu
%         \end{align*}
%         recalling $v^\mu = v(x^\mu)$ and the resemblance here to inner products.
% %
%         Using this formalism, we can choose a local representation for one forms:
%         \begin{align}
%             \omega = \sum_\mu \omega_\mu dx^\mu
%         \label{eqn:geo:dual-omegasumomegamudxmu}
%         \end{align}
%         i.e. we can express a one-form (contangent vector) in terms of the basis set of the dual space where the above is a shortened expression for:
%         \begin{align*}
%             \omega_p = \sum_\mu \omega_\mu(p) (dx^\mu)_p
%         \end{align*}
%         for $p \in U \subset\M$. The components $\omega_\mu$ of $\omega$ are \textit{functions} on $U$:
%         \begin{align*}
%             \omega_\mu(q) := \bigg\langle{\omega, \pardivx\bigg\rangle}_p
%         \end{align*}
%         where $q \in U \subset \M$.
% Such a construction shows how a one-forms can be construed as smooth cross-sections of $T^*\M$ analogous to vector fields defined as smooth sections of $T\M$ (see \cite{isham_modern_1999}).
% \subsubsection{Pullbacks of one-forms}
%  We now describe the pullback property of one-forms.  While it isn't true in general that a map $h: \M \to \N $ (between manifolds) can be used to push-foward a vector field on $\M$ i.e. we cannot always use some commuting differential form to act as our pushfoward in the general case, this map $h$ \textit{can} be used to \textit{pull-back} a one-form on $\N$. This feature is connected with the way in which the global topological structure of a manifold is reflected in \textit{DeRham cohomology groups} of $\M$ defined using differential forms and to the fact that fibre bundles also pull-back (not push-forward) (see Frankel \cite{frankel_geometry_2011} $\S13$ for detailed discussion).
% %pullback definition
% \begin{definition}[Pull-back]\label{defn:geo:Pull-back}
%     A pullback is the dual of the map between tangent spaces across manifolds. If $h: \M \to \N$ and we have the linear map (the pushfoward) $h_*: \tpn \to T_{h(p)}\N$, then then \textit{pullback map} is defined as:
%     \begin{align}
%         h^*:T_{h(p)}^*\N \to T_{p}^*\M \label{eqn:geo:pullback}
%     \end{align}
%     and is considered under certain conditions the dual of $h_*$. This means that for all maps (which are also vectors in the associated vector space) $T_{h(p)}^*\N$ and $v \in \tpn$ we have :
%     \begin{align*}
%         \braket{h^*k,v}_p := \braket{k,h_*v}_{h(p)}
%     \end{align*}
% \end{definition}
% To unpack the formalism, note that $T^*_{h(p)}\N$ is a reference to the dual of the tangent space for $p\in\M$ mapped to $h(p)\in\N$, so we can see $h^*$ as `pulling back' to the dual space of $p\in\M$. The term $\braket{h^*k,v}_p$ refers to $h^*$ (the pullback) acting on $k$ i.e. it `pulls back' the map $k$ living in $T_{h(p)}^*\N$ to a map living in $T_{h(p)}^*\M$. Thus $h^*k$ is a map living in $T_{h(p)}^*\M$ which is itself a linear map that acts on the tangent space $\tpn$, i.e. $v \in \tpn$. The definition says that this pullback is equivalent (diagrammatically) to $k$ acting on $h_*$ having been pushed forward to $T_{h(p)}\N$ which means it cans be acted on by $k \in T_{h(p)}^*\N$. In both cases, we have a mapping to $\R$.
% \\
% \\
% We can also extend pullbacks to one-forms. Recall, a one-form is an assignment of a cotangent vector $\omega_p$ to $p\in\M$ and this cotangent vector, which is a mapping from $\tpn$ to $\R$, acts on the tangent vector at $p$, i.e. $v \in \tpn$ to $\R$. We define a pullback of one-forms as follows.
% \begin{definition}[Pull-back (one-forms)]\label{defn:geo:Pull-back (one-forms)}
%     iIf $\omega$ is a one-form on $\N$, then the pullback of $\omega$ is itself a one-form $h^*\omega$ on $\M$ expressed as:
%     \begin{align*}
%         \braket{h^*\omega,v}_p := \braket{\omega,h_* v}_{h(p)}
%     \end{align*}
%     for all $p \in \M$ and $v \in \tpn$. 
% \end{definition}

% It can be shown (see \cite{isham_modern_1999} for specifics exposition) that the pullback $h^*$ of $\omega$ (again, in the dual space of $\N$) evaluated at $p \in \M$ is given by the pullback acting on that one-form $\omega$, i.e. $h^* \omega$ when then acts on the \textit{basis} elements of $\tpn$, namely the $\pardivx$ terms, mapping them to $\R$ via the bilinear form. This is then definitionally equated with the one-form $\omega$ acting on the basis element $\pardivx$ of $\tpn$ once it has been `pushed foward' to $\tpnn$ by the pushfoward map $h_*$, which also is equivalent to an evaluation of the one-form at $h(p)$ (as we are assuming the existence of $h: \M \to \N$ here). The point of the pullback is to allow the structure of maps defined on or in relation to one manifold, say $\N$, to be expressed or represented in terms of structure on or related to another manifold $\M$.

%     \subsubsection{Lie derivatives and pullbacks}
%     We now specify the relationship of Lie derivatives (and thus commutators) to pullbacks. Using definition (\ref{defn:geo:Pull-back (one-forms)}), the pull-back of a one-form $\omega$ on $\mathcal{M}$ can be related to a vector field $X$ with an associated one-parameter group of local diffeomorphisms $t \to \phi_t^X$. For each $t$, there exists an associated pull-back $\phi_t^{X^*}$. This one-parameter family of pulled-back forms describes how the one-form $\omega$ changes along the flow lines (integral curves) of $X$. In this formalism we can connect Lie derivatives to one forms and pullbacks. The \textit{Lie derivative} of $\omega$ associatef with vector field $X$ is then the \textit{rate of change} of $\omega$ along the flow-lines (integral curves) of the one-parameter group $\phi_t^X$ of diffeomorphisms associated with the vector field $X$. That is:
%     \begin{align}
%         L_{X}\omega := \left.\frac{d}{dt}\right|_{t=0} \phi_t^{X^*}\omega
%     \label{eqn:geo:liederivativepullback}
%     \end{align}
%     Note by comparison that the Lie derivative can be expressed as:
% \begin{align}
%     \frac{d}{dt}\bigg|_{t=0} \phi^X_{-t_*}(Y) = [X,Y] = L_XY
% \end{align}
% Recall that that $X$ in $\phi_t^X$ refers to the group of \textit{local} diffeomorphisms that induce the vector fields $X$. Then $\phi_t^{X^*}$ is the family of diffeomorphisms that generate the \textit{dual} cotangent vector field $X^*$. Equation (\ref{eqn:geo:liederivativepullback}) can be understood as follows. Recall that $L_Xf = Xf$ and $L_XY = [X,Y]$ (as naive multiplication of vector fields lacks the derivation quality). It can be shown that $L_X\braket{\omega,Y} = \braket{L_X\omega,Y} + \braket{\omega,L_XY}$. 
%     Recall $\phi^X_t$ representing the flow of $X$ on $\mathcal{M}$ (a one-parameter group of diffeomorphisms). This says that each value of $t$ is associated with a diffeomorphism from $\M$ to itself. The flow moves points along the integral curves of the vector field $X$. Associated with such flow ias an inverse flow, indicated by the negative sign in $\phi^X_{-t}$, in essence a rewinding of the flow (which recall is possible as a diffeomorphism). $\phi^X_{-t}$ moves points $p\in\M$ along integral curves in the opposite direction to $\phi^X_t$. In this way, we can see how the commutator (Lie derivative) $[X,Y]$ expresses the rate of change of the vector field $Y$ along integral curves of $X$. 
% \\
% \\
%  Moreover, $df$ can be used to define the \textit{exterior derivative}.
%  \begin{definition}[Exterior derivative]\label{eqn:geo:Exterior derivative}
%      The exterior derivative of $f \in \cinfm$ is given by:
%      \begin{align*}
%         \braket{df,X}:=Xf = L_xf
%     \end{align*}
% for vector fields $X$ on $\M$.
%  \end{definition}
%    In local coordinates, this has a representation as:
%     \begin{align*}
%         (df)_p = \sum_\mu^m \left( \frac{\partial}{\partial x^\mu} \right)_p f (dx^\mu)_p
%     \end{align*}
%     i.e. we represent the function in the dual basis $dx^\mu$ of $X^*$, then take the derivative with respect to the coordinates in $X$, i.e. $\partial_\mu$. Note also the commutation of the pullback $h^*$ with $f$, $h^*(df) = d(f \circ h)$. 

% \subsection{General tensors and $n$-forms}
% We can now express tensors, discussed in earlier chapters, with the geometric formalism above, which we utilise further on in terms of our discussion of time-optimal geometric control. Generalising tangent and cotangent vectors requires tensors and $n$-forms. To do this, we require the idea of the \textit{tensor product} of two vector spaces $V$ and $W$, denoted (as per definition (\ref{defn:quant:Tensor Product})) by $V \otimes W$. The tensors examined in earlier chapters can then be represented as compositions of tangent and cotangent spaces.

% \begin{definition}[Tensor types (geometric)]\label{defn:geo:Tensor types (geometric)}
%     tensors are composed of elements of the vector products of tangent spaces and cotangnet spaces. Formally, a \textit{tensor of type} $(r,s) \in T_p^{r,s}\M$ at a ponit $p\in\M$ belongs to the tensor product space:
%     \begin{align}
%         T_p^{r,s}\M := \Bigg[\otimes^r T_p\M \Bigg] \otimes \Bigg[\otimes^s T^*_p \M\Bigg]\label{eqn:geo:Trstensortype}
%     \end{align}
%      i.e. $r$ tensor products of the tangent space with itself tensor-producted with $s$ tensor products of the dual cotangent space. 
% \end{definition}
% The basis of $T^{r,s}_p\M$ can be thought of as composed of the tensor products of the basis elements of the tangent space (partial derivatives) and the basis of the dual (cotangent) space (differentials):
%         \begin{align*}
%     T_p^{r,s}\M=\Bigg[ \otimes_{i=1}^r \left( \frac{\partial}{\partial x^{\mu_i}} \right) \Bigg] \otimes \Bigg[ \otimes_{j=1}^s (dx^{v_j}) \Bigg]
%         \end{align*}
% By convention, we can designate $r=0 \to \R$ with $W \otimes \R \simeq W$ for a real vector space $W$. In this formulation with vectors and their duals, tensors as linear maps becomes apparent. For (finite) $\tpn$ and $\tpndual$, we can define tensors in terms of a vector space and its dual. We can represent the $T_p^{r,s}$ type tensor in terms of a multilinear mapping of the Cartesian product of a vector space and its dual to $\R$ which, in functional notation (Cartesian products describing the function of tensors rather the direct product) is given by:
%     \begin{align*}
%         \bigg(\times^r \tpndual\bigg) \times \bigg(\times^s \tpn\bigg) \to \R
%     \end{align*}
% In this formulation, a multilinear is viewed as a function that takes $r$ tangent vectors as input and $s$ cotangent vectors as input and maps them to $\R$ (the difference being notational, $r$ always indexes the tangent vectors, $s$ always indexes the cotangent vectors). The upper index $r$ indices the number of contravariant components of the tensor associated with $\tpn$. These are akin to `directional' components transforming in the same way as coordinate differentials $dx^i$. These contravariant components are typically denoted via superscripts corresponding to directions the tensor acts along with respect to covectors. The subscript index $s$ denotes the number of covariant components, consisting of linear functionals in $\tpndual$ (recall for duals and vectors we have components and bases). This formulation is usefully understood in terms of equation (\ref{eqn:geo:dualdelta}) i.e. $\braket{f^i, e_j} = \delta^i_j $. Each basis element of the vector and its dual either annihilate or lead to unity, thus if we denote component coefficients $a,b \in \Real$ for vectors and duals $a f^i,b e_j$, then:
% \begin{align}
%     \braket{a f^i, b e_j} = ab\braket{f^i, e_j} = ab\delta^i_j
% \end{align}
% Thus the definition of vectors and duals, as bases of $\tpn$ and $\tpndual$ shows how the tensorial map effectively acts as contraction (see below) which reduces the dimensionality of the tensor product and then multiplies the remainder by the corresponding scalar product of the real coefficients of the basis vectors for the vector and its dual so annihilated. As we see below, the usual inner product on vector spaces can be framed in the language of metric tensors (where the metric tensor acts as a bilinear form resulting in a scalar product). Framing tensors as multilinear maps connects to concepts further on of, for example, \textit{metric tensors} which act on $\tpn$ and $\tpndual$ to contract tensor products to scalars, forming the basis for measuring the time, energy or length of paths given by Hamiltonian evolution in our quest for time-optimal geodesics. We note for completeness a few types of special $(r,s)$ tensors. Note the relation between the tangent planes and cotangent planes:
%     \begin{enumerate}[(i)]
%         \item $T_p^{0,1}\M = \tpndual$ is the cotangent space at $p$ (space of covectors or one-forms). An example at $p \in \M$ would be a vector in $\tpn$ with one contravariant component;
%         \item $T_p^{1,0}\M = \tpn = (\tpndual)^*$ (dual of dual returns the tangent plane). An example would be a covector or one-form in $\tpndual$ consisting of one covariant component;
%         \item $T_p^{r,0}\M$ is the space of \textit{r-contravariant} tensors (multilinear functions of covectors);
%         \item $T_p^{0,s}\M$ is the space of \textit{s-covariant} tensors (multilinear functions of vectors); 
%         \item $T_p^{r,s}\M$ a mixed tensor comprising both contravariant (acting on vectors) and covariant (acting on covectors) elements. Such higher-rank tensors are used to represent more complex objects, such as curvature tensors or stress-energy tensors.
%     \end{enumerate}
% where \textit{covariant} tensors are multi-linear maps that take vectors (from $\tpn$) as inputs and return scalars, while \textit{contravariant} tensors take covectors (from $\tpndual$) as inputs. From this we obtain a \textit{tensor field} on $\M$, which is a smooth association of a tensor of type $(r,s)$ for $p \in \M$. It is instructive to observe how $\tpn$ is associated with contravariant transformations while $\tpndual$ is associated with covariant transformations. This is intuitively related to the fact that dual spaces (cotangent spaces) consist of linear maps that act on vectors in the tangent space, hence they transform covariantly (i.e. they co-vary with vectors). On the other hand, structures that transform `opposite to the way tangent vectors do', i.e. according to the basis changes in the cotangent space, are said to transform contravariantly. Since tensor spaces can involve multiple layers of dual spaces, we consider their transformation properties in terms of how they relate to the transformations of the basis in the tangent and cotangent spaces. Note tensors can be defined as the unique bilinear map $V^* \times W^* \to \R$ which evaluates to $\braket{k,v}\braket{l,w} \in \R$ on $(k,l) \in V^* \times W^*$. We also can now usefully define a tensorial contraction as a generalisation of equations (\ref{eqn:geo:dualdelta}). 
% Contraction is an operation that reduces the order of a tensor by pairing covariant vectors, indicated by (lower) indices with  contravariant vectors, indicated by (upper) indices and summing over the dimension of the manifold, effectively treating the contraction over indices as if they are in an inner product, akin to a trace operation. Recalling that a tensor is a mapping (a function), then we can define the contraction as a function, being a tensor, that takes as its argument another tensor. In general, the contracting tensor can be of any order, but in practice contraction is often performed using metric tensors, tensors which, as maps to $\R$, satisfy the conditions of being metric (we discuss this below). The most general form of a contraction is set out below. Following \cite{helgason_differential_1979,isham_modern_1999} first recall that vectors and their duals are related via:
% \begin{align*}
% \langle X_{i} \otimes \cdots \otimes X_{r}, \omega_{s'} \otimes \ldots \otimes \omega'_{r} \rangle &= \prod_{i,j} \omega_{j}(X'_{i})\omega'_{i}(X_{j}),
% \end{align*}
% for $X_{i}, X'_{j} \in T^r\M$ and $\omega_{j}, \omega'_{i} \in T^*\M$.
% %tensor contraction definition
% \begin{definition}[Tensor contractions]\label{defn:geo:Tensor contractions}
% A $(1,1)$-contraction is a linear mapping $C^i_j: T^r_s \M \to T^{r-1}_{s-1}\M$ with $(C^i_j(T^r_{s}))_p = C^i_j(T^r_{s,p})$ for $T \in T^r_s \M, p \in \M$. The mapping $C^i_j$ is the contraction of the $i$th contravariant index and $j$th covariant index:
% \begin{align}
% C^i_j\underbrace{(\otimes_{j=1}^r X_j \otimes_{i=1}^s \omega_i )}_{(r,s)} &= \langle X_i, \omega_j \rangle (X_1 \otimes ... \otimes \hat{X}_i ... \otimes X_r \otimes \omega_1 \otimes \cdots \otimes \hat{\omega}_j ... \otimes \omega_s)\\
% &= \delta^j_i (X_1 \otimes ... \otimes \hat{X}_i ... \otimes X_r \otimes \omega_1 \otimes \cdots \otimes \hat{\omega}_j ... \otimes \omega_s)\\
% &= \underbrace{(X_1 \otimes ... \otimes \cancel{X_j} ... \otimes X_r \otimes \omega_1 \otimes \cdots \otimes \cancel{\omega_j} ... \otimes \omega_s)}_{(r-1,s-1)} \label{eqn:geo:Tensor contractions}
% \end{align}
% Where the $\hat{X_i}$ symbol denotes removal of the $i^{th}$ element (following \cite{helgason_differential_1979}). 
% \end{definition}
% Thus contraction reduces the rank of a tensor by one in both the covariant and contravariant indices. Note that in the more general setting, we can in principle construct a more general contraction mapping the product of individual contractions. In particular we examine metric tensors, which provide a way to compute inner products between tangent vectors, thereby inducing a geometry and way of measuring distance (and thus time optimality) on $\M$.

% \subsubsection{Metric tensor}
% We now move to the definition of the \textit{metric tensor}, of fundamental importance to time optimal and machine learning approaches adopted in later chapters.
% \begin{definition}[Metric tensor]\label{def:geo:metric_tensor}
%     The metric tensor is a [0,2]-form tensor field mapping $g_p: T_p\M \times T_p\M \to \R$ given by:
%     \begin{align}
%         g := g_{ij} dx^i \otimes dx^j \qquad g_{ij} := \braket{e_i,e_j} \qquad g^{ij:}=\braket{dx^i,dx^j} \label{eqn:geo:metric_tensor}
%     \end{align}
%     where $e_i=\partial_i=\partial_{x_i}$ are basis elements of $T_p\M$ and $dx_i$ are the corresponding dual basis elements for the inverse metric tensor $g^{ij}$.
% \end{definition}
% Recall in this notation that $v = v^j e_j$ so that and similarly for $v^j$ expressed in the dual basis. The metric tensor can be described in terms of Metric tensors induce an inner product space on $T_p\M$ allowing vector both lengths (magnitudes) and angles between vectors to be calculated. The metric tensor can be used for raising and lowering indices in effect converting between vectors and their covectors. The metric tensor acts on the vector \(v\) to produce its covariant components \(v_i\) through a process known as "index lowering." This process is described by:
% \begin{equation}
%     v_i = g_{ij} v^j.
% \end{equation}
% which can be seen, assuming an orthonormal basis $\{e_i\}$ as:
% \begin{align*}
% \braket{v,e_j}=\braket{v^ie_i,e_j}=v^i\braket{e_i,e_j}=v^i\delta_{ij}=v_j
% \end{align*}
% where $g_{ij}=\delta_{ij}$ in the orthonormal case (see \cite{frankel_geometry_2011} p.lix).
% % \begin{align*}
% % \braket{v,dx^j}=v^ie_idx^j=v^i\delta_i^j=v_j
% % \end{align*}
% % Also note: \cite{frankel_geometry_2011}:
% % \begin{align}
% %     g_{ij}dx^i\otimes dx^j(A,B) = g_{ij}dx^i\otimes dx^j(A^\alpha e_\alpha,B^\beta e_\beta) = g_{ij}A^\alpha B^\beta(\delta^i_\alpha,\delta^j_\beta)
% % \end{align}

% \subsubsection{$n$-forms and exterior products}
% We conclude this section introducing $n$-forms and exterior products. Consider an $n$-form as follows here $0 \leq n \leq \dim\mathcal{M}$ with $n \in \mathbb{N}$. A $0$-form is a function in $\mathcal{C}^\infty(\mathcal{M})$. A one-form ($1$-form) at each point $p \in \mathcal{M}$,  assigns a linear functional that maps vectors in $T_p\mathcal{M}$ to $\mathbb{R}$. It is a section of the cotangent bundle $T^*\mathcal{M}$. An $n$-form is then defined as follows.
% %n-form definition
% \begin{definition}[$n$-form]\label{defn:geo:nform}
%     An $n$-form is form of a \textit{tensor field}, represented by $\omega$, of type $(0,n)$ that is \textit{totally skew-symmetric}. For any permutation $P$ of the indices $1,2,\ldots,n$:
%     \begin{align*}
%    \omega(X_1,\ldots,X_n) = (-1)^{\deg(P)}\omega(X_{P(1)},\ldots,X_{P(n)})
%     \end{align*}
% \end{definition}
%       where $X_i$ are arbitrary vector fields on $\mathcal{M}$, and $\text{deg}(P)$ is the degree of the permutation $P$ ($+1$ even, $-1$ odd). Set of all $n$-forms on $\mathcal{M}$ is denoted $A^n(\mathcal{M})$.
%       % When $n$ equals the dimension of $\mathcal{M}$, an $n$-form is a top form that can be integrated over $\mathcal{M}$ if the manifold is orientable.
% We can now define an important concept, the \textit{wedge} or \textit{exterior product} in terms of a tensor product of $n$-forms.

% \begin{definition}[Exterior product]\label{defn:geo:Exterior product}
%     For $\omega_1 \in A^{n_1}(\M),\omega_2 \in A^{n_2}(\M)$ the \textit{wedge or exterior product} of n-forms $\omega_1,\omega_2$ is the $(n_1 + n_2)$-form, denoted $\omega_1 \wedge \omega_2$ and defined as:
%     \begin{align}
%         \omega_1 \wedge \omega_2 = \frac{1}{n_1! n_2!} \sum_{\sigma(P)}(-1)^{\deg(P)}(\omega_1 \otimes \omega_2)^P \label{eqn:geo:Exterior product}
%     \end{align}
%     where $\sigma(P)$ denotes permutations over $P$.
% \end{definition}
% The permutations $\sigma(P)$ are understood as follows. For a tensor field $\omega$ of type $(0,n)$, the \textit{permuted} tensor field $\omega^P$ is defined to be the permutation map applied to the permutation index i.e:
%     \begin{align*}
%         \omega^P(X_1,...,X_n) = \omega(X_{P(1)},...,X_{P(n)})
%     \end{align*}
%     for all vector fields $X_1,...,X_n$ on the manifold $\M$. The factor $1/(n_1!n_2!)$ is a normalisation factor given the ways of permuting $\omega_1,\omega_2$, while the sum over permutations $\sigma(P)$ ensures all orderings of vectors are considered and that the result is antisymmetric with respect to exchange of vectors. When applied to vector fields, the result is a real number interpreted as an oriented valume spanned by those vectors in the manifold. Intuitively one can think of how in two dimensions the wedge (or cross) product leads to a volume (area) which can be given an orientation based on the direction of its vectors. While not a focus of this work, we note that the generalised pullback commutes with the wedge product, noting for $h:\M \to \N$ and differential forms $\alpha,\beta$, the pullback is a homomorphism $h^*(\alpha \wedge \beta) = (h^*\alpha) \wedge (h^*\beta)$. Wedge products turn vectors into a graded algebra, important in various algebraic geometry techniques. We note that the basis of $n$-forms at $p \in \M$ is given by the wedge product of differentials:
%     \begin{align*}
%         (dx^{\mu_1})_p \wedge ... \wedge (dx^{\mu_n})_p
%     \end{align*}
%     Indeed it can be shown that $d\omega(X_i)$ at $p \in \M$ only depends upon vector fields $X_i$ at $p$, a fact related to the property of the exteriror derivative being $f$-linear:
%     \begin{align*}
%     d\omega(X_1,...,fX_i,...,X_{n+1}) &= fd\omega(X_1,...,X_i,...,X_{n+1})\\
%     d\omega(fX,Y) &= fd\omega(X,Y)
% \end{align*}
% Such formulations then form the basis for important theorems related to DeRham cohomology (see Frankel \cite{frankel_geometry_2011}). In this context the \textit{exterior derivative} can be defined as follows.
% %==
% \begin{definition}[Exterior Derivative]\label{defn:geo:exterior_derivative}
% Given $A(\M) := T^\M$, the \textit{exterior derivative} is a map $d: A^n(\mathcal{M}) \to A^{n+1}(\mathcal{M})$, which takes an $n$-form to an $(n+1)$-form. For an $n$-form $\omega \in A^n(\mathcal{M})$ given locally by
% \[
% \omega = \sum_{i_1, \ldots, i_n} \omega_{i_1 \ldots i_n} dx^{i_1} \wedge \ldots \wedge dx^{i_n},
% \]
% the exterior derivative is defined as
% \begin{align}
% d\omega &= \sum_{i_1, \ldots, i_n} d\omega_{i_1 \ldots i_n} \wedge dx^{i_1} \wedge \ldots \wedge dx^{i_n}
% \end{align}
% where $\quad d\omega_{i_1 \ldots i_n} &= \sum_{j} \frac{\partial \omega_{i_1 \ldots i_n}}{\partial x^j} dx^j$.
% \end{definition}
% The exterior derivative has the property that $d(d\omega) = 0$ for any form $\omega$, and it is linear over the smooth functions on $\mathcal{M}$, i.e., for a smooth function $f$ and a form $\alpha$, we have $d(f\alpha) = df \wedge \alpha + f d\alpha$.

% \subsection{Tangent planes and Lie algebras}\label{sec:geo:Tangent planes and Lie algebras}
% In this section, we recount a few properties of Lie groups and Lie algebras from earlier chapters, connecting them explicitly to geometric formulations used in later chapters. Recall from proposition (\ref{prop:geo:Lie Group (Manifold)}) that a Lie group is a group equipped with the structure of a differentiable manifold such that the group operations are smooth i.e. where the map in parameter space that takes us from $g_1$ (parametrised by $\theta_1$) to $g_2$ in $G$ is a differentiable map. \\
% \\
% A fundamental aspect of Lie group theory is the isomorphism between the set of all left-invariant vector fields on a Lie group $G$, denoted $L(G)$, and the tangent space $T_eG$ at the identity element $e$ of $G$. This isomorphism implies that one can understand the behavior of left-invariant vector fields by examining transformations within $T_eG$. In particular, this concept is foundational when considering the exponential map. The tangent space $T_eG$ is, effectively, the Lie algebra of the Lie group $G$, and mappings between different Lie groups $G \to H$ can be studied by examining the corresponding maps between their Lie algebras $T_eG \to T_eH$. In addition, given the completeness of left-invariant vector fields $G$, we can extend integral using the group structure even if $G$ is not compact. Moreover, we can see how the exponential map is constructed by considering the unique integral curve of a left-invariant vector field at $t=0$, mapping $t \mapsto \exp(tA)$, where $A$ is an element of the Lie algebra $T_eG$. The map is formally defined as $\exp: T_eG \to G$, such that $\exp(A) = \exp(tA)$ evaluated at $t=1$. It can be demonstrated that the exponential map is a local diffeomorphism near the identity $e$, mapping a neighborhood in $T_eG$ smoothly onto a neighborhood in $G$. This elucidates that the exponential map generates a one-parameter subgroup of $G$, and, in fact, every one-parameter subgroup of $G$ can be expressed in the form $t \mapsto \exp(tA)$. This relates to the bijective correspondence between one-parameter subgroups of the Lie group $G$ and elements of its Lie algebra discussed earlier in this wek. Thus the neighborhood of $e$ in $G$, which is diffeomorphically mapped by $\exp: T_eG \to G$, is filled with the images of these subgroup maps, allowing investigations into these subgroups by examining the local structure around the identity element of the Lie algebra.
% \\
% \\
% Of importance to connecting Lie groups and algebras to geometric constructs is the existence of left and right translations of $G$ onto itself, which can be used to map the local tangent bundle around the entire group. Recall \textit{left translations} and \textit{right translations} of $G$ are diffeomorphisms given by the group actions:
%     \begin{align*}
%         r_g:& G \to G, \qquad &l_g: G \to G\\
%         &g'\mapsto g'g \qquad &g' \mapsto gg'
%     \end{align*}

% A vector field $X$ on a Lie group $G$ is \textit{left-invariant} if it is $l_g$-related to itself for all $g \in G$ i.e.:
%     \begin{align*}
%         l_{g^*}X = X, \forall g \in G
%     \end{align*}
%     or equivalently:
%     \begin{align*}
%         l_{g^*}(X_{g'}) = X_{gg'}, \forall g,g' \in G
%     \end{align*}
%     with a similar notion of \textit{right invariance}. Here $l_{g^*}$ denotes the pushforward, being the derivative map of the left action $L_g$ i.e. $g$ maps between manifolds, while $g^*$ is the corresponding push-forward. The set of left invariant vector fields is denoted $L(G)$. Lie groups that are locally compact (such as $GL(n,\R))$. Local compactness is important in quantum contexts as it relates to the existence, for example, of the Haar measure (discussed in the second chapter above) where the measure exists on $G$ if $G$ is (quasi)-invariant under left and right translations.  For vector fields $X_1, X_2$ on $\M$ that are by a pushforward $h_*$ mapped to vector fields $Y_1,Y_2$ on a manifold $\N$ where $h: \M \to \N$, then the \textit{commutator} $[X_1,X_2]$ is $h$-related to the commutator $[Y_1,Y_2]$. For left-invariant vector fields $X_1,X_2$, we then have that the commutator is invariant under the left-invariant actions (translations) of $G$, namely:
%     \begin{align*}
%         l_{g^*}[X_1,X_2] = [l_{g^*}X_1,l_{g^*}X_2] = [X_1,X_2]
%     \end{align*}
%     which shows that $[X_1,X_2] \in L(G)$.  It can be shown theh that the set $L(G)$ is a `sub-Lie algebra' of the infinite-dimensional Lie algebra of all vector fields on the manifold $G$. This is equivalent to the \textit{Lie algebra} of $G$ and represents a way of construing the Lie algebra in terms of important invariant properties of vector fields. It can also be shown that there is an isomorphism between the tangent space at the identity $e \in G$ i.e. $T_eG$ and $L(G)$, allowing $L(G)$ (and diffeomorphisms of $G$) to be explored via actions upon $T_eG$ (at the identity). The commutator $[A,B] \in T_eG$ (for $A,B \in T_eG$)i s then defined to be the unique element in $T_eG$ satisfying:
% \begin{align*}
%         L^{[A,B]} = [L^A,L^B]
%     \end{align*}
%     Here $L^A := L^A_g = l_{g_*}A, \forall g \in G$ i.e. $L^A$ is the vector field on $G$ defined by such left translation and $L^{[AB]} = l_{g_*}[A,B]$ representing hte left invariant vector field associated with the Lie bracket $[A,B] \in T_eG$. We note also the structure constants of a Lie algebra $L(G) \simeq T_eG$ arising from commutators of its basis elements $E_\alpha$ that is:
%     \begin{align*}
%         [E_\alpha,E_\beta] = \sum_{\gamma = 1}^n C_{\alpha\beta}^\gamma E_\gamma
%     \end{align*}
%     for $C_{\alpha\beta}^\gamma \in \Real$ where $C_{\alpha\beta}^\gamma$ denotes the relevant structure constant. The adjoint map also has an expression in terms of actions on $T_eG$ and that left-invariant fields $X$ such that integral curves of $X$ can be extended for all $t \in \R$.

% \subsubsection{Right and left invariance and Schr\"odinger's equation}\label{sec:geo:Right and left invariance and Schrodinger's equation}
% Because of its relevance in particular to our final chapter results, we set out the significance of left and right invariance in relation to quantum control. Our problem in that chapter is to determine the optimal time to synthesise a unitary $U_T \in G$ using only controls in $\p$, the Lie algebra corresponding to the Cartan decomposition $\g = \k \oplus \p$, where $\g$ is the Lie algebra of $G$. Now consider the Schr\"odinger equation:
% \begin{align}
%     \frac{dU}{dt} = -iH(t)U
%     \label{eqn:geo:leftrightinvarschrod}
% \end{align}
% Presented in this way with the Hamiltonian on the left of $U$, the Hamiltonian is the generator of (infinitesimal) translations (to second order) $U \to U + dU$ over increments $dt$. $U$ is our unitary at $t$ while $U + dU$ is our unitary at $t + dt$. The Hamiltonian is applied for $dt$ i.e. $dU/U = -iH(t)dt$. Thus time in equation (\ref{eqn:geo:leftrightinvarschrod}) moves from right to left. When we say right or left translation by $g$, we can think of [right translation as following the flow of time once its direction is chosen, and left translation in this case as time flowing `backwards' relative to that choice]. Thus right and left action by $h$ is expressed as follows:
% \begin{align}
%     \frac{dU}{dt}h & = -iH(t)Uh & &\text{(right action)}
% \end{align}
% whereas left action is given by:
% \begin{align}
%     h\frac{dU}{dt} & = -ihH(t)U = -i(hH(t)h^\inv) hU &\text{(left action)}
% \end{align}
% Thus we can see how, as distinct from right action, left action acts to conjugate (thus transform by an effective rotation) the Hamiltonian $H(t) \to hH(t)g^\inv$ (recalling here that the action of $h$ on $\g$ is by conjugation, expressed as the commutation $\g \to [X_h,\g]$). Thus while the representation of left or right invariance can be chosen, \textit{once chosen} in certain circumstances they are not equivalent. We explore the consequences of this asymmetry (or symmetry breaking) on Hamiltonians in our final chapter. \hl{NB: possibly leave out?}

% \subsubsection{Exponentials, integral curves and tangent spaces}\label{sec:geo:Exponentials, integral curves and tangent spaces}
% We briefly note a few connections between the exponential map (discussed in Chapter 2) and the geometric formalism above. The exponential map can be consiered in terms of integral curves, that is as the unique integral curve satisfying:
%     \begin{align*}
%         t &\to \gamma^{L^A}(t) \qquad       A=\gamma_*^{L^A} \left( \frac{d}{dt} \right)_0
%     \end{align*}
%     of the left invariant vector field $L^A$ associated with the identity in $\M$, that is $\gamma^{L^A}(0)=e$ and which is is defined for all $t \in R$. The notation $\gamma^{L^A}$ refers to the integral curve generated by the left-invariant vector field $L^A$ originating from the identity element $e \in G$. For any $g \in G$, the left translation map $L_g:G \to G, L_g(h) = gh, h \in G$ does not alter $L^A$. Here $A$ is the tangent vector to the curve $\gamma^{L^A}$ at $e$ where $\gamma_*^{L^A}$ represents the pushforward of the curve's tangent vector at $t=0$. The integral curve is then written as a mapping from the affine parameter $t \mapsto \exp(t A)$ with $A \in T_eG$. Here $\exp: T_eG \to G$ is defined via $\exp A = \exp(tA)\big|_{t=1}$, reflecting the convention that one moves from the identity $e \in G$ along the integral curve generated by $A$ to $\exp(A) \in G$ with time $t \in [0,1]$. This reflects the idea that evolution of curves in $G$ can be framed in terms of evolution from the identity element and therefore studied in terms of the canonical Lie algebra associated with $T_eG$. \\
%     \\
%     Other results mentioned in chapter 2 also apply, such as the exponential map being local diffeomorphism from $T_eG$ to $e \in G$ and that $t \mapsto \exp(At)$ is considered a unique one-parameter subgroup of $G$ (indeed that all such one-parameter subgroups are of that form for $A \in T_eG \simeq L(G)$. This reiterates the one-to-one association between one parameter subgroups of $G$ and the exponential map. \\
% \\
% Note that left-invariance also applies to $n$-forms and that Lie algebras can be said to have associated with them dual Lie algebras (see literature for standard discussion). Of note in our final chapter is the Cartan-Maurer form. The form can be understood as relating structure constants and wedge products with the derivative of a one-form. Given the Cartan-Maurer equation:
% \begin{align}
%     d\omega^\alpha + \frac{1}{2}\sum_{\beta,\gamma=1}^n C_{\beta \gamma}^\alpha \omega^\beta \wedge \omega^\gamma=0 \label{eqn:geo:Cartan-Maurer equation}
% \end{align}
% we observe that the commutator of one-forms is a two-form which can be obtained via exterior differentiation. The term $d\omega^\alpha$ is the exterior derivative of the form, and the wedge product $\omega^\beta \wedge \omega^\gamma$ is summed over the structure constants $C_{\beta \gamma}^\alpha$ of the Lie algebra, weighted by the Lie bracket.
% % \begin{definition}[Cartan-Maurer form]
% % The Cartan-Maurer form is a left-invariant vector field valued one-form $\Xi$ on $G$ that assigns to $v \in T_gG$ a \textit{left-invariant} vector field on $G$. The value of this field at $g \in G$ is the tangent vector $v$ where, if $\braket{\Xi,v}$ denotes this left-invariant vector field then:
% % \begin{align*}
% %     \braket{\Xi,v}(g') = l_{g'*}(l_{g^{-1}}v)
% % \end{align*}
% % for all $v \in T_gG$.  
% % \end{definition}
% % \hl{VERSUS}
% \begin{definition}[Maurer-Cartan Form]
% Let $G$ be a Lie group. The Maurer-Cartan form is a $\mathfrak{g}$-valued one-form $\omega$ on $G$, where $\mathfrak{g}$ is the Lie algebra of $G$. For each $g \in G$, $\omega_g: T_gG \rightarrow \mathfrak{g}$ is defined by
% \begin{align*}
% \omega_g(v) = l_{g^{-1}_*}(v)
% \end{align*}
% where $l_{g^{-1}_*}$ denotes the pushforward (differential) of the left multiplication by $g^{-1}$ in $G$, and $v \in T_gG$ is a tangent vector at $g$. 
% \end{definition}
% Essentially, $\omega_g$ relates the tangent space at any point $g \in G$ back to the tangent space at the identity, $\mathfrak{g}$, ensuring left-invariance. As Sharpe \cite{sharpe_differential_2000} notes, the equation is of profound use in classifying properties of spaces. In particular, Cartan's structural equations (see Theorem \ref{thm:geo:Cartanstructuralequations} below) can be expressed as:
% \begin{align}
%     d\omega_g = \frac{1}{2}[\omega_g,\omega_g] = 0 \qquad [\omega_g,\omega_g] := \frac{1}{2}[\omega_g,\omega_g](u,v) = [\omega_g(u),\omega_g(v)] \label{eqn:geo:cartancurvatureequation}
% \end{align}
% which is also described as the \textit{Cartan curvature} equation.  Note we can derive Cartan curvature equation (\ref{eqn:geo:cartancurvatureequation}) from equation (\ref{eqn:geo:Cartan-Maurer equation}).

% Connecting the concepts above to quantum information problems in this work, the form takes a tangent vector $v \in T_gG$ and returns a left-invariant vector field associated with $v$, meaning the field remains constant along the flow. Here $l_{g^{-1}}$ translates $v$ back to the identity then pushes it forward to $g'$ using left translation. The form is used in particular in our final chapter where we equate its relation to the Schr\"odinger equation (definition \ref{eqn:quant:schrodingerdUUinv}). This can be seen where:
% \begin{align}
%     g^\inv dg = \omega_g \qquad \qquad dU U^\inv = -iH(t)dt
% \end{align}
% where $U$ corresponds to the group element $g$ and the form $\omega_g$ corresponds to the Hamiltonian which can be regarded as a [one-form as a linear mapping on $T\M$] \hl{\textbf{FIX}}.


% As we discuss, the Cartan-Maurer form assists in identifying left-invariant vector fields invariant under the group action, simplifying equations of motion in optimal control contexts (as we show in the final chapter). For optimal control, we are also interested in transformation groups. For example, a group $G$ acting on $\M$ does so if there exists a homomorphism such that $\gamma: G \to \sigma(\M)$ with $g \mapsto \gamma_g$ where $\sigma(G)$ is the permutation group of $\M$ (with an equivalent anti-homomorphism for right action). Left action on a differential manifold can then be considered as a homomorphism from the group (of diffeomorphisms on $\M$) to curves $\gamma$, that is $g \to \gamma_g$ where $\gamma: \text{Diff}(\M) \to \M$. This gives rise to the notion of \textit{equivariant} mappings, being structure preserving maps between pairs of group actions of $G$ on manifolds $\M,\N$ where $g \mapsto \gamma_g, g\mapsto \gamma_g'$ on $\M$ and $\N$ respectively where $\gamma_g' \circ f = f \circ \gamma_g$. Equivariance has recently become of interest in quantum machine learning via the construction of equivariant neural networks where the network architecture is constructed to be equivariant \cite{meyer_exploiting_2022-1,cohen_equivariant_2021,mernyei_equivariant_2022}. 
% \\
% \\
% Moreover, we can connect different types of group actions discussed in earlier parts of this work to their geometric equivalents:
% \begin{enumerate}[(i)]
%     \item \textit{Kernel}: kernel of a $G$-action is the subgroup of $G$ defined by:
%     \begin{align*}
%         K = \{  g \in G | gp = p, \forall p \in \M \}
%     \end{align*}
%     \item \textit{Effective group action}: is where the kernel equals the identity, that is $K = \{ e \}$
%     \item \textit{Free group action}: if for all $p \in \M$ it is the case that $\{   g \in G | gp = p \} = \{e \}$ i.e. $\M$ is moved away from itself except with the exception of the unit element $e$ i.e. $e=p$ is the only element such that $gp=p$
%     \item \textit{Transitive group action}: G-action is \textit{transitive} if any pair of points $p,q\in\M$ can be \textit{connected} by an element of the group, i.e. there exists a $g \in G$ such that $p = gq$. In transitive action, the whole of $\M$ can be probed by the $G$-action. This is complementary to the idea that in an effective action the whole of $G$ can be proved by its action on the manifold $\M$
%     \item \textit{Orbit}: the orbit $O_p$ of the G-action through $p$ is the set of all points in $\M$ that can be reached from $p$, that is:
%     \begin{align}
%         O_p = \{ q \in \M | \exists g \in G, q = gp  \} \label{eqn:geo:orbit}
%     \end{align}
%     When a group $G$ acts on a set $X$ (group action on $X$) it \textit{permutes} the element of $X$. The path of an element of $X$ moves around a \textit{fixed path} is its orbit. An example is the \textit{sphere} $S^2$ acted on by the \textit{circle group} $S^1$ via rotations around the $z$ axis, this leaves the elements of the set. Such action is analogous to the action of the compact subgroup $K$ under a Cartan  decomposition $G = K \oplus P$, the intuitive idea being that each $K$ defines an orbit about which $k \in K$ translate, but that to reach different orbits, one requires the action of some element in $P$.
%     \item \textit{Stabiliser (isotropy) groups}: if G action on $\M$ is transitive with $G_p$ of the action is given by:
%         \begin{align}
%             G_p = \{ g \in G | gp = p  \} \label{eqn:geo:stabiliser}
%         \end{align}
%         and closed for Lie case.  The stabilisers of an element $p \in \M$ can be thought of as group actions (or permutations of $\M$ which form a group homomorphically mapped to $G$) which leave $p$ unchanged, i.e. the set of group action identity elements with respect to $p \in \M$. (re) Think of a set of permutations which leave $p$ unchanged or `in the same position'. Stabliser groups are fundmantal to quantum information (especially surface codes). In our final chapter, the stabliser group $K$ of $G$ is of fundamental importance, noting, for example, that stabiliser groups along an orbit are conjugate i.e. if $p,q$ belong to the same orbit of a $G$-action, they can be reached via some $g \in G$. 
% \end{enumerate}

% \subsubsection{Infinitesimal transformations and adjoint action}\label{sec:geo:Infinitesimal transformations and adjoint action}
% An important action throughout this work is the \textit{adjoint action} of $G$ on itself (discussed in Chapter 2): 
%         \begin{align*}
%             Ad_g(g') = gg'g^{-1}
%         \end{align*}
%         The kernel of this action is the centre $C(G)$ because the centre is the set of elements of $G$ that commute with every element in G, but then for an $g' \in C(G)$ we have $Ad_g(g')= gg'g^{-1}=g'gg^{-1}=g'$ i.e. the (effective) kernel of this action of conjugating by $g$ is the set of elements in $g$ that result in this action being equivalent to the identity, which is the centre. The relation between the commutator of a pair of Lie algebra elements (crucial for all quantum control problems) and the push-forward $Ad_{g*}$ of the adjoint action of $G$ can be expressed as follows. Let $A,B \in T_eG$ with Lie bracket $[A,B]$, then the bracket has a representation as differentiated adjoint:
% \begin{align*}
%     [A,B] = \frac{d}{dt}Ad_{\exp(tA)*}(B)|_{t=0}
% \end{align*}
% Recalling that the exponential is given such that $\exp(Ad_G{g*}(B)) = g(\exp(B))g^{-1}$, it can be shown that the relation between the commutator can be thought of in terms of this conjugacy:
% \begin{align*}
%     \exp(tA)\exp(B)\exp(-tA) = \exp(t[A,B] + O(t^2))
% \end{align*}
% and $X^{Ad_{g*}(A)} = \delta_{g^{-1}*}(X^A)$ where $\delta_{g^{-1}*}$ is the differential (pushfoward) of the map $g^\inv$ acting on $X^A$. That is, the vector field associated with the adjointly transformed Lie algebra element $A$ is equivalent to the transformed vector field $A$. 

% We conclude this section via reiterating in a geometric context the key results related to Lie algebra homomorphisms and connecting these to vector fields. This is an important result for further on when we introduce the \textit{connection} between vector (fibre) bundles that serves a pivotal role in our final chapter. In the theory of infinitesimal transformations, we can represent the Lie algebra $\g$ of $G$ via vector fields on $\M$ on which $G$ acts. This mapping is a homomorphism of Lie algebras and associates $X^A$ with $A \in T_eG$. Assume $G$ right-acts on $\M$. Given a mapping
%     \begin{align*}
%         A \mapsto X^A
%     \end{align*}
%     that assigns to each $A \in T_eG$ the vector field $X^A$ (denoted the \textit{induced vector field} on $\M$) is a homomorphism from the Lie algebra $L(G) \simeq T_eG$ 
%     into the infinite-dimensional Lie algebra of all vector fields on $\M$. This is denoted:
%     \begin{align*}
%         [X^A, X^B] = X^{[AB]}
%     \end{align*}
%     for all $A,B \in T_eG \simeq L(G)$. For left actions, the map $A \mapsto X^A$ is an anti-homomorphism $[X^A, X^B] = X^{[B,A]}$ from $T_eG \simeq L(G)$. If the action is effective on $\M$, then the map $A \mapsto X^A$ is an isomorphism from $T_eG \simeq L(G)$ to Lie algebras on $\M$.


% \subsection{Fibre bundles}\label{sec:geo:Fibre bundles}
% In many cases of physical importance, the vector space $V$ arises as a representation space of some \textit{internal symmetry group}, especially for example in symmetry reduction techniques used in geometric control theory. Fibre bundles allow for the study of situations where the structure of interest over each point of a base space is more complex than just a vector space, allowing, for example, gauge symmetries to be identified (e.g. where gauge symmetries are not completely represented as transformations on vector spaces). They are of particular relevance in gauge theories providing a means of describing fields and their connections over manifolds.  
% In quantum information problems involving systems with a geometric or topological character, quantum state space can be considered as sections of a fibre bundle where the base space represents a space of parameters or configurations, and the fibres represent the Hilbert spaces associated with each configuration. We briefly sketch out the theory of fibre bundles and principal bundles as these are touched upon in later chapters. In geometric control, we often look to find ways of modelling the control space modeling control inputs and state spaces as fibres. Fibre bundles are an abstraction of vector bundles and are utilised for when, for example, mappings lack vector space properties. 
% We begin with the concept of a \textit{bundle}.
% A \textit{bundle} is defined as a triple $(E, \pi, \mathcal{M})$, where $E$ and $\mathcal{M}$ are linked via a continuous projection map $\pi: E \to \mathcal{M}$. 
% Firstly, we define the important concept of a \textit{fibre}. Define a \textit{bundle space} as $E = \bigcup_{p \in \mathcal{M}} F_p$, with $F_p$ being fibres. A fibre is then defined as follows.
% \begin{definition}[Fibre]\label{defn:geo:fibre}
%     The fibre over $p$ is the inverse image of $p$ under $\pi$. It arises via the map $\pi^{-1}:\mathcal{M} \to T\mathcal{M}$, an example of a fibre bundle associating $p \in \mathcal{M}$ with the tangent space $T_p \mathcal{M}$. The projection $\pi$ associates each fibre $F_p$ with a point $p \in \mathcal{M}$, where
% \begin{align*}
%     F_p = \pi^{-1}(\{p\}),
% \end{align*}
% defines $F_p$ as the preimage of $p$ under $\pi$.
% \end{definition}
%  Certain bundles have the special property that the fibres $\pi^{-1}(\{x\}), x \in \M$ are all \textit{homeomorphic} (\textit{diffeomorphic} for manifolds) to $F$. In such cases, $F$ is known as the \textit{fibre} of the bundle and the bundle is said to be a \textit{fibre bundle}. For vectors, this is the set of all vectors that are tangent to the manifold at the point $p$. The fibre bundle is sometimes visualised in diagrammatic form:
%     \[ \begin{tikzcd}
% F \arrow{r} & E \arrow{d}{\pi} \\%
% & \M
% \end{tikzcd}
% \]
% Related to fibre bundles is the idea of a \textit{cross section}. The section of a bundle $(E,\pi,\M)$ is a \textit{map} from the base space (manifold) to the total space:
%     \begin{align*}
%         s: \M \to E
%     \end{align*}
%     such that the image of each point in the base space $x \in \M$ lies in the fibre $\pi^{-1}(\{ x\})$ over $x$ such that:
%     \begin{align*}
%         \pi \circ s = id_\M
%     \end{align*}
%     So the section is the map from the manifold such that we take an $x$, send it up to the total space $E$, then that image of $x$, when subject to $\pi$, takes us back to $x \in M$, hence $\pi \circ s$ is equivalent to the identity on $\M$. One can also define maps between bundles and pullbacks among fibres analogous to the case for vector bundles. 


% \subsubsection{Principal fibre bundles}\label{sec:geo:Principal fibre bundles}
% An important canonical fibre bundle is the principal fibre bundle whose fibre acts as a Lie group in a particular way. Importantly for our purposes, they allow for the definition of \textit{connections} (see below) which describe how fibres (or vector spaces) are connected over different points in $\M$. Connections are of fundamental importance to results in our final chapter and also to definitions of vertical and horizontal subspaces in subRiemannian control problems further on. A connection on a principal bundle defines a notion of horizontal and vertical subspaces within the tangent space of the total space. This distinction is crucial for defining parallel transport and curvature, concepts that are central to understanding the dynamics and control of systems with symmetry. 

% \begin{definition}[Principal fibre bundle]\label{defn:geo:Principal fibre bundle}
%     A principal fibre a bundle $(E,\pi,\M)$ is a \textit{G-bundle} (a \textit{fibre bundle}) if the total space $E$ is a \textit{right-G space} and if the bundle $(E,\pi,\M)$ is isomorphic in the following way:
%     \begin{align*}
%         (E,\pi,\M) \simeq (E,\rho, E/G)
%     \end{align*}
%     where $E/G$ is the \textit{orbit space} of the $G$-action on $E$ and $\rho$ is here the usual projection map such that we have the diagram:
%     \[ \begin{tikzcd}
% E \arrow{d}{\pi} \arrow{r}{u} & E \arrow{d}{\rho}\\%
% \M \arrow{r}{\simeq} & E/G
% \end{tikzcd}
% \]
% \end{definition}
% A principal fibre bundle has a typical fibre that is a Lie group $G$, and the action of $G$ on the fibres is by right multiplication, which is free and transitive. The fibres of the bundle are the orbits of the $G$-action on $E$ and hence are not generally homeomorphic to each other. All non-principal bundles are associated with the principal bundle. Principal $G$ bundles are when $G$ acts freely on $E$ (that is, \textit{free action} is when the only element of $G$ that acts as an identity element on $x \in E$ is the identity in $G$ itself). Given a closed subgroup $H \subset G$, then the quotient space $G/H$ is also an orbit space with fibre $H$. A few other concepts of relevance include:
% \begin{enumerate}[(i)]
%     \item \textit{Principal total space (P)}.  principal bundle sets $(P,\pi,\M)$ where $P$ is the principal total space together with \textit{prinpal maps} between two such bundles i.e. $u: P \to P'$ for $(P,\pi,\M)$ and $(P',\pi',\M')$. The mapping is $G$-equivariant as $u(pg) = u(p)g$. 
%     \item \textit{Triviality}. The \textit{triviality} (or \textit{trivialisation}) of a principal $G$-bundle relates to whether the bundle expressly respects the product structure of the base space with $G$. A principal $G$-bundle is trivial if it is isomorphic to the product bundle $(\M \times G, pr_1,\M)$ where $pr_1:\M \times G \to \M$ is a projection onto $\M$. Triviality requires (i) \textit{compatability} with projection maps so that diffeomorphisms $f$ respect the fibration structure of $P$ by mapping fibres in $P$ over $p \in \M$ to $\{p\} \times G$ and (ii) \textit{equivariance} with respect to $G$ such that $f(pg) = f(p)g$, where $f(p) \in \M \times G$ (such that $f$ preserves the group action structure of the bundle).
% \end{enumerate}
% For the avoidance of doubt, we have so far (with slight abuse of notation for convenience) been equating $G \equiv \M$ (as distinct from explicitly notationally indicating the group acting on the manifold $\M \times G)$, where $T_gG$ for $g \in G$ captures the infinitesimal directions in which $G$ can evolve, mapping directly to tangent spaces $T_p\M$ on the manifold. Usually the principal bundle $(P,\pi,\M)$ is introduced as a more abstract formulation to cater for wehre $G$ acts on a different manifold (where $G \neq \M$). The formulation of total space $P$ allows consideration of how the tangent spaces $T_gG$ (that is for our formulation, $T_p\M$) are related across the entirely of $\M$. Thus in our treatment, we are interested in how $G$ acts upon itself, which in the language of quantum operators is how operators act upon themselves e.g. $U_1(t)U_2(t)=U'(t)$ can be regarded as group elements acting on themselves. 

 

% We conclude this section with vector bundles, important due to their being equipped with a natural vector space structure.
% \begin{definition}[Vector bundle]\label{defn:geo:Vector bundle}
%     An $n$-dimensional complex or real vector bundle $(E,\pi,\M)$ is a a type of fibre bundle in which each fibre exhibits the structure of an $n$-dimensional vector space. For each $x \in \M$ there exists a neighbourhood $U$ and way of locally expressing  trivialisation of the bundle via $h: U \times \R^n \to \pi^{-1}(U)$ such that for all  $ y \in U, h: \{ y \} \times \R^n \to \pi^{-1}(\{ y\})$ is linear.
% \end{definition}
% Vector bundles are the primary type of fibre bundle with which we are concerned in this work. The concept has braod application, e.g. in machine learning by allowing the representation of data points that are sensitive to inherent symmetries in the data. In quantum settings, unitary operations and quantum channels, which describe the evolution of quantum states, can be seen as bundle maps that act on the sections of vector bundles. Unitary operations, representing reversible quantum evolutions, can be modeled as isomorphisms of Hilbert spaces $\Hilb$ (definition \ref{defn:quant:Hilbert Space}) as fibres which preserving their structure. Quantum channels, which describe more general (possibly irreversible if decohering) quantum evolutions, can be represented as linear maps between fibers (see \cite{bengtsson_geometry_2006} for more detail).

% % Conceptually this can include: \hl{\textbf{FIX}}
% % \begin{enumerate}[(a)]
% %     \item \textit{Parametrised unitaries}. One example is parametrised quantum circuits. Here the base manifold $\M$ can represent the parameter space of the quantum system, i.e. the configurations of the quantum registers (definition \ref{defn:quant:Quantum registers and states}), each point in the manifold being a register (parameter) configuration. Hilbert spaces $\Hilb$ can then be regarded as fibres of the bundle, representing physical states consistent with parameter configurations. Evolution on the manifold is represented by the action that transforms to a different configuration in $\M$ e.g. from $p\to q\in \M$, represented by pushing forward (transporting) vectors in $\Hilb_p \to \Hilb_q$, akin to how we regard vectors $v\in T_p\M$ as transported to $v' \in T_q\M$ via unitary evolution.
% % \end{enumerate}

% \subsection{Connections}\label{sec:geo:Connections}
% Connections are a fundamentally important concept in geometry, encapsulating the concept of differentiation of vector fields along curves on manifolds. A connection on a manifold $\mathcal{M}$, or more specifically on a tangent bundle $T\mathcal{M}$, provides a systematic way to parallel transport vectors along paths, allowing the comparison of tangent spaces at different points on $\mathcal{M}$, effectively facilitating the extension of the notion of directional derivatives to curved spaces. Intuitively the idea of a connection is a means of associating vectors between infintesimally adjacent tangent planes $T_p\M \to T_{p+dp}\M$ as one progresses from $\gamma(t)=p$ to $\gamma(t+dt)=p+dt$ on $\M$. Another way to think about them is that they provide a way of identifying how $T_p\M$ transform along the curve $\gamma(t)$, in giving conditions to be satisfied for tangent vectors $\dot\gamma(t)$ to remain parallel as they are transported along a curve (parallel transport or the vanishing of the covariant derivative, which we discuss below). 

% Connections are also a fundamental means of distinguishing between Riemannian and subRiemannian manifolds via the decomposition of fibres (and Lie algebras) into horizontal and vertical subspaces. They are thus central to quantum and classical control problems, such as the $KP$ control problem we study extensively in the final chapter. Connections, as we explain below, are related to notions of parallel transport and covariant differentiation. In Riemannian geometry, for example, Christoffel symbols represent coefficients of connection on the bundle of frames (set of bases) for $\M$. The underyling idea of parallel transport and covariant differentiation requires that one compares points in neighbouring fibres (or vector spaces, in the case of a vector bundle) in a way that isn't dependent upon a particular local coordinate system (or trivialisation). Thus a concept of directionality is needed such that vector fields point from one fibre to another. Vector fields arising from Lie algebras lack this intrinsic orientation of directional pointing. The problem is that the vector fields $X^A_p$ at $p$ are tangent to the fibre.


% Consider a principal $G$-bundle $(P, \pi, \mathcal{M})$ above. A connection on $P$ provides a smooth splitting of the tangent space $T_pP$ at each point $p \in P$ into vertical and horizontal subspaces, $T_pP = V_pP \oplus H_pP$, where $V_pP$ is tangent to the fibre and $H_pP$ is isomorphic to $T_{\pi(p)}\mathcal{M}$. To understand this formalism, we expand upon important concepts of vertical and horizontal subspaces. These are fundamental in later chapters, where synthesis of time-optimal (approximate) geodesics arise by way of choosing Hamiltonians comprising generators from horizontal subspaces (Lie subalgebras). Evolution according to horizontal subspaces in Riemannian manifolds relates to vanishing (zero) covariant derivatives.

% \begin{definition}[Vertical subspace]\label{defn:geo:Vertical subspace}
%    The vertical subspace $V_pP$ at $p \in P$ is defined as the kernel of the differential of the projection map $\pi: P \rightarrow \mathcal{M}$, i.e., 
%     \begin{align*}
%     V_pP = \ker(\pi_*|_p) = \{ v \in T_pP \mid \pi_*(v) = 0 \}.
%     \end{align*}
% \end{definition}
% Intuitively, $V_pP$ consists of tangent vectors to $P$ at $p$ that are "vertical" in the sense that they point along the fibre $\pi^{-1}(\pi(p))$. These vectors represent infinitesimal movements within the fibre itself, without leading to any displacement in the base manifold $\mathcal{M}$. Vector fields $X^A_p$ belong to the subspace $V_pP \subset T_pP$  intuitively they point `along' the fibres (re). This vertical subspace is defined by:
%     \begin{align*}
%         V_pP = \{ \tau \in T_pP | \pi_* \tau = 0 \}
%     \end{align*}

% \begin{definition}[Horizontal subspace] \label{defn:geo:Horizontal subspace}
% The horizontal subspace $H_pP$ at $p \in P$, on the other hand, is selected by the connection and complements the vertical subspace within $T_pP$. Specifically, a connection on $P$ provides a smooth assignment of a horizontal subspace to each point in $P$ such that the tangent space at any point $p$ decomposes as a direct sum:
%     \begin{align*}
%     T_pP = V_pP \oplus H_pP.
%     \end{align*} 
% \end{definition}
% The horizontal subspace consists of those vectors that are orthogonal (under a chosen Riemannian or pseudo-Riemannian metric on the bundle) to the vertical space with respect to a chosen connection. Vectors in $H_pP$ are "horizontal" in the sense that they correspond to displacements that lead to movement in the base manifold $\mathcal{M}$ when considered under parallel transport defined by the connection. This can be understood diagramatically. The projection map $\pi: P \to \M$ induces a (push-foward) map $\pi_*: T_pP \to T_{\pi(p)}\M$:
%     \begin{figure}
%         \centering
%         \[ \begin{tikzcd}
%     & TP \arrow{d} \arrow{r}{\pi_*} & T\M \arrow{ddl}\\
% G \arrow{r} & P \arrow{d}{\pi}  & \\%
% & \M  & 
% \end{tikzcd}
% \]
%         \caption{Commutative diagram showing the relationship of the connection (map from $G \to P \to \M$), the projection map $\pi: P \to \M$ and induced horizontal map (the pushforward) $\pi^*$}
% \label{fig:geo:connectionfibresetc}
%     \end{figure}
% In this structure, $A \mapsto X^A$ is an isomorphism of $L(G)$ onto $V_pP$. The vertical subspace thus comprises those vectors that are in the kernel of the map $\pi_*$, i.e. they map to the nullspace of $T\M$ and such vectors do not generate evolutions in the base manifold $\M$. Analogously, these vectors `point up' so do not specify a direction to move on $\M$, akin to a vector pointing vertically out of a surface. The horizontal subspace, by contrast, comprises vectors that generate translations on the base manifold. This is intuitively equivalent to those vectors `pointing' in some direction of translation on the manifold from say $p \to p' \in \M$. Because $p'$ has its own fibre (e.g. vector bundle), then those horizontal subspace vectors `point' horizontally towards other vector bundles associated.  
% \\
% \\
% It is useful to dwell on the notion of orthogonality between vertical and horizontal subspaces implied by the connection. Indeed in many ways it is more illuminating to begin with this concept of orthogonality to build intuition around the terms vertical and horizontal. This provides means of distinguishing between vertical and horizontal movements in $P$. The choice of horizontal subspace $H_pP$ at $p \in P$ is not arbitrary. Rather, it is subject to conditions ensuring consistency with the group action and smooth variation across $P$:
% \begin{align*}
%     \delta_{g*}(H_pP) = H_{pg}P, \quad \forall g \in G, p \in P,
% \end{align*}
% where $\delta_g(p) = pg$ denotes the right action of $G$ on $P$. This condition ensures that vectors being deemed horizontal is consistent with the geometric structure of the bundle as defined by the group action.

% Intuitively, vertical subspaces manifest the internal symmetry of the bundle encoded by the Lie group $G$, while horizontal subspaces encapsulate the geometry of how the bundle expands over the base manifold. This geometric structure, facilitated by the connection, is crucial for defining parallel transport,  curvature and ultimately geodesics (and their approximations) that characterise time-optimality.
% We can thus formally define a connection \cite{isham_modern_1999,frankel_geometry_2011} and \cite{helgason_differential_1979} in these terms.
% %Connection definition
% \begin{definition}[Connection]\label{defn:geo:Connection} A \textit{connection} on a principal $G$-bundle given as:
% \begin{align*}
%     G \to P \to \M
% \end{align*}
% is a smooth assignment of horizontal subspaces $H_pP \subset T_pP$, to each point $p$ in the total space $\in P$ such that:
% \begin{enumerate}[(i)]
%     \item $T_pP \simeq V_pP \oplus H_p P, \forall p \in P$ (i.e. decomposable into direct sum of horizontal/vertical)
%     \item $\delta_{g*}(H_pP) = H_{pg}P, \forall g \in G, p \in P$ (subject to right action)
% \end{enumerate}
% where $\delta_g(p) = pg$ denoting right action.
% \end{definition}
% The commutative diagram in Figure (\ref{fig:geo:connectionfibresetc}) illustrates how the projection map $\pi: P \to \M$ gives rise to an \textit{induced horizontal map} from the tangent space to the total space:
% \begin{align*}
%     \pi_*: T_pP \to T_{\pi(p)}\M
% \end{align*}
% By construction, the kernel of this map is the vertical subspace. Connections can also be understood usefully in terms of one forms.  Connections can be associated with certain $L(G)$-valued one-forms $\omega$ on $P$. Recall that the map $\ell: L(G) \to VFlds(P), A \mapsto X^A$, so $\ell^{-1}$ maps back to the Lie algebra $L(G)$. If $\tau \in T_pP$, then:
% \begin{align*}
%    \omega_p: T_pP \to P, \omega_p(\tau) = \ell^{-1}(V_pP(\tau))
% \end{align*}
% which maps back to $V_pP$. As this map takes us back to $L(G)$, then $\ell$ is the isomorphism of $L(G)$ with $V_pP$, so we can associate one-forms with maps between the tangent space and the Lie group as follows:
% \begin{enumerate}[(i)]
%     \item $\omega_p(X^A) = A, \forall p \in P, A \in L(G)$
%     \item $\delta_g^* = Ad_{g^{-1}}\omega$, with $\delta_g^* \omega (\tau) = Ad_{g^{-1}}\omega(\tau)$
%     \item $\tau \in H_pP \iff \omega_p(\tau) = 0 $
% \end{enumerate}
% The horizontal subspace of the tangent space $TP$ can thus be thought of as the kernel of the one-form that maps to the left-invariant Lie group (re):
% \begin{align*}
%     H_pP = \{ \tau \in T_pP | \omega_p(\tau) = 0, \omega_p(\tau) = \ell^{-1}(V_pP(\tau))  \}
% \end{align*}
% In this formulation, the connection can be expressed as an $L(G)$-valued one form on $P$ satisfying (i) to (iii) above. The map $\ell: L(G) \to VFlds(P)$ maps Lie algebra elements to vector fields on $P$ such that $\ell^{-1}(V_pP(\tau))$ would map this vertical component back to an element of the Lie algebra.

% \subsubsection{Relation to Cartan decompositions}\label{sec:geo:Relation to Cartan decompositions}
% The decomposition into vertical and horizontal subspaces discussed above is particularly relevant to time optimal control problems. In essence, given the Cartan decomposition (\ref{defn:alg:cartandecomposition}) $\g = \k \oplus \p$ we associate $\k$ as the vertical and $\p$ as the horizontal subspace. We can then understand the symmetry relations expressed by the commutators related to this vertical and horiztonal sense of directionality: i.e. given $[k,k]\subset k, [k,p]\subset p$ and $[p,p]\subset k$ we can see that the horizontal generators under the adjoint action shift from $p \in G/K$ to $p' \in G/K$, while the vertical generators in k do not translate those points in $G/K$. We introduce two definitions to elucidate this further, the \textit{Cartan connection}:
% \begin{definition}[Cartan Connection]\label{defn:geo:CartanConnection}
% A Cartan connection on a principal $G$-bundle $(P,\pi,\M)$ (with group $G$, subgroup $H$ (and subalgebra $\h$) and homogeneous space $G/H$) consists of an atlas (see definition \ref{defn:geo:Coordinate charts and atlases}) $U \in \M$ and a $\mathfrak{g}$-valued one-form $\theta_U: TU \to \g$ defined on each chart such that (a) $\mathfrak{h}$: $\theta_U \mod \mathfrak{h}$ is a linear isomorphism for every $u \in U$ and (b) for charts $U,V$, then $h: U \cap V \rightarrow H$:
% \begin{align}
%     \theta_V = \text{Ad}(h^{-1})\theta_U + h^*\omega_H \label{eqn:geo:thetaUoneformcartanmaurer}  
% \end{align}
%     where $\omega_H$ is the Maurer-Cartan form of $H$.
% \end{definition}
% Note that Cartan curvature (equation (\ref{eqn:geo:cartancurvatureequation}) can be expressed as:
% \begin{align}
% \Omega_U = d\theta_U + \frac{1}{2}[\theta_U, \theta_U] \label{eqn:geo:cartancurvatureequation2}
% \end{align}
% % \begin{definition}[Cartan Curvature]\label{defn:geo:CartanCurvature}
% % The curvature $\Omega_U$ of a Cartan connection $\theta_U$ is a system of 2-forms defined on the charts, given by

% % \end{definition}

% We can understand the commutation relations in terms of principal bundles and horizontal/vertical subspaces as follows: 
% \begin{enumerate}
%     \item \textit{Vertical subspace $\k$}. The first relation $[\mathfrak{k}, \mathfrak{k}] \subset \mathfrak{k}$ provides that the Lie bracket of two vertical generators remains within the vertical subspace. Geometrically, this means that transformations generated by elements of $\mathfrak{k}$ remain within the fibres of the principal bundle $G \rightarrow G/K$. Such vertical movements do not evolve to other points in the base space $G/K$, reflecting an intrinsic, self-contained dynamics within each fibre, akin to internal symmetries. Geometrically, translations by elements of $\mathfrak{k}$ keep points within the same orbit in $G/K$.
%     \item \textit{Horizontal to vertical}. The second commutation relation $[\mathfrak{p}, \mathfrak{p}] \subset \mathfrak{k}$, indicates that the commutator of two horizontal elements results in a vertical element. This property is particularly intriguing as it relates to the curvature of the connection in $G/K$. The horizontal generators under the adjoint action can lead to a shift that results in a vertical movement, suggesting that purely horizontal displacements can induce curvature in the space, effectively "bending" into the vertical subspace. This phenomenon is a hallmark of the non-trivial geometry in subRiemannian spaces and is crucial for understanding the underlying geometric structure of $G/K$. Elements of $\mathfrak{p}$ correspond to horizontal directions that can be projected onto the base space $G/K$, effectively causing translations from one orbit to another. This curvature is a manifestation of how horizontal translations alter the geometric structure of the space, moving points across different orbits in $G/K$ (see below).
%     \item \textit{Vertical acting on horizontal}. The relation $[\mathfrak{k}, \mathfrak{p}] \subset \mathfrak{p}$ implies that the action of vertical elements on horizontal ones results in horizontal displacements. This can be interpreted as the influence of the group's internal symmetries on the directionality of movement within $G/K$. In other words, the vertical generators, through their adjoint action, can modify the direction of horizontal generators without leaving the horizontal plane, thereby affecting the trajectory of points in $G/K$ without transitioning to vertical movement
% \end{enumerate}
% Recall that in the full Lie group $G$, orbits are generated by the action of its subgroups, including $K$, on points within $G$. For a subgroup $K$ and an element $g \in G$, the orbit of $g$ under the action of $K$ is defined as $\mathcal{O}_g = {k \cdot g \mid k \in K}$. These orbits represent continuous trajectories or paths within $G$ that are traced out by the action of $K$, reflecting the inherent symmetry structure imposed by $K$ on $G$. When considering the quotient space $G/K$, which represents the space of left cosets of $K$ in $G$, the action of $K$ on $G$ translates differently. Here, each point in $G/K$ corresponds to an orbit of $K$ in $G$, and the quotient space essentially "collapses" these orbits to single points, with the projection map $\pi: G \rightarrow G/K$ sending elements of $G$ to their corresponding orbits in $G/K$. 

% \subsubsection{Fixed points and orbits}\label{sec:geo:Fixed points and orbits}
% Translations by elements of $\mathfrak{k}$ preserve the orbit of a point in $G/K$ (reflecting the isotropy subgroup $K$'s action where $K$ is the stabiliser (see equation (\ref{eqn:geo:stabiliser})) of a point in $G/K$, translations by elements of $\mathfrak{p}$ have the capacity to navigate across different orbits, revealing the transitive but stratified nature of the action of $G$ on $G/K$. This can be related to the fixed-point operation of $K$.In the quotient space $G/K$, the orbits of $K$ in $G$ appear as if $K$ acts as a fixed-point operator. This perspective arises because, within $G/K$, each orbit $\mathcal{O}_g$ is identified with a single point, and the distinct actions of elements of $K$ on points in $G$ that would have moved them along their orbits are now seen as leaving the corresponding points in $G/K$ invariant. That is:
% \begin{align}
%     k(gK) = (kg)K = gK
% \end{align}
% for all $k \in K$ and $g \in G$, where $gK$ denotes the coset (or point in $G/K$) corresponding to $g$. The action of $K$ on any $g \in G$ thus translates to the invariance of the coset $gK$ in $G/K$, effectively rendering $K$ as acting by fixed points in the quotient space. To this end, each fibre of $G/K$ can be thus regarded as an equivalence class of orbits. For any Lie group $G$ and a subgroup $K$, the quotient space $G/K$ is constructed by partitioning $G$ into equivalence classes under the equivalence relation:
% \begin{align*}
%     g \sim g' \longleftrightarrow g' = gk
% \end{align*}
% for $k \in K$. This relation groups elements of $G$ into sets where each set, or equivalence class, contains elements that can be transformed into one another by the right action of elements of $K$. Mathematically, an equivalence class of $g \in G$ can be denoted by the coset $gK = {gk \mid k \in K}$, which represents an orbit of $g$ under the action of $K$.

% In the quotient topology of $G/K$, each point corresponds to one such equivalence class or orbit. The projection map $\pi: G \rightarrow G/K$ maps each element $g \in G$ to the equivalence class $gK$ it belongs to. The preimage $\pi^{-1}(\pi(g)) = gK$ under this map is a fibre over the point $\pi(g)$ in $G/K$. Therefore, each fibre of $G/K$ is representative of an orbit in $G$ under the action of $K$, signifying that the entire set of elements in $G$ that are related through multiplication by elements of $K$ are collapsed to a single point in $G/K$. This illustrates how the quotient space encapsulates the idea of moving from the specific (individual group elements in $G$) to the general (equivalence classes or orbits in $G/K$) by abstracting away the internal symmetries represented by $K$.

% This explicitly builds intuition for the symmetry reducing properties of $KP$ decompositions and the fundamental role of connections in defining such symmetries on manifolds. Moreover, as we discuss below, the synthesis of connections in terms of vertical and horizontal spaces, related to the homogeneous space $G/K$ allows for a detailed understanding of Riemannian and subRiemannian geometry and, in turn, geometric control theory.

% \subsection{Parallel transport and horizontal lifts}\label{sec:geo:Parallel transport and horizontal lifts}
% We come now to important concepts related to geodesics and time optimality explored in later chapters. We are interested in the concept of parallel transport in a principal bundle $\xi = (P,\pi,\M)$ with a connection given (via the one-form) $\omega$. We are interested in \textit{horizontal vector fields} whose flow lines move from one fibre to another, intuitively constituting translation across a manifold via generators in the horizontal subspace.  Parallel transport shifts vector fields vectors along integral curves such that they "parallel" according to a specified connection. The concept of horizontal lifts is central to this process by enabling (i) preservation of a concept of direction and (ii) preserving `horizontality' such that the notion of straightness or parallelism of Euclidean space can be extended to curved manifolds, essential for the study of geodesics.

% \begin{definition}[Horizontal lift]\label{defn:geo:Horizontal lift}
%     Given a vector field $X$ on $\mathcal{M}$ and connection expressed in terms of $\omega$, its horizontal lift $X^{\uparrow}$ is a vector field on $P$ that is everywhere horizontal with respect to $\omega$ such that given $\pi_*: H_p P \to T_{\pi(p)}\M$ is an isomorphism, for all $X$ on $\M$ there exists a \textit{unique} vector field $X^{\uparrow}$ satisfying the following for all $p \in P$:
%     \begin{enumerate}[(i)]
%         \item $\pi_*(X^{\uparrow}_p) =  X_{\pi(p)}$
%         \item $V_p(X^{\uparrow}_p)=0$
%     \end{enumerate}
% The vector field $(X^{\uparrow}_p)$ is called the \textit{horizontal lift} of $X$ as it `lifts' up the vector field $X$ on $\M$ into the \textit{horizontal subspace} of $TP$
% \end{definition}
% The requirement of $V_p(X^{\uparrow}_p) = 0$, indicates that that $X^{\uparrow}$ lies entirely in the horizontal subspace $H_p\M$, encapsulates the essence of parallel transport as maintaining the direction of $X$ through the fibres of $P$. For a smooth curve $\gamma$ in $\mathcal{M}$, a horizontal lift $\gamma^\uparrow: [a,b] \to P$ is a curve whose tangent vectors are in the horizontal subspaces $H_{\gamma^\uparrow(t)}P$ as:
% \textit{horizontal} in that:
%     \begin{align*}
%         &V_p[\gamma^\uparrow] = 0\\
%         & \pi(\gamma^\uparrow(t)) = \gamma(t), \forall t \in [a,b]
%     \end{align*}
% Given a point $p \in P$ above $\gamma(a)$, there exists a unique horizontal lift $\gamma^\uparrow$ starting at $p$. This uniqueness underscores the connection's role in determining a specific way to transport points along curves in $\mathcal{M}$, embodying the geometric intuition behind parallel transport.
% \begin{definition}[Parallel vector fields]\label{def:geo:parallelvectorfields}
%    For a curve $\gamma(t) \in \M$, the vector field $X$ is parallel along $\gamma(t)$ if the covariant derivative vanishes along the curve, that is if:
%    \begin{align}
%        \nabla_{\dot \gamma(t)}X(t) = 0 \qquad \forall t \in [a,b]
% \end{align}
% where $\nabla$ is the covariant derivative defined below.
% \end{definition}
% Parallel transport of $v \in T_{\gamma(a)}\M$ along $\gamma(t)$ for $t \in [a,b]$ is then defined by the following map $\tau$ which takes $v$ to the corresponding vector field $X(b) \in T_{\gamma(b)\M}$. The vectof field $X$ is the unique vector field along $\gamma$ such that $X(a)=v$ and $\nabla_{\dot \gamma(t)}X(t) = 0$ is satisfied. Parallelism is expressible in terms of horizontal lifts as follows \cite{isham_modern_1999,frankel_geometry_2011}.
% %parallel transport
% \begin{definition}[Parallel transport]\label{def:geo:Paralleltransport} 
% For $\gamma: [a,b] \to\M$, the notion of \textit{parallel transport} along $\gamma$ from $\gamma(a)$ to $\gamma(b)$ is defined as a map $\tau: T_{\gamma(a)}\M \to T_{\gamma(b)}\M$ satisfying the following:
%     \begin{align*}
%         \tau: \pi^{-1}(\{ \gamma(a) \}) \to \pi^{-1}(\{ \gamma(b) \})
%     \end{align*}
%     The map represents assigning, to each $\pi^{-1}(\{ \gamma(a) \})$, a point in the horizontal lift of $\gamma(b)$. That is, assigning $\gamma^\uparrow(b) \in \pi^{-1}(\{ \gamma(b) \})$ to $\pi^{-1}(\{ \gamma(a) \})$ where $\gamma^\uparrow$ is the \textit{horizontal lift} of the curve $\gamma$ that passes $p$ at $t=a$.
% \end{definition}
% Parallel transport is defined across fibres, where horizontal curves are mapped into horizontal curves by the right action of $\delta$ of $G$ on $P$, for all $g \in G$ that commutes with $\tau$ i.e. $\tau \circ \delta_g = \delta_g \circ \tau$. It can be shown that if $p_1 = \tau(p)$ then $p_1g = \tau(p)g = \tau(pg)$ with the result that $\tau$ is a bijection among fibres. The concept of parallel transport is then extended to fibres via the holonomy group. This is important in our final chapter where we are interested in holonomic paths for time-optimal synthesis. The holonomy group $\text{Hol}_x(\omega)$ consists of all elements of $G$ that can be realized as the result of parallel transporting a reference fibre along closed curves (loops) starting and ending at $x$.
% \begin{definition}[Holonomy group]\label{defn:geo:holonomy}
% For a loop $\gamma: [0,1] \rightarrow \mathcal{M}$ with $\gamma(0) = \gamma(1) = x$ and a horizontal lift $\gamma^{\uparrow}$ of $\gamma$ starting at a point $p \in P$ above $x$, the endpoint of $\gamma^{\uparrow}$ is related to $p$ by an element of $G$. The set of all such elements, for all possible loops $\gamma$ based at $x$, forms the holonomy group $\text{Hol}_x(\omega)$.
% \end{definition}
% For a vector field $X$ to be parallel along $\gamma$ (for all $t \in [a,b]$), the requirement $\nabla_{\dot \gamma(t)}X(t) = 0$ says that the rate of change of the vector field and the connection's adjustment of that rate of change sums to zero. Holonomy reflects how connections on $\M$ influence the paths taken by curves on the manifold, where curves traced out by the action of the holonomy group constitute (time-optimal) subRiemannian or Riemannian geodesics (discussed further on in this work).


% \subsection{Covariant differentiation}\label{sec:geo:Covariant differentiation}
% We now come the important concept of covariant differentiation. As noted in the literature, the challenge of identifying the derivative of a section lies in how to compare neighbouring points in two different fibres in a way that does not depend on the local coordinate frame. For bundles equipped with a connection that allows a pullback points one fibre to those in another, this comparison can be undertaken. Consider the map $\psi: \mathcal{M} \rightarrow P_V$ where $\psi$ is a section, being a smooth map that assigns a vector in the fibre each point in $\mathcal{M}$ (here $P_V$ is the total space of the vector bundle where each fibre is a vector space isomorphic to $V$ (following the notation of \cite{isham_modern_1999})). We wish to understand how $\psi$ varies along curves in the manifold. This concept is expressed via the \textit{covariant derivative} as a generalised gradient (definition \ref{defn:geo:gradient}). Recall that $\mathfrak{X}(\mathcal{M})$ denotes the set of smooth vector fields on $\M$. 
% %covarient derivative
% \begin{definition}[Covariant derivative]\label{defn:geo:covariantderivative}
%     Denote a principal $G$-bundle $\xi = (P, \pi, \mathcal{M})$ with $V$ a vector space linear representation of $G$. Consider the curve $\gamma : [0, \epsilon] \to \mathcal{M}$ such that $\gamma(0) = p_0 \in \mathcal{M}$, and let $\psi : \mathcal{M} \to PV$ be a section of the associated vector bundle. Then the covariant derivative of $\psi$ in the direction $\gamma$ at $p_0$, is
% \begin{align*}
% \nabla_{\gamma}\psi := \lim_{t \to 0} \frac{\tau_{t}^{-1} \psi(\gamma(t)) - \psi(p_0)}{t}
% \label{eqn:geo:covariantderiv1}
% \end{align*}
% where $\tau_{t}^{-1}$ is the parallel transport operator from the vector space $\tau_{t}^{-1}(\{\gamma(t)\})$ to the vector space $\tau_{t}^{-1}(\{x_0\})$.
% \end{definition}
% Note we use a slight abuse of notation where $\nabla_\gamma$ refers more properly to $\nabla_{\dot\gamma}$ where $\dot\gamma(t)$ is the tangent vector to the curve $\gamma$ at the point $\gamma(t)$. Here $\tau_{t}^{-1}$ transports vectors back along $\gamma(t) \to \gamma(0)$ while preserving parallelism. We interchange with the notation $\nabla_X$ which typically refers to the covariant derivative along a vector field $X \in \mathfrak{X}(\M)$ on a manifold $\mathcal{M}$. Here, $X$ is a smooth section of the tangent bundle $T\mathcal{M}$, and $\nabla_X$ is an operator that acts on a vector field or section of a vector bundle. If two curves $\gamma_1,\gamma_2$ are tangent at $p\in\M$ then we have $\nabla_{\gamma_1}\psi = \nabla_{\gamma_2}\psi$. Morover, connecting with the notation:
% \begin{enumerate}[(a)]
%     \item For $v \in T_x\M$, the covariant derivative of $\psi$ of $P_V$ along $v$ is represented as $\nabla_v \psi = \nabla_\gamma \psi$ where $\gamma$ here is any curve in the equivalence class $v=[\gamma]$.
%     \item For the vector field $X$ on $\M$, the covariant derivative along $X$ is the linear operator: 
%     \begin{align*}
%         \nabla_X: \Gamma(P_V) \to \Gamma(P_V)
%     \end{align*}
%     on the set of cross sections $\Gamma(P_V)$ of the vector bundle $P_V$ associated with $p \in M$, that is:
%     \begin{align*}
%         \nabla_X\psi(p) = \nabla_{X_p}\psi
%     \end{align*}
% \end{enumerate}

% An important concept for understanding such differentiation comes from understanding affine connections. The covariant differential operators $\nabla$ arises from such considerations. We begin with affine connections, noting $\mathfrak{X}(\M)$ is also denoted $\Gamma(P_V)$. We note that $\nabla_X$ on $\mathfrak{X}(\M)$ exihibits the structure of derivation:
% \begin{align}
%     \nabla_X(f\psi) = f\nabla_X\psi + X(f)\psi
% \end{align}
% for $f \in \cinfm$. The $\nabla_X$ operator is also linear in $\mathfrak{X}(\M)$ (which can also be regarded as a module over $\cinfm$). These properties are expressed by considering $\nabla_X$ as an \textit{affine connection}.
% %affine connection
% \begin{definition}[Affine connection]\label{defn:geo:Affine connection}
%     An affine connection on $\M$ is an operator $\nabla: \mathfrak{X}(\M) \times \mathfrak{X}(\M) \to \mathfrak{X}(\M)$ which associates with $X \in \mathfrak{X}(\M)$ a linear mapping $\nabla_X$ of $\mathfrak{X}(\M)$ into itself i.e. $(X,Y) \mapsto \nabla(X,Y)=\nabla_XY$ satisfying the following two conditions:
% \begin{align*}
% (\nabla_1) \quad &\nabla_{fX+gY} = f\nabla_X + g\nabla_Y; \\
% (\nabla_2) \quad &\nabla_X(fY) = f\nabla_X(Y) + (Xf) Y
% \end{align*}
% for $f, g \in C^\infty(M), X, Y \in \mathfrak{X}(\M)$.  
% \end{definition}
% The affine connection is one way to define the covariant derivative $\nabla_X$ on a vector bundle $(P_V,\pi_V,\M)$, which in turn can be related to the connection one-form on the principal bundle $\xi$ (see above). The affine connection together with a local coordinate chart $(U,p)$ can be defined via:
% \begin{align*}
%     \nabla_{\partial_i} = \Gamma^k_{ij} \partial_k
% \end{align*}
% where $\Gamma^k_{ij} = (\nabla_{\partial_i} \partial_j)^k$ are \textit{Christoffel symbols of the second kind} and $(\cdot)^k$ indicates the $k$-th component. For the covariant derivative of $Y$ with respect to $X$, such $k$-th coordinate is given by:
% \begin{align*}
% \left(\nabla_X Y\right)^k = X^i (\nabla_i Y)^k = X^i \left(\frac{\partial Y^k}{\partial x^i} + \Gamma^k_{ij} Y^j\right).
% \end{align*} 

% \subsection{Geodesics and parallelism}\label{sec:geo:Geodesics and parallelism}
% We can use the above concepts to define a notion of parallelism leading to a definition of geodesics. Denote $\gamma: I \to \M, t \mapsto \gamma(t)$ for an interval $I \subset \Real$ (which we generally without loss of generality specify as $I=[0,1]$) with an associated tangent vector $\dot\gamma(t)$. Here $\gamma$ is regular. Two vector fields $X,Y$ are parallel along $\gamma(t)$ if:
% \begin{align*}
%     \nabla_XY = 0 \qquad \forall t \in I
% \end{align*}
% This definition of parallelism involves values of $X,Y$ only on the curve $\gamma$. In local coordinates $\{x_i\}$, it can be shown that their exist coordinate functions $X^i,Y^j$ for $i,j \leq m$ on the coordinate neighbourhood $U$ as per above such that:
% \begin{align*}
%     X = \sum_i X^i \left(\frac{\partial}{\partial_{x_i}} \right) \qquad Y = \sum_j Y^j \left(\frac{\partial}{\partial_{x_j}} \right)
% \end{align*}
% \begin{align*}
% \nabla_X(Y) &= \sum_k \left( \sum_i X^i \frac{\partial Y^k}{\partial x_i} + \sum_{i,j} X^i Y^j \Gamma^k_{i,j} \right) \frac{\partial}{\partial x_k} \quad \text{on } U
% \end{align*}
% with the result:
% \begin{align*}
% \frac{dY^k}{dt} + \sum_{i,j} \Gamma^k_{i,j} \frac{dx_i}{dt} Y^j &= 0 \quad (t \in J) \label{eqn:geo:geodesicchristoffel1}
% \end{align*}
% which can be shown \cite{helgason_differential_1979} to represent equation (\ref{eqn:geo:covariantderiv1}) in the limit as $t \to 0$. Equation (\ref{eqn:geo:geodesicchristoffel1}) indicates that the component form of the covariant derivative along $\gamma(t)$ is zero (hence indicative of parallel transport). The covariant derivative operator $\nabla_X$ has a number of properties, including that (i) it is a derivation (an $(r,s)$-tensor being drawn from the derivation space of tangent and cotangent vectors respectively), (ii) it preserves tensors (i.e. it maps $(r,s)$ tensors to $(r,s)$ tensors) $\nabla_X: T^{r,s}\M \to T^{r,s}\M$ and (iii) commutes with all contractions $C^i_j$ (see above). From this we come to the first iteration of a \textit{geodesic}.
% %geodesic definition
% \begin{definition}[Geodesic]\label{defn:geo:Geodesic}
%     A curve $\gamma: I \to \M, t \mapsto \gamma(t)$in $\M$ is denoted a geodesic if the set of tangent vectors $\{\dot\gamma(t)\} = T_{\gamma(t)}\M$ is parallel with respect to $\gamma$, corresponding to the condition that $\nabla_{\gamma}\dot\gamma=0$, which we denote the geodesic equation. 
% \end{definition}
% In a coordinate fame the geodesic equation is expressed as:
% \begin{align*}
%     \frac{d^2u^\gamma }{ds^2} +   \Gamma^\gamma_{\alpha \beta} \frac{du^\alpha }{ds} \frac{du^\beta }{ds} = 0 \label{eqn:geo:geodesiccoordinateframe}
% \end{align*}
% where:
% \begin{align*}
% \Gamma^\gamma_{\alpha \beta} = \frac{1}{2} g^{\gamma \mu} \left( \frac{\partial g_{\mu \alpha}}{\partial u^\beta} + \frac{\partial g_{\mu \beta}}{\partial u^\alpha} - \frac{\partial g_{\alpha \beta}}{\partial u^\mu} \right)
% \end{align*}
% are the Christoffel symbols of the second kind (essentially connection coefficients) with $g^{\gamma \mu}$ the inverse of the metric tensor and $ds$ usually indicates parametrisation by arc length. It can be shown that given an affine connection above, for any $p \in \M$ and $X_p$, there exists a unique [maximal] geodesic $t \mapsto \gamma(t)$ such that $\gamma(0)=p$ and $\dot\gamma(0)=X_p$, i.e. it cannot be extended to a larger interval. As \textbf{NIELSEN INFO} notes, the geodesic equation is solved either (a) as an initial value problem by specifying $\gamma(0)=p,\dot\gamma(0)=v$ for $v \in T_p\M$, or (b) a boundary value problem for $\gamma(0)=p$ and $\gamma(1)=q$ using variational methods.

% \section{Riemannian manifolds}\label{sec:geo:Riemannian manifolds}
% The covariant derivative / affine connection $\nabla$ on $\M$ allows us to define concepts of \textit{torsion} and \textit{curvature} tensor fields. First, we define the celebrated Riemann curvature tensor. The tensor intuitively represents 

% \begin{definition}[Riemann curvature tensor]\label{defn:geo:Riemann curvature tensor}
% Given an $(\M,g)$ Riemannian manifold (see below) and set of vector fields $\mathfrak{X}(\M)$, define the following $(1,3)$ tensor field:
% \begin{align}
%     &\mathfrak{X}(\M) \times \mathfrak{X}(\M) \times \mathfrak{X}(\M) \to \mathfrak{X}(\M) \\
%     &(X,Y,Z) \mapsto R(X,Y)Z &= (\nabla_X\nabla_Y - \nabla_Y\nabla_X - \nabla_{[X,Y]})Z \\
%     & &= \nabla_X\nabla_Y Z - \nabla_Y\nabla_X Z - \nabla_{[X,Y]}Z
% \end{align} 
% for any vector fields $X, Y, Z \in \mathfrak{X}(\mathcal{M})$, where $\nabla$ denotes the Levi-Civita connection associated with the metric $g$.
% \end{definition}
% The Riemann curvature tensor measures the extent to which the affine connection (covariant derivative) is not commutative i.e. the failure of the covariant derivatives to commute and therefore the extent of intrinsic curvature of the manifold. In this way, it corresponds to the non-holonomy of $\M$. Recall $\text{Hol}_x(\omega)$ for a loop $\gamma$ reflects parallel transportation of a vector $v \in T_p\M$ to and from $x \in \M$ along $\gamma$. The deviation of $v$ from its initial position can be given by the action of the Riemann curvature tensor along the loop expressed by the Ambrose-Singer Holonomy Theorem which states that the Lie algebra of $\text{Hol}_x(\omega)$ at $x \in \M$ is generated by the values of the curvature $\Omega$ over all horizontal two-planes in $T_pP$ where $p$ is the fibre over $x$ (see also section \ref{sec:geo:sectionalcurvature} below). The properties of $\text{Hol}_x(\omega)$ that describe how parallel transport around closed loops $\gamma$ distort vectors are related to the curvature experienced by these vectors in plans spanned by tangent vectors at $T_x\M$. Integrating $R_{\mu \nu}$ overa all such two-dimensional subspaces identifies the set of possible curvatures that parllel transport can induce i.e. each element in $\text{Hol}_x(\omega)$ corresponds to a unique way of parallel transporting and the relation to curvature quantifies the amount of twisting or distortion of the vector ($R_{\mu \nu}$ being responsible for \textit{both} the curvature experienced and the Lie algebra of $\text{Hol}_x(\omega)$ ) [\textbf{AMBROSE 1953}].


% Given on Riemannian manifolds the affine connection is given by the Levi-Civita connection that is metric compatible and torsion free, the Riemann curvature tensor has an expression in terms of the second covariant derivative:
% \begin{align*}
%     R(X,Y) = \nabla^2_{X,Y} - \nabla^2_{Y,X}
% \end{align*}
% Given the relationship between second derivatives and curvature, one can see how the Riemann curvature tensor gives rise to a measure of curvature on manifolds. In coordinate notation, it is denoted as:
% \begin{align*}
%     R^{\alpha}_{\beta\gamma\delta} = \Gamma^{\alpha}_{\beta\delta,\gamma} - \Gamma^{\alpha}_{\beta\gamma,\delta} + \Gamma^{\mu}_{\beta\delta} \Gamma^{\alpha}_{\mu\gamma} - \Gamma^{\mu}_{\beta\gamma} \Gamma^{\alpha}_{\mu\delta},
% \end{align*}
% To obtain measures of curvature, one can then perform contractions with the metric tensor $g$ to obtain the \textit{Ricci tensor} which is obtained by performing a tensor contraction over the first and third indices i.e. $R_{\mu\nu} = R^\lambda_{\mu\lambda\nu}$. Scalar curvature is then obtained via contraction with the inverse metric tensor $R = g^{\mu\nu}R_{\mu\nu}$, which is in effect a trace operation.
% Given the definitions
% \begin{align*}
% T(X, Y) &= \nabla_X(Y) - \nabla_Y(X) - [X, Y] \qquad (\text{torsion tensor}) \\
% R(X, Y) &= \nabla_X\nabla_Y - \nabla_Y\nabla_X - \nabla_{[X,Y]} \qquad (\text{curvature tensor}),
% \end{align*}
% With an appropriate one-form, we can then define a a \textit{torsion tensor field} as the argument for the one-form mapping $\omega: T*\M \times T\M \times T\M  \to \R$ with $(\omega,X,Y) \mapsto\omega(T(X,Y))$ where $T(X,Y) \in T^1_2\M$ (i.e. a type (1,2) tensor). We can define the \textit{curvature tensor field} $\omega: T*\M \times T\M \times T\M  \times T\M \to \R$ with $(\omega,X,Y,Z) \mapsto\omega(R(X,Y) \cdot Z)$ where $R(X,Y) \cdot Z \in T^1_3\M$. It can be shown that the relevant one-forms in turn determine the structure of the covariatn derivative on $\M$, while it can be shown (via Cartan's structure equations) that the forms $\omega$ are themselves described by the torsion and curvature tensor fields as per below (adapted from Theorem 8.1 in \cite{helgason_differential_1979}, $\S$8).

% \begin{theorem}[Cartan structural equations]\label{thm:geo:Cartanstructuralequations}
% Given a principal bundle connection (definition \ref{defn:geo:Connection}), Cartan's structural equations are given by:
% \begin{align}
%     d\omega^i &= - \sum_{p} \omega^i_p \wedge \omega^p + \frac{1}{2} \sum_{j,k} T^i_{jk} \omega^j \wedge \omega^k \\
%     d\omega^i_l &= - \sum_{p} \omega^i_p \wedge \omega^p_l + \frac{1}{2} \sum_{j,k} R^i_{ljkp} \omega^j \wedge \omega^k
% \end{align}
% \end{theorem}
% Here for completness, $d\omega^i$ represents the exterior derivative (how $\omega^i$ changes in all directions), $\omega^i_p$ is a one form representing connection coefficients, encoding information about non-linear behaviour, the $\wedge$ product captures the idea of an oriented area spanned by the one-forms $\omega^i$. Cartan's structural equations provide an important tool for using the local behaviour of a connection to understand global properties of $\M$, such as curvature and torsion. 

% \subsection{Riemannian Manifolds and Metrics}\label{sec:geo:Riemannian Manifolds and Metrics}
% We now come to identifying how to calculate lengths of curves on manifolds relevant to later chapters. Firstly, we define a (pseudo)-Riemannian structure in terms of a tensor field. In doing so we gain further insight into metrics in terms of tensor fields of type (0,2). A Riemannian manifold is the tuple $(\M,g)$ (i.e a manifold $\M$ with a metric $g$) where to each $p \in \M$ is assigned a positive definite map $g_p: T_p\M \times T_p\M \to \R$ (described usually in terms of being an inner product) and an associated norm $||X_p||: T_p\M \to \R$. We integrate these concepts in the formalism above as follows.
% \begin{definition}[Riemannian structure]\label{defn:geo:(Pseudo)-Riemannian structure}
%     Define a pseudo-Riemannian structure on $\M$ as a type-(0,2) tensor field $g$ such that (a) $g(X,Y) = g(Y,X)$ (symmetric) and (b) for $p \in \M$, $g$ is a nondegenerate bilinear form $g_p: T_p\M \times T_p\M \to \R$.
% \end{definition}
% If we assume $g_p$ is positive definite for all $p \in \M$ then we speak of Riemannian structures and manifolds as follows.
% \begin{definition}[Riemannian Manifold]\label{defn:geo:Riemannian Manifold}
%     A Riemannian manifold is a connected $\cinfm$ manifold with a Riemannian structure such that there exists a unique affine connections satisfying the following:
%     \begin{enumerate}[(i)]
%         \item $\nabla_X Y - \nabla_Y X = [X,Y]$ (namely the torsion tensor $T=0$); and 
%         \item $\nabla_Z g = 0$ (parallel transport preserves the inner product on tangent spaces).
%     \end{enumerate}
% \end{definition}
% By applying $\nabla_Z$ to the tensor field formed from $X \otimes Y \otimes g$, can specify the Riemann connection. We understand this as follows. An affine connection $\nabla$ is metric compatible with a metric $g$ when: 
% \begin{align*}
% X\inner{Y}{Z} = \inner{\nabla_X Y}{Z} +  \inner{Y}{\nabla_X Z},
% \end{align*}
% which can be expressed using the metric $g$ as:
% \begin{align*}
%     Xg({Y},{Z}) = g({\nabla_X Y},{Z}) +  g({Y},{\nabla_X Z})
% \end{align*}
% Metric-compatible connections preserve angles, orthogonality and lenths of vectors in $T_p\M$ when transported along $\gamma(t)$. The fundamental theory of Riemannian geometry is an existence and uniqueness theorem which asserts the existence of a torsion-free metric compatible connection, denoted the \textit{Levi-Civita connection}, which can be expressed via the Koszul formula as per below.
% \begin{align}
%     2g(X, \nabla_Z Y) = Z g(X,Y) + g(Z,[X,Y]) + Y g(X,Z) + g(Y,[X,Z]) - Xg(Y,Z) - g(X,[Y,Z])
% \end{align}
% An example of a connection where torsion is non-zero yet remains metric compatible is the Weitzenb\"ock connection. The metric $g$ determines the local structure but not global structure. We now define the Riemannian metric.
% \begin{definition}[Riemannian metric]\label{defn:geo:Riemannian metric}
%     A Riemannian metric is an assignment to each $p \in \M$ of a positive-definite inner product:
%     \begin{align*}
%         g_p: T_p\M \times T_p\M \to \R
%     \end{align*}
%     with an induced norm:
%     \begin{align*}
%         ||\cdot ||_p&: T_p\M \to \Real\\
%         (v,w)&\mapsto \sqrt{g_p(v,w)}
%     \end{align*}
% \end{definition}
% The Riemannian metric is a $(0,2)$-form thus a tensor, aligning definition (\ref{def:geo:metric_tensor}). Recall $(0,2)$-forms at $p \in \M$ have a representation as the tensor product of two cotangent vectors at $p$. Given a coordinate basis for $T^*_pM$ at $p$, denoted $\{dx^1, dx^2, \ldots, dx^n\}$. In the case of a $(0,2)$-form $g$, we can express it in this basis as:
% \begin{align*}
% \omega &= \sum_{i,j} \omega_{ij} \, dx^i \otimes dx^j,
% \end{align*}
% where the $g_{ij}$ are the components of the form with respect to the basis, and they can be functions on the manifold. We can then identify an induced norm on $\M$ using this metric. For $X \in T_pM$, denote:
% \begin{align}
%     \left(g_p(X,X)\right)^{1/2} \dot = || X ||
% \end{align}
% We may now define the important concept of arc (curve) length which is fundamental to later chapters. Given the curve (segment) $t \mapsto \gamma(t)$ with $t \in [\alpha,\beta]$ and metric $g_\gamma = g$, define the \textit{arc length} of $\gamma$ as follows:
% \begin{definition}[Arc length]\label{defn:geo:arclength}
%     Given a curve $\gamma(t) \in \M$ with $t \in [\alpha,\beta]$ and metric $g$, the arc length of the curve from $\gamma(0)$ to $\gamma(t)$ is given by:
%     \begin{align}
%     L(\gamma) = \int_\alpha^\beta \left( g(\dot\gamma(t),\dot\gamma(t)) \right)^{1/2} dt 
%     \label{eqn:geo:arclength}
% \end{align}
% \end{definition}
% Given any normal neighbourhood $N_0$ of $0 \in \M$ and defining $N_p = \exp(N_0)$, then for any $q \in N_p$, denote the unique geodesic in $N_p$ joining $p$ to $q$ as $\gamma_{pq}$. In this case it can be shown that $L(\gamma_{pq}) < L(\gamma)$ for each curve segment joining $p$ and $q$. Under this assumption, we can impose a metric upon the Riemannian manifold $\M$ as follows. Assuming $\M$ is simply connected, then all $p,q \in \M$ can be joined via a curve segment. The \textit{distance} of $p,q$ is then defined by the infimum of the shortest curve measured according to the equation (\ref{eqn:geo:arclength}) above and is defined as:
% \begin{align}
%     d(p,q) = \inf_\gamma L(\gamma)
%     \label{eqn:geo:riemannmetric}
% \end{align}
% Here $d(p,q)$ satisfies the usual axioms of metrics, namely (a) symmetry $d(p,q) = d(q,p)$, (b) triangle inequality $d(p,q) \leq d(p,r) + d(r,q)$ and (c) positive definite $d(p,q) = 0$ if and only if $p=q$.
% It can then be shown that for such a Riemannian manifold $\M$ with metric $d$ given by equation (\ref{eqn:geo:riemannmetric}) together with a curve $\gamma_{pq}$ joining $p,q \in \M$, then if $L(\gamma_{pq} = d(p,q)$ then $\gamma_{pq}$ is a geodesic. Then consider an open ball around $p$ with radius $r$, $B_r(p)$ and associated sphere around $p$ denoted $S_r(p)$. Then assume an open ball $V_r(0) = \{X \in T_p \M | 0 \leq ||X|| \leq r \}$ is a normal neighbourhood of $0 \in T_p\M$. In this case it can be shown that $B_r(p) = \exp(V_r(0))$. For complete Riemann manifolds (where every sequence in $\M$ is convergent), each pair of points $p,q \in \M$ can be joined by a geodesic of length $d(p,q)$. Recall isometries are distance preserving mappings of $\M$ onto itself. 

% The preservation of distances can then be understood in terms of total geodesicity of manifolds. 
% A sub-manifold $S$ of a Riemannian manifold $\M$ is \textit{geodesic at} $p$ if each geodesic tangent to $S$ at $\p$ is also a curve in $S$. The submanifold $S$ is \textit{totally geodesic} if it is geodesic for all $p \in S$. It can then be shown that if $S$ is totally geodesic, then parallel translation along $\gamma \in S$ always transports tangents to tangents, that is $\tau: S_p\M \to S_p\M$. Summarising the above points: 
% \begin{itemize}
%     \item \textit{Riemann Connection}: 
% This refers to the affine connection on a Riemannian manifold $\M$, representing differentiation of vector fields $\mathfrak{X}(\M)$ along curves $\gamma$ and for calculations related to parallel transport.
% \item \textit{Riemann metric}: This provides a notion of distance on $\M$, providing a means of measuring lengths of curves and angles between vectors, thereby defining the manifold geometry. 
% \item \textit{Riemann curvature tensor}: This tensor $R_{\mu\nu}$ quantifies curvature on $\M$ and derives from the   Riemann connection. Importantly, it is  independent of any coordinate embedding.
% \item \textit{Levi-Civita Connection}: Given all connections on a Riemannian manifold with metric $(\M,g)$, the Levi-Civita connection is the unique connection that is both torsion-free and metric-compatible, i.e. preserving the Riemannian metric under parallel transport (under which the covariant derivative of the metric tensor vanishes).
% \end{itemize}



% \subsection{Fundamental forms}\label{sec:geo:Fundamental forms}
% In this section we briefly set out a few key theorems and definitions from standard differential geometry relating to fundamental forms and curvature which are familiar for differential geometry on Euclidean spaces. In particular we connect standard results to the coordinate-free formalism adopted above.
% \begin{enumerate}[(i)]
%     \item \textit{First fundamental form}. The first fundamental form is an expression of the metric tensor $g$ on $\M$ and is denoted:
%     \begin{align}
%         I_p(X,Y) = g_p(X,Y) \qquad X,Y \in T_p\M
%     \end{align}
%     Given a coordinate chart $\phi:\R^2 \to \M$ where $\phi(X,Y) \to p\in\M$ then define as usual $\phi_X = \partial_X \phi$ and similarly for $v$ and dual $X'=dX/dt$. Then (recalling $g(X,V)=\braket{X,Y}$):
%     \begin{align}
%         E &= g(\phi_X,\phi_X) \qquad F = g(\phi_X,\phi_Y)\qquad G = g(\phi_Y,\phi_Y)\\
%         g_{ij} &= \pmat{E}{F}{F}{G}\\
%         I_p &= E (u')^2 + 2Fu'v' + G(v')^2 = g_{ij}\frac{dx^i}{dt}\frac{dx^j}{dt} = ds^2{dt}
%     \end{align}
%     with equivalents for higher-dimensional manifolds. The first fundamental form thus represents a quadratic form associated with the metric tensor \cite{frankel_geometry_2011}.
%     \item \textit{Second fundamental form}. The second fundamental form describes how surfaces curve in ambient space i.e. by reference to a normal to surface. In general, define a level set function $f: \M \to \R$ as the set of points $p \in \M$ such that $f(p)=c \in \R$:
%     \begin{align}
%         S_c = \{ p \in \M | f(p) = c\}
%     \end{align}
%     $S_c \subset \M$ will be a submanifold if $\Delta f \neq 0, \forall p \in S_c$. Recall that $\nabla f$ points in the direction of the steepest incease in $f$. For $\nabla f(p) \neq 0$, $f$ is non-constant except along directions tangent to $S_c$. Thus $S_c$ resembles a hypersurface in $\M$ (where $\dim S_c = \dim \M-1$), which is a generalisation of $\M$ being, for example, $\R^3$ with $S_c = \R^2$ and $\nabla_f$ being the normal vector `pointing out' of the surface. Thus we can denote a generalised unit normal vector via $N = \nabla f/||\nabla f||$. The second fundamental form is then defined as:
%     \begin{align*}
%         II_p(X,Y) = g(\nabla_X N,Y) = \braket{S(X),Y}
%     \end{align*}
%     for $X,Y \in T_p\M$. Here $S(X)=\nabla_X N$, the shape operator which encodes information about a manifold's (or submanifold's) curvature by describing how the normal vector field $N$ changes along the vector field $X$ for $X \in T_p\M$ (i.e. as one moves tangent to the surface). We then have in the coordinate frame:
%         \begin{align*}
%         e&=-\braket{N_u, \phi_u} \qquad        f=-\braket{N_u, \phi_v} = -\braket{N_v, \phi_u}\qquad 
%         g=\braket{N_v, \phi_v}\\
%        II_p&=e (u')^2 + 2fu'v' + g(v')^2
%     \end{align*}
%     \item \textit{Gauss and Codazzi equations}. The Gauss equation provides that the Gauss curvature is a measure of intrinsic curvature of the manifold. In a coordinate frame, given the first and second fundamental forms in a coordinate basis with components $\phi_u,\phi_v$ with principal curvatures given by $dN = \text{diag}(k_1,k_2)$. Gaussian curvature is then:
%     \begin{align}
%         K & = \frac{\det (h_{ij})}{\det (g_{ij})} = \frac{eg -f^2}{EG - F^2}   k_1 k_2 \\
%         H& = \frac{1}{2} (k_1 - k_2) = \frac{1}{2}\frac{eE - 2fF + gG}{EG-F^2}
%     \end{align}
%     where $H$ is mean curvature (the average of principal curvatures $k_1,k_2$. Gaussian curvature is extrinsic to the manifold, while mean curvature depends on how it is embedded in ambient space. In coordinate free form, the Gauss equation can be exprssed as:
%     \begin{align}
%         [\nabla_X,\nabla_Y]Z = -K \det(X,Y)JZ
%     \end{align}
%     where $\det(X,Y)$ is the \textit{area form} of a Riemannian manifold and $J$ is an endomorphism (mapping) $J:\M \to \M$ such that $\braket{JX,Y}=\det(X,Y)$ and is denoted an\textit{almost complex structure} $J^2=-I$ (and so intuitively acts to rotate by $\pi/2$ in a way that transitions for example $JX\to Y$. These results provide that the Gaussian curvature $K$ is invariant under local isometry, a statement of Gauss's celebrated \textit{theorem egregium}. Additionally, the \textit{Codazzi equation} provides that the covariant derivative of $II_p$ is symmetric, that is:
%     \begin{align}
%        [\nabla_X,\nabla_Y]N =  (\nabla_X \nabla_Y - \nabla_Y \nabla_X)N = \nabla_{[X,Y]}N \label{eqn:geo:Codazzi equation}
%     \end{align}
%     which, when satisfied, ensures that the local shape of the surface given by normal curvature $\nabla_X N$ is consistent with the global properties of the manifold (thereby providing an integrability condition). 
% \end{enumerate}

% \subsection{Curvature and forms}\label{sec:geo:curvatureandforms}
% Curvature is a concept of fundamental importance in geometric methods across quantum information, algebra, machine learning and control. Curvature also plays a profound role in the classification of symmetric space of interest in quantum information, where in many cases computations may be expressed in terms of the evolution of curves over unitary Lie group manifolds generated by Hamiltonians drawn from corresponding Lie algebras. In this section, we contextualise curvature in the language of differential forms, beginning with the concepts of sectional curvature and revisiting curvature tensor fields on the way to defining the celebrated Riemann curvature tensor.

% \subsection{Sectional curvature}\label{sec:geo:sectionalcurvature}
% We now define sectional curvature on the way to defining the formalism of Riemannian symmetric spaces, the subject in particular of our final chapter. Sectional curvature $K(\sigma_p)$ provides a means of classifying curvature on Riemannian manifolds via a two-dimensional sub-bundle $\sigma_p \subset T_p\M$. Geometrically it corresponds to the Gaussian curvature with plane $\sigma_p$ constructed from tangents to geodesics $\gamma$ in the direction of $\sigma_p$.  Recall the definition of the section of a fibre bundle.
% \begin{definition}[Section of a Fibre Bundle]\label{defn:geo:Section of a Fibre Bundle}
% Let $ \pi: E \to M $ be a fibre bundle with total space $ E $, base space $ M $, and fibre $ F $. A section of this fibre bundle is a continuous map $ s: M \to E $ such that $ \pi \circ s = \text{id}_M $, the identity map on $ M $. In other words, for each point $ p \in M $, $ s(p) $ is a point in the fibre over $ p $, i.e., 
% \begin{align}
% \pi(s(p)) = p, \quad \forall p \in M.
% \end{align}
% \end{definition}
% This condition ensures that the section "lifts" each point in the base manifold back to a specific point in the total space, intersecting each fibre exactly once. For a \textit{vector bundle section} then the section is a map assigning to each $p \in \M$ a vector in the corresponding fibre. We now define the sectional curvature as taking a two-dimensional sub-bundle of the section in order to calculate curvature. The intuitive idea is that one can observe how a plane .
% \begin{definition}[Sectional curvature]\label{def:geo:sectionalcurvature}
%     For a Riemannian manifold $\M$ and point $p \in \M$ with a two-dimensional sub-bundle $\sigma_p \subset T_p\M$ with $X,Y \in \sigma_p$, define the sectional curvature $K: T_p\M \times T_p\M \to \R, (X,Y) \to K(X,Y)$ as:
%     \begin{align*}
% K(X, Y) &= \frac{g(R(X, Y)Y, X)}{g(X,X)g(Y,Y) - g(X,Y)^2}\\
% &=\frac{\langle R(X, Y)Y, X\rangle}{\langle X, X\rangle \langle Y, Y\rangle - \langle X, Y\rangle^2}
% \end{align*}
% where $R$ is the Riemann curvature tensor, $g$ is the Riemannian metric tensor and $g(X,Y)=0$ (orthogonal).
% \end{definition}
% Sectional curvature $K$ thus measures how the Riemann curvature tensor, when acting on $X,Y$ relates to the area spanned by $X$ and $Y$. This spanning of an area is also described by a ``2-Grassmanian bundle'', which intuitively speaking is the set of  
% Riemannian manifold then has constant curvature $c$ if $K(H) = c$. Indeed it can be shown (see \cite{helgason_differential_1979}, Prop. 12.3) that sectional curvature determines the Riemannian curvature such that if for two bundles $T_p\M,T_{q}\M$, $K_p = K_{q}$, then $R_p=R_q$. For a two-dimensional manifold, the sectional curvature of the plane spanned by $(X,Y)$ is the Gaussian curvature at that point. Given Gaussian curvature is [restricted] to two-dimensions, sectional curvature in one sense allows a generalisation of Gaussian curvature measurement to higher-dimension manifolds. 



% \section{Symmetric spaces}\label{sec:geo:Symmetric spaces}
% \subsection{Overview}
% Symmetric spaces were originally defined as Riemannian manifolds whose curvature tensor is invariant under all parallel translation. Locally, they resemble Riemannian manifolds. Locally they are manifolds of the form $\R^n \times G/K$ where $G$ is a semi-simple lie group with an involutive automorphism whose fixed point set is the compact group $K$ while $G/K$, as a homogeneous space, is provided by a $G$-invariant structure. Cartan thus allowed the classification of all symmetric spaces in terms of classical and exceptional semi-simple Lie groups. Cartan's classification of symmetric spaces (see Chapters IV and IX of \cite{helgason_differential_1979}) is of seminal importance. 

% As Helgason notes, Cartan adopted two methods for the classification problem. The first, bsed on holonomy groups provides that for $p \in \M$ Riemannian, then the holonomy group (definition \ref{defn:geo:holonomy}) of $\M$ is the group of all linear transformations of the tangent space $T_p\M$ corresponding to parallel transportation of closed curves $\gamma \in \M$. Parallel translation is equated with the action of the holonomy group and leaves the Riemannian metric invariant, leading to a method of classification. The more direct second method involves demonstrating the invariance of the curvature tensor under parallel transport is equivalent geodesic symmetry being a local isometry for all $p \in \M$ through which the geodesic cure passes.  As Helgason notes, such spaces with geodesic symmetry and global isometry are equipped with a transistive group of isometries $K$ such that space is represented as a coset space $G/K$ with an involutive isomorphism whose fixed point is the isometry group $K$.  The study of symmetric spaces then becomes a question of studying specific involutive automorphisms of semi-simple Lie algebras, thus connecting to the classification of semi-simple Lie groups. 
% \textit{Geodesic symmetry} is defined in terms of diffeomorphisms $\varphi$ of $\M$ which fix $p \in \M$ and reverses geodesics through that point (i.e. when acting the map $f: \gamma(1) = q \to \gamma(-1)=q'$, such that $d\varphi)p = -I$ where $I$ denotes the identity in $T_p\M$.  The manifold $\M$ is then \textit{locally (Riemannian) symmetric} if each geodesic symmetries is isometric that is, if there is at least one geodesic symmetry about $p$ which is an isometry (and globally so if this applies for all $p \in \M$). As noted in the literature, this is equivalent to the vanishing of the covariant derivative of the curvature tensor along the geodesic. A globally symmetric space is one where geodesic symmetries are isometries for all $\M$.
% A manifold being \textit{affine locally symmetric} is one which, given $\nabla$, the torsion tensor $T$ and curvature tensor $R$, $T=0$ and $\nabla_Z R=0$ for all $Z \in T\M$. 
% %Riemannian local symmetric space
% \begin{definition}[Riemannian local symmetric space]\label{defn:geo:Riemannian local symmetric space}
%     A Riemannian manifold $\M$ if for all $p \in \M$ there exists a normal neighbourhood $N_p$ where the geodesic symmetry for $p$ is an isometry. In other words, a Riemanninan local symmetric space is a manifold $\M$ where the Riemann curvature tensor is invariant under all parallel translations, that is:
%     \begin{align*}
%         \nabla_X R = 0
%     \end{align*}
% \end{definition}
% It can be shown that this is equivalent to the sectional curvature being invariant under parallel translations. In the formalism of Helgason, given a Riemannian manifold $\M$ with Riemannian structure $Q$, an analytic Riemannian manifold is one where both $\M$ and $Q$ are analytic. From this we obtain the global form i.e. a \textit{Riemannian globally symmetric} space if all $p \in \M$ are fixed points of an involutive symmetry $\theta$ such that $\theta^2(p) = \theta$. In this case $\theta$ is also a geodesic symmetry in that $\theta(p)$ induces $\dot\gamma_p \to -\dot\gamma_p$ i.e. a reflection symmetry along the geodesic. As Helgason, following Cartan, notes, in such cases certain facts follow from being a Riemannian globaly symmetric space $G/K$ (in which case $(G,K)$ is sometimes denoted a Riemannian symmetric pair), with a Cartan decomposition as discussed above and an association of $H_p\M \sim \p$ and $V_p\M \sim \k$. 
% It can be shown then that the Riemann curvature tensor for the symmetric space (homogeneous) $G/K$ with a Riemannian metric allows for curvature, via $R$, to be related to the Lie triple property, namely:
% \begin{align}
%     R_p(X,Y)Z = -[[X,Y],Z] \qquad X,Y,Z \in \p
% \end{align}
% The theorem has the consequence that the curvature $R$ at $p$ can be analysed by studying the Lie brackets of generators in $\p$ and is reflective of the Lie triple property: 
% \begin{align}
%     [[\p,\p],\p] \subseteq \p \label{eqn:geo:lietripleproperty}
% \end{align}
% Moroever, the curvature tensor is independent of the group action of $h \in G$, that is, the curvature tensor remains invariant. In geometric terms, this is reflected by the fact that the pullback of the metric tensor by $h$ corresponds to the original metric tensor itself. This $G$-invariance property of symmetric spaces $G/K$ means that the parallel transport of vectors remains the same.

% Curvature plays an important role in the classification of symmetric spaces. Three classes of symmetric space can be classified according to their sectional curvature as follows. Given a Lie algebra $\g$ equipped with an involutive automorphism $\theta^2=I$, with corresponding group $G$ with $G/K$ as above, we have a $G$-invariant structure on the Riemannian metric i.e. $g(X,Y) = g(hX,hY)$ for $h\in G/K$. Then the three types of symmetric space are:
% \begin{enumerate}[(i)]
%     \item $G/K$ compact, then $K(X,Y) > 0$;
%     \item $G/K$ noncompact, then $K(X,Y) < 0$; and
%     \item $G/K$ Euclidean, then $K(X,Y)=0$
% \end{enumerate}
% The non-compactness or compactness can be calculated via the rank of $\M=G/K$, beign the maximum dimension of a subspace of $T\M$ where $K=0$.

% \subsection{Curvature and commutators}\label{sec:geo:Curvature and commutators}
% To round off this section, we briefly note how the Maurer-Cartan form and Cartan curvature can be used to demonstrate the curvature of symmetric spaces. The commutator relation $[\mathfrak{p}, \mathfrak{p}] = \mathfrak{k}$ is interpreted as having curvature because the commutator of two horizontal elements (from $\mathfrak{p}$) yields an element in the vertical space (from $\mathfrak{k}$), indicating a deviation from flatness (see Sharpe \cite{sharpe_differential_2000} for advanced discussion in relation to Cartan geometries). Recalling the Cartan curvature equation (\ref{eqn:geo:cartancurvatureequation2}) modified for Lie algebra elements $X,Y \in \g$:
% \begin{align*}
% \Omega(X,Y) = d\theta(X,Y) + \frac{1}{2}[\theta(X), \theta(Y)]
% \end{align*}
% where $d\theta$ denotes the exterior derivative (of the one-form $\theta$) and recall that $\theta$ (equation (\ref{eqn:geo:thetaUoneformcartanmaurer}) is a $\g$-valued one-form, which means the image of $\theta(X),\theta(Y) \in \g$. For $\g = \k \oplus \p$ we then have that $\theta$ can be decomposed as:
% \begin{align}
%     \theta_\g= \theta_\k + \theta_p
% \end{align}
% noting $\theta_\k \in \k,\theta_\p \in \p$.  Calculating the exterior derivatives (definition \ref{defn:geo:exterior_derivative}) and gru:
% \begin{align}
%     d\theta_k + \frac{1}{2}[]
% \end{align}
% \hl{\textbf{FIX}}


% \subsection{Classification of symmetric spaces}\label{sec:geo:Classification of symmetric spaces}
% The classification of Riemannian symmetric spaces by Cartan (see Knapp \cite{knapp_lie_1996} and Helgason \cite{helgason_differential_1979} for detailed discussion, especially Helgason Chapter IX) terms of simple Lie groups is set out below. Type I spaces are non-compact and are associated with non-compact simple Lie groups, while Type II spaces are their compact counterparts. Type III spaces are distinct in that they are Riemannian duals of themselves. Type IV spaces involve complex structures and are related to complexifications of simple Lie algebras. The families of simple Lie groups are denoted by $A_n$, $B_n$, $C_n$, and $D_n$, where $A_n$ corresponds to the special linear group $\text{SL}(n+1, \mathbb{C})$, $B_n$ to the special orthogonal group $\text{SO}(2n+1)$, $C_n$ to the symplectic group $\text{Sp}(n)$, and $D_n$ to the special orthogonal group $\text{SO}(2n)$. Additionally, the exceptional Lie groups are denoted as $E_6$, $E_7$, $E_8$, $F_4$, and $G_2$, each signifying a unique algebraic structure that induces specific geometric properties on the associated symmetric spaces.


% \begin{table*}[h!]
% \footnotesize
% \caption{\label{tab:classification}Classification of Riemannian Globally Symmetric Spaces}
% \begin{ruledtabular}
% \begin{tabular}{llll}
% Type & Lie Algebra Class & Symmetric Space & Alternative Description \\
% \hline
% I (II) & AI($n$) & $SU(n)/SO(n)$ & - \\
% I (II) & AII($2n$) & $SU(2n)/Sp(2n)$ & $SU(2n)^*/Sp(2n)$ \\
% I (II) & AIII($n,r$) & $U(n)/[U(r)\times U(n-r)]$ & $U(r,n-r)/[U(r)\times U(n-r)]$ \\
% I (II) & BDI($n,r$) & $SO(n)/[SO(r)\times SO(n-r)]$ & $SO(r,n-r)/[SO(r)\times SO(n-r)]$ \\
% I (II) & DIII($n$) & $SO(2n)/U(n)$ & $SO(2n)^*/U(n)$ \\
% I (II) & CI($n$) & $Sp(2n)/U(n)$ & $Sp(2n,\mathbb{R})/U(n)$ \\
% I (II) & CII($n,r$) & $Sp(2n)/[Sp(2r)\times Sp(2n-2r)]$ & $Sp(2r,2n-2r)/[Sp(2r)\times Sp(2n-2r)]$ \\
% III (IV) & A($n$) & $SU(n) \times SU(n) / SU(n)$ & - \\
% III (IV) & BD($n$) & $SO(n) \times SO(n) / SO(n)$ & $SO(n,\mathbb{C}) / SO(n)$ \\
% III (IV) & C($n$) & $Sp(2n) \times Sp(2n) / Sp(2n)$ & - \\
% \end{tabular}
% \end{ruledtabular}
% \end{table*}





% \section{SubRiemannian geometry}\label{sec:geo:SubRiemannian geometry}
% We now discuss subRiemannian geometry which is fundamental to the last two chapters of this work where the problem at hand is to develop techniques for time optimal synthesis in relation to subRiemmanian manifolds. SubRiemannian geometry involves a manifold $\M$ together with a distribution upon which an inner product is defined. Most of the material is drawn from Montgomery's seminal work on subRiemannian geometry \cite{montgomery_tour_2002} together with other standard source material on topic. Distribution in this context refers to a linear sub-bundle of the tangent bundle of $\M$ and corresponds to the horizontal subspace of $T\M$ discussed above and where the vertical subspace is non-null. SubRiemannian manifolds are characterised where the distribution is not the entire bundle, or in the language of Lie algebra, where for a decomposition $\g = \k \oplus \p$, we have $\p \subset \g$ rather than the identity. This means, as discussed above, the generators or vector fields $\mathfrak{X}\M$ are constrained to limited directions. A transformation not in the horiztonal distribution may be possible (as we discuss for certain subspaces where $[p,p]\subseteq k$, but in a sense these are indirect such that the geodesic paths connecting the start and end points will be longer than for a Riemannian geometry on $\M$. 

% \begin{definition}[SubRiemannian manifold and distributions]\label{defn:geo:SubRiemannian manifold}
% A subRiemannian manifold (geometry) on $\M$ consists of a distribution $\Delta$, being a [vector] sub-bundle $H_p\M \subset T\M$ together with a fibre inner product on $H_p\M$. The sub-bundle corresponds to the \textit{horizontal distribution}, having the meaning ascribed to horizontal subspace $H_p\M$ above.
% \end{definition}
%  We use the notation interchangeably throughout. A curve on $\M$ is a \textit{horizontal curve} if it is tangent to $H_p\M$. Similar to Riemannian manifolds, \textit{subRiemannian length} $\ell = \ell(\gamma)$ (for $\gamma$ smooth and horizontal) is then defined similarly as:
% \begin{align*}
%     \ell(\gamma) = \int || \dot \gamma(t) || dt
% \end{align*}
% where $||\dot \gamma(t)|| = \sqrt{\braket{\dot\gamma(t),\dot\gamma(t)}}$ computed over the horizontal subspace $H\M$. As with the Riemannian case, \textit{subRiemmanian distance} $d_S$ is defined as the infimum of all such lengths, namely $d_S(A,B) = \inf \ell(\gamma)$ of all curves connecting $A,B \in \M$. To [guarantee] that a horizontal curve has a minimal or geodesic distance, we reuqire that the curve $\gamma$ be absolutely continuous which is to say that its derivative $\dot\gamma(t) \in H_p\M$ for all $t$. In this case we can define a subRiemannian \textit{minimising geodesic} as that absolutely continuous horiztonal path that realises the distance between two points in $\M$. Sometimes we define the \textit{energy} of a horizontal curve as:
% \begin{align}
%     E(\gamma) = \int_\gamma \frac{1}{2}||\dot\gamma(t)||^2 \label{eqn:geo:energyhorizontalcurve}
% \end{align}
% as it can be more convenient to minimise this quantity rather than $\ell(\gamma)$. A horizontal curve $\gamma$ that minimises $E$ among all curves also minimises length and can be parametrised by constant speed (analogous to parametrisation by constant arc length for minimal geodesics) via $d(q_0,q_1)/T$ for $\gamma(0)=q_0, \gamma(T)=q_1 \in \M$.

% \subsubsection{SubRiemannian Geodesics}\label{sec:geo:SubRiemannian Geodesics}
% As Montgomery notes, while a Riemannian metric is defined by a covariant $(0,2)$ form. In subRiemannian geometry, the metric is defined only on a subset of the tangent space (the horizontal distribution), unlike in Riemannian geometry where it is defined over all $T_\M$. 

% Instead, it is usual for a \textit{subRiemannian metric} to be encoded as a contravariant symmetric two-tensor as a section of the bundle. We denote this the \textit{cometric} as follows:
% \begin{definition}[SubRiemannian (co)metric]\label{defn:geo:SubRiemannian (co)metric}
%     The subRiemmanian metric, or cometric, is a section of the bundle $T\M \otimes T\M$ of symmetric bilinear forms on the cotangent bundle $T^*\M$. This gives rise to a fibre-bilinear form:
%     \begin{align*}
%         \braket{\cdot,\cdot}: T^*\M \otimes T^*\M \to \R
%     \end{align*}
% \end{definition}
% The form  defines a symmetric bundle that maps $\beta: T^*\M \to T
% \M, \alpha(\beta_p(\mu)) = ((\alpha,\mu))_q$ where $\alpha,\mu \in T^*_p\M$ and $p \in \M$. Symmetric here refers to the fact that $\beta$ equals its adjoint $\beta^*$. The cometric then satisfies the conditions that $Im(\beta_p)=H_p\M$ and it considered a subRiemannian inner product $\alpha(v) = \braket{\beta_p(\alpha),v}_p$ for $v \in H_p\M$, $\alpha \in T^*\M$. From the subRiemannian metric we specify a system of Hamilton-Jacobi equations on $T^*\M$ the solution to which is a subRiemmanian geodesic.

% This subRiemannian Hamiltonian formalism can be used to define a \textit{subRiemannian Hamiltonian} given by $H(p,\alpha) = \frac{1}{2}(\alpha,\alpha)_p$ where $\alpha \in T^*\M$ and $(\cdot,\cdot)_p$ is the cometric. As Montgomery notes, $\beta$ uniquely determines the subRiemannian structure. The formalism also has its own form of Hamiltonian differential equations (see \cite{montgomery_tour_2002} Appendix A) given by $\dot x^i = \partial H\partial p_i, \dot\partial p_i = -\partial H/\partial x^i$, denoted the \textit{normal geodesic equations}. Here $x^i$ are the coordinates and $p_i$ are momenta functions for coordinate vector fields. 

% In this sense, Riemannian geometry is a special case of subRiemannian geometry where the distribution $\Delta = \g$ or the entire tangent bundle and with the cometric $g^{\mu\nu}$. As with the Riemannian case, there are equivalent existence theorems regarding minimal geodesics.
% \begin{definition}[Normal subRiemannian geodesics]\label{defn:geo:Normal subRiemannian geodesics}
%     Given a solution to the subRiemannian equations on $T^*\M$ given by $(\gamma(t),p(t))$ with $\gamma(t) \in \M$, then every sufficiently short curve segment $\gamma(t)$ is a minimising subRiemannian geodesic and $\gamma$ is the unique minimising geodesic between endpoints $\gamma(0)=q,\gamma(T)=p$. 
% \end{definition}
% Here $\gamma(t)$ is a projected curve, i.e. a curve constituted via projection onto the subRiemannian manifold. As noted in the literature, there are subRiemannian geometries for which minimal geodesics exist that are not solutions to subRiemannian Hamiltonian equations, so-called `singular' geodesics. The existence of subRiemannian geodesics and importantly the ability for curves generated by distributions $\Delta$ to effectively cover the entirety of $\M$ (thus, in a quantum information context, making any $U(t)$ in principle reachable via only the subset $\p$), relies upon braket-generating properties of $\Delta$ and Chow's theorem.
% %Bracket generating
% \begin{definition}[Bracket generating]\label{defn:geo:bracketgenerating}
%     A distribution $\Delta$ (as a collection of vector fields $\{X_i\}$ is called bracket generating if the application of the Lie derivative among all $X_i$ spans the entire tangent bundle. Equivalently, a distribution (in our case defined by a control subalgebra of the Lie algebra) $\Delta = \h \subset \g$ for a Lie algebra $\g$ is bracket generating if repeated application of the Lie derivative (commutator) (definition \ref{defn:alg:Lie algebraliederivative}) obtains the entirely of $\g$.
% \end{definition}
% By a theorem of Chow and Raschevskii (see \cite{montgomery_tour_2002}), it can be shown that if $\M$ is connected with a bracket generating distribution and complete (with respect to the subRiemannian metric), then there exists a minimising geodesic connecting any two points of $\M$. For a decomposition $\g = \k \oplus \p$, then we are interested in bracket generating control subalgebras $\p$ such that $[\p,\p]=\k$ such that we have access to the entirety of $\g$. Recall $\p$ is our horizontal subspace (distribution) $H_p \M$. 


% A subRiemannian structure on $\M$ is, as noted above, given by the sub-bundle distribution $\Delta \subseteq H_p\M$. Noting the canonical [projection] [\textbf{ref above}] $\pi_\Delta: \Delta \to \M$ being the canonical projection of the bundle with fibres at $p \in \M$ given by $\Delta_p = \pi^\inv_\Delta \subseteq H_p\M$. Assuming $\dim \Delta_p = m$, independent from the dimension of $p \in \M$. Such a setup corresponds to, in traditional control contexts, the existence of $m$ smooth vector fields $\mathfrak{X}_p = \{ X_1,...,X_m \}$ such that all points $p \in \M$ share the same distribution i.e. $\Delta_p$. We assume that $\mathfrak{X}_p$ is bracket generating such that it is the smallest $\p$ which can generate the entire $\g$. With the assumption that $\Delta_p$ is the same for all $p\in\M$, then we have that for all $p \in \M$, $\g = T_p\M$. The Riemannian metric restricted to $\Delta_p \in T_p\M$ provides a smooth, positive definite inner product for generators in $\Delta_p$. Denote this subRieammian metric $\braket{\cdot,\cdot}_S$. We assume the usual orthonormality of vectors and covectors.

% \section{Geometric control theory}\label{sec:geo:Geometric control theory}
% \subsection{Overview}
% The primary problem we are concerned with in our final two chapters is solving time optimal control problems for certain classes of Riemannian symmetric space. In our case, time optimal contorl is equivalent to finding the time-iminimising subRiemannian geodesics on a manifold $\M$ corresponding to the homogeneous symmetric space $G/K$. Our particular focus is the $KP$-problem, where $G$ admits a Cartan $KAK$ decomposition where $\g = \k \oplus \p$, with the control subalgebra (Hamiltonian) comprised of generators in $\p$. In particular such spaces exhibit the Lie triple property $[[\p,\p],\p] \subseteq \k$ given  $[\p,\p]\subseteq \k$. In such cases $\g$ remains in principle reachable, but where minimal time paths constitute subRiemannian geodesics. Such methods rely upon \textit{symmetry reduction} [\textbf{ENRIQUEZ; ALBERTINI}]. As D'Alessandro notes \cite{dalessandro_introduction_2007}, the primary problem in quantum control involving Lie groups and their Lie algebras is whether the set of reachable states $\mathcal{R}$ (defined below) for a system is the connected Lie group $G$ generated by $\mathcal{L} = \spn\{-H(u(t))\}$ for $H \in \g$ (or some subalgebra $\h \in \g$) and $u \in U$ (our control set, see below). This is manifest then in the requirement that $\mathcal{R} = \exp(\mathcal{L})$. In control theory $\mathcal{L}$ is designated the \textit{dynamical Lie algebra} and is generated by the Lie bracket (derivative) operation among generators in $H$. The dynamical addage is a reference to the time-varying control functions $u(t)$.
% %
% %
% \subsection{Geometric control preliminaries}\label{sec:geo:Geometric control preliminaries}
% Returning to horizontal curves above, we assume that such curves $\gamma: \Real \supset [0,T] \to \M$ satisfy certain usual Lipschitz continuity requirements (almost everywhere differentiable as per above). We assume \textbf{RELATE TO BANACH SPACES} that $||\dot\gamma(t)||$ is essentially bounded as follows.
% \begin{definition}[Essentially bounded]\label{defn:geo:Essentially bounded}
% A tangent $\dot\gamma(t)$ is essentially bounded where there exists a constant $N$ and mapping $H: [0,T] \to T\M, t \mapsto H(t) = \dot \gamma$ such $\braket{H(t),H(t)}_S \leq N$ for all $t \in [0,T]$.     
% \end{definition}
% This condition ensures that $H(t) = \dot\gamma(t)$ almost everywhere along the curve (which we assume to be regular $\dot\gamma \neq 0$). As discussed above, horizontal curves are then those whose tangents (generators) are in the horizontal distribution for such a curve, that is where $\dot\gamma(t) \in \Delta_{\gamma(t)}$. Recalling our vector fieds $X_j$ are differential operators on $\gamma(t)$, we can then write the curve in terms of control functions and generators.
% %curve control functions and generators
% \begin{definition}[Horizontal control curves]\label{defn:geo:Horizontal control curves}
%     Given $\gamma(t) \in \M$ with $\dot\gamma(t) \in \Delta_{\gamma} \subseteq H_p\M$, we can define horizontal control curves as:
%     \begin{align}
%         \dot\gamma(t) = \sum_j^m u_j(t) X_j(\gamma(t))
% \label{eqn:geo:horizontalcurves}
%     \end{align}
%     where $u_j$ are the control functions given by:
%     \begin{align}
%         u_j(t) = \braket{X_j(\gamma(t)),\dot\gamma(t)} \label{eqn:geo:controlshorizontal}
%     \end{align}
% \end{definition}
% The boundedness of $\dot\gamma(t)$ sets an overal bound on $u_j(t)$. Following above [\textbf{REF}], the length of a horizontal curve is given by:
% \begin{align}
%     \ell(\gamma) = \int_0^T ||\dot \gamma(t)|| dt =  \int_0^T \sqrt{\braket{\dot\gamma(t),\dot\gamma(t)}} dt = \int_0^T \sqrt{\sum_j^m u^2_j(t)} dt \label{eqn:arclengthparamby}
% \end{align}
% When $[0,T]$ is normalised this is equivalent to parametrisation by arclength. As noted in \cite{albertini_symmetries_2018}, the consequence of the Chow-Raschevskii theorem, $\M$ being connected and $\mathfrak{X}$ being bracket generating renders $(M,d)$ a (subRiemannian) metric space where $d_S$ is the subRiemannian distance function.

% \subsection{Time optimal control}\label{sec:geo:Time optimal control}
% For subRiemmanian and Riemannian manifolds, the problem addressed in our final two chapters in particular is, for a given target unitary $U_T \in G$, how to identify the minimal time for and Hamiltonian to generate a minimal geodesic curve such that $\gamma(0)=U_0$ and $\gamma(T)=U_T$ for $\gamma:[0,T] \to \M$. This is described \cite{albertini_symmetries_2018} as the \textit{minimum time optimal control problem} \cite{jurdjevic_geometric_1997}. In principle, the problem is based upon the two equivalent statements (a) $\gamma$ is a minimal subRiemmanian (normal) geodesic between $U_0$ and $U_T$ parametrised by constant speed (arc length); and (b) $\gamma$ is a minimum time trajectory subject to $||\vec u|| \leq L$ almost everywhere (where $u$ stands in for the set of controls via control vector $\vec u$). SubRiemannian minimising geodesics starting from $q_0$ to $q_1$ (our $U_T$) subject to bounded speed $L$ describe \textit{optimal synthesis} on $\M$. We now discus two loci of geodesics related to their optimality.
% \begin{enumerate}[(i)]
%     \item \textit{Critical locus} ($CR(\M)$) being the set of points where minimising geodesics are not optimal. This is defined such that for $p \in CR(\M)$, the horizontal curve $\gamma$ is a minimising geodesic for all points $t \in [0,T]$ but not for infinitesimally extended interval $[0,T+\epsilon]$, the set of such points being \textit{critical points}; and
%     \item \textit{Cut locus} $(CL(\M))$ being the set of points $p \in \M$ reached by more than one minimising geodesic $(\gamma_i,\gamma_j)$ over $t \in [0,T]$, where at least one is optimal (such points $p \in \M$ then being \textit{cut points}).
% \end{enumerate}
% When minimising $\gamma$ are analytic functions of $t \in [0,\infty)$ i.e. $CL(\M) \subseteq CR(\M)$, then cut points are critical points. An important concept with a geometric framing and one drawn from control theory is that of a reachable set.
% %reachable set definition
% \begin{definition}[Reachable set]\label{defn:geo:Reachable set}
%     The set of all points $p \in \M$ such that, for $\gamma(t): [0,T] \to \M$ there exists a bounded function $\vec u, ||\vec u||\leq L$ where $\gamma(0)=q_0$ and $\gamma(T) = p$ is called the reachable set and is denoted $\mathcal{R}(T)$.
% \end{definition}
% Note for reachable sets under usual assumptions we have $T_1 \leq T_2$ implies $\mathcal{R}(T_1) \subseteq \mathcal{R}(T_2)$. For optimal trajectories, $p = \gamma(T)$ belong on teh boundary of $\mathcal{R}(T)$. In general, targets are in $\M/G$ the space of equivalence class of orbits of $[p]$. For our particular case, we assume that $G=\M$. For convenience and notational efficiency we denote by $g \in G$ the relevant group diffeomorphisms of $\M$. We also make reasonable assumptions about the existence of a minimal orbit type and that for points on the same orbit $q_2 = g q_1$, then one can transition between minimising geodesics parametrised by constant speed $L$ via the group action $\gamma_1 = g \gamma_2$, which effectively pushes $\gamma$ around the orbit while satisfying time optimality.  

% \subsection{Variational methods} \label{sec:geo:variational methods}
% Of fundamental importance to optimal control solutions (in geometric and other cases) is the application of variational calculus in terms of Euler-Lagrange, Hamiltonian and control optimisation formalism. We follow Jurdjevic's geometric framing of the Pontryagin maximum principle (PMP) (see \cite{jurdjevic_geometric_1997}, Chapter 11). The maximum principle represents an extension of techniques developed by Weierstrass and others, with a particular focus on optimality conditions and the distinction between `weak' (Euler-Lagrangian) and `strong' (PMP) minima. In essence the PMP represents the application of variational techniques tailored for optimal control.

% \subsubsection{Pontryagin Maximum Principle}\label{sec:geo:Pontryagin Maximum Principle}
% Consider as our differentiable manifold $\M \sim \R^n$ on which we define $\cinfm$ functions $(f_1(\gamma,u),...,f_m(\gamma,u))$ where our coordinate charts $\phi \in S \subset \R^n$ parametrise curves $\gamma(t) \in \M$ (i.e. such that $\phi_i(t) \simeq \dot\gamma(t)$). We have as our control variable $u \in U \subset \R^m$ where $U$ is our control set. Both are parametrised as $u=u(t),\gamma=\gamma(t)$ for $t \in I = [t_0,t_1]$ (assuming boundedness and measurability). The evolution of $\gamma \in \M$ is determined by the state and the control, according to the differential equation. We have:
% \begin{align}
%     \dot\gamma_i(t) = f_i(\gamma(t),u(t)) \label{eqn:geo:pontrydotgamma}
% \end{align}
% for almost all $t \in I$. Solution curves $\gamma(t)$ can in typical circumstances be regarded as unique.  The classical PMP approach then posits a \textit{variational equation} such that for the integral curve $\gamma(t)$, which expresses how small variations in the initial conditions of a dynamical system affect its evolution. For a solution curve $\gamma(t)$, the matrix:
% \begin{align}
%     A_{ij}(t) = \frac{\partial f_i}{\partial \gamma_j}(\gamma(t),u(t))
% \end{align}
% expresses how the vector field (whose components are $f_i)$ changes around $\gamma(t)$. The \textit{variational system} along the curve $\gamma(t), u(t)$ is then:
% \begin{align}
%     \frac{dv_i}{dt}=\sum_j^n A_{ij}(t)v_j(t)
% \end{align}
% a set of differential equations describing the evolution of a small perturbation (i.e. a variation) of $\gamma(t)$ by $v(t)$. The solution to $v(t)$ describes how sensistive the system is to such perturbations over time and thus how stable it is. Related to the variational system is the \textit{adjoint system} a set of differential equations for optimality with respect to $p(t)$:
% \begin{align}
%     \frac{dp_i}{dt} = -\sum_j^n p_j A_{ji}(t) \label{eqn:geo:pontryadjointsystem}
% \end{align}
% Solutions to equation (\ref{eqn:geo:pontryadjointsystem}) allow construction of the time optimal Hamiltonian. Solutions $\gamma(t),v(t)$ satisfy:
% \begin{align}
% \sum_{i=1}^{n} p_i(t) v_i(t) = c,
% \end{align}
% for some constant $c$, such that the solutions have a constant inner product over time, constituting level sets in their applicable phase space. The systems can be expressed via the Hamiltonian as a function of $\gamma, p$ and $u$ as follows:
% \begin{align}
%     H(\gamma, p, u) &= p_0 f_0(\gamma, u) + \sum_{i=1}^{n} p_i f_i(\gamma, u) \label{eqn:geo:PMPHamiltonian}
% \end{align}
% with:
% \begin{align}
% \frac{d\gamma_i}{dt} &= \frac{\partial H}{\partial p_i}(\gamma(t), p(t), u(t)) = f_i(\gamma(t),u(t)) \\
% \frac{dp_i}{dt} &= -\frac{\partial H}{\partial \gamma_i}(\gamma(t), p(t), u(t)) = \sum_j^n p_j \frac{\partial f_i}{\partial x_i}(\gamma(t),u(t)) \label{eqn:geo:pontryHamiltonianequations}
% \end{align}
% Note that $f_0(\gamma(t),u(t))$ is the function we seek to minimise (hence $p_0 \leq 0$ below) while costates $p_i$ act as in effect Lagrange multiplier terms such that $f_i$ represent the rate of cost for exerting control $u(t)$ given state $\gamma(t)$
% Optimisation is then expressed in terms of a \text {cost functional} which quantifies the evolution along the curve from points $p(t_0)$ to $p(t_1)$ in $S \in \M$:
% \begin{align*}
%     C(u) = \int_{t_0}^{t_1} f_0(\gamma(t), u(t)) dt \label{eqn:geo:costfunctional}
% \end{align*}
% where $(\gamma(t),u(t))$ is denoted a \textit{trajectory} and $C(u)$ the cost function. A trajectory is \textit{optimal} relative to $\gamma(t_0)=a,\gamma(t_1)=b$ if it is the minimal cost among all trajectory costs from $a$ to $b$. Note that the cost function involves $f_0$. The optimal control problem is then constituted by finding an optimal trajectory. The PMP then specifies necessary conditions that any optimal trajectory must satisfy. From this, we have the concept of the \textit{maximal Hamiltonian} $H_M$ associated with an integral curve $(\gamma(t),p(t),u(t))$:
% \begin{align}
%     H_M(\gamma(t),p(t)) = \sup_{u\in U}H(\gamma(t),p(t),u(t))
% \end{align}
% The PMP transforms the problem of minimising $C(u)$ into one of Hamiltonian maximisation. It does so by the introduction of the costate variables $p(t)$ which are analogous to Lagrange multipliers, enabling inclusion of system dynamics in the optimisation. Thus the Hamiltonian is defined to include the dynamics and cost function with co-state variables. In essence it assumes an optimal minimum length given by the cost $p_0f_0(\gamma,u)$ term which is negative and then adds to the Hamiltonian the $\sum_i p_i f_i(\gamma,u)$ representing the additional energy or cost from the controls. The condition for optimality is that the time-optimal curve and controls $(\gamma,u)$ will be such that (a) at any point in time, the Hamiltonian 

% \begin{definition}[Pontryagin maximum principle]\label{defn:geo:Pontryagin maximum principle}
%     The maximum principle for solving the optimal control problem provides that for a trajectory $(\gamma(t),u(t))$ evolving from $a \to b$ over interval $t \in I=[0,T]$, there exists a non-zeo absolutely continuous cirve $p(t)$ on $I$ satisfying:
%     \begin{enumerate}[(i)]
%         \item $(\gamma(t),p(t),u(t))$ is a solution curve to the Hamiltonian equations (\ref{eqn:geo:pontryHamiltonianequations}).
%         \item $H(x(t), p(t), u(t)) = H_M(x(t), p(t))$ for almost all $t \in [0, T]$; and
%     \item $p_0(T) \leq 0$ and $H_M(x(T), p(T)) = 0$.
%     \end{enumerate}
% \end{definition}

% %PMP and quantum control
% \subsubsection{PMP and quantum control}\label{sec:geo:PMP and quantum control}
% Following \cite{dalessandro_introduction_2007,jurdjevic_geometric_1997}, typical quantum control problems are fundamentally  take one of three forms: (a) the problem of Mayer (where $C(u) = C(\gamma(T),T)$, (b) Lagrange where $C(u) = \int_0^T L(\gamma(t), u(t), t), dt$ where $C_T$ denotes some cost functional for time $T$, combined into a more general Bolza form:
% \begin{align}
%     C(u) = C_T(\gamma(T),T) + \int_0^T L(\gamma(t), u(t), t) dt \label{eqn:geo:PMPBolzaloss}
% \end{align}
% subject to the constraint imposed by the Schr\"odinger equation \ref{eqn:quant:schrodingersequation}). Both the Hamiltonian and unitary target $U$ are complex-valued, however they can be represented in real values via the mapping $\C^n \to \R^{n^2}$. For the optimal solution, one assumes the existence of a set of optimal controls $u_j(t)$ which may be unknown and replaces them with a control approximating $u$, given by $u^\epsilon$. The cost function is then:
% \begin{align}
%     C(u^\epsilon) - C(u) \geq 0
% \end{align}
% Following this, there are then two types of variation condition, known as \textit{strong variation} and \textit{weak variation} describing how varied the choice of $u^\epsilon$ is from the true $u$, which can be used to optimise. The PMP problem above is based upon a \textit{strong variation} then involves assumptions about how much $u^\epsilon$ varies over intervals. One assumes that for $\tau \in (0,T]$:
% \begin{align}u^\epsilon =
%       \begin{cases}
%       u & \text{if }t \in [0,\tau - \epsilon] \&  (\tau-\epsilon,\tau]\\
%       v & t \in (\tau,T]    
%       \end{cases}\label{eqn:geo:PMPtimes}
% \end{align}
% where $v$ is any value in the admissible control set $U \in \R^m$. In this context, the PMP is then expressed as that assuming $u(t)$ as the optimal control and $\gamma(t)$ as a solution equation (\ref{eqn:geo:pontrydotgamma}) in the form of Schr\"odinger's equation exist, there exists a non-zero (vector) solution to the adjoint equations and terminal equation at $T$:
% \begin{align}
%     \dot p^T = -p^T f_i(\gamma(t),u(t)) \qquad p^T(T)=-\phi_\gamma(\gamma(T))
% \end{align}
% where for all $\tau \in (0,T]$:
% \begin{align}
%     p^T(\tau)f(\gamma(\tau),u(\tau) \geq p^T(\tau)f(\gamma(\tau),u(\tau)
% \end{align}
% Practically speaking the PMP in quantum contexts, the following procedure is used. First we define the Hamiltonian (equation (\ref{eqn:geo:pontryHamiltonianequations})). For each state $\gamma$ and costate $p$, we maximise the Hamiltonian over $u \in U$ such that:
% \begin{align}
%     H(p,\gamma,u) \geq H(p,\gamma,v) \label{eqn:geo:PMPHgeqH}
% \end{align}
% recalling $v$ is determined as per equation (\ref{eqn:geo:PMPtimes}). The solutions to this maximisation problem enable us to write $u = u(\gamma,p)$ i.e. as a function of the state and costate. We can convert the general loss (equation (\ref{eqn:geo:PMPBolzaloss})) into a `Mayer form' via expressing $\phi$ as a function of $\gamma$ and the [loss Lagrangian] $L$. In this case, the differential equations (\ref{eqn:geo:pontryHamiltonianequations}) then become:
% \begin{align}
% p_i^\T = -p_i^T f_i(\gamma_i,u(\gamma_i,p_i) - \mu L \qquad \dot \mu = 0
% \end{align}
% with boundary conditions that $\gamma(0)=\gamma_0$ (and that $p^T(T)=-\phi_\gamma(\gamma(T))$. Controls that satisfy these conditions are denoted \textit{extremal}. The Hamiltonian then is written as follows as a function of the controls:
% \begin{align}
%     H(p,\gamma,u) &= p^T f(\gamma,u) - L(\gamma,u)\\
%     &=p^T H(u)\gamma - L(\gamma,u)\\
%     &=H(u)p + L(\gamma,u) \qquad \text{(by skew-symmetry)}
% \end{align}
% with adjoint equations:
% \begin{align}
%     \dot p^T = -p^T H(u) _ L^T \qquad p(T) = -\phi^T(\gamma(T))
% \end{align}
% For a typical qubit control problem where $H \in \g = \su(2)$ for final state target $U_f \in G=$ SU(2), with Pauli generators $\sigma_j$ where $H=\sum_j u_j(t) \sigma_j$. The cost function is then of the form:
% \begin{align}
%     J(u_j) = Re(U^\dagger(T)U_f) + \eta \int_0^T \sum_j u_j(t)\sigma_j dt
% \end{align}
% It can be shown (see \cite{dalessandro_introduction_2007} $\S 6$) that the optimal controls are then of the form:
% \begin{align}
%     u_j(t) = A \cos(\omega t + B)
% \end{align}
% where $A,\omega$ and $B$ are free parameters which can be determined through a minimisation procedure. As noted in the literature, the solutions to the PMP equations are extremal curves such that the trajectories $\gamma(t)$ can be said to reside on the boundary of the reachable set $\mathcal{R}$. Solving the PMP can be challenging. One class of tractable problems is when the targets $U_T \in G$ belong to a Riemannian symmetric space where the symmetry properties of the related Cartan decomposition can, in certain cases, allow the control solutions $u_j$ to be found in closed form. This is the main focus of our final Chapter. In Chapter \ref{chapter:Quantum Geometric Machine Learning}, we also discuss and examine the work of Nielsen et al. and others on geometric quantum control \cite{gu_quantum_2008,dowling_geometry_2008,nielsen_geometric_2006} where minimisation of paths on corresponding Lie group SU($2^n$) manifolds is related to obtaining minimum bounds on circuit complexity (a research programme built upon in later work by Brown and Susskind \cite{brown_complexity_2019,lin_complexity_2020}).


% %=========CONTROL AND LIE GROUPS
% \subsection{Time optimal problems with Lie groups}\label{sec:geo:Time optimal problems with Lie groups}
% In this section, we examine the general variational problem above framed in terms of the geometric and algebraic formalism of Lie groups. For optimal control problems involving Lie groups draws upon the theory of Hamilton systems, anchored in the fact the cotagnent bundle of $G$ corresponds to the product of $G$ and the dual of $\g$, i.e. the symplectic structure $T*G = G \times L^*$. As Jurdjevic notes \cite{jurdjevic_geometric_1997}, for variational problems exhibiting left or right-invariant symmetries, projecting Hamilton's equations onto $L^*$ accounts for the conservation laws arising from the structure of $G$. \hl{\textbf{ALSO CHECK HALL ON THIS}}. Hamiltonians are then exprssed as arbitrary functions on $T*G$. In this setting, we regard Hamiltonians of left-invariant vector fields are linear functions on $L^*$, while right-invariant vector fields depend on $G \times l^*$

% \subsubsection{PMP for Lie Groups}\label{sec:geo:PMP for Lie Groups}
% We now summarise the PMP principle applied to Lie groups, following standard presentations in \cite{sachkov_control_2009,jurdjevic_geometric_1997} in particular. Frame the optimal control problem as follows:
% \begin{align}
%     \dot \gamma(t) &= f(\gamma,u) &\gamma(t) &\in \M &u \in U \subset \R^m\\
%     \gamma(0) &= p &\gamma(T)&=q\\
%     C(u)&=\min_{u}\int_0^T \varphi(\gamma(t),u(t)) dt
% \end{align}
% where $f,\varphi \in \cinfm$ and controls $u(t)$ are measurable and locally bounded. Recall that $v \in T_q\M$ can be decomposed in the dual basis as $v=\sum_i^n x_i dx^i$ such that the $2n$-tuple $(x_1,...,x_n; dx_1,...,dx_n)$ forms a set of canonical coordinates for the cotangent bundle $T^*\M$. Assume canonical projects $\pi:T^*\M \to \M$.

% \subsubsection{Dynamical Lie algebras}\label{sec:geo:Dynamical Lie algebras}
% Other approaches use the language of \textit{dynamical Lie algebras} defined by the criterion that:
% \begin{align}
%     \mathcal{R} = \exp(\h) \label{eqn:geo:liealgebracontrollable}
% \end{align}
% for some Lie algebra $\h$ where $\h = \spn\{ -iH(u(t))\}$. `Dynamical' here refers to the fact that $\h$ is composed of generators multiplied by control functions $u(t)$ which are time-dependent and thus dynamic. Such a condition is equivalent to complete controllability, namely that every $U_T \in G$ is obtainable via a particular sequence of controls $u(t)$. The condition relies upon the bracket-generating characteristics of $\h$ (see definition \ref{defn:geo:bracketgenerating}) to recover the full Lie algebra $\g$. In some literature \cite{dalessandro_introduction_2007}, the number of applications of the commutator in order to obtain $\g$ is denoted the \textit{depth} of the bracket. Moreover, the condition in equation (\ref{eqn:geo:liealgebracontrollable}) relies upon the fact that $\exp(\h) \subset G$ and that $G$ is compact. This is an important point: in our final chapter (and in subRiemannian geometric control problems generally) admitting a Cartan decomposition $\g = \k \oplus \p$, the isometry group $\exp(\k)$ is not compact (as $[\k,\k] \subseteq \k$. One cannot reach arbitrary states (limits) in $\p$. However, symmetric spaces admitting such a decomposition exhibit the Lie triple property with respect to $\p$, namely that $[\p,[\p,\p]] \subset \k$ where $[\p,\p] \subseteq \k$, which is a necessary requirement. Controllability is sometimes segmented into three types: (a) \textit{pure state controllable}, where for $U(0),U(T) \in G$, there exist controls $\{ u_j(t) \}$ rendering both reachable; (b) \textit{equivalent state controllable}, where $\{ u_j(t) \}$ exist to reach $U_1(T)$ upt to some phase factor $\phi$ such that $U(T) = \exp(i\phi)U_1(T)$; and (c) \textit{density-matrix controllable} such that there exist controls $\{ u_j(t) \}$ enabling $\rho_i \to \rho_k$ for all $\rho_i.\rho_k \in \mathcal{B}(\Hilb)$ (i.e. any state is reachable from any other). 

% Recall from equation (\ref{eqn:alg:cartankakandpk}) that $U \in G$ can be decomposed as either the product of group elements in $P,K$ or via the $KAK$ decomposition. 
% %
% %
% %
% \\
% \\
% \subsubsection{Symplectic manifolds and Hamiltonian flow}\label{sec:geo:Symplectic manifolds and Hamiltonian flow}
% \hl{Note relation of symplectic manifolds to phase space and quantum recurrence} We can express the above in terms of symplectic manifolds and Hamiltonians which elucidates the deep connection between Hamiltonian dynamics and the geometric formalism above. Given a control system defined on $\M$, the Hamiltonian can be represented as a map $H:T^*\M \to \R$ which generates a flow (see definition \ref{sec:geo:Local flows}) on the cotangent bundle which represents the phase space of the quantum system (as we discuss below). As discussed below (definition \ref{defn:geo:Hamiltonian vector field}), one forms define a Hamiltonian vector field associated with the Hamiltonian

% As Hall \cite{hall_quantum_2013} notes, intuitively a symplectic manifold $\M$ is one with sufficient structure to define the Poisson bracket of two functions $f_1,f_2 \in \cinfm$ on it.
% \begin{definition}[Symplectic manifold]
% A symplectic manifold is a smooth differentiable manifold equipped with a non-degenerate $(0,2)$-form $\omega$ on $\M$.  
% \end{definition}
% Symplectic manifolds are even dimensional as odd-dimensional bundles cannot be equipped with non-degenerate skew bilinear forms. Thus we assume $\M$ is of dimension $2n$ for convenience. As noted in the literature, it can be shown that the cotangent bundle $T^*\M$ of any manifold has the structure of a symplectic manifold. Given a coordinate system $x_i$ then, as per our discussion above, we can represent an element in $T_p^*\M$ as $\phi = X^j dx_j$ with $p_j$ the coordinate functions in $\R$. Recall that $\pi^\inv: M \to T^*M$. 

% Define a one-form $\theta(X) = \phi(\pi^*(X))$ sometimes denoted the \textit{tautological one-form} (so called because it returns the value of $\theta$ acting on tangent vectors at $p$). Define a (0,2)-form via the [\hl{exterior product}] $\omega = d\theta = dp_j \wedge dx_j$. As discussed above, the non-degeneracy of $\omega$ allows the identifiaction of $T_p\M$ with $T^*_p\M$. The two-form $\omega$ also has a corresponding dual defined on $T^*\M$ (taking duals as its arguments) given by $\omega^\inv: T^*\M \times T^*\M \to \R$. Then, given $f,g \in \cinfm$, we can define the Poisson bracket in differential formalism as:
% \begin{align}
%     \{f,g\} = -\omega^\inv(df,dg) \label{eqn:geo:symplecticomegapoisson}
% \end{align}
% which anti-commutes $\{g,f\} + \{f,g\}=0$ with $\{f,gh\} = \{f,g\}h+ g\{f,h\}$. The term $\omega^\inv$ is taken from Hall \cite{hall_quantum_2013} an denotes the bilnear form on $T^*\M$ that arises by way of the canonical identification of $T^*\M$ with $T\M$ if $\omega$ is non-degenerate. With these identifications and in particular the isomorphism describe dabove, we can define the \textit{Hamiltonian vector field} as follows.
% \begin{definition}[Hamiltonian vector field]\label{defn:geo:Hamiltonian vector field}
%     For $f \in \cinfm$, we denote $X_f \in T\M$ the Hamiltonian vector field associated to $f$ if:
%     \begin{align}
%         df = w(X_f,\cdot)
%     \end{align}
%     where $X_f$ corresponds to $df$ under such isomorphism given by $\omega$.
% \end{definition}
% In this case, we can relate such Hamiltonian vector field to the Poisson bracket via:
% \begin{align}
%     X_f(g) = \{f,g\} = -X_g(f) \qquad \omega(X_f,X_g) = -\{f,g\}
% \end{align}
% for $f,g \in \cinfm$. Thus conceptually we  connect vector fields to Poisson brackets in Hamiltonian formalism. We then define the \textit{Hamiltonian flow} generated by $f$, as a local flow $\varphi^f$ being the local flow generated by $-X_f$, such flow preserving $\omega$, expressed via $L_{X_f}\omega = 0$. 

% We then have that $f,g,h \in \cinfm$ form a Lie algebra under the Poisson bracket satisfying the Jacobi equation, which in turn allows us to transition from the Poisson bracket to the commutator via:
% \begin{align}
%     [X_f,X_g] = X_{\{f,g\}} \label{eqn:geo:commutatorpoisson}
% \end{align}
% For the flow $\varphi$ generated by $-X$ on $\M$, if $\varphi$ preserves $\omega$ then we can represent $X = X_f$. In this case, we can assert that the flow is locally (or, if applicable to all $\M$, globally) Hamiltonian. We then have the concept of a \textit{Hamiltonian generator} where $\varphi = \varphi^f$ \hl{CHECK}. As Hall notes \cite{hall_quantum_2013}, any smooth function on a symplectic manifold $\M$ generates a Hamiltonian flow. We can then define the familiar Hamiltonian $H$ defined on $T*\M$. We then obtain the definition of a Hamiltonian and Hamiltonian system in such geometric terms.
% %Hamiltonian systems and Hamiltonians
% \begin{definition}[Hamiltonian systems and Hamiltonians]\label{eqn:geo:Hamiltonian systemsandHamiltonians}
%     A Hamiltonian system on a symplectic manifold $\M=T^*\M$ is a tuple $(\M, \Phi^H)$ where $\Phi^H$ represents the Hamiltonian flow generated by the Hamiltonian $H$ on $\M$. Conserved quantities for the Hamiltonian system are represented by functions $f$ such that $f(\Phi^H(v))$ is independent of $t$ for each $v \in \M$ 
% \begin{align}
% \frac{d}{dt} f(\Phi^H_t(z)) = \{ f, H \}(\Phi^H_t(z)),
% \end{align}
% for all $z \in N$, or, more concisely,
% \begin{align}
% \frac{df}{dt} = \{ f, H \}.
% \end{align}
% The functions $f$ are conserved quantities if and only if $\{ f, H \} = 0$.
% \end{definition}
% The fundamental structure of a symplectic manifold $\mathcal{M}$ is the non-degenerate closed 2-form $\omega$, which provides a way to measure the "volume" of phase space regions and defines the Poisson bracket operation crucial for the dynamics.

% While $H$ dictates the flow or vector field on this manifold by determining the direction and rate of change of $U \in \M$. \\
% We briefly connect to the formulation of Hamiltonians, as the generator of time translations, in terms of controls $u_j(t)$ and generators in $\g$. The Hamiltonian determines a Hamiltonian vector field on the symplectic manifold $T^*\M$ (the cotangent bundle of $\M$). The $(0,2)$-symplectic form $\omega$ encodes information about the evolution of $\gamma(t) \in \M$ as shown in equation (\ref{eqn:geo:symplecticomegapoisson}) which shows that Hamilton's equations [\textbf{FIX}].  


% % \subsection{TEMP}
% % \subsubsection{Symplectic manifolds and Hamiltonian flow}

% % The material presented above can be further illuminated through the language of symplectic manifolds and Hamiltonian dynamics. As articulated in \cite{hall_quantum_2013}, a symplectic manifold $\mathcal{M}$ is a structure that inherently possesses the necessary elements to define the Poisson bracket of two functions $f_1, f_2 \in C^{\infty}(\mathcal{M})$.

% % \begin{definition}[Symplectic manifold]
% %     A symplectic manifold is a smooth, differentiable manifold endowed with a non-degenerate, closed $(0,2)$-form $\omega$, known as the symplectic form. This form provides the framework for the Poisson bracket structure and Hamiltonian dynamics.
% % \end{definition}

% % Typically, symplectic manifolds are of even dimension, as it is a requisite for the existence of non-degenerate skew-symmetric bilinear forms. Thus, we may consider $\mathcal{M}$ to be of dimension $2n$. It is well-established that the cotangent bundle $T^*\mathcal{M}$ of any manifold $\mathcal{M}$ inherits the structure of a symplectic manifold. 

% % If we consider a coordinate system $(x^i)$ on $\mathcal{M}$, an element of $T_p^*\mathcal{M}$ can be represented as $\phi = p_j \mathrm{d}x^j$, with $p_j$ as the coordinate functions in $\mathbb{R}^n$. Here, the canonical projection $\pi: T^*\mathcal{M} \rightarrow \mathcal{M}$ allows us to map elements of the cotangent bundle to the manifold itself. Given a one-form $\theta$ on $T^*\mathcal{M}$, we can construct a $(0,2)$-form by taking the exterior derivative $\omega = \mathrm{d}\theta = \mathrm{d}p_j \wedge \mathrm{d}x^j$.

% % The symplectic form $\omega$ is non-degenerate, enabling the identification of the tangent and cotangent spaces at each point of $\mathcal{M}$. For two functions $f,g \in C^{\infty}(\mathcal{M})$, the Poisson bracket can be expressed in this differential framework as
% % \begin{align}
% %     \{f,g\} = -\omega^{\sharp}(\mathrm{d}f, \mathrm{d}g),
% % \end{align}
% % where $\omega^{\sharp}$ is the musical isomorphism associated with $\omega$, mapping covector fields to vector fields.

% % The \textit{Hamiltonian vector field} $X_f$ corresponding to a function $f$ on $\mathcal{M}$ is then defined such that
% % \begin{align}
% %     \mathrm{d}f = \iota_{X_f} \omega,
% % \end{align}
% % where $\iota$ denotes the interior product. This association between vector fields and Poisson brackets within the Hamiltonian framework is crucial. The \textit{Hamiltonian flow} generated by $f$ preserves the symplectic structure, as indicated by the condition $L_{X_f}\omega = 0$, where $L$ denotes the Lie derivative.

% % Furthermore, for $f,g,h \in C^{\infty}(\mathcal{M})$, we find that they form a Lie algebra under the Poisson bracket, satisfying the Jacobi identity. This relationship is mirrored in the commutator of the associated Hamiltonian vector fields, given by
% % \begin{align}
% %     [X_f,X_g] = X_{\{f,g\}}.
% % \end{align}

% % For a flow $\varphi$ on $\mathcal{M}$ generated by the vector field $-X$, the preservation of the symplectic form $\omega$ implies that the flow is locally (and globally if the manifold is simply connected) Hamiltonian. In such cases, $\varphi$ is referred to as the Hamiltonian flow associated with the Hamiltonian generator $f$, or $\varphi = \varphi^f$. As noted by Hall, any smooth function on a symplectic manifold generates a Hamiltonian flow, a fact that lies at the heart of Hamiltonian mechanics.


% \subsection{KP Problems}\label{sec:geo:KP Problems}
% A particular type of subRiemannian optimal control problem with which we are concerned in the final chapter is the $KP$-problem. In control theory settings, the problem was articulated in particular via Jurdjevic's extensive work on geometric control \cite{jurdjevic_abstract_1970,jurdjevic_control_1972,jurdjevic_control_1981,jurdjevic_controllability_1978}, drawing on the work of [\textbf{Brockett} \cite{brockett_sub-riemannian_nodate} as particularly set out in \cite{jurdjevic_geometric_1997} and \cite{jurdjevic_hamiltonian_2001}. Later work building on Jurdjevic's contribution includes that of Boscain \cite{boscain_introduction_2021,boscain_k_2002,boscain_invariant_2008}, D'Alessandro \cite{dalessandro_introduction_2007,dalessandro_k-p_2019} and others. $KP$ problems are also the focus of a range of classical and control problems focused on the application of Cartan decompositions of target manifolds $G=K \oplus P$, such as in nuclear magnetic resonance \cite{khaneja_time_2001} and others (see our final chapter). The essence of the $KP$-problem is where $\M$ corresponds to a semi-simple Lie group $G$ together with right-invariant vector fields $\mathfrak{X}$ equivalent to the corresponding Lie algebra $\g$. In this formulation, the Lie group and Lie algebra can be decomposed according to a Cartan decomposition (definition \ref{defn:alg:cartandecomposition}) which is, recalling equation:
% \begin{align*}
%     \g = \k \oplus \p
% \end{align*}
% together with the Cartan commutation relations (Lie triple):
% \begin{align*}
%     [\k,\k] \subseteq \k \qquad [\k,\p] \subseteq \p \qquad [\p,\p] \subseteq \k
% \end{align*}
% and equipped with a Killing form (definition \ref{defn:alg:Killing form}) which defines an implicit positive definite bilinear form $(X,Y)$ which in turn allows us to define a Riemannian metric restricted to $G/K$ in terms of the Killing form. Thus for our purposes, we understand the $KP$ problem as a minimum time problem for a subRiemannian symmetric space $G/K$. 

% \subsection{SubRiemannian control and symmetric spaces}\label{sec:geo:SubRiemannian control and symmetric spaces}
% Assume our target groups are connected matrix Lie groups (definition \ref{defn:alg:connected_matrix_lie_group}). Recall equation (\ref{eqn:geo:horizontalcurves}) can be expressed as:
% \begin{align}
%     \dot\gamma(t) = \sum_j X_j(\gamma) u_j(t)
% \end{align}
% where $X_j \in \Delta = \p$, our control subalgebra. For the $KP$-problem, we can situate $\gamma(0) = 1 \in \M$ (at the identity) $||\hat u|| \leq L$, [in turn specifying] a reachable set $\mathcal{R}(T)$.  As D'Alessandro et al. \cite{albertini_symmetries_2018,dalessandro_time-optimal_2020} note, reachable sets for $KP$-problems admit reachable sets for a larger class of problems. Connecting with the language of control, we can frame equation (\ref{eqn:geo:horizontalcurves}) in terms of \textit{drift} and \textit{control} parts with:
% \begin{align}
%     \dot\gamma(t) = A \gamma(t) + \sum_j X_j(\gamma_j) u_j(t) \label{eqn:geo:horizontalcontroSchrod}
% \end{align}
% where $A\gamma(t)$ represents a drift term for $A \in \k$. Our unitary target in $G$ can be expressed as:
% \begin{align}
%     \dot \gamma(t) = \sum_j \exp(-At)X_j\exp(A t) \gamma(t) u_j
%     \label{eqn:geo:dotU=sumjKAKdal}
% \end{align}
% for bounded $||A_p|| = L$. For the $KP$ problem, the PMP equations are integrable. One of Jurdjevic's many conributions was to show that in such $KP$ problem contexts, optimal control for $\vec u$ is related to the fact that there exists $A_k \in \k$ and $A_p \in \p$ such that:
% \begin{align}
%     \sum_j^m X_j u_j(t) = \exp(At)X_j\exp(-A t)
% \end{align}

% Following Jurdjevic's solution  \cite{jurdjevic_hamiltonian_2001} (see also \cite{albertini_symmetries_2018}), optimal pathways are given by:
% \begin{align}
%     \dot\gamma(t) &= \exp(A_kt)A_p\exp(-A_k t) \gamma(t) \qquad \gamma(0)=1 \\
%     \gamma(t) &= \exp(-A_k t) \exp((A_k + A_p)t)
% \end{align}
% resulting in analytic curves. As we explore in our final chapter and as noted in the literature, one can select $A_p \in \a \subset \p$ where $\a$ is the non-compact part of a maximally abelian Cartan subalgebra in $\p$. In this regard, we see conjugation of a Cartan subalebra element by elements of $K$, reminiscent of the $KAK$ decomposition itself. It is also worth noting that $\a$ being a maximal subalgebra means that equation (\ref{eqn:geo:dotU=sumjKAKdal}) is invariant under the action of $K \in \k$, reflected in the commutation relation $[\k,\p] \subseteq \p$. Albertini et al. \cite{albertini_symmetries_2018} note that for $\gamma(t) \notin CL(\M)$ with $H$ the isotropy group of $\gamma$ then the tuple $(A_k,A_p)$ minising the geodesic is invariant under the action of $h \in H$. This gives rise to a general method for time optimal $KP$ control problems set out in \cite{albertini_symmetries_2018}: (i) identify the symmetry group of the problem, (ii) specify $G/K$, (iii) find boundaries of $\mathcal{R}$ (which may require numerical solution), (iv) find the first value of $t$ such that $\pi(\gamma(t)) \in \pi(\mathcal{R})$ and (v) identifying the orbit space within which the optimal control exists and then moving within an orbit to the final target $U_T = \gamma(T)$. We draw the reader's attention to work of Jurdjevic \cite{jurdjevic_optimal_1999,jurdjevic_geometric_1997} for discussion and in particular D'Alessandro \cite{dalessandro_introduction_2007} ($\S6.4.2$) for detailed exposition of this Cartan-based solution to the $KP$ problem. In our final chapter, we revisit this method demonstrating how our novel use of a global Cartan decomposition and variational methods give rise to time optimal synthesis results consistent with the literature.


==> ebackupChapter3b.tex <==
% %==========
% %==========
% %====BACKGROUND: ackground: Geometry, Lie Theory and Representation Theory



% \chapter{Background: Algebra}
% \label{chapter:Background: Geometry, Lie Algebras and Representation Theory}
% \section{Introduction}
% \subsection{Overview}
% A major focus of this work on the topic of quantum geometric machine learning is the framing of quantum control problems in terms of geometric control where target quantum computations are represented as $U_T \in G$ where $G$ is a Lie group of interest. In this generic model, we are interested then in constructing time-optimal Hamiltonians composed of generators from the associated Lie algebra $\g$ (or some subalgebra thereof) and associated control functions $u(t)$ so as to evolve the quantum system towards the target $U_T$ in the most efficient manner possible. Doing so according to optimality criteria, such as optimal (minimum) time or energy in turn requires a deep understanding of both quantum information processing concepts, but also algebraic and geometric concepts at the heart of much modern quantum and classical physics. By using methods that leverage symmetry properties of quantum systems, time-optimal solutions can often be more easily approximated to find solutions or solution forms that would otherwise be intractable or numerically infeasible to discover. This synthesis of geometry and algebra is one of the grand stories of modern mathematics, prefigured in much ancient meditations of natural philosophy and becoming a central motivation for so much of 19th century mathematical innovations in geometry, analysis, algebra and number theory that led to the hitherto unparalleled development of the field from Hilbert onwards. The widespread application of ideas drawn from these disciplines has been of significance within physics and other quantitative sciences, including more recently computer science and machine learning fields.

% In this chapter, we cover the key elements of the theory of Lie algebras and Lie groups relevant to the quantum geometric machine learning programme and greybox machine learning architectures discussed in this work. The exegesis below is far from complete and we have assumed a level of familiarity with elementary group and representation theory. The chapter focuses on key principles relevant to understanding Lie groups and their associated Lie algebras, with a particular focus on matrix groups and foundational concepts such as bilinear (Killing) forms, the Baker-Campbell-Hausdorff theorem and other elementary principles. We then proceed into a short discussion of elements of representation theory, including a discussion of semi-simple Lie group classification (of relevance to later chapters), adjoint action, Cartan decompositions and abstract root systems. The material in this chapter is related throughout to the novel results in this work in later chapters, as well as the other background chapters themselves. The chapter is also interconnected with the following chapter on geometric principles (originally a single chapter, it was split for readability), especially regarding differentiable manifolds, geodesics and geometric control. Most of the material is sourced from standard texts such as those by Knapp \cite{knapp_lie_1996,knapp_representation_2001}, Helgason \cite{helgason_differential_1979}, Hall \cite{hall_lie_2013} and others. As with the other background chapters, proofs are largely omitted (being accessible in the referenced texts). Readers with sufficient background in the topics herein may skip this chapter. 


% \subsection{Historical background}\label{sec:alg:Historical background}
% Understanding the historical development of geometric methods is a useful \textit{aid\'e-memoire} for situating the modern adoption of differential geometry within quantum information and machine learning contexts. The development of geometry and algebra, two of the four [standard] pillars of modern mathematics \cite{gowers_princeton_2010}, has been tandem. Philosophically, the relationship between algebra and geometry has exhibited a symbiotic waxing and waning throughout the development of mathematics' early formalism between the then-canonical ancient distinctions of the science of magnitude (geometry) and the science of multitude (arithmetic) \cite{detlefsen_formalism_2007}. Geometric and algebraic (or what today would be regarded as proto-algebraic) proofs or demonstration took relatively distinct forms. For example, Euclid's geometric proofs in the \textit{Elements} \cite{heath_thirteen_1956} were characterised by geometric demonstrative visual methods, while alternative proofs, such as the celebrated proof of the infinity of primes, relied upon explicit logical inference and deduction.
% %
% % \subsubsection{Erlangen programme}
% The late nineteenth-century \textit{Erlangen Program} of Felix Klein \cite{gray_felix_2005} put forward a systematic means of describing geometries in terms of their symmetry properties, as described by the mathematics of groups. In particular, the unification of geometry and group theory via the identification of geometries with specific transformation groups originally developed by Sophus Lie. Lie's \textit{id\'ee fixe} in describing the transformation of geometric objects in terms of underlying symmetries formed a primary motivation for his later development of the theory of continuous transformation groups (Lie groups). \\
% \\
% As Sharpe notes \cite{sharpe_differential_2000}, Klein's insight that non-Euclidean geometries could be recognised as examples of coset spaces $G/H$ (for Lie groups) seemed incompatible with the other central trend of nineteenth century geometry, the development of Riemannian geometry. As Knapp \cite{knapp_lie_1996} notes, the development of representation theory and Lie theoretic-methods has taken diverse approaches within the literature. Some tomes have emphasised primarily the algebraic and group-theoretic basis of Cartan decompositions and [optimisation]. Others, such as the work of Helgason \cite{helgason_differential_1962,helgason_differential_1979}, have followed more closely Cartan's genesis, an approach that elucidates the concurrent development of differential-geometric principles and Lie theory together. Indeed the unification of geometry, symmetry and algebra via Cartan's seminal classification of Riemannian symmetric spaces according to the taxonomy of semi-simple Lie groups is regarded as one of the 20th century's most elegant mathematical achievements. 



% % \subsubsection{Cartan's revolution}

% \section{Lie theory}\label{sec:alg:Lie theory}


% \subsection{Overview} 
% An essential concept in physics is \emph{symmetry}, especially \emph{rotational} and \emph{Lorentz symmetry} in various physical systems. Symmetries are often described by \emph{continuous groups}—parameterized groups with a manifold structure that allows smooth operations. These are known as \emph{Lie groups}, which possess a differentiable manifold structure that supports smooth group operations. The tangent space at the identity element of a Lie group forms a \emph{Lie algebra} through a natural bracket operation, encoding the properties of the Lie group while being more tractable due to its linear structure.

% In quantum mechanics, symmetry is reflected in the Hilbert space through a \emph{unitary action} of a symmetry group. This is formalized by a \emph{unitary representation}, a continuous homomorphism from a symmetry group $G$ into the group of unitary operators $U \in \mathcal{B}(\mathcal{H})$ acting on the quantum Hilbert space $\Hilb$ (axiom \ref{axiom:quant:quantumstates}). However, in reality, physical states correspond to unit vectors in $H$ differing by a phase, so we use \emph{projective unitary representations}, mapping $G$ into the quotient $U(H)/U(1)$, where $U(1)$ is the group of phase factors, or complex numbers of unit magnitude. This captures the essence of physical state representations, as an ordinary or projective representation of a Lie group induces a corresponding representation of its Lie algebra. For example, angular momentum operators are a representation of the Lie algebra of the rotation group. Understanding the representation of Lie groups and their algebras in a way relevant to quantum information processing is therefore central to solving geometric quantum control problems, especially using machine learning. To this end, we set out background theory below.

% \subsection{Lie groups}\label{sec:alg:Lie groups}
% A topological group is a group $G$ equipped with a topology uch that the group's binary operation and inverse function are continuous functions with respect to the topology. Such groups exhibit both algebraic structure and topological structure, allowing algebraic operations (due to group structure) and continuous functions on the group manifold (due to its topology). A \textit{continuous group} is one equipped with continuous group operations i.e. that $G$ is parameterised by a parameter that is continuous (and even smooth) on its domain e.g. $\theta \in I \subset \R$. If $G$ has Hausdorff ($T_2$ topology) and that parameter is differentiable, then $G$ exhibits the structure of a Lie group. 

% \begin{definition}[Lie groups]\label{defn:alg:liegroups}
%     A Lie group $G$ is a Hausdorff topological group equipped with a smooth manifold structure, namely one that supports group operations that are smooth maps.
% \end{definition}
% Lie groups encapsulate the concept of a \textit{continuous group} allowing the study of infitesimal transformations (such as translatiosn and rotations) and associated symmetry properties. The ability to analyze infinitesimal transformations is what connects Lie groups to differential geometry and physics, particularly in the context of studying continuous symmetries relevant to symmetry reduction. The corresponding Lie Groups are also equipped with product and inverse maps $\mu: G \times G \to G, \ell: G \to G$. An important property of Lie groups is left translation and the related concept of left invariance, central to the construction of invariant measures (such as the Haar measure) on groups. For a Lie group $G$, left translation by $g \in G$, denoted $L_g: G \to G, L_g(h)\mapsto gh$ for $h \in G$, is a diffeomorphism from $G$ onto itself. Right translations are similarly defined as $R_g(h) \mapsto hg$.  An important concept is that of left invariance of a vector field $X$ where $X$ is left invariance if $(dL_{g^\inv h})(X_g) = X_h$ (i.e. that $X$ commutes with left translations) i.e if, for all $g \in G$, we have $dL_g(X_e) = X_g$, where $e$ is the identity element in $G$ and $dL_g$ is the differential of left translation by $g$.

% Given a smooth function $f:G \to \R$, we denote $f_g(h) = f(gh)$ for $g,h \in G$ the left translate. A vector field $X$ on $G$ is itself left invariant if $(Xf)_g = X(f_g)$. Such left invariant $X$ form the Lie algebra $\g$ of $G$. The vector field $X$ can then be regarded as a set of tangent vectors $X_g$ at $g \in G$. The special relationship with the identity is then further understood as follows: the mapping $X \to X_I$ (where $I$ is the identity element of $G$) is a vector space isomorphism between $\g$ to the tangent space $X_I$ (mapping vector fields to their vectors at the identity element, thus identifying the Lie algebra with the tangent space at the identity), thereby (as we discuss below and in the next chapter) encoding the structure of the group through its tangent space at the identity. This isomorphism preserves (and thus `carries') the Lie bracket, allowing the tangent space at the identity in $G$ to be identified \textit{as} the Lie algebra $\g$ itself. Thus the entire Lie algebra, and thus group, can be studied in terms of the infinitesimal translations near the identity.


% \subsection{Matrix Lie groups}\label{sec:alg:Matrix Lie groups}
% We begin with the general linear group $GL(n; \C)$ acting on $M_n(\C)$, the set of $\dim n$ complex matrices.
% \begin{definition}[General linear group] \label{defn:alg:general linear group}
%     The group of all invertible n-dimensional complex matrices is denoted the general linear group:
%     \begin{align*}
%         GL(n;\C) = \{ A \in M_n(\C) | \det(A) \neq 0 \}
%     \end{align*}
% \end{definition}
% As we discuss later on, matrix representations of groups are central to many methods in quantum information processing. We note (as discussed in Chapter \ref{chapter:Quantum Geometric Machine Learning}) that $M_n(\C)$ may be identified (locally) $C^{n^2}=\R^{2n^2}$ via representing another dimension for the imaginary terms (each complex matrix element represented by two real numbers). A \textit{matrix Lie group} is defined as a closed subgroup of $GL(n; \C)$ i.e. each such group is a real-valued submanifold of the general linear group (closed here means in the topological sense, such that limit points of sequences remain within the subgroup). An important feature of Lie theory is the existence of Lie group homomorphisms.

% \begin{definition}[Lie group homomorphism]\label{defn:alg:Lie group homomorphism}
% Given matrix Lie groups $G_1$ and $G_2$, a Lie group homomorphism $\varphi:G_1\to G_2$ is a continuous group homomorphism. Such a homomorphism is an isomorphism if it is bijective and with a continuous inverse. Lie groups for which there exists such an isomorphism are equivalent (up to the isomorphism).
% \end{definition}
% Important groups include the group of $n-$dimensional invertible real-valued matrices $\text{GL}(n, \mathbb{R})$, and $\text{SL}(n, \mathbb{C})$ and $\text{SL}(n, \mathbb{R})$ special linear groups with determinant 1. Of particular importance is the unitary group defined below.


% \begin{definition}[Unitary matrix and unitary group]\label{defn:alg:Unitary matrix and unitary group}
% An operator $U \in M_n(\mathbb{C})$ is unitary if $U^\daggerU = UU^\dagger = I$. The set of unitary operators form the unitary group denoted $U(n)$. 
% \end{definition}
% Unitary operators preserve inner products such that $U$ is unitary if and only if $\langle Uv, Uw \rangle = \langle v, w \rangle$ for all $v, w \in \Hilb$. The special unitary group $SU(n)$ is the set of all $U(n)$ such that $\det U(n)=1$.

% \begin{proposition}[Connected Lie Group]
% \label{defn:alg:connected_matrix_lie_group}
% A (matrix) Lie group $G$ is \emph{connected} if for all $A, B \in G$ there exists a continuous path $\gamma : [0,1] \rightarrow M_n(\mathbb{C})$ such that $\gamma(0) = A$ and $\gamma(1) = B$ with $\gamma(t)\in G$ for all $t$. 
% \end{proposition}
% The connectedness of a Lie group is crucial to its representation in terms of a differentiable manifold with suitable topology for quantum information tasks.
% We characterise $G$ as \emph{simply connected} if it is connected and every continuous loop (i.e. curve such that $\gamma(0)=\gamma(t)$ in $G$ can be shrunk continuously to a point $g \in G$. A matrix Lie group $G$ is considered  \emph{compact} if it is compact as a subset of $M_n(\mathbb{C}) \cong \mathbb{R}^{2n^2}$.

% In particular, of relevance to later chapters, we note that the groups $O(n), SO(n), U(n)$ and $SU(n)$ are compact. $U(n)$ is connected allowing continuous paths between $U(0) \to U(t)$. This is an important aspect of controllability (and reachability) of quantum states in later chapters. It also impacts the learnability of unitary sequences from training data (such as discussed in Chapter \ref{chapter:Quantum Geometric Machine Learning}). The group $SU(2)$, the key group for qubit-based quantum computation, is defined as:
% \begin{align}
%     SU(2) = \left\{ \begin{pmatrix}
% \alpha & -\beta \\
% \beta & \bar{\alpha}
% \end{pmatrix} \, \middle| \, \alpha, \beta \in \mathbb{C}, \, |\alpha|^2 + |\beta|^2 = 1 \right\}.
% \label{eqn:alg:su2group}
% \end{align}

% The [allows for a consistent and complete description of qubit states and their transformations (i.e. because of guarantees of , which in turn is essential for the design and understanding of quantum algorithms and the behavior of quantum systems]. In particular, for multi-qubit computations (and even single-qubit ones), we are often interested in decomposition into a sequence of single-qubit gates. The simply connected nature of gates drawn from $SU(2)$ guarantees the density of universal gate sets, allowing approximation of (and controllability for) relevant target unitaries to any desired accuracy. We set out below a few relevant standard facts about Lie groups and Lie algebras. In particular we emphasise concepts related to characterising quantum unitary sequences as curves along Lie group manifolds generated by the corresponding Lie algebra.



% %=====Subsection: Lie algebras
% \subsection{Lie algebras}\label{sec:alg:Lie algebras}
% \begin{definition}[Lie algebra and Lie derivative]\label{defn:alg:Lie algebraliederivative}
%      An algebra $\frak{g}$ is a vector space over a field $\Km$ equipped with a bilinear form (product) $[X,Y]$ for $X,Y \in \frak{g}$ that is linear in both variables. Such an algebra is a \textit{Lie algebra} if:
% \begin{enumerate}[(a)]
%     \item $[X,X]=0$ and $[X,Y]=-[Y,X]$, $\forall X,Y \in \frak{g}$; and
%     \item the Jacobi identity is satisfied, namely:
%     \begin{align}
%         [[X,Y],Z] + [[Y,Z],X] + [[Z,X],Y]=0
%     \end{align}
% \end{enumerate}
% \end{definition}
% The product $[X,Y]$ above is denoted the \textit{Lie derivative} (sometimes the Lie bracket). In quantum information contexts, the Lie derivative is denoted the commutator. The commutator exhibits a number of properties which we set out here for completeness.

% \begin{proposition}[Lie bracket properties]\label{prop:alg:Lie bracket properties}
%     Properties of Lie bracket (commutator) include:
%     \begin{enumerate}
%         \item linearity in the first and antilinearity in the second arguments $[\alpha A, B + \beta C] = \alpha[A,B] + \alpha\beta^*[A,C]$ for $\alpha,\beta \in \C$; 
%         \item antisymmetry $[B,A] = -[A,B]$; 
%         \item derivability (Liebniz rule) $[A,BC] = [A,B]C + B[A,C]$ (related to derivations).
%     \end{enumerate}
% \end{proposition}
% In geometric contexts, the Lie bracket (commutator) is equated with the Lie derivative, satisfying the conditions above. We use these terms interchangeably as appropriate for the context. 

% Note that for $\g \subset \mathcal{A}$ (where $\mathcal{A}$ is an associative algebra), $\g$ can be constructed as a Lie algebra using the Lie bracket $[x,y] = xy-yx, \forall x,y \in \g$ (in such cases $\mathcal{A}$ is the universal enveloping algebra of $\g$). An important characteristic of Lie algebras is the action of a Lie algebra upon itself as represented by the adjoint action, realised in the form of the Lie derivative.

% %======defn: adjoint action
% \begin{definition}[Adjoint action]\label{defn:alg:Adjoint action}
%     The \textit{adjoint action} of a Lie algebra upon itself $\ad: \frak{g}\to \text{End}_\Km (\frak{g})$ is given by:
% \begin{align}
%     \ad_X(Y) = [X,Y]
% \end{align}
% where $\text{End}_\Km (\frak{g})$ represents the [set of $\Km$-scalar endomorphisms of $\frak{g}$ upon itself]. 
% \end{definition}
% More intuition about the relationship between the Lie derivative and differential [forms] is provided by showing that the adjoint action is a derivation. It can be shown that satisfying the Jacobi identity is equivalent to:
% \begin{align}
%     \ad_Z[X,Y] = [X,\ad_Z(Y)] + [\ad_Z(X),Y]
% \end{align}
% The adjoint action is a homomorphic endomorphism of $\g$ i.e. $\ad_{[X,Y]} = \ad_X\ad_Y - \ad_Y\ad_X$ with kernel $Z_\g$ below. Moreover the adjoint action is indeed a derivation $D$:
% \begin{align}
%     D[X,Y]=[X,DY] + [DX,Y]
% \end{align}
% for $D \in \text{End}_\Km (\frak{g})$. 

% In quantum information processing, Lie algebras tend to be represented via representations of $G \subset GL(n,\C)$ or its closed subgroups (closed linear group). An important result in the theory of Lie groups is that the Lie algebra $\g$ of $G$ is canonically isomorphic with the linear Lie algebra $\frak{gl}(n,\C)$ i.e. $\mu: \g \to \frak{gl}(n,\C)$ such that $X \in \g$ can be represented in terms of real and imaginary $X_I \in \frak{gl}(n,\C)$. Thus the behaviour of $\frak{gl}(n,\C)$ may be used to study that of $\g$ and thus $G$ of interest.
% \begin{definition}[Lie algebra homomorphism]\label{defn:alg: Lie algebra homomorphism} \hl{fix}
%     A \textit{Lie algebra homomorphism} from $\frak{g}$ to $\h$ is a linear map $\varphi:\frak{g} \to \frak{h}$ where:
% \begin{align}
%     \varphi([X,Y]) = [\varphi(X),\varphi(Y)]
% \end{align}
% where $\frak{a},\frak{b} \subset \frak{g}$:
% \begin{align}
%     [\frak{a},\frak{b}] = \text{span} \{ [X,Y] | X \in \frak{a}, Y \in \frak{b} \}
% \end{align}
% \end{definition}
% We then can define subalgebras (of critical importance to our discussion of Cartan methods below and control subalgebras) and ideals.
% \begin{definition}[Lie subalgebras and ideals]\label{defn:alg:Lie subalgebras and ideals}
%     A set $\h \subset \frak{g}$ is a \textit{Lie subalgebra} if $[\frak{h},\frak{h}] \subseteq \frak{h}$, in which case $\h$ is also a Lie algebra. A subalgebra is an \textit{ideal} if $[\h,\g] \subseteq \h$.
% \end{definition}
% Lie algebras can also be written as direct sums of the underlying vector spaces $\g_1,g_2$ equipped with an (induced) Lie bracket (adjoint preserving [Killing form]):
% \begin{align}
%     [(X_1,Y_1),([X_2,Y_2])]=([X_1,Y_1],[X_2,Y_2])
% \end{align}
% for $X_k,Y_k \in \g_k$.

% For Cartan decompositions, we require the classification of semi-simple Lie groups. This in turn requires other sundry definitions.
% \begin{definition}[Centralizer and Normalizer]\label{defn:alg:Centralizer and Normalizer}
%     The centralizier of $\frak{s}$ in $\g$ is a subalgebra of $\g$ comprising elements that commute with all of $\frak{s}$:
%     \begin{align}
%         Z_\g(\frak{s}) = \{ X \in \g | [X,Y]=0, \forall Y \in \frak{s} \}
%     \end{align}
%     The normalizer of $\g$ is the set of all elements of $\g$ whose commutator with $\frak{s}$ is in $\frak{s}$:
%     \begin{align}
%         N_\g(\frak{s}) = \{ X \in \g | [X,Y] \in \frak{s}, \forall Y \in \frak{s} \}
%     \end{align}
% \end{definition}
% The center $Z_\g$ is the set of $X \in G$ that commute with all elements in $\g$. To understand semi-simple Lie algebras, we can define nested commutators with a commutator series and lower central series as:
% \begin{align}
%     \g^0 &=\g \qquad \g^{j+1} = [\g^j,\g^j] \qquad \g &= \g^0 \supseteq \g^1 \supseteq ...\qquad \text{(commutator series)}\\
%     \g^0 &=\g \qquad \g_{j+1} = [\g,\g_j] \qquad \g &= \g_0 \supseteq \g^1 \supseteq ...\qquad \text{(lower central series)}
% \end{align}
% From these definitions we obtain the concepts of $\g$ being \textit{solvable} if $g^j=0$ for some $j$ and \textit{nilpotent} if $g_j=0$ for some $j$ (nilpotent implies solvable). We can now define simple and semi-simple Lie algebras as follows:
% %Simple and semisimple
% \begin{definition}[Simple and semisimple]\label{defn:alg:Simple and semisimple}
% A finite-dimensional $\g$ is simple if $\g$ is nonabelian and has no proper non-zero ideals. We say $\g$ is semisimple if $\g$ has no nonzero solvable ideals.
% \end{definition}
%  This last test for semisimplicity is equivalent to the radical $\text{rad}\g=0$. Simple $\g$ are semisimple by construction. They are algebras are closed under commutation $[\g,\g]=\g$ (important for control). Semisimple $\g$ have empty centers. 
 
% \subsection{Killing form}\label{sec:alg:Killing form}
% We now define the Killing form, a bilinear form defined on $\g$ which plays an central role in allowing algebraic concepts to be connected to geometric analogues and enabling classification of algebraic structures. In particular, as we discuss below, conditions on the Killing form allow its association as a Riemannian or subRiemannian metric (used to calculate minimal path lengths, and thus time, of curves in $G$) for symmetric spaces the subject of our final chapter. 
% \begin{definition}[Killing form]\label{defn:alg:Killing form}
%     The Killing form is a bilinear transformation given by:
% 	\begin{align}
% 	B(X,Y) = \Tr(\ad_X, \ad_Y)
% 	\end{align}
% 	for $X,Y \in \g$.
% \end{definition}
% The Killing form is an important element in Cartan's classification of semi-simple Lie algebras and, among other things, establishing appropriate metrics (and inner products) on $\g$ for variational methods discussed later on. Additionally, Cartan's criterion for semisimplicity is that the Killing form is non-degenerate, that is $\g$ is semisimple if and only if the Killing form for $\g$ is non-degenerate, namely $B(X,Y) \neq 0$ for all $X,Y \in \g$. Other concepts we briefly note are that $\g$ is \textit{reductive} if for each ideal $\a \subset \g$, there exists another ideal $\frak{b} \subset \g$ such that $\g = \a \oplus \frak{b}$ (i.e. can be written as the direct product of ideals). It can be shown this is equivalent to $\g$ being closed under the conjugate transpose (adjoint) action. Under such conditions, the Killing form can be used to define an inner product via $(X,Y) = -B(X,Y)$ and thus a metric. Moreover, the Killing form is invariant under the adjoint action of the Lie group, meaning $B(\text{Ad}_g X, \text{Ad}_g Y) = B(X,Y)$ for all $g \in G$ and $X,Y \in \g$. This invariance property of the Killing form ensures the induced metric is well-defined across the manifold $G$. We explore this in our final chapter.



% \subsection{Matrix exponential}\label{sec:alg:Matrix exponential}
% The matrix exponential is an important operation in the theory of Lie algebras and Lie groups (especially regarding their connection). Moreover, it is also a fulcrum concept that links both operationally and semantically from algebraic theory to quantum theory. The various representations of the matrix exponential serve a variety of uses, such as in terms of infinite power series (especially relating to the use of the adjoint operator in Chapter \ref{chapter:Time optimal quantum geodesics using Cartan decompositions}) and as group elements.

% \begin{definition}[Matrix exponential]\label{defn:alg:Matrix exponential}
% The matrix exponential is defined by the following  power series: 
%     \begin{align}
%         e^X = \sum_{n=0}^\infty \frac{X^n}{n!}
%     \end{align}
% \end{definition}
% This can usefully be expressed as:
% \begin{align}
%      e^X = \lim_{n \to \infty} \left( I + \frac{X}{n} \right)^n \label{eqn:alg:exponentiallimit}
% \end{align}
% where $X \in \g$ or some other vector space, such as $M_n(\C)$. The matrix exponential satisfies a number of properties (listed out in theorem (\ref{thm:alg:matrix_exponential_properties}) in the Appendix). More intuition can be obtained via the derivative of the matrix exponential function: 
% % \hl{update}
% \begin{align}
%     \left. \frac{d}{dt} e^{tX} \right|_{t=0} = X \label{eqn:alg:matrixexpderivativeatzero}
% \end{align}
% Equation (\ref{eqn:alg:matrixexpderivativeatzero}) provides an important way of understanding, via the representation of matrix groups, the connection between Lie algebras and Lie groups. It indicates that the derivative at the identity element of the group is precisely the Lie algebra element $X$, demonstrating how Lie algebras serve as the infinitesimal generators of Lie group actions. Moreover, the one-parameter subgroup theorem below, stating that for every element $X$ in the Lie algebra there corresponds a unique one-parameter subgroup in the Lie group with $A(t) = \exp{tX}$, explicitly reveals the relationship between the algebraic structure of Lie algebras and the topological and geometric structure of Lie groups. This unique mapping via the exponential allows the exploration of continuous symmetries of groups by way of their corresponding Lie algebra.
% %=========
% We note then the definition of a one-parameter subgroup of $G$.
% \begin{definition}[One-Parameter Subgroup of \(GL(n; \mathbb{C})\)]
% \label{defn:alg:one_parameter_subgroup}
% A one-parameter subgroup of \(GL(n; \mathbb{C})\) is denoted \(G(\cdot)\) and is a continuous homomorphism of $\R \to GL(n; \mathbb{C})$. Equivalently, for $A \in G(\cdot)$, it corresponds to a continuous map \(A : \mathbb{R} \rightarrow GL(n; \mathbb{C})\) such that \(A(0) = I\) and \(A(s + t) = A(s)A(t)\) for \(s, t \in \R\).
% \end{definition}
% It can then be shown that there exists a unique element of the Lie algebra (representation) used to establish the relationship between a Lie algebra and Lie group.

% \begin{theorem}[One-Parameter Subgroup Exponential Representation] 
% \label{thm:alg:one_parameter_subgroup_exponential}
% If \(G(\cdot)\) is a one-parameter subgroup of \(GL(n; \mathbb{C})\), then there exists a unique \(X \in M_n(\mathbb{C})\) such that $A(t) = \exp{tX}$ parametrised by $t \in \R$.
% \end{theorem}
% These relations show how continuous symmetries of Lie groups may be studied via the Lie algebra as a tangent space at the identity element of the group. In quantum information contexts, the matrix exponential allows the study of system's dynamics via mapping the Hamiltonian $H$ (see definition \ref{defn:quant:Hamiltonian}) to group elements represented as unitary operators (definition \ref{defn:quant:Unitary Operator}).

% \subsection{Lie algebra of matrix Lie group}\label{sec:alg:Lie algebra of matrix Lie group}
% Lie algebras are associated with Lie groups via the exponenial map.
% % \hl{Update}
% \begin{definition}[Lie Algebra of a Matrix Lie Group]
% \label{defn:alg:lie_algebra_of_matrix_lie_group}
% Given a matrix Lie group $G \subseteq GL(n; \mathbb{C})$, the Lie algebra $\mathfrak{g}$ for $G$ is defined as follows:
% \begin{align*}
%     \mathfrak{g} = \{ X \in M_n(\mathbb{C}) \mid e^{tX} \in G \text{ for all } t \in \mathbb{R} \}.
% \end{align*}
% \end{definition}
% Note that $X \in \mathfrak{g}$ if and only if the one-parameter subgroup is in closure of $G$. For $X \in \mathfrak{g}$, it is sufficient that $e^{tX} \in G$ for all $t \in \R$.
% % \hl{Paraphrased}
% For any matrix Lie group $G$, the Lie algebra $\mathfrak{g}$ of $G$ has the following properties. The zero matrix $0$ belongs to $\mathfrak{g}$. For all $X$ in $\mathfrak{g}$, $tX$ belongs to $\mathfrak{g}$ for all real numbers $t$. For all $X$ and $Y$ in $\mathfrak{g}$, $X + Y$ belongs to $\mathfrak{g}$. For all $A \in G$ and $X \in \mathfrak{g}$ we have $AXA^{-1} \in \mathfrak{g}$. For all $X$ and $Y$ in $\mathfrak{g}$, the commutator $[X, Y]$, defined by
% \begin{align*}
% [X, Y] := XY - YX = \frac{d}{dt}e^{tX}Ye^{-tX} \bigg|_{t=0}
% \label{eqn:alg:liealgderivatidentity}
% \end{align*}
% belongs to $\mathfrak{g}$. The first three properties of $\mathfrak{g}$ say that $\mathfrak{g}$ is a real vector space. Since $M_n(\mathbb{C})$ is an associative algebra under the operation of matrix multiplication, the last property of $\mathfrak{g}$ shows that $\mathfrak{g}$ is a real Lie algebra. Equation (\ref{eqn:alg:liealgderivatidentity}) also indicates that the Lie algebra $\g$ is the set of derivatives at $t=0$ of all smooth curves $\gamma(t) \in G$ where such curves equal the identity at zero. It thus provides a bridge between typical algebraic formulations of commutators and geometric representations of tangents. In the next section we provide more detail on the relationship between Lie theory and differential geometric concepts such as curves. Note that we can define the Lie algebras of $\u(n)$ and $\frak{su}(n)$:
% \begin{align}
%     \u(n)&=\{ X \in M_n(\C) | X^\dagger = -X \}\\
%     \frak{su}(n) &= \{X \in \u(n) | \Tr(X)=0  \}
%     \label{eqn:alg:xderivofetx}
% \end{align}
% The relation of Lie groups to Lie algebras can be briefly sketched. Group actions $\Phi: G \to G$ have a corresponding map in the Lie algebra $\phi:\g \to g$ such that: 
% \begin{align}
%     \Phi(e^{tX})=e^{t\phi X}
%     \label{eqn:alg:groupalgebrahomocorro}
% \end{align}
% where $\phi(X)=\frac{d}{dt}\Phi(e^{tX})|_{t=0}$ (implying smoothness for each $X$). Here $\phi$ is a linear homomorphism such that:
% \begin{align}
%     \phi([X,Y])&=[\phi(X),\phi(Y)] \qquad \phi(AXA^\inv) = \Phi(A)\phi(X)\Phi(A)^\inv
% \end{align}
% where $A\in G$ and $X \in \g$. For a group $G$ and corresponding algebra $\g$, $X \in \g$ if and only if $e^X \in G$. 


% A key feature in quantum control contexts is framing control of the evolution of quantum systems in terms of paths over unitary Lie group manifolds. For this to be the case, in essence we require that Lie group homomorphisms be characteirsed or determined by Lie algebra homomorphisms - that is, we essentially want guarantees that arbitrary paths along the manifold can be generated by applying controls to generators in $\g$. This is particularly the case when the Lie groups of interest exhibit topological properties of being simply connected (meaning any close curve in $G$ can be shrunk to an arbitrary element of $G$ itself - or that is, there are no `holes'. In a control context, the simply connected nature of the underlying group manifold also provides [guarantees] as to arbitrary controls. If a group $G$ is connected and simply connected, then it can be shown that the Lie algebra and Lie group are related such that there is unique mapping $\Phi$ such that the group-algebra homomorphism correspondence set out in equation (\ref{eqn:alg:groupalgebrahomocorro}) holds. 
% From a geometric perspective, the following relationship between Lie algebras and tangent spaces is set out.
% \begin{theorem}[Lie algebra tangent space correspondence]\label{thm:alg:Lie algebra tangent space correspondence}
%     Each Lie algebra $\g$ of $G$ [is equivalent to] the tangent space to $G$ at the identity. The algebra $\g$ is equivalent to the set of $X \in M_n(\C)$ such that there exists a smooth curve $\gamma:\R \to M_n(\C) \subseteq G$ with $\gamma(0)=I,\gamma'(0)=X$.
% \end{theorem}
% This can be seen given equation (\ref{eqn:chap-lie:xderivofetx}) in concert with $\gamma(t) = e^{X(t)}$ (such that $\gamma'(0) \in \g$). Moreover, for a matrix Lie group that is connected, then it can be shown that for $\gamma \in G$, there is a finite set of elements in $\g$ that generate $\gamma$. These facts are important to the characterisation and control of quantum unitary sequences (and circuits) in terms of paths along manifolds in Chapters \ref{chapter:Quantum Geometric Machine Learning} and \ref{chapter:Time optimal quantum geodesics using Cartan decompositions}. The relationship between Lie algebra and group homomorphisms is not simply one-for-one, as can be seen the fact that $\su(2) \simeq \so(3)$ while $SU(2)$ and $SO(3)$ are not isomorphic (see literature \cite{knapp_lie_1996,knapp_representation_2001} etc for more detail). We note finally for completeness that on occasions one is interested in the universal cover $\tilde G$ of a group $G$ which effectively is a simply connected matrix Lie group which `covers' (in the sense that there is a group homomorphism between the groups and isomorphism among their algebras that allows the study or manipulation of group $G$, which may not be simply connected, via $\tilde G,\tilde \g$. 


% \subsection{Homomorphisms}\label{sec:alg:Homomorphisms}
% The relationship between Lie algebras and Lie groups via the exponential map is considered a lifting of homomorphisms of Lie algebras to homomorphisms of (analytic) groups. That is, for $G,H$ analytic subgroups, $G$ simply connected and the Lie algebra homomorphism $\varphi: \g \to \h$, then there exists a smooth homomorphism $\Phi: G \to H$ such that $d\Phi = \varphi$. As \cite{knapp_lie_1996} notes, there are two equivalent ways to express such a lifting: either relying on lifting homomorphisms to simply connected analytic groups, or relying on existence theorems for sets of solutions to differential equations. The first approach involves defining curves $\gamma: \R \to G$ with $\gamma(t) \mapsto \exp(tX)$. One then defines $d/dt$ and $\tilde X$ as left invariant fields on $\R,G$ such that:
% \begin{align*}
%     d\gamma(t)\left(\frac{d}{dt}\right)f = \frac{d}{dt}f(\gamma(t)) = \frac{d}{dt}f(\exp(tX))= \tilde X f(\exp(tX))
% \end{align*}
% hence we see the important explicit relationship between the left-invariant vector fields $\tilde X$ and $d/dt$. Among other things, this shows the mapping $X \to \exp(X)$ is smooth (given the smoothness of $d/dt$). Expressed in local coordinate charts, the equation above represents a system of differential equations satisfied by curves $\gamma(t)$ represented as exponentials. Among other aspects, this relation enables the machinery of analysis to be brought to bear in group theoretic problems in quantum information contexts. For example, it enables the application of Taylor's theorem such that:
% \begin{align*}
%     (\tilde X^n)(g \exp (tX)) = \frac{d^n}{dt^n}(f(g\exp (tX))
% \end{align*}
% for $g\in G, f \in C^\infty$. Noting also that:
% \begin{align}
%     \tilde X f(g) = \frac{d}{dt}f(g \exp t X) \big|_{t=0}
% \end{align}
% shows again how the operation of left-invariant vector fields $\tilde X$ is equated with differential operators. 

% \subsection{Baker-Campbell-Hausdoff theorem}\label{sec:alg:Baker-Campbell-Hausdoff theorem}
% As Hall \cite{hall_lie_2013} notes, an important feature of the correspondence between Lie algebras and Lie groups is to show that the Lie group homomorphism $\Phi: G \to H$ defined by $\Phi(\exp(X)) = \exp(\phi(X))$ where $\phi: \g \to \h$ is a Lie algebra homomorphism . 
% \begin{definition}[Baker-Campbell-Hausdorff]\label{defn:alg:Baker-Campbell-Hausdorff}
% The Baker-Campbell-Hausdorff formula shows that the map $\Phi$ is identified from $U_e \in G$ into $H$ is a local homomorphism by such that for sufficiently small $X,Y, Z \in \g$:
% \begin{align}
%     \exp(X)\exp(Y) = \exp\left(X + Y + \frac{1}{2}[X,Y] + \frac{1}{12}[X,[X,Y]] +...  \right) \label{eqn:alg:Baker-Campbell-Hausdorff}
% \end{align}
% \end{definition}
% %  That is:
% % \begin{align}
% %     Z = \log(\exp(X)\exp(Y)) = X + Y + \frac{1}{2}[X,Y] + \frac{1}{12}[X,[X,Y]] -  \frac{1}{12}[Y,[X,Y]] + ...
% % \end{align} 
% (see Hall \cite{hall_lie_2013} $\S 5$ for proofs including the Poincar\'e integral form). The BCH formula is important in quantum control settings in particular as we discuss in other parts of this work. 

% %===========ROOT SYSTEMS/DIAGRAMS (MOVE)



% %==========REPRESENTATION THEORY

% \section{Representation theory}\label{sec:alg:Representation theory}
% \subsection{Overview}
% In this section, we briefly cover elements of the [representation theory of semi-simple groups.] This is particluarly relevant to geometric treatments involving Lie algebras in later chapters. Representations are abstractions (homomorphisms) of groups (in terms of actions on generalised linear (invertible) vector spaces, i.e. on  $GL(n; \C)$ the group of invertible linear transformations of a finite-dimensional vector space $V$. The associated Lie algebra is $\frak{gl}(n,\C)$. We summarise 

% \subsection{Representations}\label{sec:alg:Representations}
% We begin with the definition of representations.
% \begin{definition}[Finite-Dimensional Representation of a Lie Group]\label{defn:alg:Finite-Dimensional Representation of a Lie Group}
% \label{defn:alg:finite_dim_representation_of_lie_group}

% A finite-dimensional representation of $G$ is a continuous homomorphism of $\pi:G \to GL(V)$. A representation satisfies:
% \begin{align}
%     \pi([X,Y]) = [\pi(X),\pi(Y)]
% \end{align}
% for $X,Y \in G$ and equivalently for the lie algebra $\pi: \g \to \frak{gl}(V)$.
% \end{definition}
% An \textit{invariant subspace} for a representation $\varphi:\g \to GL(V)$ on a subspace $U \subset GL(V)$ is one such that $\varphi(X)U \subseteq U$ for $X \in \g$ (i.e. if the only $G$-invariant subspaces of $V$ under $\pi$ are the trivial subspace $\{0\}$ and $V$ itself). A representation on a non-zero space $GL(V)$ is \textit{irreducible} if the only invariant subspaces are 0 and $GL(V)$. That is, given $\pi: G \to GL(V)$, a subspace $U \subset V$ is invariant if $\Pi(g)w \in W$, for all $g \in G, w \in W$. 
% % \begin{definition}[Irreducible representations]
% % \label{defn:alg:irreducible_representation}
% % \end{definition} 
% Two representations of $G$ are isomorphic if and only if the Lie algebra representations are isomorphic. This result allows us in particular to move between the fundamental and adjoint representation with implications, for example, with respect to optimal parametrisation of invariant neural networks whose parameters are correlated to the choice of representation \cite{larocca_group-invariant_2022,larocca_theory_2023}.
% Representations $\varphi,\varphi'$ are equivalent if there exists an isomorphism between the two vector spaces $\chi:V\to V'$ such that $\chi \varphi(X) = \varphi'(X)E$. A \textit{completely reducible} subspace is then one which can be decomposed into the direct sum of irreducible representations i.e. such that $V = \oplus_i U_i$ for $U \subset V, i = 1,...,\dim V$.

% \subsection{Complex Semi-simple Lie Algebras}\label{sec:alg:Complex Semi-simple Lie Algebras}
% Of central importance to later chapters in this work are what are known as Cartan decompositions of symmetric space Lie groups as a technique for solving certain classes of time-optimal quantum control problems. In this section, we provide a brief summary of Cartan decompositions, their relationship to Lie groups and algebras together with root systems and Dynkin diagrams. The section largely summarises standard work in the literature \cite{knapp_lie_1996,hall_beyond_2007,helgason_differential_1962,helgason_differential_1979}. Quantum information processing problems in this work (and much of the field) are often related to semisimple Lie groups and Lie algebras. In such cases, Cartan subalgebras $\h \subset \g$ are abelian and we are particularly interested in certain subclasses of maximally abelian subalgebras. The Cartan subalgebra forms the generators the adjoint action of which on $\g$ enable its root-space decomposition which in turn give rise to an abstracted root system. The root system can then in turn be related (given a fixed ordering or choice of basis) to simple roots. These roots can be used to form a basis of $\g$, from which a Cartan matrix and Dynkin diagram may be constructed. The relevance of root systems, Cartan matrices and such diagrams in quantum control settings is explored primarily in the final chapter of this work.

%  %=========Adjoint action
% \subsection{Adjoint action and commutation relations} \label{sec:alg:Adjoint action and commutation relations}
% % \subsubsection{Adjoint action}
% An important representation used throughout this work is the \textit{adjoint representation}.
% \begin{definition}[Adjoint representation]\label{defn:alg:adjointrepresentation}
%     Given a Lie group $G$, Lie algebra $\g$ with smooth isomorphism $\Ad_g(h) = g h g^\inv$ where $g,h \in G$, there exists a corresponding Lie algebra isomorphism $\ad_X: \g \to \g$ such that:
%     \begin{align*}
%         \exp((\ad_\g)(X)) = g(\exp(X))g^\inv
%     \end{align*}
%     i.e. $\exp(\ad_\g(X))=\Ad_G(\exp(X))$.
% \end{definition}
% In the above, the former being the Lie algebra adjoint, the latter the group adjoint action, the two concepts being related by the exponential map. We denote $\ad_g(X) = g X g^\inv$. We note that each Lie group exhibits the structure of a manifold that is real and analytic (under multiplication and inversion and for the exponential map). Moreover, as noted in \cite{knapp_lie_1996}, it can be shown that each real Lie algebra has a one-to-one finite dimensional representation on complex vector spaces $V(\C)$.

% \subsection{Adjoint expansions} \label{sec:alg:Adjoint expansions}
% We note for completeness a few additional properties. Firstly \textit{automorphisms} of a Lie algebra $\g$ is an invertible linear maps $L$ such that $[L(X),L(Y)]=L[X,Y]$ for $X,Y \in \g$. In addition we have that $\ad_(L X) = L(\ad_X)L^\inv$. The Killing form is invariant under such automorphisms $B(LX,LY)=B(X,Y)$ for $X,Y \in G$.

% Note that the adjoint action of group elements can be expressed via conjugation as $\text{Ad}_h(g) = hgh^\inv$where $g,h \in G$. The adjoint action of a Lie algebra upon itself, which we focus on, is via the commutator namely $\ad_X(Y) = [X,Y]$ where $X,Y \in \frak{g}$. Thus terms such as $\ad_\Theta(\Phi)$ involve calculation of commutation relations among generators. Note the following used in the paper:
% \begin{align}
%     e^{i\Theta}Xe^{-i\Theta} = e^{i\ad_\Theta}(X) = \cos\ad_\Theta(X)+i\sin\ad_\Theta(X)
%     \label{eqn:alg:econjsinhcosh}
% \end{align}
% The $\cos \ad_\Theta (X)$ term can be understood in terms of the cosine expansion:
% \begin{align}
%     \cos \ad_\Theta (X) = \sum_{n=0}^\infty \frac{(-1)^n}{(2n)!} (\ad_\Theta))^{2n} (X)
% \label{eqn:alg:cosadthetaXexpansion}
% \end{align}
% Thus each term is a multiple of $\ad_\theta^2$. For [certain] choices of generators $\Theta$ and $X \in \frak{k}$ this effectively means that [acts as an involution up to coefficients]. Thus in the $SU(2)$ case, $\ad^{2n}_{J_y}(J_z) \propto J_z$ (with $n=0,1,2,...$). Each application of the adjoint action acquires a $\theta^2$ term (from $\Theta = i\theta J_y$), such that the series can be written:
% \begin{align}
%     \cos \ad_{\Theta} (-iJ_z) = \sum_{n=0}^\infty \frac{(-1)^n}{(2n)!} (\theta))^{2n} (J_z) = \cos(\theta)(-iJ_z)
% \label{eqn:alg:su2cosadthetaXexpansion}
% \end{align}
% More generally, the Cartan commutation relations exhibit such an [involutive] property given that for $\Theta \in \frak{k}$:
% \begin{align} \ad_\Theta(\frak{k})=[\Theta,\frak{k}] \in \frak{p} \qquad \ad^2_ \Theta(\frak{k})=[\Theta,[\Theta,\frak{k}]] \in \frak{k}
% \end{align}
% In the general case, assuming an appropriately chosen representation, each application of the adjoint action by even $n$ or odd $2n+1$ powers (and thus our $\cos \theta$ and $\sin \theta$ terms) will be scaled by an eigenvalue $\alpha$, such eigenvalue being the [root] (see below for an example). 
% Thus we have $\ad_{\Theta}^{2n}(\frak{k}) \subset \frak{k}$ and:
% \begin{align}
% \cos(\ad_\Theta) \Phi = \cos\alpha(\theta)\Phi 
% \label{eqn:alg:cosadthetaphi=costhetaphi}
% \end{align}
% such as in equation (\ref{eqn:main-x=1-cosadthetabigphi}) and similarly for the sine terms. Note that the assumption behind our choice of initial condition:
% \begin{equation}
% c(T) \in \Big\{c \in K : c\Theta c^\inv =\Theta \Big\} = M
% \end{equation} i.e. that $c\Theta c^\inv = \Theta$ depends upon the algebras in question for specific detail. In certain simple cases (as we discuss in the final chapter) one can  select $\phi_k = 2\pi n$ (for $n=1,2,...)$ such that $M= \{ \pm \mathbb{I} \} $ where $c$ is of the form:
% \begin{align}
%     c = e^{-i\Phi} = e^{-i(\sum_k \phi_k H_k)} \qquad H_k \in \frak{k}, \phi_k \in \Complex
% \end{align}
% For the $\sin\ad_\Theta(X)$ terms, by contrast, the adjoint action is of odd order: 
% \begin{align}
%     \sin \ad_\Theta (X) = \sum_{n=0}^\infty \frac{(-1)^{n}}{(2n+1)!} (\ad_\Theta))^{2n+1} (X)
% \label{eqn:alg:cosadthetaXexpansion}
% \end{align}
% such that $\ad_{\Theta}^{2n+1}(\frak{k}) \in \frak{p}$, hence the sine term arising in our Hamiltonian form equation (\ref{eqn:general:timeoptimalhamiltonian}) which, when cojugated with $\Lambda$ results in a Hamiltonian given in terms of control generators, namely:
% \begin{align}
%     [\sin \ad_\Theta(\frak{k}),\Lambda] \subset \frak{p}
% \end{align}
% By convention, sometimes one sees in the literature $KAK$ decompositions written in the form $e^{k_1}\frak{a}e^{k_2}$ where $k_1,k_2 \in \frak{k},e^{k_i}\in K$. Here the two exponentials are group elements while the middle $\frak{a}$ is shorthand for an exponentiated Lie algebraic element. Thus in equation (\ref{eqn:econjsinhcosh}) we write the adjoint action as conjugation given it involves the Lie group (rather than Lie algebraic) elements, while for the action of a Lie algebra on itself, we would use the commutation relation. 
% % For completeness \hl{\textbf{FIX}}: 
% % \begin{align}
% %     e^{k_1} e^{a} \approx e
% % \end{align}
% The choice is usually one of convenience (see the final chapter for more detailed discussion).


% %===========Real forms and Root systems
% \subsection{Real and complex forms}\label{sec:alg:Real and complex forms}
%  Complex Lie algebras $\g$ (over $\C$) and real Lie algebras $\g_0$ (over $\R$) are related via complexification and the related concept of the real form of a complex Lie algebra. Such complexification of Lie algebras is relevant in particular to formulating Cartan decompositions of Lie algebras and their associated groups (see Definition (\ref{defn:alg:cartandecomposition}). 
% \begin{definition}[Real form]\label{defn:alg:realforms}
%     We say that a real vector space $V(\R)$ is the real form of a complex vector space $W(\C)$ when the two are related as:
%     \begin{align*}
%         W^\R = V \oplus i V
%     \end{align*}
%     Where we denote $W$ the complexification of $V$.
% \end{definition}
% This equivalence is a statement that a real vector space can be complexified in the manner above. For Lie algebras, we often denote a real Lie algebra (as a vector space over $\R$) via a 0 subscript $\g_0$. In such terms, we may denote:
% \begin{align}
%     \g = \g_0^\C = \g_0 + i\g_0 \label{eqn:alg:liealgebracomplexification}
% \end{align}
% as the complexification of $\g_0$ (and equivalently indicating that $\g_0$ is the real form of the complex Lie algebra $\g$). Doing so allows the retention of certain properties of $\g_0$ while allowing complex coefficients yet retaining structure of interest from $\g_0$ (including decompositional structure). We can describe the real forms of $\g$ via $\g=\g_0 + i\g_0$, analogous to splitting $\C^n$ into $\R^{2n}$ (parametrising the imaginary part). In particular for $M\in M_n(\C)$ we have under this transformation (used in equation (\ref{eqn:qgml:complextorealmx}) below):
% \begin{align}
%     Z(M) &= \begin{pmatrix}
%         \text{Re} M & -\text{Im} M\\
%         \text{Im} M & \text{Re} M
%         \label{eqn:alg:complextorealmx}
%     \end{pmatrix}
% \end{align}


% \section{Cartan algebras and Root-systems}\label{sec:alg:Cartan algebras and Root-systems}
% \subsection{Complex Semi-simple Lie Algebras}\label{sec:alg:Complex Semi-simple Lie Algebras}
% Of central importance to later chapters in this work are what are known as Cartan decompositions of symmetric space Lie groups as a technique for solving certain classes of time-optimal quantum control problems. In this section, we provide a brief summary of Cartan decompositions, their relationship to Lie groups and algebras together with root systems and Dynkin diagrams. The section largely summarises standard work in the literature \cite{knapp_lie_1996,hall_beyond_2007,helgason_differential_1962,helgason_differential_1979}. Quantum information processing problems in this work (and much of the field) are often related to semisimple Lie groups and Lie algebras. In such cases, Cartan subalgebras $\h \subset \g$ are abelian and we are particularly interested in certain subclasses of maximally abelian subalgebras. The Cartan subalgebra forms the generators the adjoint action of which on $\g$ enable its root-space decomposition which in turn give rise to an abstracted root system. The root system can then in turn be related (given a fixed ordering or choice of basis) to simple roots. These roots can be used to form a basis of $\g$, from which a Cartan matrix and Dynkin diagram may be constructed. The relevance of root systems, Cartan matrices and such diagrams in quantum control settings is explored primarily in the final chapter of this work. In the following part, we define Cartan subalgebras and connect them with root systems and accompanying diagramatic and geometric intepretations. 

% A weight system (or set of weights) is associated with representations of a Lie algebra or Lie group. Weights are elements of the dual space (see definition \ref{defn:quant:Dual space}) of a Cartan subalgebra and label the eigenspaces of the representation with respect to the Cartan subalgebra.
% Root systems are primarily used in the classification and structure theory of Lie algebras, while weight systems are used in the study and classification of their representations. As noted in the literature, the process involves (a) identifying the (complex semi-simple Lie algebra) $\g$, (b) selecting a Cartan subalgebra $\h$, (c) constructing an abstract reduced root system, (d) selecting a choice of ordering and (e) then constructing a Cartan matrix.

% \subsection{Roots}\label{sec:alg:Roots}

% We define root systems as per below \cite{knapp_lie_1996,hall_lie_2013}. Given a subalgebra $\h \in \g$ with a (diagonal) basis $H$ and a dual space $\h^*$ with elements $e_j \in \h^*$, we recall that the duals are a [vector] space of functionals $e_j: V \to \C$. For a [matrix] Lie algebra, We can construct a basis of $\g$ given by $\{\h,E_{ij}\}$ where $E_{ij}$ is 1 in the $(i,j)$ location and zero elewhere. We are then interested in the adjoint action of elements of $H \in \h$ on each such eigenvector as:
% \begin{align*}
%     \ad_H(E_{ij}) = [H,E_{ij}] = (e_i(H)-e_j(H))E_{ij} = \alpha E_{ij}
% \end{align*}
% where $e_j$ sepects the $(j,j)^{th}$ element of a matrix (recalling duals $e_j(v)=v_j \delta_{ij}, v_j \in \C$ form a vector space of linear functionals). That is $\alpha = e_i - e_j$ is a linear functional on $\h$ such that $\alpha:\h \to \C$. Such functionals $\alpha$ are denoted roots. Thus $\g$ can be decomposed as:
% \begin{align}
%     \g = \h \oplus_{i\neq j} \C E_{ij} = \h \oplus_{\alpha \in \Delta} \g_\alpha \qquad \g_\alpha = \{X \in \g | \ad_H(X) = \alpha X, H \in \h \}
% \end{align}
% This is the root space decomposition of $\g$ with $X \in \g_\alpha$ the root vectors of root $\alpha$. As we see below, such decomposition is related to the existence of Cartan subalgebras and eventually Cartan decompositions, crucial to results in later chapters. The commutation relations are given by:
% \begin{align*}
% [\mathfrak{g}_{\alpha}, \mathfrak{g}_{\beta}] := \begin{cases}
% \mathfrak{g}_{\alpha + \beta} & \text{if } \alpha + \beta \text{ is a root} \\
% 0 & \text{if } \alpha + \beta \text{ is not a root or } 0 \\
% \subseteq \mathfrak{h} & \text{if } \alpha + \beta = 0.
% \end{cases}
% \end{align*}
% with $[E_{ij}, E_{ji}] = E_{ii} - E_{jj} \in \h$. Roots are then defined as positive or negative (with $-$ and may be ordered as a sequence. Each root is a  nongeneralised weight of $\ad_\h(\g)$ (a root of $\g$ with respect to $\h$). The set of roots is denoted $\Delta(\g,\h)$. 

% \subsection{Cartan subalgebras}\label{sec:alg:Cartan subalgebras}
% Given a Lie algebra representation, we can construct a system analogous to a root system, via a weight space and weight vectors, as follows.
% \begin{definition}[Weights]\label{defn:alg:weights}
%     Given a representation $\pi: \h \to V(\C)$ and roots $\alpha \in \h^*$, define the generalised weight space as:
%     \begin{align*}
%         V_\alpha = \{  v \in V | (\pi(H)-\alpha(H)1)^nv=0, \forall H \in \h \}
%     \end{align*}
%     for $V_\alpha\neq 0$.
% \end{definition}
% The elements of $v \in V_\alpha$ are generalised weight vectors with $\alpha$ the weights. If this condition holds, we say $\h$ is a nilpotent Lie algebra, such that there are finitely many generalised weights and $V = \oplus_\alpha V_\alpha$ (weight space decomposition). Weights needn't be linearly independent and are dependent upon roots. For a Lie algebra, we denote $V_\alpha$ as $\g_\alpha$. It can be shown that for such a nilpotent $\h$ relative to $\ad_g \h$ (the action on $\h$), the generalised weight vectors have the following properties: (a) $\g = \oplus \g_\alpha$, (b) $\h \subseteq \g_0$ and (c) $[\g_\alpha, \g_\beta] \subseteq \g_{\alpha + \beta}$ (zero if $\alpha + \beta$ is not a weight etc). Note that
% \begin{align*}
%     \g_\alpha &= \{  X \in \g | (\ad_H-\alpha(H)1)^nv=0, \forall H \in \h \}\\
%     \g = \h \oplus_{\alpha \in \Delta} \g_\alpha \label{eqn:alg:rootspace decompositiongalpha}
% \end{align*}
% i.e. $\pi$ is the adjoint action of $\h$ on $X \in \g$. Here $\g_0$ is then the weight space subalgebra associated with the zero weight under this adjoint action, it denotes the weight space corresponding to the zero weight in the decomposition of the Lie algebra $\g$ (the centralizer of $\h \in \g$). We come now to the definition of a Cartan subalgebra.
% \begin{definition}[Cartan subalgebra]\label{defn:alg:cartansubalgebra}
%   A Cartan subalgebra $\h \subset \g$ is a nilpotent Lie algebra of a finite-dimensional complex Lie algebra $\g$ such that $\h = \g_0$. Cartan subalgebras are maximally abelian subalgebras of $\mathfrak{g}$. 
% \end{definition}
% The algebra $\h$ is a Cartan subalgebra if it is the normalizer with respect to $\g$, that is if $N_\g(\h) = \{ X\in\g | [X,\h] \subseteq \h \}$. It can be shown that all finite complex Lie algebras $\g$ have Cartan subalgebras. For complex semisimple Lie algebras, Cartan algebras $\h$ are abelian ($B([H_k,H_j])=0$ for Killing-form $B$ and $H_k,H_j \in \h$). A Cartan subalgebra $\h$ is the maximally abelian subalgebra such that the elements of $\ad_\g(\h)$ are simultaneously diagonalisable. Moreover, all such Cartan subalgebras of $\g$ are conjugate via an automorphism of $\g$ in the form of an adjoint action. With this understanding of Cartan subalgebras we can now generalise the concepts of roots.

% \subsection{Root system properties} \label{sec:alg:Root system properties}
% Roots exhibit a number of properties \cite{knapp_lie_1996}. We set out a number of these relevant to results in later chapters and in particular our methods in Chapter \ref{chapter:Time optimal quantum geodesics using Cartan decompositions}. 
% \begin{definition}[Roots]\label{defn:alg:roots}
%     Non-zero generalised weights of $\ad_\h(\g)$ are [mapped isomporphically] denoted the \textit{roots} of $\g$ with respect to the Cartan subalgebra. Denote the set of roots $\alpha$ is $\Delta(\g,\h)$
% \end{definition}
% Given a Killing form $B(\cdot,\cdot)$, a few standard results hold: (a) $B(\g_\alpha,\g_\beta)=0$ for $\alpha,\beta \in \Delta$ (including $0$); (b) $\alpha \in \Delta \implies -\alpha \in \Delta$, (c) each root $\alpha$ is associated with a $H_\alpha \in \h$ such that we can identify a correspondence between the root functional and Killing form given by:
% \begin{align*}
%     \alpha(H) = B(H,H_\alpha) \qquad \forall H \in \h
% \end{align*}
% noting that $\Delta$ spans $\h^*$. Importantly we have that for each eigenvector $E_\alpha \in \g$ (non-zero) that:
% \begin{align*}
%     [H,E_\alpha] &= \alpha(H)E_\alpha
% \end{align*}
% (see \cite{knapp_lie_1996} for standard results e.g Lemma 2.18). Other results include that $\ad_\h(\g)$ is simultaneously diagonalisable, and that the Killing form has an expression in terms of the functional:
% \begin{align*}
%     B(H,H') = \sum_\alpha \alpha(H)\alpha(H') \qquad B: \h \times \h \to \C
% \end{align*}
% A few other standard results include normalisability (such that $B(E_\alpha,E_{-\alpha})=1)$ and standard commutation relations:
% \begin{align}
%     [H_\alpha,E_\alpha] &= \alpha(H_\alpha)E_\alpha & [H_\alpha,E_{-\alpha}] &= -\alpha(H_{-\alpha})E_{-\alpha} & [E_\alpha,E_{-\alpha}] &= H_\alpha
% \end{align}
% Finally in this section, we note concepts of relevance to Cartan matrices applied in the final chapter. We denote root strings, or $\alpha$-strings as follows: given $\alpha \in \Delta, \beta \in \Delta \cup \emptyset$, the $\alpha$-string that contains $\beta$ is the set of all elements $\beta + n\alpha \in \Delta \cup \emptyset$ for $n \in \Z$. Essentially denoting a (symmetric) string of roots $\beta + n\alpha$ for $-p \leq n \leq q$ ($p,q \geq 0)$ with:
% \begin{align*}
%     p-q = \frac{2\braket{\beta,\alpha}}{\braket{\alpha,\alpha}}
% \end{align*}

% %====Abstract root systems
% \subsection{Abstract root systems}\label{sec:alg:Abstract root systems}
% Abstract root systems are important ways of capturing the essence of the symmetries within a Lie algebra via enabling the construction of relations among roots that may be interpreted using the formalism and language of symmetry. 
% \begin{definition}[Root System]\label{defn:alg:Root System}
% A root system $(V, \Delta)$ is a finite-dimensional $\Delta \in V(\R)$ equipped with an inner product $\langle \cdot , \cdot \rangle$ and norm $|\cdot |^2$ with a subset $\Delta = \{\alpha \in V | \alpha \neq 0 \}$ satifying (a) $V = \text{span}(\Delta)$, (b) $\alpha \in \Delta$ and $c \in \mathbb{R} \implies c\alpha \in \Delta$ only if $c = \pm 1$, (c) given the linear transformation $s_{\alpha}$:
% \begin{align*}
%     s_{\alpha} \cdot \beta = \beta - 2 \frac{\langle \beta, \alpha \rangle}{\langle \alpha, \alpha \rangle} \alpha, \quad \beta \in E
% \end{align*}
% for $\alpha,\beta \in \Delta$ then $s_{\alpha} \cdot \beta$ and (d):
% \begin{align*}
%     \frac{\langle \beta, \alpha \rangle}{2 \langle \alpha, \alpha \rangle} \in \Z
% \end{align*}
% \end{definition}
% The rank of $V=\dim(V)$. The elements $\alpha \in \Delta$ are roots. Moreover, $\alpha \in \Delta \implies -\alpha \in \Delta$. A root system is reduced if it satisfies (a) to (d) above, or non-reduced if it doesn't satisfy (b). Symmetric spaces root systems of interest in this work are of the non-reduced type. $s_\alpha$ is a reflection about the hyperplane with respect to $\alpha$ (an orthogonal transformation with determinant $-1$). Such reflections are said to generate an orthogonal group of $V$, the Weyl group $W$, generated by such reflections. This general formulation allows root systems to be associated to all complex semisimple Lie algebras. 
% A reduced abstract root system in $\h_0^*$ is one where $\alpha \in \Delta$ but $2\alpha \notin \Delta$. Familiar Lie algebraic concepts apply to root systems: \textit{reducible} root systems (orthogonal decompositions $V = \oplus V_k$ such that $\alpha$ belongs to a $V_k$) and corresponding irreducible root systems. Standard results show isomorphisms between root systems. An important element in the geometric characterisation of root systems is set out below. Given $\alpha,\beta \in R$ (linearly independent) and $\braket{\alpha,\alpha} \geq \braket{\beta,\beta}$ it can be shown that there are limited allowed angles $\theta$ and length ratios among the roots via the proposition that: (a) $\braket{\alpha,\beta}=0$, (b) $\braket{\alpha,\alpha} = \braket{\beta,\beta}$ with $\theta=\pi/3$ or $2\pi/3$, (c) $\braket{\alpha,\alpha} = 2\braket{\beta,\beta}$ (for $\theta=\pi/4,3\pi/4)$ or (d) $\braket{\alpha,\alpha} = 3\braket{\beta,\beta}$ (for $\theta=\pi/6,5\pi/6)$. If $\theta \in (\pi/2,\pi)$ (obtuse) then $\alpha+\beta$ is a root or $\theta \in (0,\pi/2)$ then $\pm(\alpha-\beta)$ are roots. These angles can be used to plot the relevant root system (see Chapter \ref{chapter:Time optimal quantum geodesics using Cartan decompositions}). In more general settings, the geometric representation of roots, under certain assumptions, then exhibits certain permutation symmetries and the applicable Weyl group is defined in terms of these. 

% One final concept before coming to the Cartan matrix is that of fixing a lexicographic ordering related to the concept of positivity of roots. Given such a set of roots:
% \begin{align*}
%     \Delta = \{\alpha_1, \alpha_2, \ldots, \alpha_l\}
% \end{align*}
% we introduce an ordering as follows. A root $\beta = \sum_{i=1}^l b_i\alpha_i$ is positive with respect to the lexicographic ordering if the first non-zero coefficient $b_j$ in its expansion with respect to the basis $\Delta$ is positive. Conversely, the root $\beta$ is negative if this first non-zero coefficient is negative. The lexicographic order is defined by comparing roots: for two distinct roots $\beta = \sum_{i=1}^l b_i\alpha_i$ and $\gamma = \sum_{i=1}^l c_i\alpha_i$ in $\Phi$, we say that $\beta > \gamma$ if, at the first index $j$ where $b_j$ and $c_j$ differ, we have $b_j > c_j$. This comparison allows partitioning the root system into two disjoint sets $\Delta^+$ and $\Delta^-$ of positive and negative roots.  

% The highest root in a root system is the maximal element with respect to this lexicographic ordering and is always a positive root. This root plays a pivotal role in the structure and representation theory of semisimple Lie algebras.

% As we articulate in Chapter \ref{chapter:Time optimal quantum geodesics using Cartan decompositions}, the construction of the abstract root system for Lie algebras (related to quantum control problems of interest) involves determining root systems. We note that $\alpha$ is \textit{simple} if $\alpha > 0$ and it is linearly independent of other roots. It can be shown that any positive root can be decomposed as $\alpha = \sum_i n_i \alpha_i$ (with $\alpha_i$ simple and $n_i \geq 0$). The sum of $n_i$ is an integer denoted the \textit{level} of $\alpha$ with respect to the set of simple roots (important as the set of simple roots generates the entire root system through integer linear combinations).


% \subsection{Cartan matrices}\label{sec:alg:Cartan matrices}
% \hl{We now define the Cartan matrix used in Chapter} \ref{chapter:Time optimal quantum geodesics using Cartan decompositions}. To do so we fix a root system $\Delta$, assume each $\alpha \in \Delta$ is reduced and fix an ordering as per above. Data from Cartan matrices may be represented in diagrammatic form via Dynkin diagrams.
% \begin{definition}[Cartan matrix]
%     Given $\Delta \in V$ and simple root system $\Pi = {\alpha_k}$, $k=1,...,n=\dim V$, the Cartan matrix of $\Pi$ an $n \times n$ matrix $A = (A_{ij})$ where:
%     \begin{align}
%         A_{ij} = 2\frac{\braket{\alpha_i,\alpha_j}}{|\alpha_i|^2}
%     \end{align} 
% \end{definition}
% A variety of other standard properties apply to abstract root systems $\Delta$ constraining the roots and their ratios (e.g. $2\braket{\beta,\alpha}/|\alpha^2|=0,\pm 1,\pm 2, \pm 3, \pm 4$ and $\pm 1$ if $\alpha,\beta$ are non-proportional with $|\alpha| \leq |\beta|$). These and other constraints limit the ratios and relation of roots in ways that allow their representation in terms of Cartan matrices and diagrammatic representations. Different orderings (enumerations) of $\Pi$ lead to different $A_{ij}$, however they are all conjugate to each other. Cartan matrices satisfy certain properties e.g. $A_{ij} \in \Z, A_{ii}=2, A_{ij}\leq 0 (i\neq j), A_{ij}=0 \leftrightarrow A_{ji}=0$ and the existence of a diagonal matrix $D$
% that renders $A$ symmetric positive definite under conjugation. The (multiple) block diagonality of a Cartan matrix implies its reducibility, otherwise the matrix is irreducible. From the Cartan matrix, we can construct a Dynkin diagram (as distinct from a root diagram) as follows. 

% %===Dynkin diagram

% \begin{definition}[Dynkin diagram]\label{defn:alg:dynkindiagram}
%     A Dynkin diagram is a graph diagrm of a set of simple roots $\Pi$. Let each simple root $\alpha_i$ be a vertex of the graph, with a weight proportional to $\braket{\alpha_i,\alpha_i} = |\alpha_i|^2$. The graph construction rules are as follows. Two simple roots  $\alpha_i,\alpha_j$ are connected by $A_{ij}A_{ji}$ edges (which may be zero).
% \end{definition}
% While Dynkin diagrams are not focus for use in this work, we do relate them to quantum control results in the final chapter, hence here we mention a few sundry properties. For an $\l \times l$ Cartan matrix $A$, the associated Dynkin diagram has the following structure: (a) there are at most $l$ pairs of vertices $i<j$ having one edge (at least) between; (b) the diagram has no loops; and (c) at most three edges (triple points) connect to any node. The Cartan matrix may be used to determine a Dynkin diagram (up to scaling factors). 

% %=====Dynkin diagrams 

% \begin{figure}[h]
% \centering
% \begin{tikzpicture}
%   % Define the style for the nodes
%   \tikzset{dynkinnode/.style={circle, draw, minimum size=25pt, inner sep=0pt}}
  
%   % Draw the first node
%   \node[dynkinnode] (first) {};
  
%   % Label above the first node
%   \node[above=1mm of first] {1};
  
%   % Label below the first node
%   \node[below=1mm of first] {$\alpha_1$};

  
  
%   % Draw the second node
%   \node[dynkinnode] (second) [right=2cm of first] {};

%   \node[below=1mm of second] {$\alpha_2$};

%   % Draw the third node
%   \node[dynkinnode] (third) [right=2cm of second] {};

%   % Label below the third node
%   \node[below=1mm of third] {$\alpha_n$};
  
%   % Connect the nodes
%   \draw[-] (first) -- (second);
%   \draw[dashed] (second) -- (third);
% \end{tikzpicture}
% \caption{Expanded Dynkin diagram of type \( A_n \) with labeled vertices and edges. The numbers above the nodes indicate the length of the roots relative to each other. $A_{ij}A_{ji}$ determines the number of lines (or the type of connection) between vertices $i$ and $j$. This product can be 0 (no connection), 1 (single line), 2 (double line), or 3 (triple line), representing the angle between the corresponding roots. Additionally, when $A_{ij}A_{ji} > 1$, an arrow is drawn pointing from the longer root to the shorter root. }
% \label{fig:alg:dynkin_diagram_an_expanded}
% \end{figure}
% By constructing an abstract reduced root system, one can then show that for two complex semisimple Lie algebras with isomorphic abstract reduced root systems, the associated Cartan matrices are isomorphic.  If two complex semisimple Lie algebras have the same Dynkin diagram, they are isomorphic, thereby sharing the same algebraic structure. Operations on Cartan matrices correspond to operations on Dynkin diagrams, allowing visualisation of transformations. It can be shown that the choice of Cartan matrix is independent of the choice of positive ordering up to a permutation of index and that the Cartan matrix determines the reduced root system. The Weyl group, as the set of orthogonal transformations , can be used to deteremine $\Delta^+$ and $\Pi$.


% \section{Cartan decompositions}\label{sec:alg:Cartan decompositions}
% An important set of theorems for the results in Chapters \ref{chapter:Quantum Geometric Machine Learning} and \ref{chapter:Time optimal quantum geodesics using Cartan decompositions} are those related to the Cartan decomposition of semisimple Lie groups and their associated algebras. The Cartan decompsoistion allows decomposition of a classical matrix Lie algebra into Hermitian and skew-Hermitian components. For a given a complexified semisimple Lie algebra $\g = \g_0^\C$, a corresponding Cartan involution $\theta$ is associated with the decomposition $\g = \k \oplus \p$. In turn, this allows a global decomposition of $G=KAK$ where $K = e^\k$ and $A = e^\a$ where $\a \subset \p$ (a maximal abelian subspace of $\p$), which is a generalisation of polar decompositions of matrices. Of importance to our result in our final chapter is that Cayley transforms (see below) may be used to transform between any Cartan subalgebras up to conjugacy. We use this result to define our appropriate control decomposition in Chapter \ref{chapter:Time optimal quantum geodesics using Cartan decompositions}. We briefly set out relevant background theory below, before moving to geometric concepts and interpretation.  

% \subsubsection{Compact Real Forms} \label{sec:alg:Compact Real Forms}
% For classical semisimple groups, the matrix Lie algebra $\g_0$ over $\R,\C$ is closed under conjugate transposition, in which case $\g_0$ is the direct sum of its skew-symmetric $\k_0$ and symmetric $\p_0$ members. Recall from equation (\ref{eqn:su3:liealgebracomplexification}) that complexification of $\g_0$ is denoted $\g = \g_0^\C = \g_0 + i\g_0$. The real Lie algebra $\g_0$ has a decomposition as the direct sum $\g_0 = \k_0 \oplus \p_0$. We can construct a real vector space of complex matrices (that is, where coefficients of matrices are real) as $\u_0 = \k_0 + i\p_0$ as a subalgebra. As Knapp notes \cite{knapp_lie_1996}, there are certain requirements with respect to $\g_0$ and $\u_0$ such as $\k_0 = \g_0 \cap \u_0$ and $\p_0 = \g_0 \cap i\u_0$ which allow us to decompose $\g_0 = \k_0 \oplus \p_0$ in a way that in turn allows the complexification:
% \begin{align}
%     \g = \k \oplus \p
% \end{align}
% As the focus of this work is geometric and machine learning techniques for Lie groups and algebras of relevance to quantum control, we omit specific standard steps showing the complexification of $\g = \k_0 \oplus \p_0$ from this work, see \cite{knapp_lie_1996,knapp_representation_2001,hall_lie_2013} for more detail. Note that we can define the mapping $\theta(X) = -X^\dagger$ (negative of complex conjugate transpose) as an involution (that squares to identity) with $\theta[X,Y] = [\theta(X),\theta(Y)]$. We then define a Cartan involution as follows.
% \begin{definition}[Cartan involution]\label{defn:alg:cartaninvolution}
%     Given a Killing form $B$, $X,Y\in\g$ and an involution $\theta$, a Cartan involution is a positive definite symmetric bilinear form:
%     \begin{align}
%         B_\theta(X,Y) = -B(X,\theta Y)
%     \end{align}
% \end{definition}
% It can be shown (see below) that involutions on $\g_0$ [induce] Cartan involutions on $\g$ (for complex semisimple $\g$, the only Cartan involutions of $\g^\R$ are conjugations with respect to real forms of $\g$). 
% Cartan involutions are conjugate up to inner automorphisms Int$\g$. This result is related to the existence statement that $\g$ is equipped with a Cartain involution which are so conjugate (the proofs are usually via $\g_0$ which is then complexified). From the existence of this involution, we infer the existence of the relevant Cartan decomposition.
% %===========
% \begin{definition}[Cartan decomposition]\label{defn:alg:cartandecomposition}
%     Given a complex semisimple Lie algebra $\g$ with Cartan involution $\theta$, $\g$ can be decomposed as:
%     \begin{align}
%         \g = \k \oplus \p
%     \end{align}
%     with $\k$ the +1 symmetric eigenspace $\theta(\k)=\k$ and $\p$ the -1 anti(skew)symmetric eigenspace $\theta(\p)=-\p$ satisfying the following commutation relations:
%     \begin{align}
%         &[\k,\k] \subseteq \k &[\k,\p] &\subseteq \p & [\p,\p] \subseteq \k
%     \end{align}
% \end{definition}
% Here $\k,\p$ are orthogonal with respect to the Killing form in that $B_\g(X,Y)=0=B_\theta(X,Y)$ i.e. for $X \in \k$ and $Y \in \p$ we have $B(X,Y) = 0$. For the corresponding Lie group $G$, then the existence of the Cartan decomposition of $\g$ (where $K \subset G$ is analytic with Lie algebra $\k$) gives rise to a global Cartan decomposition of $G$. The global Cartan decomposition $G = K \exp(\p)$ together with the fact that $\p = \bigcup_{k \in K}\Ad_k\a$ means that the global Cartan decomposition is expressible as $G=KAK$ which we define below. 
% \begin{definition}[KAK Decomposition]\label{defn:alg:KAKdecomposition}
%     Given $G$ with a Cartan decomposition as in (\ref{defn:cartandecomposition}), $G$ can be decomposed as $G=KAK$ where $K = \exp(\k), A=\exp(\a)$. Every element $g \in G$ thus has a decomposition as $g=k_1 a k_2$ where $k_1,k_2 \in K, a \in A$
% \end{definition}
% Where such a Cartan decomposition is obtainable, then we denote (as discussed further on) $G/K$ as a global Riemannian symmetric space. Note that in this case we can decompose an arbitrary $U \in G$ as:
% \begin{align}
%     U = kac \qquad U = pk \label{eqn:alg:cartankakandpk}
% \end{align}
% where $k,c \in \exp(\k) = K$ and $p \in \exp(\p)$. 

% The Cartan decompositions of semi-simple Lie algebras and groups is central to results in our final chapter. It is also important to results relevant to Chapter \ref{chapter:Quantum Geometric Machine Learning} given the role of Cartan decompositions in quantum control formalism \cite{khaneja_cartan_2001,khaneja_optimal_2005,brockett_sub-riemannian_nodate,dalessandro_introduction_2007}. In particular, we rely upon the $KAK$ decomposition and the assumption that $a \in \exp(\a)$ is parametrised by a constant parameter (the `constant-$\theta$' property) which, as we demonstrate, simplifies the minimisation problem for finding certain time (and energy) optimal sequences of unitaries.

% \subsubsection{Compact and non-compact subalgebras}\label{sec:alg:Compact and non-compact subalgebras}
% For our results in Chapter \ref{chapter:Time optimal quantum geodesics using Cartan decompositions}, we require transformation of the relevant Cartan subalgebra (e.g. for $\su(3)$) to one which is [maximally non-compact] in order to prove our results relating to time-optimal control. In our case this is because we require our maximally abelian subalgebra $\a \in \h$ to be an element of our control subalgebra, i.e. we require $\a \in \p$. As noted, for Cartan decompositions $\g = \k \oplus \p$ with associated involutions, the Cartan subalgebras $\h \subset \g$ are conjugate up inner automorphisms of $\g$ (denoted $\g$, namely those which have a representation as conjugation by an element $g \in G$), that is $\h' = \text{Int}_g(\h) = g \h g^\inv$. In the literature, it can be shown that in particular any such $\h$ is thereby conjugate to a $\theta-$stable Cartan subalgebra (for involution $\theta$). Importantly, this means that we can decompose the Cartan subalgebra as $\h = \t \oplus \a$ where $\t \in \k, \a \in \p$. [As Knapp notes, the roots of $(\g,\h)$ are real on $\a_0 \oplus i\t_0$]. The [subsets] $\t$ and $\a$ are compact and non-compact subsets of $\h$, with $\dim \t$ being the compact dimension and $\dim \a$ being the compact dimension. The Cartan subalgebra $\h = \t \oplus \a$ is maximally compact if its compact subalgebra is as large as possible and maximally noncomopact in the converse case. As $\a \in \p$, for a given Carten decomposition, $\h$ is maximally compact if and only if $\a$ is a maximally abelian subspace of $\p$. Maximally noncompact $\h$ are conjugate via $K$ (and it can be shown that up to conjugacy in Int$\g_0$ there are only finitely many Cartan subalgebras of $\g$).

% %====Cayley transforms
% \subsubsection{Cayley transforms}\label{sec:alg:Cayley transforms}
% As we discuss in Chapter \ref{chapter:Time optimal quantum geodesics using Cartan decompositions}, our Cartan decomposition for quantum control problems related to symmetric spaces requires $\a \in \h$. That is, we seek a maximally noncompact Cartan subalgebra. As we note above, Cartan subalgebras $\h$ are conjugate to other Cartan subalgebras via a transformation of the form $h' = K\h K^\inv$. In certain cases, such as the typical Cartan decomposition of $SU(3)$ that we explicitly explore in our final chapter, $\h$ is not maximally non-compact (e.g. for $\su(3)$ choosing $\h = \{ \lambda_3, \lambda_8\}$ Gell-man generators renders $\h \in \k$ while $\h \cap \p = \null$. To remedy this, we apply Cayley transforms. There are two types of Cayley transforms: (a) one constructed from an imaginary noncompact root $\beta$ (denoted by Knapp as $c_\beta$) whose application to $\h$ causes the intersection $\h \cap \p$ to increase by one dimension; and (b) another constructed from a real root $\alpha$ (denoted by Knapp as $d_\alpha$) whose application to $\h$ causes the intersection $\h \cap \p$ to decrease by one dimension. Our interest is in the first of these, $c_\beta$. An example of the form of such a transformation for $\sl(2,\C)$ is given by:
% \begin{align}
%     c_\beta &= \Ad\left(\exp\left(i\frac{\pi}{4}X\right)\right) \qquad X = \overline{E}_\beta + E_\beta \in \g_\beta \subset \p
% \end{align}
% where $E_\beta \in \g_\beta, \overline{E}_\beta \in \g_{-\beta}$. In our example, we choose $\gamma = (1,\sqrt{3})$ such that:
% \begin{align*}
%     E_\gamma + E_{-\gamma} = \lambda_4
% \end{align*}
% Having covered key elements of algebra and representation theory relevant to our later chapters, we now cover relevant background in differential geometry and then geometric control theory. Our focus is largely on the synthesis of geometric and algebraic formalism, where specific Lie groups are represented in terms of differential manifolds, Lie algebras in terms of fibre bundles (the Lie algebra of a Lie group can be associated with the structure group of a principal fiber bundle, and Lie algebra-valued differential forms play a crucial role in defining connections on these bundles) and where transformations are given in terms of connections (such as Levi-Civita and others). We also relate basic elements of the theory of Riemannian and subRiemannian manifolds, geodesic theory and the application of variational methods to the theory of Lie algebras and groups articulated above in a quantum context. Finally, we integrate our algebraic and geometric exegesis into the context of geometric control theory, with a specific focus on quantum control relevant to the main results of this work. 





==> ebackupChapter4a.tex <==
% %=========BACKGROUND: QUANTUM MACHINE LEARNING CHAPTER

% \chapter{Background: Quantum Machine Learning}
% \label{chapter:Background: Classical, Quantum and Geometric Machine Learning}

% \section{Introduction}
% In this section, we survey literature from classical and machine learning relevant to later chapters. We include a high-level review of key concepts from classical machine learning, statistical learning theory and [other statistical methods] for both context and utility. We then summarise with a short overview the burgeoning field of quantum machine learning. We track how quantum analogues of classical machine and classical statistical learning have developed, noting key similarities and differences. In particular we provide an [in-depth] analysis of of learning in a quantum context, with a specific comparative analysis between quantum and classical backpropagation techniques. We map learning in quantum contexts with established results related the learnability of quantum algorithms \cite{aaronson_learnability_2007}. We also focus on the relationship between learning (in both classical and quantum contexts) and measurement, emphasissing the classical-quantum nature of QML learning protocols (in the main). We then examine how techniques from geometry, algebra and representation theory have been specifically (and relatively recently, in some cases) integrated into both classical and quantum machine learning strategies. In doing so, we provide a survey overview of geometric machine learning, together with the use of representation theory and differential geometry in relevant aspects of classical machine learning. We then briefly summarise recent results in invariant and geometric QML \cite{cerezo_building_2019,cerezo_cost_2021,cerezo_variational_2021,cerezo_challenges_2022} as a final contextualisation before our subsequent chapter introducing the first result on quantum geometric machine learning.

% % \section{Classical machine learning}

% % \section{Deep learning}
% \section{The Nature of Learning}\label{sec:ml:The Nature of Learning}

% \subsection{Taxonomies of learning}\label{sec:ml:Taxonomies of learning}
% The nature of learning in classical and quantum information science is a rich and widely studied problem. In this section, we set out a brief synopsis of key principles of machine learning, including foundational elements of supervised and unsupervised models, architectural principles regarding data, models and loss functions. We cover principles behind training, optimisation, regularisation and generalisation, together with the primary classes of algorithm used in this work. Our treatment focuses on both classical and quantum forms of machine learning. 
 

% A common taxonomy for approaching learning problems involves classifcation in terms of concepts of data, modelling, risk/loss and algorithm type (supervised or unsupervised learning) \cite{schuld_machine_2021}. The concept of \textit{learning} is then manifest in the ability of a model to accurately predict or reproduce known information (such as labels from training data) and to generalise to out-of-sample data well. Other adjuncts for characterising learning of algorithms include algorithmic expressibility or complexity mesures \cite{aaronson_quantum_2013} [\textbf{AARONSON Learnability}] The \textit{model} is then represented as an algorithm which achieves these objectives, as measured by figures of merit, such as empirical risk, training and generalisation error, algorithmic complexity and others. We discuss these in more detail with our summary of statistical learning theory concepts below. In many cases, the models in question, both classical and quantum, are extensions of well-understood statistical modelling techniques, such as generalised linear models \cite{mccullagh_generalized_1989,hastie_elements_2013}, graphical models, kernel methods \cite{cristianini_introduction_2000} or deep-learning algorithms \cite{goodfellow_deep_2016}. Quantum machine learning adapts concepts from modern machine learning (and statistical learning) theory to develop learning protocols for quantum data, or using quantum algorithms themselves. More recently, generative models \cite{wolf_transformers_2020,vaswani_attention_2017} have been adapted in quantum settings. The landscape of QML is already vast thus for the purposes of our work it will assist to situate our results within the useful schema set out in \cite{schuld_machine_2021} below in Table (\ref{table:quantumclassical}). Our results in Chapters \ref{chapter:QDataSet and Quantum Greybox Learning} and \ref{chapter:Quantum Geometric Machine Learning} fall somewhere between the second (classical machine learning using quantum data) and fourth (quantum machine learning for quantum data) categories, whereby we leverage classical machine learning and an adapted bespoke architecture equivalent to a parametrised quantum circuit \cite{benedetti_parameterized_2019} (discussed below). 

% %===QUANTUM CLASSICAL TABLE
% \begin{center}
% \begin{table}
% \begin{tabular}{ |p{3cm}||p{3cm}|p{3cm}|p{3cm}|  }
%  \hline
%  \multicolumn{4}{|c|}{QML Taxonomy} \\
%  \hline
%  \textbf{QML Division}  & \textbf{Inputs} & \textbf{Outputs} & \textbf{Process} \\
%  \hline
%  Classical ML   & Classical    & Classical &   Classical \\
%  \hline
%  Applied classical ML &   Quantum (Classical)  & Classical (Quantum)   & Classical\\
%  \hline
%  Quantum algorithms for classical problems &Classical & Classical&  Quantum\\
%  \hline
%  Quantum algorithms for quantum problems    &Quantum & Quantum&  Quantum\\
%  \hline
% \end{tabular}
% \caption{Quantum and classical machine learning table. Quantum machine learning covers four quadrants (listed in `QML Division') which differ depending on whether the inputs, outputs or process is classical or quantum.}
% \label{table:quantumclassical}
% \end{table}
% \end{center}
% % \begin{itemize}
% %     \item Data
% %     \item Models
% %     \item Risk and Loss
% %     \item Supervised and Unsupervised learning
% % \end{itemize}

% % \subsubsection{Risk minimisation in supervised and unsupervised learning}:
% % \begin{itemize}
% %     \item Minimising empirical risk as a proxy
% %     \item Quantifying generalisation
% %     \item Optimisation
% %     \item Unsupervised learning
% % \end{itemize}

% % Classical machine learning methods:
% % \begin{itemize}
% %     \item (Generalised) linear models
% %     \item Neural networks
% %     \item Graphical models
% %     \item Kernel methods
% %     \item Generative models
% % \end{itemize}

% % \subsection{Encoding data}
% % \begin{itemize}
% %     \item Basis encoding (single input and superposition)
% %     \item Amplitude encoding (amplitude efficient and qubit efficient state preparation)
% %     \item Time-evolution encoding
% %     \item Hamiltonian encoding (Hamiltonian simulation, qubit-efficient Hamiltonian simulation, density matrix exponentiation)
% %     \item Data encoding as a feature map
% % \end{itemize}

% % Quantum algorithms:
% % \begin{itemize}
% %     \item State discrimination
% %     \item Search (Grover)
% %     \item Quantum phase estimation
% %     \item Matrix multiplication and inversion
% %     \item Variational quantum algorithms
% %     \item Quantum annealling
% % \end{itemize}

% % \subsubsection{Variational quantum models}
% % \begin{itemize}
% %     \item Quantum circuits as models
% %     \item Probabilistic and quantum models
% %     \item Variational quantum classifier 
% %     \item Variational quantum generator
% %     \item Functions expressed by quantum models (linear combinations of periodic functiosns)
% % \end{itemize}

% % Training variational models:
% % \begin{itemize}
% %     \item Gradients of quantum computations
% %     \item Parameter shift rules
% %     \item Barren plateaus
% %     \item Generative training
% % \end{itemize}

% % Quantum models as kernel methods:
% % \begin{itemize}
% %     \item Connection between quantum models and kernels
% %     \item Quantum computing, feature maps and kernels
% % \end{itemize}

% \section{Statistical Learning Theory}\label{sec:ml:Statistical Learning Theory}
% % \subsection{What does it mean to learn?}

% \subsection{Classical statistical learning theory} \label{sec:ml:Classical statistical learning theory}
% The formal theory of learning in computational science is classical statistical learning theory \cite{vapnik_nature_1995,james_introduction_2013,vapnik_overview_1999,hastie_elements_2013} which sets out theoretical conditions for function estimation from data. In the most general sense, one is interested in estimating $Y$ from as some function of $X$, or $Y = f(X) + \epsilon$ (where $\epsilon$ indicates random error independent of $X$). Statistical learning problems are typically framed as \textit{function estimation models} \cite{vapnik_nature_1995} involving procedures for finding optimal functions $f: \mathcal{X} \to \mathcal{Y}, x \mapsto f(x) = y$ (where $\X,\Y$ are typically vector spaces) where it is usually assumed that $X,Y \sim \Prb_{XY}$ i.e. random variables drawn from a joint distribution with realisations $x,y$ respectively. Formally, this model of learning involves (a) a generator of the random variable $X \sim \Prb_X$, (a) a supervisor function that assigns $Y_i$ for each $X_i$ such that $(X,Y) \sim \Prb_{XY}$ and (c) an algorihtm for learning a set of functions (the hypothesis space) $f(X,\Theta)$ where $\theta \in \Theta$ parametrises such functions.

% Typically $X$ are denoted the features and $Y$ are denoted the labels. Feature and label data is usually classified into \textit{discrete} or \textit{continuous} data. The two primary types of learning problems are supervised and unsupervised learning (defined below) where the aim is to learn a \textit{model family} $\{f\}$ or distribution $\Prb$. 
% \begin{definition}[Supervised learning]
%     Given a sample $D_n = \{ X_i, Y_i\}$ comprising tuples $(X_i, Y_i) \in \mathcal{X} \times \mathcal{Y}$ (where for simplicity it is assumed $D_n$ is i.i.d) where $X,Y \sim \Prb_{XY}$, a supervised learning task consists of learning the mapping $f: \X \to \Y$ for both in-sample and out-of-sample $(X_i,Y_i)$.
% \end{definition}
% \textit{Unsupervised learning} is defined as for $D = \{X_i\}, X \sim \Pr_X$ unsupervised learning does not utilize corresponding output labels $Y_i$ for each input $X_i$. Instead, the objective is to discover underlying patterns, structures, or distributions within the dataset $D_n$, such as clusters or classifications. \textit{Semi-supervised} learning is where some but not all $X_i$ are labelled. \textit{Self-supervised learning} is where a model $f$ is trained on data in $\X$ itself (e.g. where traditionally unlabelled data is used in effect as a label, such as where $\X$ is a sequence of data and each element in the sequence is predicted using the previous items in the sequence). The primary subject of this work is supervised learning of unitary operators as elements of Lie groups of relevance to quantum information processing, with a focus on $U(t) \in G$ for $G=\text{SU}(2)$ or SU(3). 

% Finding optimal functions intuitively means minimsing the error $\epsilon = |f(x)-y|$ for a given function. This is described generically as \textit{risk minimisation} where, as we discuss below, there are various measures of risk (or uncertainty) which typically are expectations (averages) of loss. Moreover, the objective of supervised learning then becomes one of \textit{generalisation}, which is intuitively the mininimsation of risk across both in-sample and out-of-sample data. More formally, given a loss function $L:Y \times y \to R, (f(x),y) \mapsto L(f(x),y)$ and a joint probability distribution over $X \times Y$ denoted by $(X,Y) \sim P_{XY}$ and associated density $p_{XY}$ (with usual assumptions regarding applicable measure, Lebesgue for continuous, counting for discrete), then an expectation operator can be defined as:
% \begin{align}
%     E[f(X,Y)] = \int f(x,y)d P_{XY}(x,y) = \int f(x,y) p_{XY}(x,y)
% \end{align}
% The \textit{statistical risk} or \textit{true risk} of $f$ is then given by:
% \begin{align}
%     R(f) = E[L(f(X),Y) | f] \label{eqn:ml:statlearning true risk}
% \end{align}
% Statistical risk is an [average] estimator, representing the average (expected) loss of $f$ with respect to $L$. The minimum risk (\textit{Bayes risk}) is the infimum of $R(f)$ over all such measureable functions (learning rules) $f$ denoted $R^* = \underset{f \in \mathcal{F}}{\inf} R(f)$. Of course the challenge is that $P_{XY}$ is usually not known such that the estimation of $f$ relies upon random samples of training data comprising $n$ examples of input $x$ and label $y$ data, denoted $D_n = \{ X_i, Y_i\}^n$ (where for simplicity it is assumed $D_n$ is i.i.d). The learning task then becomes framed as finding an estimate $\hat{f}$ of $f$ (conditional upon $D_n$) among a set of functions (preduction rules) $\mathcal{F}$. This functional estimator conditioned on the sample is denoted $\hat{f}_n(x) = f(x; D_n)$. The learning objective then aims to minimise $R(\hat{f}_n)$ with high probability over the distribution of data, i.e. we want to minimise the \textit{expected risk} given by $E[R(\hat{f}_n)]$. Intuitively this means the average error (risk) of the prediction rules is minimised over the distribution (of samples) $D_n$ i.e. $\hat{f}_n$ [performs well] on average across $D_n$. [As \textbf{Castro} notes], the objective here is not to minimise a specific $f$, but to optimise the selection rule of $f \in \mathcal{F}$ given training data $D_n$ (i.e the algorithm that selects $f$ for a given $D_n$). 


% \subsubsection{Empirical risk}\label{sec:ml:Empirical risk}
% The concept of \textit{empirical risk} then enables an estimation of statistical risk on out of sample (unseen) data using $D_n$ is defined as follows \cite{vapnik_overview_1999}.
% \begin{definition}[Empirical risk]\label{eqn:ml:empiricalrisk}
%     Given a sample $D_n = \{X_i,Y_i\}^n$, loss function $L$ and family of [classifiers] $F$, the empirical risk is denoted:
%     \begin{align}
%     \hat{R}_n(f) = \frac{1}{n}\sum_i^n L(F(X_i),Y_i)  
%     \label{eqn:empiricalrisk}
% \end{align}
% \end{definition}
% The objective then becomes learning an algorithm (rule) that minimises empirical risk, thereby obtaining [a best] estimator across sampled and out-of-sample data, namely:
% \begin{align}
%     \hat{f}_n = \arg \underset{f \in \mathcal{F}}{\min} \hat{R}_n(f)
%     \label{eqn:fhatopt}
% \end{align}
% i.e. the $f$ that minimises $\hat{R}$. As the number of samples $n \to \infty$, then by assumption (of i.i.d. $D_n$), $\hat{R}(f) \to R(f)$. [As we discuss in more detail], (\ref{eqn:empiricalrisk}) is typically reflected in (batch) gradient descent methods that seek to solve for the optimisation task (\ref{eqn:fhatopt}). [Part of the success of neural network machine learning architectures in [such model selection tasks] lies in the [(classical) superposition] of functional estimators along with the connected nature of such networks, which enables (via backpropagation typically) [correlations] among candidate $\hat{f}$ and $D_n$ in ways that minimise empirical risk (as we discuss). Typical gradient descent rules adopt an \textit{update} rule, which can usefully (for the purposes of comparison with quantum) be conceived of as a state transition rule. An important (and dominant) class of optimisation algorithm is gradient descent (and backpropagation) which requires constraining estimators $\hat{f}$ that enable $\hat{R}_n(f)$ to be \textit{smooth} (continuous, differentiable), a requirement of $f \in C^k$, the class of all $k$-differentiable functions (ideally $C^\infty)$. Moreover, it is typical that $f$ is chosen to be a \textit{parameterised} function $f = f(\theta)$ such that the requisite analytic structure (parametric smoothness) is provided for by the parametrisation, typically where parameters $\theta \in \mathbb{R}_\theta$. The parameters $\theta$ are often denoted the \textit{weights} of a neural network, for example where $\hat{R}_n(f(\theta))$ is often just denoted as a function of the parameters (given the data is fixed). \\
% \\
% Under such assumptions, it can be shown (assuming the analyticity of $L$) that:
% \begin{align}
%      \hat{R}_n(f) = \frac{1}{n}\sum_i^n L(F(X_i(\theta)),Y_i)
% \end{align}
% is smooth in $\theta$, which implies the existence of a gradient $\nabla_\theta \hat{R}_n(f(\theta))$ which is a key requirement of backpropagation. The `update' rule is then a transition rule on $\mathbb{R}_\theta$ that maps at each iteration (epoch) $\theta_{i+1} = \theta_i - \gamma(n) \nabla_\theta \hat{R}_n(f(\theta))$. Here $\gamma(n) \geq 0$ is the \textit{step-size} whose value may depend upon the iteration (epoch) $n$ (with $\sum^\infty \gamma(n) = \infty$ and $ \sum^\infty \gamma^2(n) < \infty$, the square-integrable condition with respect to the Lebesgue measure \cite{vapnik_overview_1999}). [While usually assumed in the classical case, it is important for comparisons with quantum that the underlying measure-theoretic conditions for backpropagation are made explicit.]

% \subsubsection{Common Loss Functions}\label{sec:ml:Common Loss Functions}
% A variety of commmon loss functions are used as empirical risk estimators. Two popular choices across statistics and also machine learning (both classical and quantum) are (a) mean-squared error (MSE) and (b) root-mean sequared error (RMSE). Given data $D_n(X,Y)$ with $(X_i, Y_i) \sim \Prb_{XY}$ and a function estimator $f_\theta$ as per above, MSE is defined as follows.
% \begin{definition}[Mean Squared Error] \label{defn:ml:Mean Squared Error}
%     The MSE for a function $f$ parameterized by $\theta$ over a dataset $D_n$ is:
%     \begin{align}
%         \text{MSE}(f_\theta) = \frac{1}{n}\sum_{i=1}^n \left(\hat f_\theta(X_i(\theta)) - Y_i\right)^2 \label{eqn:ml:MSE}
%     \end{align}
% \end{definition}
% i.e. $L_2$ loss. MSE calculates the average of the squares of the differences between predicted and label values. RMSE is defined as $\sqrt{\text{MSE}(f_\theta)}$. Other common loss functions include (i) cross-entropy loss e.g. Kullback-Leibler Divergence (see \cite{hastie_elements_2013} $\S14)$ for classification tasks and comparing distributions (see section \ref{sec:quant:quantummetrics} for quantum analogues), (ii) mean absolute error loss and (iii) hinge loss. The choice of loss functions has statistical implications regarding model performance ad complexity, including bias-variance trade-offs.


% \subsubsection{Model complexity and tradeoffs} \label{sec:ml:Model complexity and tradeoffs}
% As we discuss below, there is a trade-off between the size of $\mathcal{F}$ and empirical risk performance in and out of sample. Such risk $\hat{R}_n(f)$ can always be minimised by specifying a [large class of prediction rules]. The most extreme example being $f(x) = Y_i$ when $x=X_i$ and zero otherwise (in effect, $F$ containing a trivial mapping of $X_i$ to $Y_i$ for all $X_i$ [\textbf{Castro}]). In this case, $\hat{R}_n(f) \to 0$, but performs poorly on out of sample data. Such an example also provides more context on what it means to learn, namely that learning is [properly] characterised as selecting $\mathcal{F}$ that minimises $\hat{R}_n(f)$ across in-sample and out-of-sample data. The [size and complexity] of prediction rules $\mathcal{F}$ illustrates a tradeoff between approximation and estimation (known as `bias-variance' tradeoff for squared loss functions). This tradeoff is formally represented by \textit{excess risk}, the difference between expected empirical risk and Bayes risk: [\textbf{NB: check hats}] \textcolor{red}{rephrase}
% \begin{align}
%     E[\R_n(\hat{f}_n)] - R^* = \underbrace{E[\hat{R}_n(\hat{f}_n)] - \underset{f \in \mathcal{F}}{\inf} R(f)}_{\text{estimation error}} + \underbrace{\underset{f \in \mathcal{F}}{\inf} R(f) - R^*}_{\text{approximation error}}
% \end{align}
% % \hl{\textbf{DO WE NEED OPTIMISATION ERROR?}}
% Recalling $E[\hat{R}_n(\hat{f}_n)]$ is contingent upon $\hat{f}$ estimated from $D_n(X,Y)$ (the data samples) and that the optimal $f$ (one that minimises statistical risk) is represented by $\underset{f \in \mathcal{F}}{\inf} R(f)$, estimation error captures how well $\hat{f}$, which is learnt from data, performs against all possible choices in $\mathcal{F}$. By contrast, as $R^*$ indicates the best choice of $f$ to minimise statistical risk, then the approximation error indicates the deterioration in performance arising from restricting $\mathcal{F}$ to subsets of all possible $f$. The tradeoff is characterised by the fact that if $\mathcal{F}$ becomes large (more prediction rules), estimation error tends to zero (i.e. there is little that must be learned from the data), but the approximation error increases. Recalling that by increasing the size of $\mathcal{F}$, the size of $\hat{R}_n(\hat{f})$ can be minimised (intuitively, we have a greater selection of $f$ to choose from according to which $\hat{R}_n(\hat{f})$ may be made small). But the chosen $f$ that renders $\hat{R}_n(\hat{f})$ minimal, namely $\hat{f}_n$, [will] overfit the data because $\hat{R}_n(\hat{f})$  [is not a good estimate] of the true risk $\R_n(\hat{f}_n)$.

% \subsection{Reducing empirical risk}\label{sec:ml:Reducing empirical risk}
% Two empirical risk-based minimisation methods for handling overfitting are (a) to limit the size of $\mathcal{F}$ in order to control estimation error. However, given the estimation/approximation error tradeoff, placing upper bounds on estimation error also places lower bounds on approximation error; and (b) including a penalty metric (the basis of regularisation) that penalises model complexity. In this latter case, we express the inclusion of the penalty (cost) term $C(f)$ as:
% \begin{align}
%     \hat{f}_n = \arg\min_{f \in \mathcal{F}} \{ \hat{R}_n(f) + C(f)   \}
% \end{align}
% In practice, $C(f)$ may be proportional to the degree of $f$ (e.g. for a polynomial) or the norm of the derivative of $f$. Often $C(f)$ is proportional to parameter norms. Limiting training data size $n$ is one method of limiting the size of $\mathcal{F}$ (such as the method of sieves) on the assumption that $\mathcal{F}$ increases monotonically with $n$. In Bayesian contexts, where empirical risk reflects a log likelihood function, $C(f)$ is interpretable as incorporating prior knowledge about the likelihood of models. In this case, setting $\exp(-C(f))$ is a prior probability distribution on $\mathcal{F}$ (i.e. the probability for $f$), then $f$ being probable equates to small $C(f)$ and vice versa. Other models, such as `description length methods', estimate model complexity via the number of bits required to represent the model. Other techniques include hold-out methods involving splitting training data $D$ into training sets $D_T$ and test (or validation) sets $D_V$, where $D_T$ is used to select $\hat{f}_n$ and assessed (via a separate risk measure) against $D_V$. Knowing how to partition the training data can be difficult. A common approach in machine learning is to use $k$-fold cross validation which randomly splits data into training and test sets, removing entry $k$ from $D$ and minimising the regularised empirical risk. Theoretically demonstrating guarantees for improved performance can remain challenging, however (see \cite{hastie_elements_2013} $\S7.10$ for a general discussion). 

% Regularisation and penalty-based methods are an important means of addressing empirical risk and form the basis of regularisation to deal with overfitting. We examine these in particular when reviewing the work of Nielsen et al. \cite{nielsen_geometric_2006,gu_quantum_2008,nielsen_optimal_2006} and penalty metrics for geometric quantum control.  

% \subsection{No-Free Lunch Theorems} \label{sec:ml:No-Free Lunch Theorems}
% Statistical learning theory (both classical and quantum) also has a number of \textit{no free lunch theorems} which place bounds upon the [generalisation performance] of general-purpose optimisation algorithms. The classical no free lunch theorem \cite{wolpert_no_1997} asserts that for any algorithm $A$, when averaged over all possible problems, the expected performance of $A$ is equivalent to any other algorithm $A'$. Mathematically, this can be represented in terms of risk across different types of learning problems.

% Given the set $F$ of all possible functions $f:\mathcal{X} \to \mathcal{Y}$ and the set of all distributions $\mathcal{P}$, for any two algorithms $f_A$ and $f_{A'}$ the \textit{no free lunch} theorem \cite{wolpert_no_1997} provides that:
% \begin{align}
% \int_{\mathcal{P}} R_{f_{A}}(L(f(X),Y)) \, d\mathcal{P} = \int_{\mathcal{P}}R_{f_{A'}}(L(f(X),Y)) \, d\mathcal{P},
% \end{align}
% where $R_f(L(f(X),Y))$ is the true risk (equation \ref{eqn:ml:statlearning true risk}) associated with algorithm $A$ for a particular distribution $\Prb_{XY}$ in predicting function $f$, and $f \in \mathcal{F}$. The theorem indicates that no algorithm can universally minimise true (statistical) risk across all distributions. In particular, the theorem sets bounds upon how well models can generalise. Below we discuss the quantum analogue of the no free lunch theorem.  

% \subsection{Statistical performance measures} \label{sec:ml:Statistical performance measures}
% Before moving onto consideration of deep learning algorithms, we mention a few common statistical measures (including those used in Chapter \ref{chapter:QDataSet and Quantum Greybox Learning}) in the context of statistical learning theory. Much machine learning and statistical modelling, especially classification algorithms, utilise measures such as true positive (TP), true negatives (TN), false positives (FP) and false negatives (FN) by reference to an functional binary classifier estimator $\hat f(X): \X \to \Y$ where $\Y = \{0,1\}$. These can be related in statistical learning terms as follows. \hl{FIX}
% \begin{enumerate}[(i)]
%     \item \textit{Binary classification}.  consider a binary indicator loss function $L$ where $L(f(x), y) = 0$ if $f(x) = y$ and $L(f(x), y) = 1$ otherwise:
%     \begin{align}
% \text{TP} &= \sum_{i=1}^n \mathcal{I}(f(x_i) = 1 \land y_i = 1) \\
% \text{FP} &= \sum_{i=1}^n \mathcal{I}(f(x_i) = 1 \land y_i = 0) \\
% \text{TN} &= \sum_{i=1}^n \mathcal{I}(f(x_i) = 0 \land y_i = 0) \\
% \text{FN} &= \sum_{i=1}^n \mathcal{I}(f(x_i) = 0 \land y_i = 1)
% \end{align}
% where $\mathcal{I}$ is the indicator function, which returns 1 if the condition is true and 0 otherwise.
% \item \textit{Accuracy}. Accuracy measures the proportion of correct predictions among the total number of cases examined and can be linked with the expectation of the indicator loss:
% \begin{align}
% \text{Accuracy} &= \frac{\text{TP} + \text{TN}}{\text{TP} + \text{FP} + \text{TN} + \text{FN}} \\
% &= 1 - E[L(f(X), Y)] =1 - E[\mathcal{I}] \label{eqn:ml:measures-accuracy}
% \end{align}
% \item \textit{AUC/ROCR}. The AUC of the ROC curve is a performance measure for classification problems at various threshold settings. It measures the area under the ROC curve, which is a plot of the true positive rate against the false positive rate at different thresholds:
% \begin{align}
% \text{TPR}(t) &= \frac{\text{TP}}{\text{TP} + \text{FN}} \\
% \text{FPR}(t) &= \frac{\text{FP}}{\text{TN} + \text{FP}} \\
% \text{AUC} &= \int_0^1 \text{TPR}(t) , d(\text{FPR}(t)) \label{eqn:ml:measures-AUC}
% \end{align}
% \item \textit{F1-Score}. The F1-Score is the harmonic mean of precision and recall, which are themselves ratios involving TP, FP, and FN:

% \begin{align}
% \text{Precision} &= \frac{\text{TP}}{\text{TP} + \text{FP}} \\
% \text{Recall} &= \frac{\text{TP}}{\text{TP} + \text{FN}} \\
% \text{F1-Score} &= 2 \cdot \frac{\text{Precision} \times \text{Recall}}{\text{Precision} + \text{Recall}} \\
% &= \frac{2 \text{TP}}{2\text{TP} + \text{FP} + \text{FN}} \label{eqn:ml:measures-F1}
% \end{align}
% \end{enumerate}

% \section{Deep Learning}\label{sec:ml:Deep Learning}
% Chapters 5 and 6 of this work concern the construction of a range of deep learning architectures to solve optimisation problems in quantum control. In this section, we cover the key elements of the machine learning architectures adopted in those chapters. We focus on neural network formalism, with a particular emphasis on `greybox' methods whereby neural network architectures are encoded with \textit{a priori} information relevant to the problem at hand, such as via encoding specific laws, rules or transformations (such as, in our case, the time-independent approximation of Schr\"odinger's equation) which assist the learning process. 

% \subsection{Linear models}\label{sec:ml:Linear models}
% Neural networks used in this work derive ultimately from an adaptation of statistical methods related to generalised linear models. In this section, we briefly survey the key features of generalised linear models as they relate to neural networks. We subsequently define neural network architecture in terms of non-linear functional composition of a variety of (usually) linear models, via layers in a deep neural network having a representation as a directed graph. Tracking the construction of neural networks by building up intuition through linear models and then non-linear networks is a useful way of both demystifying much of the jargon around neural networks, but also serves to connect the architecture to concepts across our prevoius chapters. We begin with basic linear models.
% \begin{definition}[Linear models]
%     Given $X \in \R^m$ and $Y \in \R$ where samples $(X,Y) \sim \Prb_{XY}$ are identically and independently distributed, we define a basic linear model for estimating $Y$ (assuming it as a scalar for simplicity) as:
%     \begin{align}
%         \hat Y = \hat \beta_0 + \sum_j^m X_j \hat \beta_j + \epsilon
%     \end{align}
%     where $\hat \beta_0 \in \R$  is the estimate of bias while $\beta \in \R^m$ is a vector of coefficients (with $\epsilon$ uncorrelated (random) errors).
% \end{definition}
% Sometimes $\beta_0$ (being constant) is absorbed such that $\hat Y = X^T \hat \beta$. The coefficients $\hat \beta$ are determined according to a chosen minimum estimate of empirical risk, usually least squares. As discussed in the previous chapter, where $\beta_j \in \R^m$ satisfies smoothness and other (mathematically) nice properties, then we can regard $\beta_j$ as being drawn from a differentiable manifold $\M \simeq \R^m$ (homeomorphically) where the basis of $\beta_j$ can be considered to be (tangent) vectors, each of which has directions $j=1,...,m$. An extension to forms of generalised additive model can then be undertaken by considering \textit{projection pursuit regression} (used by Hastie et al. \cite{hastie_elements_2013} as we see below to connect with neural network architecture). In generalised linear model theory, minimising [empirical] risk is often undertaken by imposting penalty metrics in [objective/loss] functions in order to steer models away from high-variance (and thus overfitting of) classes of estimates $\hat f$. Such methods are sometimes denoted `shrinkage methods' in the vernacular of statistical learning as they aim to minimise coefficient variance while retaining predictive power. \textit{Ridge regression}, common across the sciences, is one such model utilising ridge functions, being functions that are a combination of univariate functions with an affine transformation. Ridge coefficients are then those $\hat\beta$ which minimise a penalised loss function, parametrised by some parameter $\lambda \in \R$ (so higher values of $\|\beta\|_2^2$ incur a higher penalty): 
% \begin{align}
%     % General form of ridge regression
% \hat{\beta}_{\text{ridge}} = \arg\min_{\beta} \left\{ L(\mathbf{y}, \mathbf{X}\beta) + \lambda \|\beta\|_2^2 \right\}
% \end{align}
% As we can see (via the loss function, for simplicity we assume $L \in \R$), $f:\R^m \to \R$, while we can regard the addition of the ridge expression as in effect a \textit{regularisation} technique to address overfitting. A useful way of connecting generalised linear models with neural networks is to via projection pursuit models which represent linear combinations of non-linear ridge functions. We do so in order to elucidate the geometric and directional nature of statistical learning in this way, in turn connecting with intuition for quantum geometric machine learning. A ridge function defined as $f(X) = g\braket{X, a}$ for $X \in \R^m$, $g: \R \to \R$ being a univariate function (a function on the loss function in effect), $a \in \R^m$ with the inner product as defined prevoiusly. The ridge function is constant along directions orthogonal to $a_m$. By construction, vectors in hyperspaces of $R^m$, denoted $a_1,...,a_{m-1}$ are orthogonal to $a_m$ i.e. $\braket{a_j,a_m}=0$ for $j=1,...,m-1$. Thus:
% \begin{align*}
% f\left(X + \sum_{j=1}^{m-1} b_j a_j\right) = g\left(\braket{X, a_m} + \sum_{j=1}^{m-1} b_j \braket{a_j , a_m}\right) = g(\braket{X,a}) = f(X)
% \end{align*}
% which elucidates the invariance under the affine transformation. Ridge functions then form the basis for what in statistical learning is denoted project pursuit regression \cite{hastie_elements_2013} with the general form [\textbf{FRIEDMAN}]: \hl{\textbf{FIX INDEXING/DIMENSIONALITY}}
% \begin{align*}
%     f(X) = \sum_n^N g_n(\omega_m^T X)
% \end{align*}
% Recall $X \in \R^m$ and we assume ... In this formulation, $\omega_m$ are $m$ unit vectors in the $m$-directions of the manifold $\M$. The key element is that the estimator $\hat Y=f(X)$ is a function of derived features $V_m = \omega_m X$ rather than $X$ directly. Later on we consider $\omega$ as a [tensor] constructed from at update according to optimisation methods (e.g. gradient descent) reflecting the directional nature of the manifold $\R^m$ and connecting with foregoing geometric concepts of mappings over manifolds and \hl{fibres}. 

% \subsection{Neural networks}\label{sec:ml:Neural networks}
% The ridge functions $n_m(\omega_n^T X)$ vary only in the directions defined by $\omega_n$ where the feature $V_m = \omega_m^T X$ can be regarded as the projection of $X$ onto the unit vector $\omega_m$. As $g_m$ is general, a large number of non-linear functions of linear arguments $V_m$ can be obtained. As Hastie et al. \cite{hastie_elements_2013} note, if $N$ is sufficiently large, then the model can approximate \textit{any} continuous function in $\R^m$. Thus projection pursuit regression models can be regarded as \textit{universal approximators}, a key characteristic of the success of neural networks. The formal definition of neural networks by Fiesler \cite{fiesler_neural_1994} 
% \begin{definition}[Neural network] \label{def:ml:neuralnetworkgeneral}
%     A neural network can be formally defined as a nested 4-tuple $NN=(T,C,S(0),\Phi)$ where $T$ is network topology, $C$ is connectivity, $S(0)$ denotes initial conditions and $\Phi$ denotes transition functions. 
% \end{definition}
% The formal definition of a neural network has influenced later literature and technical work in the field. We discuss briefly some of the elements below:
% \begin{enumerate}
%     \item \textit{Topology}. A directed graph $G=(V,E)$ of functional composition, with vertices $V$ representing neurons and $E$ edges between neurons comprising. The topology comprises (a) a framework of $L_n$ layers each with $N_n$ neurons; and (b) a set of connectivity relations between source neurons in $L_0$ exhibiting certain properties such as (i) intraconnectivity, self-connectivity or supraconectivity, (ii) symmetry or asymmetry and (iii) order;
%     \item \textit{Constraints}. Bounds upon (a) weight value range $||\omega_{ij}|| \leq K_1 \in \R$, (b) local thresholds (biases of offsets) and (c) activation range i.e. $||\sigma|| \leq K_2 \in \R$;
%     \item \textit{Initial state}. covering initialisation of (a) weights, (b) local thresholds and (c) activation values; and
%     \item \textit{Transition functions}. These are transition functions for (a) neuron functions (specifying output of neuron via activation function), (c) learning rules (updating weights and offsets), (c) clamping functions (that keep certain neurons constant and (d) ontogenic functions that change network topology.
% \end{enumerate}
% Modern formulations generally track, with some differences, this taxonomy, with each category and subcategory being a widely studied subdiscipline of machine learning research, such as those concerned with optimal network topology, pretraining and tuning of hyperparameters (see \cite{goodfellow_deep_2016}). Of note is that while statistical learning theory and computer science can provide some theoretical bases for network design, in general there are few or limited theoretical guarantees relating network architectural features (such as network topology or choice of initialisation). As such, tuning such architectural characteristics (which are often represented as hyperparameters of a model or architecture) tends to be experimental (or in reality trial-and-error) and empirical in nature. Moreover, as we show in particular in Chapter 6, network architecture and connectivity is often a key and important element in both the performance of networks but also their description via visual or other means.\\
% \\
% \subsubsection{Neural network components}\label{sec:ml:Neural network components}
% An elementary neural network can then be understood as an extension of the non-linearisation of [generalised linear models] discussed above within the network taxonomy. Consider a simple three-layer fully-connected feed-forward network comprising an input layer $L_0$ comprising $m$ inputs $X_m$ (which for generality can be considered identity neuron functions $\sigma(X_m)\to X_m$) , a single hidden layer $L_1$ of and a final output layer $L_2$. We set out a few definitions.
% %========
% \begin{definition}[Activation function]
%     Given an input vector $X \in \R^n$, weight [tensor] $\omega \in \R^{m \times n}$ and bias term $\beta_0 \in \R^m$ we define the affine transformation $z = \omega X + \beta_0 \in \R^m$. An activation function is then defined as:
%     \begin{align*}
%         \sigma:\R^m \to \R^m \qquad \sigma(z) = \sigma(\omega X + \beta_0) = \begin{pmatrix}
%             \sigma(z_1), \sigma(z_2),\ldots, \sigma(z_m)
%         \end{pmatrix}^T
%     \end{align*}
%     where the activation function $\sigma(z_i)$ is (usually) applied element-wise to each $z_i$.
% \end{definition}
% Activation functions are generally classified into one of the following types: (i) \textit{ridge functions} (as described above) where $f(X) = g(\omega X + \beta_0)$ for a non-linear ridge function $g:\R \to \R$, (ii) \textit{radial functions} where $f(X) = g(||X - c||)$ where $c$ is the centre of the radial basis function (e.g. for a radius $r = ||X-c||$), $g:\R \to \R$ is a non-linear function with $||\cdot||$ a norm (usually Euclidean) or (iii) \textit{fold functions} such as the softmax function. Fold functions, such as softmax, are particularly important as they are often interpreted formally or heuristically as probabilities relating to classification. 
% Let $ \sigma: \mathbb{R}^m \rightarrow S $ be a function, where $ S $ is the standard $(m-1)$-simplex defined as:
% \begin{align*}
% S = \left\{ p\in \mathbb{R}^m \mid p_i \geq 0, \forall i \in \{1, \dots, m\}, \text{ and } \sum_{i=1}^m p_i = 1 \right\}
% \end{align*}
% Each point within the simplex $ S $ represents a possible probability distribution over $m$ discrete outcomes, where $p_i$ is the probability of the $i$-th outcome.
% The function $\sigma$ transforms a vector $z \in \mathbb{R}^m$ into a vector $p \in S$ such that each component of $p$, denoted as $p_i$, can be interpreted as the probability of the $i$-th outcome. Framed in this way, the activation satisfies requirements for interpretation [as] a probability distribution, namely (i) $p_i \geq 0$ (non-negativity) and (ii) $\sum_{i=1}^m p_i = 1$. An important activation function [\textbf{and one we adopt}] is the \textit{softmax function}, being a type of fold function:
% \begin{align}
% p_i = \frac{e^{z_i}}{\sum_{j=1}^m e^{z_j}} \label{eqn:ml:activationsoftmax}
% \end{align}

% \subsubsection{Layers in neural networks}\label{sec:ml:Layers in neural networks}
% As discussed above, clustering or layering of neurons is a hallmark of neural network architecture. While fully-connected feed-forward networks (where each neuron in each layer is forward-connected to each other) exhibit relatively [symmetric?] structure, not all networks are as simply described given concurrent parallel neworks, or common practices such as [\textit{residual connections}] that may connect initial layers to layers further down the hierarchy directly rather than through intermediate layers. Nevertheless, for exposition we consider in essence a fully-connected feedfoward network. To do so, we describe a canonical multi-layer perceptron model of a feed-forward network (directly related to one of the candidate models used in Chapter 6, namely the fully-connected model).
% \begin{definition}[Feed-forward neural network]
%     A feed-foward neural network (also known as a multi-layer perceptron network) consists of multiple layers $a^l_i$ of neurons such that each neuron in each layer (other than the first input layer) is a (composition) function of each neuron in the preceding layer. Formally:
%     \begin{align}
%     a_i^{(l)} = \sigma^{l}_i\left(\sum_{j=1}^{n_{l-1}} w_{ij}^{(l)} a_j^{(l-1)} + \beta_i^{(l)}\right) \label{eqn:ml:feedforwardactivation-al}
% \end{align}
% where $l$ indexes each layer, $i$ each neuron in that layer $a^l_i$ valued by an activation function $\sigma^{(l)}_i$ for that neuron in that layer which is itself a function of the sum of weight matrices $\omega_{ij}^{(l)}$ applied to the output of each neuron of the previous layer $a_j^{(l-1)}$ together with a bias term $\beta_i^{(l)}$.
% \end{definition}


% Following the classification of networks above, a fully-connected neural network with layers indexed from $l=0,...,L$ can then be formally described below. 
% \subsubsection{Neural network schema}\label{sec:ml:neuralnetworkschema}
% A schema of the toy model is set out in Figure \ref{fig:ml:fullyconnectedNNwithmatrix}:
% \begin{enumerate}
%     \item \textit{Input layer}. The input layer is represented by $X_j$, $j=1,...,m$ inputs or equivalently input neurons $\sigma_i(X_j)=X_j$. For the input layer ($l=0$), $a_j^{(0)} = x_j$, the $j$-th component of the input vector $\mathbf{x}$.
%     \item \textit{Hidden layer}. Represented by $Z_i$ neurons each a function of all neurons in the immediately preceding layer.
% \item \textit{Output layer}. The output layer $a^L$ is then chosen to accord with the problem at hand, so for classification problems it may be either a binary classification or link-function (such as a logit function) giving an outcome $\sigma_l \in [0,1]$ interpretable as a probability. 
% The overall output of the network is the estimator $\hat Y$, denoted as $\hat Y = (\hat Y_1, \hat Y_2, ..., \hat Y_{n_L})^T$, where $n_L$ is the number of neurons in the layer:
% \begin{align}
%    f(X) = \hat Y = a^{(L)} = \left( a_1^{(L)}, a_2^{(L)}, ..., a_{n_L}^{(L)} \right).
% \end{align}
% \end{enumerate}
% Note that often the output layer may itself be subject to an additional transformation. Thus denoting the penultimate $(l-1)$the layer as $T=(a_1^{(l-1)},...,a^{(l-1)_k})$, then we often have:
% \begin{align}
%     f_k(X) = g_k(T) \qquadk=1,...,K
% \end{align}
% The output function $g_k(T)$ typically allows a final transformation of $T$. This might typically be, for classification, a softmax function $g_k(T) = \exp(T_k)/(\sum_l^K \exp(T_l))$. As Hastie et al. note, the non-linearity of the activation functions $\sigma$ expand the size of the class of candidate functions $F$ that can be learnt. Functionally, the network can be regarded as a functional composition, with each layer representing a function comprising linear inputs into nonlinear activations $\sigma^l$ applied sequentially. We can regard the whole function $f^(\l) \simeq a^{(l)}$ as $f: \mathbb{R}^{m} \to \mathbb{R}^{n}$ via composition as:
% \begin{align}
%     f(X) = \sigma_L \circ f^{(L)} \circ \sigma_{L-1} \circ f^{(L-1)} \circ ... \circ \sigma_1 \circ f^{(1)}(X),
% \end{align}
% While not the focus here, in geometric contexts doing so can allow us to frame the network as maps among differentiable manifolds. We also note that multilayer feedforward networks are of particular significance due to the universal approximation theorem \cite{hornik_multilayer_1989} for learning arbitrary functions (and other universal and function approximation results) with a quantum analogue that functions can be represented to arbitrary error at exponential depth (impratical of course).  

% %========diagram

% \begin{figure}
%     \centering
%     % NEURAL NETWORK activation
% % https://www.youtube.com/watch?v=aircAruvnKk&list=PLZHQObOWTQDNU6R1_67000Dx_ZCJB-3pi&index=1
% \begin{tikzpicture}[x=2.7cm,y=1.6cm]
%   \message{^^JNeural network activation}
%   \def\NI{5} % number of nodes in input layers
%   \def\NO{4} % number of nodes in output layers
%   \def\yshift{0.4} % shift last node for dots
  
%   % INPUT LAYER
%   \foreach \i [evaluate={\c=int(\i==\NI); \y=\NI/2-\i-\c*\yshift; \index=(\i<\NI?int(\i):"n");}]
%               in {1,...,\NI}{ % loop over nodes
%     \node[node in,outer sep=0.6] (NI-\i) at (0,\y) {$a_{\index}^{(0)}$};
%   }
  
%   % OUTPUT LAYER
%   \foreach \i [evaluate={\c=int(\i==\NO); \y=\NO/2-\i-\c*\yshift; \index=(\i<\NO?int(\i):"m");}]
%     in {\NO,...,1}{ % loop over nodes
%     \ifnum\i=1 % high-lighted node
%       \node[node hidden]
%         (NO-\i) at (1,\y) {$a_{\index}^{(1)}$};
%       \foreach \j [evaluate={\index=(\j<\NI?int(\j):"n");}] in {1,...,\NI}{ % loop over nodes in previous layer
%         \draw[connect,white,line width=1.2] (NI-\j) -- (NO-\i);
%         \draw[connect] (NI-\j) -- (NO-\i)
%           node[pos=0.50] {\contour{white}{$w_{1,\index}$}};
%       }
%     \else % other light-colored nodes
%       \node[node,blue!20!black!80,draw=myblue!20,fill=myblue!5]
%         (NO-\i) at (1,\y) {$a_{\index}^{(1)}$};
%       \foreach \j in {1,...,\NI}{ % loop over nodes in previous layer
%         %\draw[connect,white,line width=1.2] (NI-\j) -- (NO-\i);
%         \draw[connect,myblue!20] (NI-\j) -- (NO-\i);
%       }
%     \fi
%   }
  
%   % DOTS
%   \path (NI-\NI) --++ (0,1+\yshift) node[midway,scale=1.2] {$\vdots$};
%   \path (NO-\NO) --++ (0,1+\yshift) node[midway,scale=1.2] {$\vdots$};
  
%   % EQUATIONS
%   \def\agr#1{{\color{mydarkgreen}a_{#1}^{(0)}}} % green a_i^j
%   \node[below=16,right=11,mydarkblue,scale=0.95] at (NO-1)
%     {$\begin{aligned} %\underset{\text{bias}}{b_1}
%        &= \color{mydarkred}\sigma\left( \color{black}
%             w_{1,1}\agr{1} + w_{1,2}\agr{2} + \ldots + w_{1,n}\agr{n} + b_1^{(0)}
%           \color{mydarkred}\right)\\
%        &= \color{mydarkred}\sigma\left( \color{black}
%             \sum_{i=1}^{n} w_{1,i}\agr{i} + b_1^{(0)}
%            \color{mydarkred}\right)
%      \end{aligned}$};
%   \node[right,scale=0.9] at (1.3,-1.3)
%     {$\begin{aligned}
%       {\color{mydarkblue}
%       \begin{pmatrix}
%         a_{1}^{(1)} \\[0.3em]
%         a_{2}^{(1)} \\
%         \vdots \\
%         a_{m}^{(1)}
%       \end{pmatrix}}
%       &=
%       \color{mydarkred}\sigma\left[ \color{black}
%       \begin{pmatrix}
%         w_{1,1} & w_{1,2} & \ldots & w_{1,n} \\
%         w_{2,1} & w_{2,2} & \ldots & w_{2,n} \\
%         \vdots  & \vdots  & \ddots & \vdots  \\
%         w_{m,1} & w_{m,2} & \ldots & w_{m,n}
%       \end{pmatrix}
%       {\color{mydarkgreen}
%       \begin{pmatrix}
%         a_{1}^{(0)} \\[0.3em]
%         a_{2}^{(0)} \\
%         \vdots \\
%         a_{n}^{(0)}
%       \end{pmatrix}}
%       +
%       \begin{pmatrix}
%         b_{1}^{(0)} \\[0.3em]
%         b_{2}^{(0)} \\
%         \vdots \\
%         b_{m}^{(0)}
%       \end{pmatrix}
%       \color{mydarkred}\right]\\[0.5em]
%       {\color{mydarkblue}\mathbf{a}^{(1)}} % vector (bold)
%       &= \color{mydarkred}\sigma\left( \color{black}
%            \mathbf{W}^{(0)} {\color{mydarkgreen}\mathbf{a}^{(0)}}+\mathbf{b}^{(0)}
%          \color{mydarkred}\right)
%     \end{aligned}$};
  
% \end{tikzpicture}
%     \caption{Schema of the first two layers of a fully-connected feed-forward neural network together with associated matrix and algebraic representation. Here $a_i^{(l)}$ are the input layer eurons, $\omega_{l,j}$ are the weights for neuron $a_j^{(l)}$. $W$ is the [weight] tensor with bias $b^{(l-1)}$ and $\sigma$ the activation function. [\textbf{REF: tikz.net}]}
%     \label{fig:ml:fullyconnectedNNwithmatrix}
% \end{figure}
% %========diagram


% \section{Optimisation methods}\label{sec:ml:Optimisation methods}
% \subsection{Optimisation and Gradient Descent}\label{sec:ml:Optimisation and Gradient Descent}
% The main optimisation algorithm used across most machine learning involves some sort of \textit{stochastic gradient descent} whereby parameters $\theta$ of estimated functions $\hat f(\theta)$ are updated according to a generalised directional derivative. In keeping with the geometric framing of much of this work, we present a definition below.
% \hl{REDO}
% Let $M$ be a smooth manifold representing the parameter space of a model, with a Riemannian metric $g$. Consider a loss function $L: M \to \mathbb{R}$ which is a smooth function on $M$. In the context of machine learning, stochastic gradient descent is an optimization technique to find a local minimum of $L$. \hl{EDIT}\\
% \\
% Given a neural network is parametrised by a set of unknown weights $\theta$ which are updatable (learnable) by means of updating according to an optimsation procedure. The set $\theta$ can be said to comprise:
% \begin{enumerate}[(i)]
%     \item \textit{Hidden layer weights}. For $m=1,...,M$ hidden layers, we can denote the parameters as $\{\alpha_{0m},\alpha_m \}$ (the bias and weight for each neuron) (the initial input layer is not considered to have any weights). 
%     \item \textit{Output layer weights}. Weights denoted for the final layer $\{\beta_{0k},\beta_k\}$ where $k=1,...,K$.
% \end{enumerate}
% In this context, we now discuss probably the most important optimisation technique in quantum machine learning (as with classical), namely backpropagation.

% \hl{SECTION ON COMMON LOSS FUNCTIONS E.G. MSE}

% \subsection{Backpropagation}\label{sec:ml:Backpropagation}
% Backpropagation \cite{rumelhart_learning_1986,werbos_backpropagation_1990,lecun_optimal_1990,lecun_gradient-based_1998} is a stochastic gradient descent-based method for optimising model performance across neural network layers. Fundamentally it represents, subject to a number of conditions, an efficient way of updating parameters $\theta$ of models $f_\theta$ in order to minimise figures of merit such as empirical risk (equation (\ref{eqn:ml:empiricalrisk}) by, having calculated an estimate $\hat f_\theta(X)$, propagating the error $\delta \sim |\hat f_\theta - Y|$ through the network. Propagation here refers to the use of the calculated error $\delta$ in updating parameters $\theta$ across network layers. Backpropagation consists of two phases: (a) a \textit{forward pass}, this involves calculating each layer's activation function $a_i^{(l)}$ (see equation (\ref{eqn:ml:feedforwardactivation-al})); and (b) a \textit{backward pass} where the backpropagation updates are calculated. We now focus on the backward pass. Assume a [loss] function given by $R(\theta)$ (in our case we use mean square error). For neural networks, the most common approach is to use the method of \textit{gradient descent} to update parameters, with the particular method by which this update is calculated being via backpropagation equations. Firstly, for gradient descent recall the directional derivative \ref{eqn:geo:directionalderivative}) in differential form for Riemannian and subRiemmanian manifolds and gradient (definition \ref{defn:geo:gradient}).
% We then define the use of gradient descent for optimisation using these definitions as follows.
% \begin{definition}[Gradien descent optimisation]\label{defn:ml:Gradien descent optimisation}
%     Optimisation by gradient descent is defined as a mapping:
%     \begin{align}
% \beta_{km}^{(r+1)} &= \beta_{km}^{(r)} - \gamma_r \sum_{i=1}^{N} \frac{\partial R_i}{\partial \beta_{km}^{(r)}} = \beta_{km}^{(r)} - \gamma_r \sum_{i=1}^{N} \nabla_{\beta_{km}} R_i \\
% \alpha_{m\ell}^{(r+1)} &= \alpha_{m\ell}^{(r)} - \gamma_r \sum_{i=1}^{N} \frac{\partial R_i}{\partial \alpha_{m\ell}^{(r)}}  = \alpha_{m\ell}^{(r)} - \gamma_r \sum_{i=1}^{N} \nabla_{\alpha_{m\ell}} R_i \label{eqn:ml:backpropupdatemain}
% \end{align}
% where (a) $R_i$ are loss/error values for the $i$th datapoint in the training set $D_n(X,Y)$, (b) $\beta_{km}$ denate the weights of the $m$th neuron \hl{FIX} and (c) $\gamma_r$ the learning rate. 
% \end{definition}
% Here $r$ indexes each epoch of the learning procedure (e.g. training run). In the above definition:
% \begin{align}
% \frac{\partial R_i}{\partial \beta_{km}} =\delta_{ki}z_{mi}   \qquad 
% \frac{\partial R_i}{\partial \alpha_{m\ell}} &= s_{mi} x_{i\ell} \label{eqn:ml:gradientdescent-errors}
% \end{align}
% denote error quantities $\delta_{ki}$ and $s_{mi}$. 
% \hl{explain why gradient descent optimises}

% The \textit{backpropagation equations} are then given by the following.
% \begin{align}
% s_{mi} = \sigma'(\alpha_{m\ell}^T X_i) \sum_{k=1}^{K} \beta_{km} \delta_{ki} \label{eqn:ml:backpropagationequationssdelta}
% \end{align}
% The equations (\ref{eqn:ml:backpropagationequationssdelta}) represent a means of implementing gradient descent optimisation above. They can then explained as follows. The $\sigma'(\alpha_{m\ell}^T X_i)$ term denotes the derivative of $\sigma$ with respect to $\alpha_{m\ell}^T X_i$. This term determines how changes in the weights affect the loss. \hl{FIX} Recall that the error gradient with respect to the output gradient for each output neuron $a_k^(L)$ is denoted:
% \begin{align}
%     \delta_k^(L) = \frac{\partial R_i}{\partial a_k^{(l)}}
% \end{align}
% with:
% \begin{align}
% \delta^{(l)}_m = \sigma' \left( \sum_{j} w^{(l+1)}_{mj} a^{(l)}_j \right) \sum_{k} w^{(l+1)}_{mk} \delta^{(L)}_k
% \end{align}
% In the forward pass, the estimates $\hat f_k(X)$ are computed. In the backward pass, first $\delta_k^L$ are computed, following which they are `back-propagated' throughout the network via the backpropagation equations (\ref{eqn:ml:backpropagationequationssdelta}). Doing so then allows computation of the gradients in equation (\ref{eqn:ml:gradientdescent-errors}). A \textit{training epoch} is then one full round of forward and backward passes. Note that equation (\ref{eqn:ml:backpropupdatemain}) sums over the training set, referred to as \textit{batch learning} (the most common case). Alternatively, one can perform backpropagation point-wise based on single observations $(X_i,Y_i) \in D_n$. 

% \textit{Quantum backpropagation} also brings with it a number of subtleties arising because of the effect of measurement on quantum states. Thus the classical analogue of backpropagation does not carry over one-for-one to the quantum case. In many cases, models learn classically parametrised quantum circuit features via implementing offline classical backpropagation (as per above) conditional upon measurement statistics. Examples of quantum-related backpropagation proposals include, for example, a series of papers by Verdon et al. \cite{verdon_learning_2019,verdon_quantum_2017,verdon_quantum_2019,verdon_universal_2018} where continuous parameters are quantised and encoded in a superposition of quantum registers enabling a backpropagation-style algorithm. Other examples, including quantum neural network proposals \cite{beer_quantum_2021,beer_quantum_2022,beals_quantum_2001} provide automatic differentiation as a means of propagating a form of automatic measurement that is then propagated through a quantum analogue of a fully-connected network. In each case, one must remember that the optimisation strategy relies upon \textit{measurement} which (as per definition \ref{defn:quant:Measurementchannel}) is an inherently quantum-to-classical channel. In this work, because we are interested in parametrising control functions $u_j(t)$, we are focused on offline optimisation of the classical type. 


% \subsection{Natural gradients}\label{sec:ml:Natural gradients}
% We briefly mention the concept also of \textit{natural gradients} here, drawn primarily from \textit{geometric information theory} \cite{nielsen_geometric_2015,nielsen_elementary_2020} as a means of connecting with the formalism of Chapter \ref{chapter:Background: Geometry, Lie Algebras and Representation Theory}. As noted in the literature \cite{nielsen_elementary_2020,amari_information_2016}, local gradient descent based optimisation depends on the choice of local parameters. Given (in the scalar case) two parameterisations $\eta$ and $\theta$, with initialisations $\theta_0=\theta(\eta_0)$ and $\eta_0 = \eta(\theta_0)$, we will usually have $\eta(\theta) \neq \theta$ such the path and stationary endpoint of gradient descent in parameter space may be different:
% \begin{align}
%     \theta_{t+1} &= \theta_t - \alpha_t \nabla_\theta L_\theta(\theta_t) \neq 
%     \eta_{t+1} = \eta_t - \alpha_t \nabla_\eta L_\eta(\eta_t)
% \end{align}
% referring to a generic smooth loss function is $L \in \cinfm$. The solution to this problem is to select a \textit{natural gradient} \cite{amari_natural_1998} which provides a directional derivative in the intrinsically steepest direction with respect to the (Riemann) metric tensor. In information theory, parameter space can be modelled in terms of a differentiable manifold where updating parameters corresponds to routes or curves on the manifold. In this case, points on the manifold $p \in \M$ have a representation, for example, as a set of parmeters (say a vector) associated with that point i.e. $\theta_p$. Stochastic gradient descent on Riemannian manifolds ($\M,g$) \cite{bonnabel_stochastic_2013}, denoted by $\nabla_{\M}$, utilises the exponential map (definition \ref{defn:alg:Matrix exponential}) $\exp:T_p\M \to \M$ for its update protocol such that:
% \begin{align}
%     p_{t+1} = \exp_{p_t}(-\alpha_t \nabla_{\M}L(p_t)) \qquad \nabla_{\M}L(p) = \nabla_v(L(\exp_p(v)))\big|_{v=0} \label{eqn:geo:naturalSGD-Riemanngradient}
% \end{align}
% where $\nabla_v$ is the directional derivative given in equation \ref{eqn:geo:directionalderivative} and $\alpha$ is step size (see section \ref{sec:ml:Regularisation and Hyperparameter tuning}). Because calculating the exponential term in equation (\ref{eqn:geo:naturalSGD-Riemanngradient}) can be difficult, instead a mapping to the parameter [fibre bundle] is used instead a first-order Taylor expansion of the exponential \textit{Euclidean retraction} $Rt_E$ (adapted from \cite{nielsen_elementary_2020}):
% \begin{align}
%     \theta_{t+1} =  R_{\theta_t}\left(-\alpha_t \nabla_{\theta} L_\theta(\theta_t)\right)
% \end{align} 
% which shifts $p$ by some infinitesimal amount. Natural gradient descent is then given by:
% \begin{align}
%     \theta_{t+1}= \theta_t-\alpha_t g^{-1}_\theta(\theta_t) \nabla_{\theta} L_\theta(\theta_t)
% \end{align}
% wher the \textit{natural gradient} $\nabla_N$ is defined as:
% \begin{align}
%     \nabla_N L_\theta(\theta) := g^{-1}_\theta(\theta) \nabla_\theta L_\theta(\theta)
% \end{align}
% Note the presence of $g^\inv$ indicates that the gradient, which transforms contravariantly. The benefit of the natural gradient is that it is invariant under coordinate transformations, though there are some subtleties regarding convergence discussed in the literature \cite{bonnabel_stochastic_2013,nielsen_geometric_2015,amari_natural_1998}. The quantum analogue of natural gradient descent is briefly touched upon in Chapter \ref{chapter:Background: Classical, Quantum and Geometric Machine Learning} as a technique for optimisation.

% \subsection{Regularisation and Hyperparameter tuning}\label{sec:ml:Regularisation and Hyperparameter tuning}
% As the abstract definition of neural networks (\ref{def:ml:neuralnetworkgeneral}) indicates, there is a wide combinatorial landscape of parameters for the design of neural network architectures, including topology, choices of activation functions, loss functions, regularisation, dropout and so on. Hyperparameters are settings of a neural network model which are not adapted or updated by the learning protocol of the model in a direct sense (though model performance may inform ancillary hyperparametric models). In effect changing the hyperparameter changes the neural network model itself. We set out briefly a few such parameters, techniques and hyperparameters used in the results detailed in later chapters.
% \begin{enumerate}[(i)]
%     \item \textit{Learning rate}. The learning rate parameter $\gamma_r$ (or \textit{gain} in adaptive learning) in equations (\ref{eqn:ml:backpropupdatemain}) represent the step size at each iteration. Mathematically it represents a scaling of the (directional derivative) $\nabla_\omega R(\theta)$ and is among the most important hyperparameters for network performance.
%     \item \textit{Epochs}. The number of epochs over which training (a full forward- and backward-pass of the backpropagation algorithm in equation (\ref{eqn:ml:backpropagationequationssdelta}) is a tunable parameter of neural networks. In principle the number of epochs can affect the sensitivity of weights to training data and can risk overparametrisation such that models do not generalise well. Conversely, insufficient epochs may not sufficiently minimise empirical risk (definition \ref{eqn:ml:empiricalrisk}).
%     \item \textit{Regularisation}. As flagged above, regularisation is a means of seeking to minimise variance, and thus overfitting, of models trained on in-sample training data where inference (i.e. predicting / infering label outputs $Y$) is undertaken on out-of-sample feature data $X$.
%     \item \textit{Generalisation}. Generalisation refers to a statistical measure of risk that captures the out-of-sample performance of a model. 
% \end{enumerate}


% % \subsubsection{Epoch number}

% % \subsubsection{Generalisation and validation}
% % As discussed above, optimsing functional estimators (models) $f: \X \to \Y$

% % \subsection{Objective (loss) functions}
% % The choice of loss functions is an important feature of neural network design. Recall the generic aim of empirical risk minimisation [\textbf{REF}] seeks to minimise the average error between the realisation $y_i$ and estimate $\hat f_i(X)$.


% % \subsection{Neural network types}

% % \section{Geometric Concepts in Machine Learning}

% % \subsection{Gradient descent }\label{sec:ml:Gradient descent}
% % \begin{itemize}
% %     \item Gradient descent in terms of manifolds
% %     \item Manifold of parameters $\theta$ i.e. $\M_\theta$
% %     \item $\M$ as a manifold where $\theta \in \R^m$ for example are charts or vector bundles on manifold (?)
% %     \item How should we think about this? $f \in \cinfm$ functions on $\M$, then $f = f(\theta)$ and $\theta$ is itself drawn from a [vector bundle] of some other manifold $\M_\theta$. In our quantum example, our elements of the maniolf are $U_T \in \M \simeq G = SU(3),SU(2)$ for example
% %     \item Natural verus usual gradient descent (Nielsen)
% %     \item Backpropagation in terms of gradients
% % \end{itemize}

% \section{Quantum Machine Learning} \label{sec:ml:Quantum Machine Learning}
% In this section we consider how the principles of classical statistical learning and classical machine learning algorithms are related to the hybrid quantum-classical models explored later on in this work. In line with our taxonomy focusing on data, models and metrics (measures), we start with a brief synopsis of how data (quantum or classical) is actually encoded for use in quantum machine learning scenarios. In this section, we cover a number of important differences between classical and quantum machine learning. We only sketch a few germane points related to the objectives of our work. As we discuss in the next Chapter, quantum machine learning is now a vast and variegated discipline combining elements of quantum computation and information processing, statistical learning theory, communication theory and other areas. The unifying factor behind quantum machine learnig is the use of quantum data or quantum information processes in ways that enable, constitute, or rely upon some type of learning protocol as measured or indicated by relevant metrics, usch as in-sample performance, variance, accuracy and so on. The spectrum of quantum machine learning algorithms is expansive, covering quantum neural networks, parametrised (variational) quantum circuits, quantum support vector machines and other formulations \cite{cerezo_challenges_2022}. Similarly, the application of deep learning principles to quantum algorithm design, such as via quantum neural networks (see \cite{schuld_machine_2021,beer_quantum_2022} for an overview), quantum deep learning architectures (including quantum analogues of graph neural networks, convolutional neural networks and others \cite{verdon_learning_2019,verdon_universal_2018,verdon_quantum_2019,verdon_quantum_2017} speaks to the diversity of approaches now studied in the field. Coupled with these approaches, emerging trends in the use of symmetry techniques, such as dynamical Lie algebraic neural networks, symmetry-preserving learning protocols and geometric quantum machine learning approaches (discussed in particular in section \ref{sec:ml:Geometric QML}) offer new method for improving on problem-solving in the quantum and classical domain. Moreover, much literature is also devoted to understanding the differences, some subtle, some less-so, between classical and quantum machine learning both at the theoretical level of statistical learning, down to the practical implementation of algorithms in each case. Some such literature draws upon extensive work in quantum algorithm design and complexity theory \cite{aaronson_how_2022} In this section, we provide a short high-level summary of some of the key features of quantum machine learning relevant to Chapters \ref{chapter:QDataSet and Quantum Greybox Learning} and \ref{chapter:Quantum Geometric Machine Learning}, with a particular focus on variational or parametrised quantum machine learning circuits. First-off, we consider a few key principle differences between classical and quantum approaches in machine learning, starting with the fundamental distinction between the need for quantum channels to preserve unitarity (definition \ref{defn:quant:Unitary Channel}) versus the dissipative nature of classical neural networks \cite{schuld_quest_2014}. 


% \subsection{Neural networks and quantum systems} \label{sec:ml:Neural networks and quantum systems}
% As Schuld et al. note \cite{schuld_quantum_2014}, the challenge for adapting classical neural network architecture to the quantum realm in part lies in structural distinctions between classical and quantum computing. Classical neural network architectures are fundamentally based upon non-linear and often dissipative dynamics, as distinct from the linear unitary dynamics of quantum computing. Early progenitors of quantum machine learning architectures adapting principles form neural networks include \textit{Hopfield networks} \cite{hopfield_neural_1982}, being a (directed) graph network where weights are indexed by $i$ and the neurons by $j$). Hopfield networks exhibit \textit{associative (content-addressable) memory}, which allows retireval of the network state state from $P$ stored network states 
% \begin{align*}
%     X^P = \{ (x^1_1,...,x_N^1),...,(x_1^P,...,x_1^P)\}
% \end{align*}
% Associative memory therefore allows computation using incomplete input information instead of the pattern's exact storage address in RAM (basis of human memory and learning). Modern day neural networks represent functional compositions of non-linear equations. Early progenitors of neurons included \textit{perceptrons} (sometimes denoted binary neurons or linear threshold functions) such as the McCulloch-Pitt neuron. Fundamentally, as noted in the literature, if quantum neural networks or machine learning circuits merely induced measurements in order to update the parameters, then they would proceed classically and in effect destroy (due to measurement collapse (axiom \ref{axiom:quant:effectofmeasurement}) \cite{schuld_quest_2014}. Early for addressing this implicit challenge included leveraging quantum measurement to select system eigenstates \cite{kak_quantum_1995}, the use of dissipative quantum systems (being revisited now in light of thermodynamic hybrid quantum computing), encoding parameter evolution in quantum terms \cite{perus_neural_2000}, use of entanglement \cite{behrman_quantum_1996}, teleportation and back-action based approaches \cite{abrams_quantum_1999}.

% \subsection{Quantum statistical learning} \label{sec:ml:Quantum statistical learning}
% Quantum learning tasks are similarly contingent upon the particular functional forms to be learnt. For example, \cite{huang_information-theoretic_2021} consider a class of learning problems concerned with learning the function:
% \begin{align}
%     f(x) = \text{tr}(O \mathcal{E}(\ket{x}\bra{x}))
%     \label{eqn:ml:preskillfn}
% \end{align}
% where $O$ represents a typical known observable (operator) and $\mathcal{E}$ represents a completely positive trace preserving map i.e. a channel representing physical (possibly quantum) state evolution. Equation (\ref{eqn:ml:preskillfn}) is generic, representing classical inputs mapped to real numbers (e.g. results of Hermitian measurement operators $O$). Observation (measurement) constitutes an interaction between an experiment and the physical (quantum) system $\mathcal{E}$, which can be thought of as querying $\mathcal{E}$ by way of $O$.  As with classical, the learning problem is to estimate a function $h(x) \approx f(x)$ while minimising statistical and empirical risk, but with the added constraint of minimising the number of queries on $\mathcal{E}$. 

% The model in \cite{huang_information-theoretic_2021} is in many ways generic and reflective of many QML architectures. A comparison with quantum control is again useful in this regard. For hybrid classical-quantum structures, empirical risk minimisation is with respect to a \textit{classical} representation $f(x)$ (e.g. contingent upon measurement outcomes $m$ given measurement operator $M$) with respect to typically a classical loss function (e.g. fidelity measures, quantum Shannon entropy or some other function of input and output state representations). Physical intuition is useful here: classical gradient descent then enters into Hamiltonian $H$ governing the evolution (and transition) of the quantum system via controls (e.g. coefficients $c_i$ that affect generator amplitudes). Other results in quantum-related statistical learning include bounds on the expressibility of variational quantum circuits \cite{du_learnability_2020,raghu_expressive_2017} [\textbf{DU EXPRESSIVE}]. In particular, it can be shown \\ \\


% The limits of quantum machine learning algorithms from a statistical learning perspective have been examined  \cite{ciliberto_statistical_2020}. For example, it is shown in \cite{ciliberto_statistical_2020} that challenges persist for quantum machine learning algorithms with polyalgorithmic time complexity in input dimensions. In this situation, the statistical error of the QML algorithm is polynomially dependent upon the number of samples in the training set, such that the best error rate $\varepsilon$ is achievable only if statistical and approximation error scale equivalently, which in turn requires approximation error to scale polynomially with the number of samples. For logarithmic dependency on sampling, it is shown that the additive sampling error from measurement further introduces a polynomial dependency on the number of samples. Such constraints affect the viability of whether certain popular or mooted QML algorithms may in fact provide any advantage over classical analogues. 
% Thus in many cases proposed QML algorithms face challenges posed by barren plateaux, entanglement growth and statistical learning barriers. Thus there is, as with classical machine learning, a need to consider how algorithms may (if at all) be architected in order to solve such scaling challenges. Doing so is one of the motivations for this work and its exploration of techniques from geometry, topology and symmetry algebras. As discussed in the introduction, in a machine learning context, the ability to encode prior or knowl information, offers one route to such efficiency, hence our synthesis of what we denote (and further articular) as \textit{greybox} QML together with geometric QML. 

% \subsubsection{Quantum measurement and machine learning} \label{sec:ml:Quantum measurement and machine learning}
% As discussed in Chapter 2, quantum systems are constructed on the basis of underlying measurement instruments and their accompanying theory. In quantum information processing, measurement is an integral [causal] part of the evolution and characterisation of systems as distinct from classical theory. Measurement [\textbf{REF}], recall, can be considered in terms of the operation of an $n$-form from a [tensorial] Hilbert space $M:\otimes_n \Hilb \to \R^n$, such process by the Born rule being stochastic in nature. Thus the question arises as to how machine learning models of quantum phenomena, trained on stochastic quantum measurement data (such as reconstructions of unitaries from measurement statistics) ought to integrate such stochasticity [and measurement practices] into their algorithms. Our models of quantum simulation in Chapter 5 specifically incorporate simulation measurement data into the QDataSet [and accompany algorithms]. By contrast, in Chapter 6, we train a greybox neural network to generate [geodesics] on [time-optimal] geodesic approximations generated from horiztonal distributions $\Delta$. Our target (label) data in that case are unitary targets $U_T$, but the construction of these ultimately depends upon measurement, which we assume has been undertaken (we do this in order to focus upon the key objectives of modelling time optimal paths rather than tomographical reconstruction). We discuss a few of these issues below in the context of parameter shift rules.

% \subsubsection{Barren Plateaus}\label{sec:ml:Barren Plateaus}
% Barren plateaus are a phenomena related to training of QML algorithms that first emerged in the literature around [2015]. They are the quantum analogue of the \textit{vanishing gradient problem} \cite{pascanu_difficulty_2013,goodfellow_deep_2016}. Early papers on quantum algorithm-related barren plateaus \cite{mcclean_barren_2018} identified the phenomena where the variance of a gradient expectation was shown to decrease exponentially in the number of qubits. The vanishing variance of the gradient is understood as follows.
% As the name hints at, barren plateaus intimates a geometric intuition where the process of gradient descent seeking (local or global minima) finds itself in sparse of `flat' (zero-manifold curvature) region. This in line with the principle underlying the directional derivative (see definition \ref{eqn:geo:directionalderivative} and gradients \ref{defn:geo:gradient}) generally, zero curvature implies a form of (pseudo)-isotropy where there is no necessary preferred direction of steepest descent, thus confounding the gradient descent protocol. Since the original paper, a plethora of studies \cite{holmes_barren_2021,holmes_connecting_2022,liu_presence_2021,patti_entanglement_2021} have examined conditions under which barren plateaus may or may not arise, together with strategies for preprocessing or tuning initial conditions (such as parameter initialisation strategies $\theta$ \cite{marrero_entanglement-induced_2021} or Bayesian methods \cite{rad_surviving_2022}) to mitigate or even side-step such issues. Other examples using control paradigms include \cite{larocca_diagnosing_2022} who leverage Lie algebras encoded within certain ansatzes (including popular Hamiltonian variational ansatzes \cite{mele_avoiding_2022}) to show guarantees for avoiding barren plateaus using such ansatzes may not exist, or showing noise-induced barren plateaus for variational quantum algorithms \cite{wang_noise-induced_2021}. Conversely, for certain classes of QML algorithms such as quantum convolutional neural networks, barren plateaus may be absent assuming the architecture is appropriately chosen \cite{pesah_absence_2021}. Examples or strategies to address barren plateaus include using adaptive quantum natural gradients for greater stability and optimised descent \cite{haug_optimal_2021}, the use of parameter initialisation \cite{liu_parameter_2021} (a state efficient ansatz) ground state preparation, the use of Gaussian parameter initialisations \cite{zhang_gaussian_2022} or even category-theory methods \cite{zhao_analyzing_2021}. Experimentally, we found, when tuning our quantum deep learning architectures in Chapters \ref{chapter:QDataSet and Quantum Greybox Learning} and \ref{chapter:Background: Classical, Quantum and Geometric Machine Learning}, initialising parameters as per \cite{pascanu_difficulty_2013} worked effectively. Barren plateaus are particularly something for researchers to take into consideration in the design of QML algorithms, such as those envisaged for use with the QDataSet below.

% %==========
% \subsection{Encoding data in quantum systems} \label{sec:ml:Encoding data in quantum systems}
% Most quantum information optimisation problems involve information encoded in quantum systems, either by construction in an experiment involving quantum systems themselves, or via encoding exogenous or classical information into quantum systems (such as qubits) in order to leverage the benefits of quantum computation. Both approaches involve the input into quantum states in a process known as \textit{state preparation}. The way in which data is encoded in quantum systems affects the performance and expressiveness many quantum algorithms \cite{schuld_machine_2021}. Information is usually encoded using one of four standard encoding methods including: (a) basis encoding, (b) amplitude encoding, (c) qsample encoding and (d) dynamic encoding. The first of these, \textit{basis encoding}, is a technique that encodes classical information into quantum basis states. Usually, such procedures involve transformation of data into classical binary bit-strings $(x_1,...,x_d), x_i \in \{0,1\}$ then mapping each bit string to the quantum basis state of a set of qubits of a composite system. For example, for $x \in \Real^N$, say a set of decimals, is converted into a $d$-dimensional bit string (e.g. $0.1\to 00001..., -0.6 \to 11001..$) suitably normalised such that $x = \sum_k^d (1/2^k)x_k$. The sequence $x$ is given a representation via $\ketpsi \propto \ket{000001\,11001}$ (see \cite{schuld_supervised_2018}). \textit{Amplitude encoding} associates normalised classical information e.g. for an $n$-qubit system (with $2^n$ different possible (basis) states $\ket{j}$), a normalised classical sequence $x\in \Complex^{2^n}, \sum_k |x_k|^2=1$ (possibly with only real parts) with quantum amplitudes $x=(x_1,...,x_{2^n})$ can be encoded as $\ket{\psi_x}=\sum_j^{2^n} x_j \ket{j}$. Other examples of sample-based encoding (e.g. \textit{Qsample} and \textit{dynamic} encoding are also relevant but not addressed here). From a classical machine learning perspective, such encoding regimes also enable both features and labels to be encoded into quantum systems.

% %===POSSIBLY MOVE

% %====Basis orthonormal

% In Chapters \ref{chapter:QDataSet and Quantum Greybox Learning} and \ref{chapter:Quantum Geometric Machine Learning}, we assume the standard orthonormal computational basis $\{\kz,\ko\}$ such that $\braket{1 | 0}=\braket{0 | 1}=0$ and $\braket{1|1}=\braket{0|0}=1$. Quantum states encode information of interest and use in optimisation problems. They are not directly observable, but rather their structure must be reconstructed from known information about the system. In machine learning contexts, quantum states may be used as inputs, constituent elements in intermediate computations or label (output) data. For example, in the QDataset (explored in Chapter \ref{chapter:QDataSet and Quantum Greybox Learning}), intermediate quantum states at any time step may be reconstructed using the intermediate Hamiltonians and unitaries for each example. The code repository for the QDataSet simulation provides further detail on how quantum state representations are used to generate the QDataSet \cite{perrier_QDataSet_2021}. Depending on machine learning architecture, quantum states will usually be represented as matrices or tensors and may be used as inputs (for example, flattened), label data or as an intermediate input, such as in intermediate layers within a hybrid classical-quantum neural network (see \cite{perrier_quantum_2020, youssry_modeling_2020}). For example, consider the matrix representation of eigenstates of a Pauli $\sigma_z$ operator below:
% \begin{align}
% \sigma_z = \begin{pmatrix} 
% 1 & 0 \\
% 0 & -1
% \end{pmatrix} 
% \end{align}
% In the computational basis, this operator has two eigenstates $\kz,\ko$ for eigenvalues $\lambda=1,-1$:
% \begin{align}
% \kz =
% \begin{pmatrix} 
% 1 \\
% 0
% \end{pmatrix} \qquad \text{for} \qquad \lambda = 1 \qquad
% \ko =
% \begin{pmatrix} 
% 0 \\ 
% 1
% \end{pmatrix} \qquad \text{for} \qquad  \lambda=-1 
% \end{align}
% where we have adopted the formalism that the $\lambda=1$ eigenstate is represented by $\kz$ and the $\lambda=-1$ eigenstate is represented by $\ko$ (our choice is consistent with Qutip - practitioners should check platforms they are using for the choice of representation). These eigenstates have a density operator representation as:
% \begin{align}
% \rho_{\lambda=1}=\kz\bz \qquad  \rho_{\lambda=-1} = \ko\bo
% \end{align}
% with matrix representations:
% \begin{align}
% \kz\bz = \begin{pmatrix} 
% 1 & 0 \\
% 0 & 0
% \end{pmatrix}\qquad  \ko\bo = \begin{pmatrix} 
% 0 & 0 \\
% 0 & 1
% \end{pmatrix}
% \end{align}
% Each element $\ketbra{a}{b}=E_{a,b}$ can be considered as an operator basis representation for the relevant density operators (not to be confused with root system vectors in representation theory below). 
% For machine learning practitioners, one way to think about density operators is associating rows and columns with bra and ket vector representations:
% \begin{align}
% \rho = a\kz\bz + b\kz\bo + c\ko\bz + d\ko\bo \dot{= }
% \begin{blockarray}{ccc}
% & \bz & \bo \\
% \begin{block}{c (cc)}
% \kz \qquad & a & b  \\
% \ko \qquad & c & d  \\
% \end{block}
% \end{blockarray}
% \end{align}
% where $a,b,c,d \in \Complex$ are the complex-values amplitudes respective. Given $\rho = \sum_{p_i} \rho_i$, the diagonal elements $a_{n}$ of the density matrix describe the probability $p_n$ of the system residing in state $\rho_n$, that is 
% \begin{align}
% \rho_{nn} = a_{n}a_n^* = p_n \geq 0
% \end{align}
% For pure states, the diagonal along the density matrix will only have one non-zero element (i.e. it will be 1) so that $\rho = \rho_i$. A mixed state will have multiple entries along the diagonal such that $ 0 \leq a_n < 1 $. For example, the $\sigma_z$ eigenvectors have the representation:
%    \begin{align} 
%    \kz\bz \dot{=} 
% \begin{blockarray}{ccc}
%  & \bz & \bo \\
% \begin{block}{c (cc)}
%   \kz \qquad & 1 & 0  \\
%   \ko \qquad & 0 & 0  \\
% \end{block}
% \end{blockarray}
% \qquad
%  \ko\bo \dot{=} 
% \begin{blockarray}{ccc}
%  & \bz & \bo \\
% \begin{block}{c (cc)}
%   \kz \qquad & 0 & 0  \\
%   \ko \qquad & 0 & 1  \\
% \end{block}
% \end{blockarray}
%  \end{align}
% Sometimes the density matrix representation of a state will be equivalent to the outer product of the state, but caution should be applied as this is not generally the case. Translating between the nomenclature and symbolism of quantum information to a more familiar matrix representation used in machine learning assists machine learning researchers to develop their algorithmic architecture. The QDataSet simulation code utilises state space representations of data and operations thereon in order to generate the output contained in the datasets themselves. To recover a quantum state $\ket{\psi(t_j)} = U(t_j)\ket{\psi_0} \approx \prod_i U_i^j \ket{\psi_0}$, one can simply apply the sequence $U_i$ up to $i=j$ (note the order of application is such that $U_j...U_0 \ketpsi$).



% \section{Variational quantum circuits}\label{sec:ml:Variational quantum circuits}
% In this section, we sketch the general use of variational quantum algorithms adopted in Chapters 5 and 6. As Schuld et al. \cite{schuld_machine_2021} note, variational quantum circuits can be interpreted as both deterministic and probabilistic machine learning models for functions $f_\theta: \X \to \Y$ (or learning a probability distribution $\Prb_\theta$). As noted in the literature, quantum circuits parametrised by $\theta$ which are updated according to some objective (cost) function as part of an optimisation process can in some sense naturally be regarded as akin to machine learning models \cite{benedetti_parameterized_2019,cerezo_variational_2022}. Firstly, we define a \textit{parametrised quantum circuit} in terms of a unitary $U(\theta)$ dependent upon parameters $\theta \in \R^m$.
% \begin{definition}[Parametrised quantum circuits]\label{eqn:ml:Parametrised quantum circuits}
%     A parametrised unitary operator is a unitary $U(\theta)(t)$ operator acting on a Hilbert space $\Hilb$ parametrised by a set of parameters $\theta \in \R^m$. A parametrised quantum circuit is then a sequence of unitary operations:
%     \begin{align}
%         U(\theta,t) = \mathcal{T}_+ \exp\left(-i\int_0^T H(\theta,t')dt'\right)\label{eqn:ml:parametrised circuit-timedependent}
%     \end{align}
%     In the time-independent approximation, we have
%     \begin{align}
%         U(\theta,t)\bigg|_{t=T} = U_{T-1}(\theta_{T-1})(\Delta t)...U_1(\Delta t)(\theta) \label{eqn:ml:parametrised circuit-time-independent}
%     \end{align}
%     acting on the initial state $\ket{\psi(0)}$ which we can represent via $U_0(t)$. We assume left-action on states $\ket{\psi}$ where dependence upon $t$ is understood.
% \end{definition}
% Recall each $U_i(\theta_i)(t)$ above is the solution to the time-dependent Schr\"odinger equation (equation \ref{eqn:quant:schrodingersequation}) as a sequence of integrals. For simplicity, we assume the time-independent approximation (equation (\ref{eqn:quant:timeindependentschrodunitary}). The aim of a variational quantum algorithm (VQA) is to find an optimal set of parameters minimising a cost functional on the parameter space given by $C(\theta): \R^\m \to \R$ such that:
% \begin{align*}
%     \theta_* = \arg\min_\theta C(\theta)
% \end{align*}
% The term variational in this quantum context \cite{peruzzo_variational_2014} derives from the underlying principles of variational calculus of finding optimal solutions, such as (originally speaking) computing, for example, lowest energy states of a system. As Schuld et al. notes, the term \textit{variational quantum circuit} is sometimes used interchangeably with parametrised quantum circuit (see Benedetti et al. for a still-salient review \cite{benedetti_parameterized_2019}). In this work, we adopt this association between the two. In geometric terms, 
% We set out the deterministic and probabilistic form below. For a deterministice model, we let $f_\theta:\X \to \Y$ and denote $U(X,\theta)$ (a quantum circuit) for initial state $X \in \X$ and parameters $\theta \in \R^m$. Let $\{O_k\}$ represent the set of (Hermitian) observable (measurement) operators. Then the following function represents a deterministic model:
%     \begin{align*}
%         f_\theta(X) = \trace(O \rho(X,\theta) \label{eqn:ml:qml-VQC-ftheta}
%     \end{align*}
%     where $\rho(X,\theta)=U(\X,\theta)\rho_0 U(\X,\theta)^\dagger$.
% % \begin{definition}[Deterministic quantum model]
% % \end{definition}
% Common approaches to the form of $U(X,\theta)$ include, in analogy with classical machine learning, $U(X,\theta)=W(\theta)S(X)$ where $W(\theta)$ represents a parametrised weight tensor with $S(X)$ representing the encoding of initial features. In this work, we adopt geometric quantum control-style architectures where the unitary channel layers in each network constructed from Hamiltonian layers comprising dynamical Lie algebra generators $X_j \in \g$ (see section \ref{sec:geo:Dynamical Lie algebras}) and associated time-dependent control functions $u_j(t)$ (sometimes denoted $c_j(t)$) (see for example equation (\ref{eqn:bch})). In terms of measurement statistics, then for $U(\theta)\ket{\psi(0)} = \ket{\psi(t)}$, then the class of functions in equation (\ref{eqn:ml:qml-VQC-ftheta}) we seek to learn are reprsentated by mesurement statistics, i.e. a mapping from inputs (e.g. quantum data $x$) to $\R$ as:
% \begin{align}
%     f_\theta(x) = \sum_j m_j p(m_j)
% \end{align}
% ranging over measurements $m_j$. In practice because of post-measurement state collapse, one takes the [expectation] to estimate $f_\theta$ as $\hat f_\theta(x) = (1/N)\sum_i^N m^{(s)}$ where $m^{(s)} \in \{ m \}$ i.e. the outcome of a random measurement from the set of possible outcomes. Reducing error $f_\theta - \hat f_\theta \leq \epsilon$ requires $\mathcal{O}(\epsilon^{-2})$ measurements, growing quickly with precision. Thus one must repeat the experiment $N$ times depending on $\epsilon$ sought. In general we are interested in learning distributions of measurement statistics (from which to reconstruct states or operators) given inputs $x \in \X$ and conditional upon labels (outputs) $\Y$. In measurement terms, we regard $y_i \in \Y$ as measurement outcomes so we interested in a \textit{supervised probabilistic quantum model} for a conditional distribution given by $\Prb_\theta(m|x)$, not just $\Prb_\theta(x)$ itself. Because probabilistic quantum models generate samples, they are often considered \textit{generative models}. \\
% Returning then to the variational / parametrised quantum circuit above, we are therefore interested in learning the parametrised function $f_\theta: \mathcal{B}(\Hilb) \to \Y$ where $\theta$ are trainable parameters (e.g. via gradient descent or some quantum implementation thereof \cite{stokes_quantum_2020}). For our purposes, we work with unitary channels that are parametrised by parameters $\theta$ which are our controls $u_j(t)$ (section \ref{sec:quant:controlsystem}). The quantum channel $U_\theta: \mathcal{B}(\Hilb) \to \mathcal{B}(\Hilb), \rho \mapsto U_\theta \rho U_\theta^\dagger$... 
% \\
% \\
% The typical supervised QML task for unitary synthsesis involves a data space $D_n(\X,\Y)$ where feature data is drawn from quantum state data for a Hilbert space $\X \sim \Hilb$ and $\Y \sim \Km$ (which can be real $\R$ or complex $\C$ -valued) labels. In many cases, including our two machine learning-based chapters, $\Hilb$ is a tensor product for qubits $\Hilb_\otimes = \otimes_n \Hilb$ where $\dim \Hilb_\otimes = 2^n$. The form of $D_n(\X,\Y)=\{ \rho_i, y_i \}_i$ where $D_n$ is sampled from an underyling population. In Chapter \ref{chapter:Quantum Geometric Machine Learning} for example, the training data generated is somewhat unusual in that label data (that which we want to accurately predict) is the the sequence $n$ unitaries $(U_n)$ (i.e. so $(U_n) \in \Y$) where the target (final state) unitary $U_T$ is actually fed in via an input layer (i.e. $U_T \in \X$). In that case, as we discuss, what we are interested in is conditioned on $U_T$, what set of controls $c_j(\Delta t)$ can be generated such that the resulting sequence $(U_n(\Delta t_n))$ leads to $U_T$. Conversely, for the QDataSet in Chapter \ref{chapter:QDataSet and Quantum Greybox Learning}, the training data may vary, such as being classical measurement statistics arising from $m$ Pauli measurements (in which case $\Y \subset \R^m$). As noted in our discussion on measurement (section \ref{sec:quant:Measurement}), for our final two chapters we assume access to a measurement process that allows us data about (of) $U$. 

% \subsubsection{QML Optimisation}\label{sec:ml:QML Optimisation}
% The quantum supervised learning problem above then becomes to learn the distribution $\Prb_\theta(y|x)$. The most common technique for PQCs is \textit{automatic differentiation} \cite{bartholomew-biggs_automatic_2000} via which one can implement stochastic gradient descent and backpropagation algorithms.
% As with the classical case, a loss function is chosen. Typically in the quantum case this requires Given the cost function $C(f_\theta,\hat f_\theta) = C(\theta)$. Thus for example a loss function based on the \textit{fidelity} metric (definition \ref{defn:quant:Fidelity}) adopted in equation (\ref{eqn:batchfidelity}) in Chapter \ref{chapter:Quantum Geometric Machine Learning}, denoted \textit{batch fidelity} takes the mean squared error (MSE, see equation (\ref{eqn:ml:MSE}) above) of the loss (difference) between fidelity of our unitary estimator and the target unitary for empirical risk as:
% \begin{align}
%     C(F,1) = \frac{1}{n}\sum_{j=1}^n (1 - F(\hat{U}_j,U_j))^2 \label{eqn:ml:batchfidelityMSE}
% \end{align}
% This equation implicitly relies upon assumptions regarding measurement protocols that allow us to specify $\hat U_j$ and $U_j$. Because we are using channels $U_j$ for states $\rho_j \in \mathcal{B}(\Hilb)$ we could equivalently specify equation (\ref{eqn:ml:batchfidelityMSE}) in terms of the measurement statistics required to (tomographically) reconstruct $U_j$ (something we touch upon in Chapter \ref{chapter:QDataSet and Quantum Greybox Learning}), in which case it could be written in terms of informationally complete measurement statistics (see section \ref{sec:quant:Informational completeness and POVMs}) with loss functions given in terms of expectation statistics (equation \ref{eqn:quant:measurementdensitymatrixtrace}) continent upon parameters (i.e. controls) $\theta$. Before moving onto a sketch of our greybox variational quantum architecture adopted in Chatpers \ref{chapter:QDataSet and Quantum Greybox Learning} and \ref{chapter:Quantum Geometric Machine Learning}, it is worth saying a few words about differences in implementation of gradient descent in the classical and quantum case and parameter shift rules in particular. 

% \subsubsection{QML Gradients} \label{sec:ml:QML Gradients}
% The discussion of gradient-based optimisation methods above is classically focused, relying on mathematically nice properties of differentiable manifolds $\M$ (such as configuration space or registers parametrisating quantum states or operators). Parameter shifts \cite{mitarai_quantum_2018,wierichs_general_2022} in the context of gradient descent represent a method of calculating gradients by shifts of parameters. By evaluating the cost function $C(\theta)$ at the value of two different parameters $\theta, \theta + \epsilon_\theta$, the rescaled difference $\nabla_\theta - \nabla_{\theta + \epsilon_\theta}$ forms an unbiased estimate of $\nabla_\theta$, usually restricted to gates with two different eigenvalues \cite{wierichs_general_2022}. The reason this matters is because in certain cases classical stochastic gradient descent is inappropriate or unable to obtain a well-defined gradient.
% \begin{enumerate}[(i)]
%     \item \textit{Quantum natural gradietns}
%     \item \textit{Parameter shift rules}
%     \item \textit{Quantum autodifferentiation}. In a series of papers, Beer et al. \cite{beer_quantum_2021,beer_quantum_2022,beer_training_2020} propose a quantum analogue of autodifferentiation and backpropagation for (fully connected for the most part) quantum neural network architectures. 
% \end{enumerate}






 


% \section{Symmetry-based QML}\label{sec:ml:Symmetry-based QML}
% In this final section, we sketch an outline of the general structure of greybox variational quantum circuits that are the subject of our next two chapters. We connect the general architecture to three related fields in quantum and classical machine learning (a) Lie algebraic methods (such as Lie group machine learning \cite{moskalev_liegg_2023,lu_survey_2020}), (b) geometric machine learning (\cite{bronstein_geometric_2021} and (c) geometric quantum machine learning \cite{nguyen_theory_2022,larocca_group-invariant_2022}. 

% \subsection{QML Optimal Control} \label{sec:ml:QML Optimal Control}
% In terms of the discussion of optimal control examined in the previous chapter, the backpropagation algorithms are designed to learn function estimates $f_\theta$ that map from time-optimal geodesic data to sequences of controls. An effective learning protocol would thereby, in principle, learn controls (and thus unitary sequences) satisfying the requisite PMP conditions. These approaches seek to learn parameterised functions $u_j(t)$ in the case of control theory and weights $\omega$ in the case of neural networks to optimise an objective function (maximising the PMP Hamiltonian or minimising the loss/cost function $L$ in backpropagation). In essence the conceptual connection between controls acting on [generators], updated to satisfy the constraints of the optimal control problem, with updatable weights acting on input features in order to satisfy the objective function of minimising loss provides a [bridge] between classical control theory and machine learning. Indeed the deep connections between the two are very much manifest across the literature, especially in the work of Bellman \cite{bellman_dynamic_1956,bellman_introduction_2016}. In Chapter \ref{chapter:Quantum Geometric Machine Learning}, we assume that the sequence of unitaries (generated from a theoretically justified means of obtaining subRiemannian geodesics) is time-optimal and thus bounded by total time (path-length) $L$, thus adopt a learning protocol that seeks to learn the sequence of controls $u(t) \in [0,1]$ which minimises the error (fidelity) of $\hat U_j(t)$ versus $U_j(t)$ for a sequence of unitaries $j=1,...,n$. Put another way, we assume by reason of the assumption that training data consists of geodesic paths (represented by sequences of unitaries) whose length is therefore minimal and unique. From equation \ref{eqn:geo:arclength}, because the controls set the length $\ell(\gamma)$, the sequence of controls obtaining $\hat U_j(t) \simeq U_j(t)$ will be minimal (up to some error tolerance).

% \subsection{Geometric information theory} \label{sec:ml:Geometric information theory}
% Geometric information theory emerged ..... The fundamental organising principle is to regard information-theoretic problems of interest in terms of geometric concepts. Thus information is presented as [inhering within] a differentiable manifold [e.g. Riemannian or Kahler manifold]. Information theory [\textbf{ref}] often has measures of information. As Amari [\textbf{AMARI}] (credited with first equating Fisher information and the Riemannian metric) notes, information geometry is a means of exploring the world using modern (differential) geometry, as a disciplien arising from the use of such techniques to study symmetry and invariance properties involved in statistical inference. In the interests of time and space, we do not in this work delve into information geometry in any significant way, however note its use in machine learning in a variety of areas, such as clustering, support vector machines, belief propagation and boosting. The underlying idea of information geometry is to cast information and probability distributions in terms of geometric structures such as differentiable manifolds.

% \subsection{Lie group machine learning}\label{sec:ml:Lie group machine learning}


% \bsubsection{Geometric QML} \label{sec:ml:Geometric QML}
% the use of dynamical Lie group generators, bespoke Hamiltonian formation and exponential activation functions as a means of connecting layer-based outputs to unitary evolution. We situate these works with concurrent related, but distinct, work in geometric quantum machine learning, representation-based QML and other related areas. 

% \subsection{Geometric QML}\label{sec:ml:Geometric QML}
% In recent years, interest in applying geometric techniques to assist in symmetry reduction and symmetry-enhanced quantum machine learning network design have gained prominent. We summarise some of the key results relevant to our complementary work below. This emerging subdiscipline, sometimes named geometric quantum machine learning \cite{cerezo_challenges_2022,larocca_theory_2021} seeks to incorporate symmetry properties into the design of machine learning architecture as a means of improving figures of merit, such as runtime complexity, metrics (such as fidelity) or generalisation and overparamterisation. This is often achieved via seeking to build parametrised quantum circuits or quantum neural network architectures which, as functional compositions, respect underyling symmetries of input data, or which lead to outputs which respect symmetry properties, such as outputs in terms of unitaries or parametrisations thereof. For example, \cite{schatzki_theoretical_2022} design quantum neural network layers $\mathcal{F}$ that permutation symmetry under the action of the permutation group $S_n$. In this case, $\sigma\mathcal{F(\sigma)} = \mathcal{F}(\sigma(\psi))$ for $\sigma \in S_n$.\\
% \\
% Central to the GQML programme is the use of symmetry-respective architectures. This is usually in the form of [neural network layers] consistent of unitaries generated by generatores of dynamical Lie groups (see section \ref{sec:geo:Dynamical Lie algebras}). [The use of symmetry reduction is shown in a number of works to, for example, reduce the effective parametrisation required in order to meet certain performance thresholds [\textbf{REF}]]. Relatedly, the reduction in parametrisation [owing to such embedded symmetries] has been shown to improve other architectural features, such as the risk of \textit{barren plateaus} (the quantum analogue of the vanishing gradient problem [\textbf{ARJOVSKY}].


% \section{Greybox machine learning} \label{sec:ml:Greybox machine learning}
% Our approach in the subsequent two chapters of this work represents a related, but distinct, stream of research leveraging algebraic and geometric techniques for solving time-optimal unitary synthesis problems. Our general approach to architecture, focusing on quantum geometric machine learning, is set out below. The method is a hybrid of quantum and classical architectures which we denote \textit{greybox architecture} or greybox learning. The underyling idea is that known a priori information is encoded within a classical neural network stack, obviating the need for the network to learn such rules (such as requirements regarding unitarity or Hamiltonian construction) and thereby affording guarantees (such as unitarity of outputs) in a way that blackbox learning only at best approximates. 
% We can analogise between directionality of [gradient descent updates] to estimate $\hat Y$ and using machine learning methods to solve time-optimal problems. Sketching this out, in our previous chapter we articulated how $U_T \in G \simeq \M$ (for Lie group $G$) are generated (via Hamiltonian flow) by Hamiltonians $H$ from the corresponding Lie algebra $\g$. By the correspondence between tangent vectors and Lie algebra basis elements, we can then regard learning optimal control functions $u_j(t)$ (for directions $j$ where $j = 1,...,\dim \g$ as equivalent optimisation in a machine learning context. The controls $u_j(t)$ in effect parametrise our system consistent with the generalised Pontryagin method, with the adjustment of the control functions to minimise our loss functions (explicated below in terms of fidelity $F(\hat U_T,U_T)$) geometrically represented as transformations in one or more of the directions of elements of $H_p\M$ (our distribution $\Delta$). The \textit{geometric} features we are seeking to leverage are the symmetry properties of subRiemannian symmetric spaces, in particular discovering strategies for learning sequences of controls for generating time-optimal geodesic paths along the manifold of interest. We describe this relationship below.
% %
% %
% %
% \begin{enumerate}[(i)]
%     \item \textit{Objective}. Firstly, our problem is one of using machine learning to synthesise time-optimal unitaries relevant to quantum computational contexts. Specifically, this means using machine learning architecture to solve certain control systems expressed through the Pontryagin Maximum Principle (definition \ref{defn:geo:Pontryagin maximum principle}). Our approach focused on quantum control lends itself to variational quantum algorithms from a design-choice perspective.
%     \item \textit{Control optimisation}. Our aim is to therefore generate a sequence of control pulses that may be applied to corresponding Lie algebra generators (in our case corresponding to single and multi-qubit systems) in order to generate sequences of time-optimal (or as approximately time-optimal as we can get) unitary operators. given the objectives and constraints required, including (a) ensuring outputs respect unitary constraints and (b) controls (and by extension path-length) respects minimisation (and geodesic) constraints.
%     \item \textit{Inputs}. The inputs layers $a^{(0)}$ of the network take as their feature data unitaries $U(t) \in G$ or in the case of multi-qubit systems, $G \otimes G$ where $G$ for the first two chapters $G=\text{sU}(2)$. The unitaries have a representation by way of the usual representation of SU(2) in terms of the matrix group $M_2(\C)$ (see definition \ref{defn:alg:connected_matrix_lie_group}). Denoting such matrices $X \in M_2(\C)$ (or $X_1 \otimes X_2 \in M_2(\C) \otimes M_2(\C)$ (by the single $X$ for conveniencE), the intial layers tend to transform (e.g. flatten) such matrices into a realised form [\textbf{CROSS REF}]. The activation function of these input layers tends to then just be the identity:
% \begin{align}
%     a^{(0)} = I(X)
% \end{align}
% consistent with the generic neural network schema in section \ref{sec:ml:neuralnetworkschema}.
% \item \textit{Feedforward layers}. The input layers are then fed into a sequence of typical classical neural network layer, in our case feed-forward layers:
% \begin{align}
%     a^{(1)}&=\sigma(W^T a^{(0)} + b)
% \end{align}
% The feed-forward layers tend to be, at least in our examples, fully-connected and dense. 
% \item \textit{Control pulse layers}.  As we sketch below, parameter network layers (parametrised by $\theta$) feed into layers comprising control pulses $u_j(t)$. The neurons within these layers are characterised by activation functions such that $u_j(t) \in [0,1]$, where we rely implicitly on the fact that for the bounded control problem, we can arbitrarily scale (normalise) controls to fit within minimum length $L$ (see definition \ref{defn:geo:arclength}).
% \item \textit{Hamiltonian and Unitary layers}.  The control pulse layers then feed into bespoke layers to (i) construct the Hamiltonian from fixed Lie algebra generators in $\g$ which is then (ii) input into a layer comprising an exponential activation that constructs time-independent approximation to time-dependent unitary operator. In all cases, our target of interest is the optimal unitary for time $t_j$. In Chapter \ref{chapter:Quantum Geometric Machine Learning}, we are interested in the sequence of controls $(u_i(t))$ that generate a sequence of unitary operators $(U(t))$ which, under the assumption of time-independence (see definition \ref{eqn:quant:timeindependentschrodunitary}), allows us to generate our target $U(T) \in G$. Each node generating a unitary has $k$ generators and control functions $u_i(t), i=1,...k$ where $k=\dim\g$ (or whatever the control subalgebra is). Our labels and our function estimates are \textit{sequences} of unitaries and, as we note below, the target $U_T$ is actually one of the inputs to the models.
% \item \textit{Optimisation}. The optimisation occurs by reference to a cost function based on the fidelity metric (definition \ref{defn:quant:Fidelity}). The fidelity of each unitary esimate in the sequence $\hat U_j(t)$ is estimated. 
% From a control theory perspective, the optimisation is classical offline control, where an exogenous protocol is used to optimise and then adjust the parameters $\theta$ accordingly which ultimately feed into adjusting the controls $u_i(t)$. Several classes of network are used, including a vanilla (basic) fully-connected feedfoward network, an LSTM (see the Chapter for details) and the greybox approach which we detail here. The networks are trained on data $D_n(X,Y)$ generated from distribution $\Delta \in \su(2)$, such that the resulting Hamiltonians (and thus curves on $\M$) are time-optimal, these are subRiemannian geodesics.
% \item \textit{Measurement}. In Chapter \ref{chapter:QDataSet and Quantum Greybox Learning}, measurement statistics for each time slice are captured in the data (from which one can reconstruct unitaries or Hamiltonians for such time slice), whereas for Chapter \ref{chapter:Quantum Geometric Machine Learning}, the existence of an external process that allows for $\hat U(t)$ and $\hat U(t)$ to be constructed is assumed.
% \end{enumerate}








% % \subsubsection{Neurons}
% % The basic building block of deep learning networks is the [neuron]. The early progenitors of neurons were 

% % A multi-layer perceptron (MLP) is a class of feedforward artificial neural network (ANN) composed of multiple layers of nodes in a directed graph, where each layer fully connects to the next one. At the core of the MLP is the perceptron, the simplest neural network building block, which computes a weighted sum of its input, adds a bias, and then passes it through a nonlinear activation function. Mathematically, an MLP can be described as follows:

% % Consider an MLP with $L$ layers, where each layer $l$ contains $n_l$ neurons. Let the input vector to the network be $\mathbf{x} \in \mathbb{R}^{n_0}$, where $n_0$ is the dimensionality of the input space. The output of the $i$-th neuron in the $l$-th layer, denoted as $a_i^{(l)}$, is computed as

% % \begin{align}
% %     a_i^{(l)} = \sigma\left(\sum_{j=1}^{n_{l-1}} w_{ij}^{(l)} a_j^{(l-1)} + b_i^{(l)}\right),
% % \end{align}

% % where $\sigma$ is the activation function (e.g., sigmoid, ReLU), $w_{ij}^{(l)}$ represents the weight from the $j$-th neuron in the $(l-1)$-th layer to the $i$-th neuron in the $l$-th layer, $b_i^{(l)}$ is the bias term for the $i$-th neuron in the $l$-th layer, and $a_j^{(l-1)}$ is the output of the $j$-th neuron in the $(l-1)$-th layer. For the input layer ($l=0$), $a_j^{(0)} = x_j$, the $j$-th component of the input vector $\mathbf{x}$.

% % The overall output of the MLP, denoted as $\mathbf{y} = (y_1, y_2, ..., y_{n_L})^T$, where $n_L$ is the number of neurons in the output layer, is thus given by the outputs of the last layer:

% % \begin{align}
% %     \mathbf{y} = \mathbf{a}^{(L)} = \left( a_1^{(L)}, a_2^{(L)}, ..., a_{n_L}^{(L)} \right)^T.
% % \end{align}







% %==========GEOMETRIC MACHINE LEARNING
% % \section{Geometric Machine Learning}
% % \hl{\textbf{NB: complete background summary}}.
% % \begin{itemize}
% %     \item Otto symmetry in machine learning paper
% %     \item Brunstein paper
% %     \item Lee on Lie theory and ML
% % \end{itemize}
% % \subsection{Overview}
% % Geometric techniques have been of increasing interest in the machine learning community. 

% % \subsection{Geometric deep learning}
% % Geometric deep learning has, over the last few years, become an increasing focus as machine learning practitioners have sought to leverage techniques from related disciplines to solve persistent challenges relating to scaling, generalisability and entropy. Geometric machine learning often crosses-over or is cross-classified with other subdisciplines such as graph-based machine learning. Thus early surveys of Cao et al. \cite{cafaro_geometric_2017} examine typical graph and convolutional machine learning techniques [\textbf{NOTE: RELATED TO PAPER}]

% % Bronstein et al. \cite{bronstein_geometric_2021} provide a relatively comprehensive introduction to the application of largely Riemannian and Euclidean geometry to machine learning problems. 

% % \subsection{Algebraic geometry and statistical learning}
% % A fruitful line of research intersecting geometric, algebraic and machine learning techniques is also found in the work of Watanabe [\textbf{WATANABE}]. The connections between algebraic geometry and statistical learning theory are explored in `singularity learning theory'. Other approaches utilising topological and physics' principles include [\textbf{CARROLL}] (phase transitions in neural networks). 

% % %==========QUANTUM MACHINE LEARNING

% % \subsection{Lie group machine learning} Another related, but distinct, subset of machine learning and representation theory has been \textit{Lie group machine learning}. Early work canvassed connections between Lie algebras and machine learning/neural network architectures \cite{li_lie_2019}


% % \subsubsection{Barren plateaux}







